Drug Selection via Joint Push and Learning to Rank

Selecting the right drugs for the right patients is a primary goal of precision medicine. In this manuscript, we consider the problem of cancer drug selection in a learning-to-rank framework. We have formulated the cancer drug selection problem as to accurately predicting 1). the ranking positions of sensitive drugs and 2). the ranking orders among sensitive drugs in cancer cell lines based on their responses to cancer drugs. We have developed a new learning-to-rank method, denoted as pLETORg , that predicts drug ranking structures in each cell line via using drug latent vectors and cell line latent vectors. The pLETORg method learns such latent vectors through explicitly enforcing that, in the drug ranking list of each cell line, the sensitive drugs are pushed above insensitive drugs, and meanwhile the ranking orders among sensitive drugs are correct. Genomics information on cell lines is leveraged in learning the latent vectors. Our experimental results on a benchmark cell line-drug response dataset demonstrate that the new pLETORg significantly outperforms the state-of-the-art method in prioritizing new sensitive drugs.

==> IEEEtran/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> figures/gene_selection.tex <==
\begin{tikzpicture}


  \definecolor{response}{RGB}{255,51,76}
  \definecolor{geneexp}{RGB}{0, 0, 255}
  \definecolor{geneweight}{RGB}{255, 153, 0}


  \def\csize{0.25} % cell size


  %%%%%%%%%%%%%%%%%%%%%%%%%%%
  % left matrix
  %%%%%%%%%%%%%%%%%%%%%%%%%%%
  \def\nDrug{1}
  \def\nCell{6}
  \def\xResStart{0}
  \def\yResStart{0}
  \def\xResEnd{\xResStart+\nDrug*\csize}
  \def\yResEnd{\yResStart+\nCell*\csize}

  \node[rotate=90] at (\xResStart-\csize          , {0.5*(\yResStart+\yResEnd)}) {\footnotesize{cell lines}};
  \node[rotate=0 ] at ({0.5*(\xResStart+\xResEnd)}, \yResEnd+\csize            ) {\footnotesize{drug $\drug_i$}};
  \node[rotate=0 ] at ({0.5*(\xResStart+\xResEnd)}, \yResStart-2*\csize        ) {\small{drug response}};
  \draw[step=0.25cm,color=black] (\xResStart, \yResStart) grid (\xResEnd, \yResEnd);

  % add color
    \foreach \x in {1}
      \foreach \y in {1,...,6}
        {\pgfmathsetmacro\k{random(5, 50)}
         \node[fill=response!\k, draw=response!\k] at (\xResStart+\csize*\x-0.5*\csize, \yResStart+\csize*\y-0.5*\csize) {};
        }



  %%%%%%%%%%%%%%%%%%%%%%%%%%%
  % equal sign
  %%%%%%%%%%%%%%%%%%%%%%%%%%%
  \node[rotate=0 ] at (\xResEnd+3*\csize, {0.5*(\yResStart+\yResEnd)}) {$=$};


  %%%%%%%%%%%%%%%%%%%%%%%%%%%
  % middle matrix
  %%%%%%%%%%%%%%%%%%%%%%%%%%%
  \def\nGenexpD{7}
  \def\nCell{6}
  \def\xGenexpStart{\xResEnd+6*\csize}
  \def\yGenexpStart{0}
  \def\xGenexpEnd{\xGenexpStart+\nGenexpD*\csize}
  \def\yGenexpEnd{\yGenexpStart+\nCell*\csize}

  \node[rotate=90] at (\xGenexpStart-\csize, \yGenexpStart+0.5*\nCell*\csize)    {\footnotesize{cell lines}};
  \node[rotate=0 ] at (\xGenexpStart+0.5*\nGenexpD*\csize, \yGenexpEnd + \csize) {\footnotesize{genes}};
  \node[rotate=0 ] at (\xGenexpStart+0.5*\nGenexpD*\csize, \yGenexpStart-2*\csize) {\small{gene expressions}};
  \draw[step=\csize,color=black] (\xGenexpStart-0.001, \yGenexpStart) grid (\xGenexpEnd, \yGenexpEnd);

  % add color
  %  \foreach \i in {1,...,\nGenexpD}
  %    \foreach \j in {1,...,\nCell}
  %      {\pgfmathsetmacro\k{random(5, 50)}
  %       \node[fill=blue!\k] at (\xGenexpStart+\csize*\i-0.5*\csize, \yGenexpStart+\csize*\j-0.5*\csize) {};
  %      }
  \node[fill=geneexp!23, draw=geneexp!23] at (\xGenexpStart+\csize* 1-0.5*\csize, \yGenexpStart+\csize* 1-0.5*\csize) {};
  \node[fill=geneexp! 8, draw=geneexp! 8] at (\xGenexpStart+\csize* 2-0.5*\csize, \yGenexpStart+\csize* 1-0.5*\csize) {};
  \node[fill=geneexp!53, draw=geneexp!53] at (\xGenexpStart+\csize* 3-0.5*\csize, \yGenexpStart+\csize* 1-0.5*\csize) {};
  \node[fill=geneexp!51, draw=geneexp!51] at (\xGenexpStart+\csize* 4-0.5*\csize, \yGenexpStart+\csize* 1-0.5*\csize) {};
  \node[fill=geneexp!26, draw=geneexp!26] at (\xGenexpStart+\csize* 5-0.5*\csize, \yGenexpStart+\csize* 1-0.5*\csize) {};
  \node[fill=geneexp!30, draw=geneexp!30] at (\xGenexpStart+\csize* 6-0.5*\csize, \yGenexpStart+\csize* 1-0.5*\csize) {};
  \node[fill=geneexp!26, draw=geneexp!26] at (\xGenexpStart+\csize* 7-0.5*\csize, \yGenexpStart+\csize* 1-0.5*\csize) {};
  \node[fill=geneexp!24, draw=geneexp!24] at (\xGenexpStart+\csize* 1-0.5*\csize, \yGenexpStart+\csize* 2-0.5*\csize) {};
  \node[fill=geneexp! 7, draw=geneexp! 7] at (\xGenexpStart+\csize* 2-0.5*\csize, \yGenexpStart+\csize* 2-0.5*\csize) {};
  \node[fill=geneexp!54, draw=geneexp!54] at (\xGenexpStart+\csize* 3-0.5*\csize, \yGenexpStart+\csize* 2-0.5*\csize) {};
  \node[fill=geneexp!52, draw=geneexp!52] at (\xGenexpStart+\csize* 4-0.5*\csize, \yGenexpStart+\csize* 2-0.5*\csize) {};
  \node[fill=geneexp!24, draw=geneexp!24] at (\xGenexpStart+\csize* 5-0.5*\csize, \yGenexpStart+\csize* 2-0.5*\csize) {};
  \node[fill=geneexp!35, draw=geneexp!35] at (\xGenexpStart+\csize* 6-0.5*\csize, \yGenexpStart+\csize* 2-0.5*\csize) {};
  \node[fill=geneexp!27, draw=geneexp!27] at (\xGenexpStart+\csize* 7-0.5*\csize, \yGenexpStart+\csize* 2-0.5*\csize) {};
  \node[fill=geneexp!25, draw=geneexp!25] at (\xGenexpStart+\csize* 1-0.5*\csize, \yGenexpStart+\csize* 3-0.5*\csize) {};
  \node[fill=geneexp! 9, draw=geneexp! 9] at (\xGenexpStart+\csize* 2-0.5*\csize, \yGenexpStart+\csize* 3-0.5*\csize) {};
  \node[fill=geneexp!59, draw=geneexp!59] at (\xGenexpStart+\csize* 3-0.5*\csize, \yGenexpStart+\csize* 3-0.5*\csize) {};
  \node[fill=geneexp!49, draw=geneexp!49] at (\xGenexpStart+\csize* 4-0.5*\csize, \yGenexpStart+\csize* 3-0.5*\csize) {};
  \node[fill=geneexp!26, draw=geneexp!26] at (\xGenexpStart+\csize* 5-0.5*\csize, \yGenexpStart+\csize* 3-0.5*\csize) {};
  \node[fill=geneexp!28, draw=geneexp!28] at (\xGenexpStart+\csize* 6-0.5*\csize, \yGenexpStart+\csize* 3-0.5*\csize) {};
  \node[fill=geneexp!27, draw=geneexp!27] at (\xGenexpStart+\csize* 7-0.5*\csize, \yGenexpStart+\csize* 3-0.5*\csize) {};
  \node[fill=geneexp!23, draw=geneexp!23] at (\xGenexpStart+\csize* 1-0.5*\csize, \yGenexpStart+\csize* 4-0.5*\csize) {};
  \node[fill=geneexp! 9, draw=geneexp! 9] at (\xGenexpStart+\csize* 2-0.5*\csize, \yGenexpStart+\csize* 4-0.5*\csize) {};
  \node[fill=geneexp!52, draw=geneexp!52] at (\xGenexpStart+\csize* 3-0.5*\csize, \yGenexpStart+\csize* 4-0.5*\csize) {};
  \node[fill=geneexp!51, draw=geneexp!51] at (\xGenexpStart+\csize* 4-0.5*\csize, \yGenexpStart+\csize* 4-0.5*\csize) {};
  \node[fill=geneexp!27, draw=geneexp!27] at (\xGenexpStart+\csize* 5-0.5*\csize, \yGenexpStart+\csize* 4-0.5*\csize) {};
  \node[fill=geneexp!34, draw=geneexp!34] at (\xGenexpStart+\csize* 6-0.5*\csize, \yGenexpStart+\csize* 4-0.5*\csize) {};
  \node[fill=geneexp!30, draw=geneexp!30] at (\xGenexpStart+\csize* 7-0.5*\csize, \yGenexpStart+\csize* 4-0.5*\csize) {};
  \node[fill=geneexp!25, draw=geneexp!25] at (\xGenexpStart+\csize* 1-0.5*\csize, \yGenexpStart+\csize* 5-0.5*\csize) {};
  \node[fill=geneexp!10, draw=geneexp!10] at (\xGenexpStart+\csize* 2-0.5*\csize, \yGenexpStart+\csize* 5-0.5*\csize) {};
  \node[fill=geneexp!60, draw=geneexp!60] at (\xGenexpStart+\csize* 3-0.5*\csize, \yGenexpStart+\csize* 5-0.5*\csize) {};
  \node[fill=geneexp!55, draw=geneexp!55] at (\xGenexpStart+\csize* 4-0.5*\csize, \yGenexpStart+\csize* 5-0.5*\csize) {};
  \node[fill=geneexp!27, draw=geneexp!27] at (\xGenexpStart+\csize* 5-0.5*\csize, \yGenexpStart+\csize* 5-0.5*\csize) {};
  \node[fill=geneexp!35, draw=geneexp!35] at (\xGenexpStart+\csize* 6-0.5*\csize, \yGenexpStart+\csize* 5-0.5*\csize) {};
  \node[fill=geneexp!26, draw=geneexp!26] at (\xGenexpStart+\csize* 7-0.5*\csize, \yGenexpStart+\csize* 5-0.5*\csize) {};
  \node[fill=geneexp!26, draw=geneexp!26] at (\xGenexpStart+\csize* 1-0.5*\csize, \yGenexpStart+\csize* 6-0.5*\csize) {};
  0\node[fill=geneexp!10, draw=geneexp!10] at (\xGenexpStart+\csize* 2-0.5*\csize, \yGenexpStart+\csize* 6-0.5*\csize) {};
  \node[fill=geneexp!58, draw=geneexp!58] at (\xGenexpStart+\csize* 3-0.5*\csize, \yGenexpStart+\csize* 6-0.5*\csize) {};
  \node[fill=geneexp!52, draw=geneexp!52] at (\xGenexpStart+\csize* 4-0.5*\csize, \yGenexpStart+\csize* 6-0.5*\csize) {};
  \node[fill=geneexp!25, draw=geneexp!25] at (\xGenexpStart+\csize* 5-0.5*\csize, \yGenexpStart+\csize* 6-0.5*\csize) {};
  \node[fill=geneexp!34, draw=geneexp!34] at (\xGenexpStart+\csize* 6-0.5*\csize, \yGenexpStart+\csize* 6-0.5*\csize) {};
  \node[fill=geneexp!30, draw=geneexp!30] at (\xGenexpStart+\csize* 7-0.5*\csize, \yGenexpStart+\csize* 6-0.5*\csize) {};







  %%%%%%%%%%%%%%%%%%%%%%%%%%%
  % multiplication sign
  %%%%%%%%%%%%%%%%%%%%%%%%%%%
  \node[rotate=0 ] at (\xGenexpEnd+2*\csize, {0.5*(\yGenexpStart+\yGenexpEnd)}) {$\times$};


  %%%%%%%%%%%%%%%%%%%%%%%%%%%
  % right matrix
  %%%%%%%%%%%%%%%%%%%%%%%%%%%
  \def\xGenwtStart{\xGenexpEnd+4*\csize}
  \def\yGenwtStart{\yGenexpEnd}
  \def\xGenwtEnd{\xGenwtStart+1*\csize}
  \def\yGenwtEnd{\yGenwtStart-\nGenexpD*\csize}


  \node[rotate=90] at (\xGenwtEnd+\csize, {0.5*(\yGenwtStart+\yGenwtEnd)}) {\footnotesize{gene weights}};
  \draw[step=0.25cm,color=black] (\xGenwtStart-0.001, \yGenwtStart) grid (\xGenwtEnd, \yGenwtEnd);

  % add color
    \foreach \i in {1}
      \foreach \j in {1,...,\nGenexpD}
        {\pgfmathsetmacro\k{random(5, 50)}
         \node[fill=geneweight!\k, draw=geneweight!\k] at (\xGenwtStart+\i*\csize-0.5*\csize, \yGenwtStart-\j*\csize+0.5*\csize) {};
        }



%  \node[fill=geneweight!19, draw=geneweight!19] at (4.875, 1.375)  {};
%  \node[fill=geneweight!20, draw=geneweight!20] at (4.875, 1.125)  {};
%  \node[fill=geneweight!0 , draw=geneweight!0 ] at (4.875, 0.875)  {};
%  \node[fill=geneweight!29, draw=geneweight!29] at (4.875, 0.625)   {};
%  \node[fill=geneweight!30, draw=geneweight!30] at (4.875, 0.375)   {};
%  \node[fill=geneweight!74, draw=geneweight!74] at (4.875, 0.125)   {};
%  \node[fill=geneweight!70, draw=geneweight!70] at (4.875, -0.125)  {};









\end{tikzpicture}


==> figures/random_cellline.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5040.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,1604){\rotatebox{-270}{\makebox(0,0){\strut{}cell lines}}}%
      \put(2695,678){\makebox(0,0){\strut{}drugs}}%
      \csname LTb\endcsname%
      \put(616,1203){\makebox(0,0)[r]{\strut{}$\cellline_1$}}%
      \put(616,1397){\makebox(0,0)[r]{\strut{}$\cellline_2$}}%
      \put(616,1592){\makebox(0,0)[r]{\strut{}$\cellline_3$}}%
      \put(616,1786){\makebox(0,0)[r]{\strut{}$\cellline_4$}}%
      \put(616,1981){\makebox(0,0)[r]{\strut{}$\cellline_5$}}%
      \put(973,898){\makebox(0,0){\strut{}$\drug_1$}}%
      \put(1362,898){\makebox(0,0){\strut{}$\drug_2$}}%
      \put(1752,898){\makebox(0,0){\strut{}$\drug_3$}}%
      \put(2141,898){\makebox(0,0){\strut{}$\drug_4$}}%
      \put(2531,898){\makebox(0,0){\strut{}$\drug_5$}}%
      \put(2920,898){\makebox(0,0){\strut{}$\drug_6$}}%
      \put(3310,898){\makebox(0,0){\strut{}$\drug_7$}}%
      \put(3699,898){\makebox(0,0){\strut{}$\drug_8$}}%
      \put(4089,898){\makebox(0,0){\strut{}$\drug_9$}}%
      \put(4478,898){\makebox(0,0){\strut{}$\drug_{10}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{random_cellline}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/selected_cl/mat_BL70_insensitive.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6192.00,2160.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1584,791){\makebox(0,0)[r]{\strut{}\footnotesize{BRD-A36275421}}}%
      \put(1584,972){\makebox(0,0)[r]{\strut{}\footnotesize{BRD-K01877528}}}%
      \put(1584,1154){\makebox(0,0)[r]{\strut{}\footnotesize{BRD-K86525559}}}%
      \put(1584,1335){\makebox(0,0)[r]{\strut{}\footnotesize{BRD-K15108141}}}%
      \put(1584,1517){\makebox(0,0)[r]{\strut{}\footnotesize{BRD-K17743125}}}%
      \put(1584,1698){\makebox(0,0)[r]{\strut{}\footnotesize{BRD-K15600710}}}%
      \put(1898,480){\makebox(0,0){\strut{}1}}%
      \put(2261,480){\makebox(0,0){\strut{}2}}%
      \put(2624,480){\makebox(0,0){\strut{}3}}%
      \put(2987,480){\makebox(0,0){\strut{}4}}%
      \put(3350,480){\makebox(0,0){\strut{}5}}%
      \put(3713,480){\makebox(0,0){\strut{}6}}%
      \put(4076,480){\makebox(0,0){\strut{}7}}%
      \put(4439,480){\makebox(0,0){\strut{}8}}%
      \put(4802,480){\makebox(0,0){\strut{}9}}%
      \put(5165,480){\makebox(0,0){\strut{}10}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(154,1244){\rotatebox{90}{\makebox(0,0){\strut{}\small{drug ID}}}}%
      \put(3531,260){\makebox(0,0){\strut{}\small{latent dimension}}}%
      \csname LTb\endcsname%
      \put(5751,709){\makebox(0,0)[l]{\strut{}\footnotesize{-6}}}%
      \put(5751,996){\makebox(0,0)[l]{\strut{}\footnotesize{-3}}}%
      \put(5751,1282){\makebox(0,0)[l]{\strut{}\footnotesize{0}}}%
      \put(5751,1569){\makebox(0,0)[l]{\strut{}\footnotesize{3}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{mat_BL70_insensitive}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/selected_cl/mat_BL70_sensitive.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6192.00,2160.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1584,791){\makebox(0,0)[r]{\strut{}\footnotesize{BRD-A81541225}}}%
      \put(1584,972){\makebox(0,0)[r]{\strut{}\footnotesize{BRD-A28746609}}}%
      \put(1584,1154){\makebox(0,0)[r]{\strut{}\footnotesize{BRD-A05821830}}}%
      \put(1584,1335){\makebox(0,0)[r]{\strut{}\footnotesize{BRD-K76674262}}}%
      \put(1584,1517){\makebox(0,0)[r]{\strut{}\footnotesize{BRD-K23547378}}}%
      \put(1584,1698){\makebox(0,0)[r]{\strut{}\footnotesize{BRD-K35708212}}}%
      \put(1898,480){\makebox(0,0){\strut{}1}}%
      \put(2261,480){\makebox(0,0){\strut{}2}}%
      \put(2624,480){\makebox(0,0){\strut{}3}}%
      \put(2987,480){\makebox(0,0){\strut{}4}}%
      \put(3350,480){\makebox(0,0){\strut{}5}}%
      \put(3713,480){\makebox(0,0){\strut{}6}}%
      \put(4076,480){\makebox(0,0){\strut{}7}}%
      \put(4439,480){\makebox(0,0){\strut{}8}}%
      \put(4802,480){\makebox(0,0){\strut{}9}}%
      \put(5165,480){\makebox(0,0){\strut{}10}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(154,1244){\rotatebox{90}{\makebox(0,0){\strut{}\small{drug ID}}}}%
      \put(3531,260){\makebox(0,0){\strut{}\small{latent dimension}}}%
      \csname LTb\endcsname%
      \put(5751,709){\makebox(0,0)[l]{\strut{}\footnotesize{-6}}}%
      \put(5751,996){\makebox(0,0)[l]{\strut{}\footnotesize{-3}}}%
      \put(5751,1282){\makebox(0,0)[l]{\strut{}\footnotesize{0}}}%
      \put(5751,1569){\makebox(0,0)[l]{\strut{}\footnotesize{3}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{mat_BL70_sensitive}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/selected_cl/mat_CAL51_insensitive.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6192.00,2160.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1584,700){\makebox(0,0)[r]{\strut{}\footnotesize{BRD-K66175015}}}%
      \put(1584,881){\makebox(0,0)[r]{\strut{}\footnotesize{BRD-M68452404}}}%
      \put(1584,1063){\makebox(0,0)[r]{\strut{}\footnotesize{BRD-M46138460}}}%
      \put(1584,1245){\makebox(0,0)[r]{\strut{}\footnotesize{BRD-K58550667}}}%
      \put(1584,1426){\makebox(0,0)[r]{\strut{}\footnotesize{BRD-K08177763}}}%
      \put(1584,1608){\makebox(0,0)[r]{\strut{}\footnotesize{BRD-A36630025}}}%
      \put(1584,1789){\makebox(0,0)[r]{\strut{}\footnotesize{BRD-K67844266}}}%
      \put(1898,389){\makebox(0,0){\strut{}1}}%
      \put(2261,389){\makebox(0,0){\strut{}2}}%
      \put(2624,389){\makebox(0,0){\strut{}3}}%
      \put(2987,389){\makebox(0,0){\strut{}4}}%
      \put(3350,389){\makebox(0,0){\strut{}5}}%
      \put(3713,389){\makebox(0,0){\strut{}6}}%
      \put(4076,389){\makebox(0,0){\strut{}7}}%
      \put(4439,389){\makebox(0,0){\strut{}8}}%
      \put(4802,389){\makebox(0,0){\strut{}9}}%
      \put(5165,389){\makebox(0,0){\strut{}10}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(154,1244){\rotatebox{90}{\makebox(0,0){\strut{}\small{drug ID}}}}%
      \put(3531,169){\makebox(0,0){\strut{}\small{latent dimension}}}%
      \csname LTb\endcsname%
      \put(5751,763){\makebox(0,0)[l]{\strut{}\footnotesize{-2}}}%
      \put(5751,1107){\makebox(0,0)[l]{\strut{}\footnotesize{0}}}%
      \put(5751,1450){\makebox(0,0)[l]{\strut{}\footnotesize{2}}}%
      \put(5751,1794){\makebox(0,0)[l]{\strut{}\footnotesize{4}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{mat_CAL51_insensitive}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/selected_cl/mat_CAL51_sensitive.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(6192.00,2160.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1584,700){\makebox(0,0)[r]{\strut{}\footnotesize{BRD-K62479592}}}%
      \put(1584,881){\makebox(0,0)[r]{\strut{}\footnotesize{BRD-K64890080}}}%
      \put(1584,1063){\makebox(0,0)[r]{\strut{}\footnotesize{BRD-K92093830}}}%
      \put(1584,1245){\makebox(0,0)[r]{\strut{}\footnotesize{BRD-K82109576}}}%
      \put(1584,1426){\makebox(0,0)[r]{\strut{}\footnotesize{BRD-A31107743}}}%
      \put(1584,1608){\makebox(0,0)[r]{\strut{}\footnotesize{BRD-K06792661}}}%
      \put(1584,1789){\makebox(0,0)[r]{\strut{}\footnotesize{BRD-K15108141}}}%
      \put(1898,389){\makebox(0,0){\strut{}1}}%
      \put(2261,389){\makebox(0,0){\strut{}2}}%
      \put(2624,389){\makebox(0,0){\strut{}3}}%
      \put(2987,389){\makebox(0,0){\strut{}4}}%
      \put(3350,389){\makebox(0,0){\strut{}5}}%
      \put(3713,389){\makebox(0,0){\strut{}6}}%
      \put(4076,389){\makebox(0,0){\strut{}7}}%
      \put(4439,389){\makebox(0,0){\strut{}8}}%
      \put(4802,389){\makebox(0,0){\strut{}9}}%
      \put(5165,389){\makebox(0,0){\strut{}10}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(154,1244){\rotatebox{90}{\makebox(0,0){\strut{}\small{drug ID}}}}%
      \put(3531,169){\makebox(0,0){\strut{}\small{latent dimension}}}%
      \csname LTb\endcsname%
      \put(5751,763){\makebox(0,0)[l]{\strut{}\footnotesize{-2}}}%
      \put(5751,1107){\makebox(0,0)[l]{\strut{}\footnotesize{0}}}%
      \put(5751,1450){\makebox(0,0)[l]{\strut{}\footnotesize{2}}}%
      \put(5751,1794){\makebox(0,0)[l]{\strut{}\footnotesize{4}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{mat_CAL51_sensitive}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plot/a_1_2prc_d_ap.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4030.00,2160.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(-99,704){\makebox(0,0)[r]{\strut{}\small{0.56}}}%
      \put(-99,1101){\makebox(0,0)[r]{\strut{}\small{0.59}}}%
      \put(-99,1366){\makebox(0,0)[r]{\strut{}\small{0.61}}}%
      \put(-99,1762){\makebox(0,0)[r]{\strut{}\small{0.64}}}%
      \put(-99,2159){\makebox(0,0)[r]{\strut{}\small{0.67}}}%
      \put(96,275){\makebox(0,0){\strut{}\small{5}}}%
      \put(1055,275){\makebox(0,0){\strut{}\small{10}}}%
      \put(2015,275){\makebox(0,0){\strut{}\small{15}}}%
      \put(2974,275){\makebox(0,0){\strut{}\small{30}}}%
      \put(3933,275){\makebox(0,0){\strut{}\small{50}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(-869,1299){\rotatebox{-270}{\makebox(0,0){\strut{}metric values}}}%
      \put(2014,0){\makebox(0,0){\strut{}$\alpha$}}%
      \csname LTb\endcsname%
      \put(792,1986){\makebox(0,0)[r]{\strut{}\scriptsize{AP@$5$}}}%
      \csname LTb\endcsname%
      \put(792,1766){\makebox(0,0)[r]{\strut{}\scriptsize{AP@$10$}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{a_1_2prc_d_ap}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plot/a_1_2prc_d_ci.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4030.00,2160.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(-99,440){\makebox(0,0)[r]{\strut{}\small{0.67}}}%
      \put(-99,870){\makebox(0,0)[r]{\strut{}\small{0.70}}}%
      \put(-99,1299){\makebox(0,0)[r]{\strut{}\small{0.73}}}%
      \put(-99,1729){\makebox(0,0)[r]{\strut{}\small{0.76}}}%
      \put(-99,2159){\makebox(0,0)[r]{\strut{}\small{0.79}}}%
      \put(96,275){\makebox(0,0){\strut{}\small{5}}}%
      \put(1055,275){\makebox(0,0){\strut{}\small{10}}}%
      \put(2015,275){\makebox(0,0){\strut{}\small{15}}}%
      \put(2974,275){\makebox(0,0){\strut{}\small{30}}}%
      \put(3933,275){\makebox(0,0){\strut{}\small{50}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(-869,1299){\rotatebox{-270}{\makebox(0,0){\strut{}metric values}}}%
      \put(2014,0){\makebox(0,0){\strut{}$\alpha$}}%
      \csname LTb\endcsname%
      \put(264,1986){\makebox(0,0)[r]{\strut{}\scriptsize{$\rCI$}}}%
      \csname LTb\endcsname%
      \put(264,1766){\makebox(0,0)[r]{\strut{}\scriptsize{$\CI$}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{a_1_2prc_d_ci}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plot/a_1_5prc_d_ap.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4030.00,2160.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(-99,440){\makebox(0,0)[r]{\strut{}\small{0.69}}}%
      \put(-99,784){\makebox(0,0)[r]{\strut{}\small{0.71}}}%
      \put(-99,1128){\makebox(0,0)[r]{\strut{}\small{0.73}}}%
      \put(-99,1471){\makebox(0,0)[r]{\strut{}\small{0.75}}}%
      \put(-99,1815){\makebox(0,0)[r]{\strut{}\small{0.77}}}%
      \put(-99,2159){\makebox(0,0)[r]{\strut{}\small{0.79}}}%
      \put(96,275){\makebox(0,0){\strut{}\small{0.00}}}%
      \put(1055,275){\makebox(0,0){\strut{}\small{0.05}}}%
      \put(2015,275){\makebox(0,0){\strut{}\small{0.10}}}%
      \put(2974,275){\makebox(0,0){\strut{}\small{0.50}}}%
      \put(3933,275){\makebox(0,0){\strut{}\small{1.00}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(-869,1299){\rotatebox{-270}{\makebox(0,0){\strut{}metric values}}}%
      \put(2014,0){\makebox(0,0){\strut{}$\alpha$}}%
      \csname LTb\endcsname%
      \put(792,1986){\makebox(0,0)[r]{\strut{}\scriptsize{AP@$5$}}}%
      \csname LTb\endcsname%
      \put(792,1766){\makebox(0,0)[r]{\strut{}\scriptsize{AP@$10$}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{a_1_5prc_d_ap}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plot/a_1_5prc_d_ci.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4030.00,2160.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(-99,440){\makebox(0,0)[r]{\strut{}\small{0.67}}}%
      \put(-99,1013){\makebox(0,0)[r]{\strut{}\small{0.70}}}%
      \put(-99,1586){\makebox(0,0)[r]{\strut{}\small{0.73}}}%
      \put(-99,2159){\makebox(0,0)[r]{\strut{}\small{0.76}}}%
      \put(96,275){\makebox(0,0){\strut{}\small{5}}}%
      \put(1055,275){\makebox(0,0){\strut{}\small{10}}}%
      \put(2015,275){\makebox(0,0){\strut{}\small{15}}}%
      \put(2974,275){\makebox(0,0){\strut{}\small{30}}}%
      \put(3933,275){\makebox(0,0){\strut{}\small{50}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(-869,1299){\rotatebox{-270}{\makebox(0,0){\strut{}metric values}}}%
      \put(2014,0){\makebox(0,0){\strut{}$\alpha$}}%
      \csname LTb\endcsname%
      \put(264,1986){\makebox(0,0)[r]{\strut{}\scriptsize{$\rCI$}}}%
      \csname LTb\endcsname%
      \put(264,1766){\makebox(0,0)[r]{\strut{}\scriptsize{$\CI$}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{a_1_5prc_d_ci}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plot/backup/plot_holdout_2prc.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(2880.00,2160.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(-132,440){\makebox(0,0)[r]{\strut{}\small{0.72}}}%
      \put(-132,870){\makebox(0,0)[r]{\strut{}\small{0.75}}}%
      \put(-132,1300){\makebox(0,0)[r]{\strut{}\small{0.78}}}%
      \put(-132,1729){\makebox(0,0)[r]{\strut{}\small{0.81}}}%
      \put(-132,2159){\makebox(0,0)[r]{\strut{}\small{0.84}}}%
      \put(148,220){\makebox(0,0){\strut{}\small{50}}}%
      \put(517,220){\makebox(0,0){\strut{}\small{100}}}%
      \put(886,220){\makebox(0,0){\strut{}\small{150}}}%
      \put(1255,220){\makebox(0,0){\strut{}\small{200}}}%
      \put(1624,220){\makebox(0,0){\strut{}\small{250}}}%
      \put(1993,220){\makebox(0,0){\strut{}\small{300}}}%
      \put(2362,220){\makebox(0,0){\strut{}\small{350}}}%
      \put(2731,220){\makebox(0,0){\strut{}\small{400}}}%
      \put(3011,440){\makebox(0,0)[l]{\strut{}\small{0.59}}}%
      \put(3011,870){\makebox(0,0)[l]{\strut{}\small{0.63}}}%
      \put(3011,1300){\makebox(0,0)[l]{\strut{}\small{0.67}}}%
      \put(3011,1729){\makebox(0,0)[l]{\strut{}\small{0.71}}}%
      \put(3011,2159){\makebox(0,0)[l]{\strut{}\small{0.75}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(-704,1299){\rotatebox{-270}{\makebox(0,0){\strut{}\small{AP@$5$}/\small{AP@$10$}}}}%
      \put(3582,1299){\rotatebox{-270}{\makebox(0,0){\strut{}\small{$\rCI$}/\small{$\CI$}}}}%
      \put(1439,0){\makebox(0,0){\strut{}$\alpha$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{plot_holdout_2prc}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plot/backup/plot_holdout_5prc.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(2880.00,2160.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(-132,440){\makebox(0,0)[r]{\strut{}\small{0.86}}}%
      \put(-132,870){\makebox(0,0)[r]{\strut{}\small{0.88}}}%
      \put(-132,1300){\makebox(0,0)[r]{\strut{}\small{0.90}}}%
      \put(-132,1729){\makebox(0,0)[r]{\strut{}\small{0.92}}}%
      \put(-132,2159){\makebox(0,0)[r]{\strut{}\small{0.94}}}%
      \put(148,220){\makebox(0,0){\strut{}\small{50}}}%
      \put(517,220){\makebox(0,0){\strut{}\small{100}}}%
      \put(886,220){\makebox(0,0){\strut{}\small{150}}}%
      \put(1255,220){\makebox(0,0){\strut{}\small{200}}}%
      \put(1624,220){\makebox(0,0){\strut{}\small{250}}}%
      \put(1993,220){\makebox(0,0){\strut{}\small{300}}}%
      \put(2362,220){\makebox(0,0){\strut{}\small{350}}}%
      \put(2731,220){\makebox(0,0){\strut{}\small{400}}}%
      \put(3011,440){\makebox(0,0)[l]{\strut{}\small{0.64}}}%
      \put(3011,784){\makebox(0,0)[l]{\strut{}\small{0.66}}}%
      \put(3011,1128){\makebox(0,0)[l]{\strut{}\small{0.68}}}%
      \put(3011,1471){\makebox(0,0)[l]{\strut{}\small{0.70}}}%
      \put(3011,1815){\makebox(0,0)[l]{\strut{}\small{0.72}}}%
      \put(3011,2159){\makebox(0,0)[l]{\strut{}\small{0.74}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(-704,1299){\rotatebox{-270}{\makebox(0,0){\strut{}\small{AP@$5$}/\small{AP@$10$}}}}%
      \put(3582,1299){\rotatebox{-270}{\makebox(0,0){\strut{}\small{$\rCI$}/\small{$\CI$}}}}%
      \put(1439,0){\makebox(0,0){\strut{}$\alpha$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{plot_holdout_5prc}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plot/backup/plot_holdout_baseline_2prc.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(2880.00,2160.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(-132,440){\makebox(0,0)[r]{\strut{}\small{0.72}}}%
      \put(-132,870){\makebox(0,0)[r]{\strut{}\small{0.75}}}%
      \put(-132,1300){\makebox(0,0)[r]{\strut{}\small{0.78}}}%
      \put(-132,1729){\makebox(0,0)[r]{\strut{}\small{0.81}}}%
      \put(-132,2159){\makebox(0,0)[r]{\strut{}\small{0.84}}}%
      \put(148,220){\makebox(0,0){\strut{}\small{50}}}%
      \put(517,220){\makebox(0,0){\strut{}\small{100}}}%
      \put(886,220){\makebox(0,0){\strut{}\small{150}}}%
      \put(1255,220){\makebox(0,0){\strut{}\small{200}}}%
      \put(1624,220){\makebox(0,0){\strut{}\small{250}}}%
      \put(1993,220){\makebox(0,0){\strut{}\small{300}}}%
      \put(2362,220){\makebox(0,0){\strut{}\small{350}}}%
      \put(2731,220){\makebox(0,0){\strut{}\small{400}}}%
      \put(3011,440){\makebox(0,0)[l]{\strut{}\small{0.60}}}%
      \put(3011,1013){\makebox(0,0)[l]{\strut{}\small{0.67}}}%
      \put(3011,1586){\makebox(0,0)[l]{\strut{}\small{0.74}}}%
      \put(3011,2159){\makebox(0,0)[l]{\strut{}\small{0.81}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(-704,1299){\rotatebox{-270}{\makebox(0,0){\strut{}\small{AP@$5$}/\small{AP@$10$}}}}%
      \put(3582,1299){\rotatebox{-270}{\makebox(0,0){\strut{}\small{$\rCI$}/\small{$\CI$}}}}%
      \put(1439,0){\makebox(0,0){\strut{}$\alpha$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{plot_holdout_baseline_2prc}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plot/backup/plot_holdout_baseline_5prc.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(2880.00,2160.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(-132,440){\makebox(0,0)[r]{\strut{}\small{0.85}}}%
      \put(-132,956){\makebox(0,0)[r]{\strut{}\small{0.88}}}%
      \put(-132,1471){\makebox(0,0)[r]{\strut{}\small{0.91}}}%
      \put(-132,1987){\makebox(0,0)[r]{\strut{}\small{0.94}}}%
      \put(148,220){\makebox(0,0){\strut{}\small{50}}}%
      \put(517,220){\makebox(0,0){\strut{}\small{100}}}%
      \put(886,220){\makebox(0,0){\strut{}\small{150}}}%
      \put(1255,220){\makebox(0,0){\strut{}\small{200}}}%
      \put(1624,220){\makebox(0,0){\strut{}\small{250}}}%
      \put(1993,220){\makebox(0,0){\strut{}\small{300}}}%
      \put(2362,220){\makebox(0,0){\strut{}\small{350}}}%
      \put(2731,220){\makebox(0,0){\strut{}\small{400}}}%
      \put(3011,440){\makebox(0,0)[l]{\strut{}\small{0.63}}}%
      \put(3011,1013){\makebox(0,0)[l]{\strut{}\small{0.69}}}%
      \put(3011,1586){\makebox(0,0)[l]{\strut{}\small{0.75}}}%
      \put(3011,2159){\makebox(0,0)[l]{\strut{}\small{0.81}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(-704,1299){\rotatebox{-270}{\makebox(0,0){\strut{}\small{AP@$5$}/\small{AP@$10$}}}}%
      \put(3582,1299){\rotatebox{-270}{\makebox(0,0){\strut{}\small{$\rCI$}/\small{$\CI$}}}}%
      \put(1439,0){\makebox(0,0){\strut{}$\alpha$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{plot_holdout_baseline_5prc}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plot/d_15_5prc_legend.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,720.00)%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(2744,492){\makebox(0,0)[r]{\strut{}AP@$5$}}%
      \csname LTb\endcsname%
      \put(4391,492){\makebox(0,0)[r]{\strut{}AP@$10$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{d_15_5prc_legend}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plot/plot_2prc_ap_eval.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(-99,788){\makebox(0,0)[r]{\strut{}0.73}}%
      \put(-99,1485){\makebox(0,0)[r]{\strut{}0.75}}%
      \put(-99,2182){\makebox(0,0)[r]{\strut{}0.77}}%
      \put(-99,2879){\makebox(0,0)[r]{\strut{}0.79}}%
      \put(393,275){\makebox(0,0){\strut{}\small{\hspace{-5pt}5}}}%
      \put(785,275){\makebox(0,0){\strut{}\small{\hspace{-5pt}10}}}%
      \put(1178,275){\makebox(0,0){\strut{}\small{15}}}%
      \put(2356,275){\makebox(0,0){\strut{}\small{30}}}%
      \put(3926,275){\makebox(0,0){\strut{}\small{50}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(-737,1659){\rotatebox{-270}{\makebox(0,0){\strut{}metric values}}}%
      \put(2159,0){\makebox(0,0){\strut{}latent dimension $d$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{plot_2prc_ap_eval}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plot/plot_2prc_ci_eval.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(-99,440){\makebox(0,0)[r]{\strut{}\small{0.63}}}%
      \put(-99,1003){\makebox(0,0)[r]{\strut{}\small{0.66}}}%
      \put(-99,1566){\makebox(0,0)[r]{\strut{}\small{0.69}}}%
      \put(-99,2316){\makebox(0,0)[r]{\strut{}\small{0.78}}}%
      \put(-99,2504){\makebox(0,0)[r]{\strut{}\small{0.79}}}%
      \put(-99,2691){\makebox(0,0)[r]{\strut{}\small{0.80}}}%
      \put(-99,2879){\makebox(0,0)[r]{\strut{}\small{0.81}}}%
      \put(393,275){\makebox(0,0){\strut{}\small{\hspace{-5pt}5}}}%
      \put(785,275){\makebox(0,0){\strut{}\small{\hspace{-5pt}10}}}%
      \put(1178,275){\makebox(0,0){\strut{}\small{15}}}%
      \put(2356,275){\makebox(0,0){\strut{}\small{30}}}%
      \put(3926,275){\makebox(0,0){\strut{}\small{50}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(-869,1659){\rotatebox{-270}{\makebox(0,0){\strut{}metric values}}}%
      \put(2159,0){\makebox(0,0){\strut{}latent dimension $d$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{plot_2prc_ci_eval}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plot/plot_2prc_eval.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(2160.00,4320.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(-99,0){\makebox(0,0)[r]{\strut{}\small{0.70}}}%
      \put(-99,864){\makebox(0,0)[r]{\strut{}\small{0.72}}}%
      \put(-99,1728){\makebox(0,0)[r]{\strut{}\small{0.74}}}%
      \put(-99,2591){\makebox(0,0)[r]{\strut{}\small{0.76}}}%
      \put(-99,3455){\makebox(0,0)[r]{\strut{}\small{0.78}}}%
      \put(-99,4319){\makebox(0,0)[r]{\strut{}\small{0.80}}}%
      \put(196,-165){\makebox(0,0){\strut{}\small{\hspace{-5pt}5}}}%
      \put(393,-165){\makebox(0,0){\strut{}\small{\hspace{-5pt}10}}}%
      \put(589,-165){\makebox(0,0){\strut{}\small{15}}}%
      \put(1178,-165){\makebox(0,0){\strut{}\small{30}}}%
      \put(1963,-165){\makebox(0,0){\strut{}\small{50}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(-869,2159){\rotatebox{-270}{\makebox(0,0){\strut{}metric values}}}%
      \put(1079,-440){\makebox(0,0){\strut{}latent dimension $d$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{plot_2prc_eval}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plot/plot_5prc_ap_eval.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(-99,440){\makebox(0,0)[r]{\strut{}\small{0.78}}}%
      \put(-99,1050){\makebox(0,0)[r]{\strut{}\small{0.80}}}%
      \put(-99,1659){\makebox(0,0)[r]{\strut{}\small{0.82}}}%
      \put(-99,2269){\makebox(0,0)[r]{\strut{}\small{0.84}}}%
      \put(-99,2879){\makebox(0,0)[r]{\strut{}\small{0.86}}}%
      \put(393,275){\makebox(0,0){\strut{}\small{\hspace{-5pt}5}}}%
      \put(785,275){\makebox(0,0){\strut{}\small{\hspace{-5pt}10}}}%
      \put(1178,275){\makebox(0,0){\strut{}\small{15}}}%
      \put(2356,275){\makebox(0,0){\strut{}\small{30}}}%
      \put(3926,275){\makebox(0,0){\strut{}\small{50}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(-869,1659){\rotatebox{-270}{\makebox(0,0){\strut{}metric values}}}%
      \put(2159,0){\makebox(0,0){\strut{}latent dimension $d$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{plot_5prc_ap_eval}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plot/plot_5prc_ci_eval.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4320.00,2880.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(-99,440){\makebox(0,0)[r]{\strut{}\small{0.63}}}%
      \put(-99,1050){\makebox(0,0)[r]{\strut{}\small{0.68}}}%
      \put(-99,1660){\makebox(0,0)[r]{\strut{}\small{0.73}}}%
      \put(-99,2269){\makebox(0,0)[r]{\strut{}\small{0.78}}}%
      \put(-99,2879){\makebox(0,0)[r]{\strut{}\small{0.83}}}%
      \put(393,275){\makebox(0,0){\strut{}\small{\hspace{-5pt}5}}}%
      \put(785,275){\makebox(0,0){\strut{}\small{\hspace{-5pt}10}}}%
      \put(1178,275){\makebox(0,0){\strut{}\small{15}}}%
      \put(2356,275){\makebox(0,0){\strut{}\small{30}}}%
      \put(3926,275){\makebox(0,0){\strut{}\small{50}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(-869,1659){\rotatebox{-270}{\makebox(0,0){\strut{}metric values}}}%
      \put(2159,0){\makebox(0,0){\strut{}latent dimension $d$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{plot_5prc_ci_eval}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plot/plot_5prc_eval.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(2160.00,4320.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(-99,0){\makebox(0,0)[r]{\strut{}\small{0.63}}}%
      \put(-99,864){\makebox(0,0)[r]{\strut{}\small{0.68}}}%
      \put(-99,1728){\makebox(0,0)[r]{\strut{}\small{0.73}}}%
      \put(-99,2591){\makebox(0,0)[r]{\strut{}\small{0.78}}}%
      \put(-99,3455){\makebox(0,0)[r]{\strut{}\small{0.83}}}%
      \put(-99,4319){\makebox(0,0)[r]{\strut{}\small{0.88}}}%
      \put(196,-165){\makebox(0,0){\strut{}\small{\hspace{-5pt}5}}}%
      \put(393,-165){\makebox(0,0){\strut{}\small{\hspace{-5pt}10}}}%
      \put(589,-165){\makebox(0,0){\strut{}\small{15}}}%
      \put(1178,-165){\makebox(0,0){\strut{}\small{30}}}%
      \put(1963,-165){\makebox(0,0){\strut{}\small{50}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(-869,2159){\rotatebox{-270}{\makebox(0,0){\strut{}metric values}}}%
      \put(1079,-440){\makebox(0,0){\strut{}latent dimension $d$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{plot_5prc_eval}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plot/plot_gene_latent_sim.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(3888.00,2520.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,594){\makebox(0,0)[r]{\strut{}\scriptsize{0.30}}}%
      \put(858,831){\makebox(0,0)[r]{\strut{}\scriptsize{0.40}}}%
      \put(858,1069){\makebox(0,0)[r]{\strut{}\scriptsize{0.50}}}%
      \put(858,1306){\makebox(0,0)[r]{\strut{}\scriptsize{0.60}}}%
      \put(858,1544){\makebox(0,0)[r]{\strut{}\scriptsize{0.70}}}%
      \put(858,1781){\makebox(0,0)[r]{\strut{}\scriptsize{0.80}}}%
      \put(858,2019){\makebox(0,0)[r]{\strut{}\scriptsize{0.90}}}%
      \put(858,2256){\makebox(0,0)[r]{\strut{}\scriptsize{1.00}}}%
      \put(990,484){\makebox(0,0){\strut{}\scriptsize{0.90}}}%
      \put(1490,484){\makebox(0,0){\strut{}\scriptsize{0.92}}}%
      \put(1990,484){\makebox(0,0){\strut{}\scriptsize{0.94}}}%
      \put(2491,484){\makebox(0,0){\strut{}\scriptsize{0.96}}}%
      \put(2991,484){\makebox(0,0){\strut{}\scriptsize{0.98}}}%
      \put(3491,484){\makebox(0,0){\strut{}\scriptsize{1.00}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(220,1425){\rotatebox{-270}{\makebox(0,0){\strut{}latent similarity}}}%
      \put(2240,154){\makebox(0,0){\strut{}gene expression similarity}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{plot_gene_latent_sim}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plot/plot_holdout_2prc.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(2880.00,2160.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(-132,686){\makebox(0,0)[r]{\strut{}\small{0.61}}}%
      \put(-132,1177){\makebox(0,0)[r]{\strut{}\small{0.63}}}%
      \put(-132,1668){\makebox(0,0)[r]{\strut{}\small{0.65}}}%
      \put(-132,2159){\makebox(0,0)[r]{\strut{}\small{0.67}}}%
      \put(148,220){\makebox(0,0){\strut{}\small{50}}}%
      \put(517,220){\makebox(0,0){\strut{}\small{100}}}%
      \put(886,220){\makebox(0,0){\strut{}\small{150}}}%
      \put(1255,220){\makebox(0,0){\strut{}\small{200}}}%
      \put(1624,220){\makebox(0,0){\strut{}\small{250}}}%
      \put(1993,220){\makebox(0,0){\strut{}\small{300}}}%
      \put(2362,220){\makebox(0,0){\strut{}\small{350}}}%
      \put(2731,220){\makebox(0,0){\strut{}\small{400}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(-704,1299){\rotatebox{-270}{\makebox(0,0){\strut{}\small{$\rCI$}}}}%
      \put(1439,0){\makebox(0,0){\strut{}$\holdoutsize$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{plot_holdout_2prc}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plot/plot_holdout_5prc.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(2880.00,2160.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(-132,440){\makebox(0,0)[r]{\strut{}\small{0.58}}}%
      \put(-132,870){\makebox(0,0)[r]{\strut{}\small{0.64}}}%
      \put(-132,1300){\makebox(0,0)[r]{\strut{}\small{0.70}}}%
      \put(-132,1729){\makebox(0,0)[r]{\strut{}\small{0.76}}}%
      \put(-132,2159){\makebox(0,0)[r]{\strut{}\small{0.82}}}%
      \put(148,220){\makebox(0,0){\strut{}\small{50}}}%
      \put(517,220){\makebox(0,0){\strut{}\small{100}}}%
      \put(886,220){\makebox(0,0){\strut{}\small{150}}}%
      \put(1255,220){\makebox(0,0){\strut{}\small{200}}}%
      \put(1624,220){\makebox(0,0){\strut{}\small{250}}}%
      \put(1993,220){\makebox(0,0){\strut{}\small{300}}}%
      \put(2362,220){\makebox(0,0){\strut{}\small{350}}}%
      \put(2731,220){\makebox(0,0){\strut{}\small{400}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(-704,1299){\rotatebox{-270}{\makebox(0,0){\strut{}\small{$\CI$}}}}%
      \put(1439,0){\makebox(0,0){\strut{}$\holdoutsize$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{plot_holdout_5prc}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plot/plot_holdout_baseline_2prc.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(2880.00,2160.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(-132,440){\makebox(0,0)[r]{\strut{}\small{0.81}}}%
      \put(-132,870){\makebox(0,0)[r]{\strut{}\small{0.85}}}%
      \put(-132,1300){\makebox(0,0)[r]{\strut{}\small{0.89}}}%
      \put(-132,1729){\makebox(0,0)[r]{\strut{}\small{0.93}}}%
      \put(-132,2159){\makebox(0,0)[r]{\strut{}\small{0.97}}}%
      \put(148,220){\makebox(0,0){\strut{}\small{50}}}%
      \put(517,220){\makebox(0,0){\strut{}\small{100}}}%
      \put(886,220){\makebox(0,0){\strut{}\small{150}}}%
      \put(1255,220){\makebox(0,0){\strut{}\small{200}}}%
      \put(1624,220){\makebox(0,0){\strut{}\small{250}}}%
      \put(1993,220){\makebox(0,0){\strut{}\small{300}}}%
      \put(2362,220){\makebox(0,0){\strut{}\small{350}}}%
      \put(2731,220){\makebox(0,0){\strut{}\small{400}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(-704,1299){\rotatebox{-270}{\makebox(0,0){\strut{}\small{AP@$5$}}}}%
      \put(1439,0){\makebox(0,0){\strut{}$\holdoutsize$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{plot_holdout_baseline_2prc}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plot/plot_holdout_baseline_5prc.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(2880.00,2160.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(-132,440){\makebox(0,0)[r]{\strut{}\small{0.75}}}%
      \put(-132,727){\makebox(0,0)[r]{\strut{}\small{0.78}}}%
      \put(-132,1013){\makebox(0,0)[r]{\strut{}\small{0.81}}}%
      \put(-132,1777){\makebox(0,0)[r]{\strut{}\small{0.89}}}%
      \put(-132,1968){\makebox(0,0)[r]{\strut{}\small{0.91}}}%
      \put(-132,2159){\makebox(0,0)[r]{\strut{}\small{0.93}}}%
      \put(148,220){\makebox(0,0){\strut{}\small{50}}}%
      \put(517,220){\makebox(0,0){\strut{}\small{100}}}%
      \put(886,220){\makebox(0,0){\strut{}\small{150}}}%
      \put(1255,220){\makebox(0,0){\strut{}\small{200}}}%
      \put(1624,220){\makebox(0,0){\strut{}\small{250}}}%
      \put(1993,220){\makebox(0,0){\strut{}\small{300}}}%
      \put(2362,220){\makebox(0,0){\strut{}\small{350}}}%
      \put(2731,220){\makebox(0,0){\strut{}\small{400}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(-704,1299){\rotatebox{-270}{\makebox(0,0){\strut{}\small{AP@$10$}}}}%
      \put(1439,0){\makebox(0,0){\strut{}$\holdoutsize$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{plot_holdout_baseline_5prc}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plot/plot_holdout_legend.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(10080.00,1152.00)%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(1877,924){\makebox(0,0)[r]{\strut{}\small{\BMTMKL($\theta=2$)}}}%
      \csname LTb\endcsname%
      \put(4184,924){\makebox(0,0)[r]{\strut{}\small{\MTCRP($\theta=2$)}}}%
      \csname LTb\endcsname%
      \put(6491,924){\makebox(0,0)[r]{\strut{}\small{\BMTMKL($\theta=5$)}}}%
      \csname LTb\endcsname%
      \put(8798,924){\makebox(0,0)[r]{\strut{}\small{\MTCRP($\theta=5$)}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{plot_holdout_legend}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plot/plot_sim_corr.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(8928.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(-132,2640){\makebox(0,0)[r]{\strut{}\small{0.0}}}%
      \csname LTb\endcsname%
      \put(-132,3068){\makebox(0,0)[r]{\strut{}\small{0.2}}}%
      \csname LTb\endcsname%
      \put(-132,3497){\makebox(0,0)[r]{\strut{}\small{0.4}}}%
      \csname LTb\endcsname%
      \put(-132,3925){\makebox(0,0)[r]{\strut{}\small{0.6}}}%
      \csname LTb\endcsname%
      \put(-132,4354){\makebox(0,0)[r]{\strut{}\small{0.8}}}%
      \csname LTb\endcsname%
      \put(-132,4782){\makebox(0,0)[r]{\strut{}\small{1.0}}}%
      \put(235,2508){\rotatebox{90}{\makebox(0,0)[r]{\strut{}melanoma (51)}}}%
      \put(470,2508){\rotatebox{90}{\makebox(0,0)[r]{\strut{}lung nsc (99)}}}%
      \put(705,2508){\rotatebox{90}{\makebox(0,0)[r]{\strut{}colorectal (47)}}}%
      \put(940,2508){\rotatebox{90}{\makebox(0,0)[r]{\strut{}lung small cell (38)}}}%
      \put(1175,2508){\rotatebox{90}{\makebox(0,0)[r]{\strut{}breast (39)}}}%
      \put(1410,2508){\rotatebox{90}{\makebox(0,0)[r]{\strut{}pancreas (38)}}}%
      \put(1644,2508){\rotatebox{90}{\makebox(0,0)[r]{\strut{}ewings sarcoma (8)}}}%
      \put(1879,2508){\rotatebox{90}{\makebox(0,0)[r]{\strut{}n/a (29)}}}%
      \put(2114,2508){\rotatebox{90}{\makebox(0,0)[r]{\strut{}stomach (32)}}}%
      \put(2349,2508){\rotatebox{90}{\makebox(0,0)[r]{\strut{}glioma (41)}}}%
      \put(2584,2508){\rotatebox{90}{\makebox(0,0)[r]{\strut{}ovary (35)}}}%
      \put(2819,2508){\rotatebox{90}{\makebox(0,0)[r]{\strut{}neuroblastoma (15)}}}%
      \put(3054,2508){\rotatebox{90}{\makebox(0,0)[r]{\strut{}lymphoma other (26)}}}%
      \put(3289,2508){\rotatebox{90}{\makebox(0,0)[r]{\strut{}aml (29)}}}%
      \put(3524,2508){\rotatebox{90}{\makebox(0,0)[r]{\strut{}lymphoma dlbcl (15)}}}%
      \put(3759,2508){\rotatebox{90}{\makebox(0,0)[r]{\strut{}esophagus (23)}}}%
      \put(3994,2508){\rotatebox{90}{\makebox(0,0)[r]{\strut{}endometrium (25)}}}%
      \put(4229,2508){\rotatebox{90}{\makebox(0,0)[r]{\strut{}upper aerodigestive (28)}}}%
      \put(4464,2508){\rotatebox{90}{\makebox(0,0)[r]{\strut{}liver (22)}}}%
      \put(4698,2508){\rotatebox{90}{\makebox(0,0)[r]{\strut{}bcell all (8)}}}%
      \put(4933,2508){\rotatebox{90}{\makebox(0,0)[r]{\strut{}urinary tract (21)}}}%
      \put(5168,2508){\rotatebox{90}{\makebox(0,0)[r]{\strut{}lymphoma hodgkin (8)}}}%
      \put(5403,2508){\rotatebox{90}{\makebox(0,0)[r]{\strut{}tcell all (12)}}}%
      \put(5638,2508){\rotatebox{90}{\makebox(0,0)[r]{\strut{}soft tissue (15)}}}%
      \put(5873,2508){\rotatebox{90}{\makebox(0,0)[r]{\strut{}kidney (19)}}}%
      \put(6108,2508){\rotatebox{90}{\makebox(0,0)[r]{\strut{}multiple myeloma (26)}}}%
      \put(6343,2508){\rotatebox{90}{\makebox(0,0)[r]{\strut{}mesothelioma (8)}}}%
      \put(6578,2508){\rotatebox{90}{\makebox(0,0)[r]{\strut{}cml (12)}}}%
      \put(6813,2508){\rotatebox{90}{\makebox(0,0)[r]{\strut{}bile duct (7)}}}%
      \put(7048,2508){\rotatebox{90}{\makebox(0,0)[r]{\strut{}lymphoma burkitt (10)}}}%
      \put(7283,2508){\rotatebox{90}{\makebox(0,0)[r]{\strut{}leukemia other (5)}}}%
      \put(7517,2508){\rotatebox{90}{\makebox(0,0)[r]{\strut{}thyroid (10)}}}%
      \put(7752,2508){\rotatebox{90}{\makebox(0,0)[r]{\strut{}prostate (6)}}}%
      \put(7987,2508){\rotatebox{90}{\makebox(0,0)[r]{\strut{}osteosarcoma (6)}}}%
      \put(8222,2508){\rotatebox{90}{\makebox(0,0)[r]{\strut{}other (3)}}}%
      \put(8457,2508){\rotatebox{90}{\makebox(0,0)[r]{\strut{}medulloblastoma (3)}}}%
      \put(8692,2508){\rotatebox{90}{\makebox(0,0)[r]{\strut{}chondrosarcoma (2)}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(-572,3839){\rotatebox{-270}{\makebox(0,0){\strut{}correlation}}}%
      \csname LTb\endcsname%
      \put(4548,4886){\makebox(0,0)[r]{\strut{}gene expression vs drug sensitivity (\gd)}}%
      \csname LTb\endcsname%
      \put(4548,4666){\makebox(0,0)[r]{\strut{}gene expression vs latent vector\textcolor{white}{aaa} (\gl)}}%
      \csname LTb\endcsname%
      \put(4548,4446){\makebox(0,0)[r]{\strut{}latent vector vs drug sensitivity (\ld)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{plot_sim_corr}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plot/trans_a_05_2prc_d_top.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(3600.00,2160.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(-99,440){\makebox(0,0)[r]{\strut{}\small{45}}}%
      \put(-99,1013){\makebox(0,0)[r]{\strut{}\small{55}}}%
      \put(-99,1586){\makebox(0,0)[r]{\strut{}\small{65}}}%
      \put(-99,2159){\makebox(0,0)[r]{\strut{}\small{75}}}%
      \put(86,275){\makebox(0,0){\strut{}\small{5}}}%
      \put(943,275){\makebox(0,0){\strut{}\small{10}}}%
      \put(1800,275){\makebox(0,0){\strut{}\small{15}}}%
      \put(2656,275){\makebox(0,0){\strut{}\small{30}}}%
      \put(3513,275){\makebox(0,0){\strut{}\small{50}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(-605,1299){\rotatebox{-270}{\makebox(0,0){\strut{}AT@$5$/@$10$\%}}}%
      \put(1799,0){\makebox(0,0){\strut{}latent dimension d}}%
      \csname LTb\endcsname%
      \put(660,1986){\makebox(0,0)[r]{\strut{}\scriptsize{AT@$5$\%}}}%
      \csname LTb\endcsname%
      \put(660,1766){\makebox(0,0)[r]{\strut{}\scriptsize{AT@$10$\%}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{trans_a_05_2prc_d_top}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plot/trans_a_1_5prc_d_top.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(3600.00,2160.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(-99,440){\makebox(0,0)[r]{\strut{}\small{50}}}%
      \put(-99,1013){\makebox(0,0)[r]{\strut{}\small{60}}}%
      \put(-99,1586){\makebox(0,0)[r]{\strut{}\small{70}}}%
      \put(-99,2159){\makebox(0,0)[r]{\strut{}\small{80}}}%
      \put(86,275){\makebox(0,0){\strut{}\small{5}}}%
      \put(943,275){\makebox(0,0){\strut{}\small{10}}}%
      \put(1800,275){\makebox(0,0){\strut{}\small{15}}}%
      \put(2656,275){\makebox(0,0){\strut{}\small{30}}}%
      \put(3513,275){\makebox(0,0){\strut{}\small{50}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(-605,1299){\rotatebox{-270}{\makebox(0,0){\strut{}AT@$5$/@$10$\%}}}%
      \put(1799,0){\makebox(0,0){\strut{}latent dimension d}}%
      \csname LTb\endcsname%
      \put(660,1986){\makebox(0,0)[r]{\strut{}\scriptsize{AT@$5$\%}}}%
      \csname LTb\endcsname%
      \put(660,1766){\makebox(0,0)[r]{\strut{}\scriptsize{AT@$10$\%}}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{trans_a_1_5prc_d_top}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> relatedWork.tex <==
%**********************************************************************************************%
%\subsection{Drug Selection}
%\label{sec:background:review:ds}
%**********************************************************************************************%

\begin{comment}
% categorization
Current computational efforts for precision cancer drug selection %~\cite{Niz2016}
are primarily focused on using regression methods (e.g., random forests~\cite{Haider2015},
%kernel based methods~\cite{Gonen2012},
ridge regression~\cite{Geeleher2014},
and deep neural networks~\cite{Dahl2014}) to predict drug response values numerically,
and then selecting drugs of optimal response values in each cell line~\cite{Costello2014}, 
%
\end{comment}
\begin{comment}
For example, in Menden \emph{et al.}~\cite{Menden2013},
cell line features (e.g., sequence variation, copy number variation) and drug
features (e.g., physicochemical properties) are jointly used to train a neural
network that predicts drug IC$_{50}$%~\cite{IC50}
values. % in a cell line.
\end{comment}
\begin{comment}
%
%Similarly, Dahl \etal~\cite{Dahl2014} used multi-task deep nerual networks to predict drug
%sensitivity.
%Other popular regression methods in drug selection include random
%forests~\cite{Haider2015}, kernel based methods~\cite{Gonen2012},
%ridge regression~\cite{Geeleher2014},
%deep nerual networks~\cite{Dahl2014}, etc. 
%
%
%Another focus of the existing methods is on effectively using omics information on
with omics information on
cell lines and features on drugs leveraged to improve regression~\cite{Hejase2015, Jang2014}.
%, Gonen2012
% to improve the
%regression~\cite{Hejase2015, Gonen2012, Jang2014}. % and classification
%
\end{comment}
\begin{comment}
For example, in Ammad-ud-din \emph{et al.}~\cite{Ammad2014}, a kernel is constructed
on each type of drug and cell line features to measure their respective similarities,
and drug sensitivity is predicted from the combination of projected drug kernels and cell
line kernels.
\end{comment}
%
\begin{comment}
These regression based methods for drug selection may suffer from the fact that
their accuracy is largely affected by non-effective drugs, which constitute
the majority of drugs, 
and therefore, accurate drug response regression does not necessarily lead to
accurate drug prioritization.
%
%
Instead, learning-to-rank (\LETOR)
methods represent a more natural and effective alternative that directly prioritizes drugs.
Actually, regression based drug selection corresponds to point-wise learning to
rank~\cite{Liu2009}, %{Li2011,Liu2009}, %~\cite{Furnkranz2010,Li2011,Liu2009},
which has been demonstrated~\cite{Cao2007} to perform
suboptimally compared to pairwise~\cite{Burges2007} and listwise ranking
methods~\cite{Lebanon2002}. 
%
\end{comment}


%**********************************************************************************************%
%\subsection{Learning to Rank}
%\label{sec:background:review:ltr}
%**********************************************************************************************%

%Two lines of research in Computer Science are highly related:  
%Learning to Rank (\LETOR) and Collaborative Filtering (\CF). 
%
%The most relevant research areas to the work in this paper include learning to rank (\LETOR). 
%
Learning to Rank (\LETOR)~\cite{Furnkranz2010} 
focuses on developing machine learning methods and models that can produce accurate rankings of
interested instances,
rather than using pre-defined scoring functions to sort the instances. 
%
\LETOR is the key enabling 
technique in information retrieval~\cite{Li2011}.
%
Existing \LETOR methods fall into three categories:  
1). pointwise methods~\cite{Cao2007}, which learn a score on each individual instance that
will be used to sort/rank all the instances; 
%
2). pairwise methods~\cite{Burges2007}, which optimize
pairwise ranking orders among all instances to induce good ranking orders among
the instances; and
%
3) listwise methods~\cite{Lebanon2002}, which model the full
combinatorial structures of ranking lists.
%
It has been demonstrated~\cite{Cao2007} that 
pairwise and listwise ranking methods outperform pointwise methods in general.
%
This is because in pairwise and listwise methods, the ordering structures among
instances are leveraged in learning, whereas in pointwise methods, no ordering information is used.
%
Moreover, listwise methods are more computationally challenging than the others,
due to the combinatorial nature of ranking lists as a whole.
%
Thus, pairwise methods are the choice in many ranking problems, given the trade-off
between ranking performance and computational demands. 


%
The idea of using \LETOR approaches to prioritize compounds has also drawn some recent
attention~\cite{Liu2017, Zhang2015, Liu2017a}.
%
For example, Agarwal \etal~\cite{Agarwal2010} developed bipartite
ranking~\cite{Agarwal2005} to rank chemical structures for Structure-Activity-Relationship (SAR)
modeling such that active compounds and inactive compounds are well separated in the ranking lists.
%
Liu and Ning~\cite{Liu2017a} developed a ranking method with
bi-directional powered push strategy to prioritize selective compounds from multiple bioassays. 
%
However, \LETOR has not been widely used in prioritizing drugs in computational medicine
domain. 
 
%
In \LETOR, a particular interest is to improve the performance on the top of the
ranking lists~\cite{Boyd2012, Narasimhan2013},
that is, instead of optimizing the entire ranking
structures, only the top of the ranking lists 
will be optimized (i.e., to rank the most relevant instances on top), while
the rest of the ranking lists, particularly the bottom of the ranking lists, is of
little interest. 
%
An effective technique to enable good ranking performance on top in \LETOR is via
push~\cite{Rudin2009, Agarwal2011, Liu2017}.
%
%The key idea is to have a quantitative measurement on the ranking positions of relavent items 
%in the ranking lists, and explicitly include such measurement as part of the objective to
%optimize.
The key idea is to explicitly push relevant instances onto top during optimization. 
Various optimization algorithms are developed to deal with the non-trivial objective functions 
when push is involved~\cite{Burges2007,Li2014}. 
%


==> tables/gene_list.tex <==
\begin{ThreePartTable}
    \begin{TableNotes}[flushleft]  %%% This should come before longtable and it is not tablenotes but TableNotes
  \small
  \item
%    \begin{footnotesize}
%        \bgroup
%%        \def\arraystretch{0.5}%       
%        \setstretch{1}
%              \textcolor{red}{Some footnotes here.}
%	      \par
%         \egroup
%    \end{footnotesize}
  \end{TableNotes}
  \begin{longtable}{
      @{\hspace{0pt}}>{}p{0.13\textwidth}@{\hspace{5pt}}
      @{\hspace{0pt}}>{}p{0.13\textwidth}@{\hspace{5pt}}
      @{\hspace{0pt}}>{}p{0.13\textwidth}@{\hspace{5pt}}
      @{\hspace{0pt}}>{}p{0.13\textwidth}@{\hspace{5pt}}
      @{\hspace{0pt}}>{}p{0.13\textwidth}@{\hspace{5pt}}
      @{\hspace{0pt}}>{\arraybackslash}p{0.13\textwidth}@{\hspace{0pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
    }
    \caption{\mbox{List of Selected Genes}}
    \label{supp:tbl:gene-list}\\
  %
    \hline\hline
    \multicolumn{6}{c}{Gene Encodings}\\
    \hline
    \endfirsthead
  %
    \multicolumn{6}{c}{\tablename\ \thetable{} -- continued from previous page}\\
    \hline\hline
    \multicolumn{6}{c}{Gene Encodings}\\
    \hline
    \endhead
  %
    \hline
    %  \midrule
    \multicolumn{6}{c}{Continued on next page} \\
    \hline
    %\midrule
    \endfoot
    %
    \hline\hline
    %\bottomrule
    \insertTableNotes         %% this added
    \endlastfoot
    %
    \input{tables/gene_list_data.tex}
    \hline
  \end{longtable}
\end{ThreePartTable}


==> tables/gene_list_data.tex <==
       ABCB1	&	       ABCC3	&	      ABLIM3	&	       ACADM	&	        ACN9	&	       ACSL3	\\
        ACTB	&	       ACTG1	&	       ACTN4	&	      ACTR10	&	        ADAR	&	        ADI1	\\
         ADM	&	     ADORA2B	&	        ADSL	&	      AGPAT9	&	        AGR2	&	        AHCY	\\
         AHR	&	       AHSA1	&	        AIDA	&	       AIFM2	&	        AIM1	&	      AKR1B1	\\
     AKR1B10	&	      AKR1C1	&	      AKR1C2	&	      AKR1C3	&	     ALDH1A1	&	     ALDH1A3	\\
       ALDH2	&	     ALDH3A1	&	     ALDH3A2	&	     ALDH9A1	&	       ALDOA	&	        ALG8	\\
      ALYREF	&	      AMIGO2	&	      AMOTL2	&	      ANKMY2	&	        ANLN	&	      ANP32B	\\
      ANP32E	&	       ANXA2	&	     ANXA2P2	&	       ANXA3	&	       ANXA4	&	       ANXA5	\\
       ANXA7	&	       AP1S2	&	       AP2M1	&	       AP2S1	&	       AP3S1	&	       APEX1	\\
     APOA1BP	&	    APOBEC3B	&	        APOD	&	       ARCN1	&	        ARF4	&	    ARHGAP15	\\
    ARHGAP18	&	    ARHGAP29	&	     ARHGEF6	&	     ARL6IP1	&	     ARL6IP5	&	      ARMCX6	\\
       ARNT2	&	      ARPC1A	&	      ARPC1B	&	       ARPC2	&	       ARPC3	&	      ARRDC4	\\
       ASAP2	&	      ASRGL1	&	        ASS1	&	        ASUN	&	        ATF4	&	        ATIC	\\
       ATOX1	&	      ATP1B1	&	       ATP5B	&	      ATP5C1	&	       ATP5I	&	       ATP5J	\\
       ATP5L	&	        ATP6	&	     ATP6AP1	&	     ATP6V0B	&	     ATP6V0C	&	    ATP6V0D1	\\
    ATP6V0E2	&	    ATP6V1E1	&	     ATP6V1F	&	        AUP1	&	       AVPI1	&	         AXL	\\
       AZGP1	&	         B2M	&	       BACE2	&	        BAG3	&	       BAMBI	&	       BANF1	\\
      BCAP31	&	       BCAR3	&	       BCAT1	&	      BCL11A	&	        BDNF	&	        BEX2	\\
       BICC1	&	       BIRC2	&	       BLCAP	&	     BLOC1S2	&	       BLVRB	&	        BMI1	\\
        BMP4	&	       BNIP3	&	       BOLA3	&	        BST2	&	       BUD31	&	        BZW1	\\
        BZW2	&	   C10ORF116	&	    C11ORF10	&	    C12ORF23	&	    C12ORF57	&	    C12ORF75	\\
   C14ORF119	&	   C14ORF166	&	     C14ORF2	&	    C15ORF48	&	    C16ORF54	&	    C16ORF80	\\
    C17ORF58	&	    C19ORF10	&	    C19ORF33	&	    C19ORF53	&	       C1QBP	&	     C1ORF51	\\
    C20ORF24	&	    C20ORF30	&	     C2ORF28	&	     C4ORF19	&	     C5ORF43	&	      C9ORF3	\\
        CA12	&	       CAMLG	&	        CAP1	&	        CAP2	&	        CAPG	&	      CAPNS1	\\
        CAV1	&	        CAV2	&	        CBX1	&	      CCDC72	&	      CCDC99	&	        CCL2	\\
       CCNB1	&	       CCND1	&	       CCNG1	&	        CCT2	&	        CCT3	&	       CCT6A	\\
        CCT7	&	       CD151	&	       CD164	&	        CD24	&	        CD55	&	        CD59	\\
        CD63	&	        CD81	&	        CD99	&	      CDC123	&	       CDC20	&	    CDC42EP3	\\
      CDCA7L	&	        CDH1	&	       CDIPT	&	     CDK2AP1	&	        CDK4	&	      CDKN1B	\\
      CDKN2C	&	       CDKN3	&	     CEACAM6	&	       CEBPB	&	       CENPW	&	      CEP170	\\
       CERS2	&	       CETN2	&	        CFL1	&	        CFL2	&	      CHCHD1	&	     CHCHD10	\\
      CHCHD2	&	      CHCHD8	&	      CHMP2A	&	      CHMP4C	&	       CHMP5	&	        CHN1	\\
        CIB1	&	      CIRH1A	&	       CISD1	&	         CKB	&	       CKS1B	&	        CKS2	\\
       CLDN3	&	        CLGN	&	       CLIC1	&	       CLIC3	&	       CLIP4	&	        CMC2	\\
        CNIH	&	        CNN3	&	      CNRIP1	&	      COL4A2	&	      COL5A2	&	      COL6A3	\\
      COMMD3	&	      COMMD8	&	       COPB2	&	       COPS5	&	      CORO1A	&	       COTL1	\\
        COX1	&	        COX2	&	      COX6B1	&	       COX6C	&	      COX7A2	&	     COX7A2L	\\
       COX7C	&	       COX8A	&	         CPE	&	       CREG1	&	       CRIM1	&	       CRIP1	\\
       CRIP2	&	       CRNDE	&	       CRYAB	&	        CRYZ	&	          CS	&	       CSDE1	\\
      CSNK2B	&	        CSTA	&	       CTBP2	&	        CTGF	&	     CTNNAL1	&	        CTSA	\\
        CTSD	&	        CTSH	&	       CTSL1	&	       CTSL2	&	        CUTA	&	       CWC15	\\
       CXXC5	&	      CYB5R3	&	        CYC1	&	      CYFIP1	&	      CYP1B1	&	     CYP51A1	\\
       CYR61	&	      CYSTM1	&	        DAB2	&	        DAD1	&	         DAP	&	        DAP3	\\
        DARS	&	         DBI	&	       DCTN3	&	      DCTPP1	&	         DDC	&	       DDOST	\\
        DDR1	&	        DDX1	&	       DDX21	&	      DDX39A	&	       DDX47	&	       DEGS1	\\
         DEK	&	     DENND5A	&	      DEPDC7	&	       DFNA5	&	      DHCR24	&	       DHX15	\\
        DKK1	&	      DNAJA1	&	     DNAJB11	&	       DNMT1	&	        DPM1	&	        DPP4	\\
       DPY30	&	      DPYSL2	&	        DRG1	&	        DSG2	&	         DSP	&	      DUSP23	\\
       DUSP4	&	       DUSP5	&	       DUSP6	&	         DUT	&	     DYNC1I2	&	      DYNLL1	\\
      DYNLT1	&	      DYNLT3	&	        EBPL	&	       ECHS1	&	        ECI2	&	        ECM1	\\
        EDF1	&	      EEF1A1	&	      EEF1A2	&	      EEF1B2	&	       EEF1G	&	        EEF2	\\
        EID1	&	       EIF2A	&	       EIF3D	&	       EIF3E	&	       EIF3G	&	       EIF3H	\\
       EIF3I	&	      EIF4A1	&	      EIF4A3	&	       EIF4H	&	        EIF6	&	      ELOVL7	\\
         EMB	&	        EMP2	&	        EMP3	&	        ENC1	&	        ENO2	&	       EPCAM	\\
       EPDR1	&	       EPHA2	&	       EPHX1	&	        EPRS	&	        EPS8	&	         ERH	\\
       ERP29	&	      ERRFI1	&	       ESRP1	&	        ETFA	&	        ETFB	&	       ETHE1	\\
       EVI2A	&	          F3	&	       FABP5	&	     FAM101B	&	    FAM108C1	&	    FAM114A1	\\
     FAM127A	&	    FAM171A1	&	     FAM176A	&	     FAM210B	&	     FAM216A	&	      FAM83D	\\
      FAM96A	&	      FAM96B	&	         FAS	&	        FAT1	&	         FAU	&	         FBL	\\
        FBN1	&	      FERMT2	&	       FGF13	&	        FGF2	&	      FGFBP1	&	        FHL2	\\
        FIS1	&	       FKBP9	&	         FN1	&	      FNBP1L	&	         FOS	&	       FOSL1	\\
       FOXQ1	&	       FRMD6	&	        FTH1	&	      FTH1P5	&	         FTL	&	       FUCA2	\\
       FXYD3	&	       FXYD5	&	        G6PD	&	     GABARAP	&	   GABARAPL2	&	     GALNT11	\\
       GANAB	&	       GAPDH	&	        GARS	&	      GAS2L3	&	        GBAS	&	        GBE1	\\
        GBP3	&	        GCH1	&	        GDI2	&	         GEM	&	        GGCT	&	         GGH	\\
       GHITM	&	         GHR	&	        GJA1	&	         GLA	&	      GLIPR1	&	       GLIS3	\\
        GLO1	&	       GLRX2	&	       GLRX5	&	       GLUD1	&	        GMFG	&	        GMNN	\\
       GNA15	&	        GNB1	&	       GNG11	&	       GNG12	&	        GNG5	&	       GNPAT	\\
      GOLPH3	&	     GORASP2	&	        GOT2	&	         GPI	&	       GPM6B	&	     GPR137B	\\
       GPR56	&	       GPR87	&	      GPRC5A	&	        GPX1	&	        GPX2	&	        GPX3	\\
        GPX4	&	        GPX8	&	      GRAMD3	&	       GSTA4	&	       GSTO1	&	       GSTO2	\\
       GSTP1	&	      GTF3C6	&	       GULP1	&	        GYG1	&	        GYPC	&	        H1F0	\\
       H2AFV	&	       H2AFZ	&	       H3F3B	&	       HADHB	&	        HAT1	&	       HBXIP	\\
       HCLS1	&	       HDAC1	&	        HDGF	&	     HEATR5A	&	       HEBP1	&	       HEBP2	\\
     HERPUD1	&	        HEXB	&	        HEY1	&	       HIAT1	&	       HIF1A	&	      HIGD2A	\\
       HINT1	&	   HIST1H2BK	&	    HIST1H4C	&	       HLA-A	&	       HLA-B	&	       HLA-C	\\
     HLA-DRA	&	        HLTF	&	       HMGB1	&	       HMGN1	&	       HMGN2	&	       HMGN3	\\
       HMGN4	&	       HMOX1	&	         HN1	&	     HNRNPA1	&	      HNRNPK	&	       HOXB2	\\
       HOXC6	&	      HPCAL1	&	       HSBP1	&	    HSD17B10	&	    HSP90AA1	&	    HSP90AB1	\\
     HSP90B1	&	      HSPA1A	&	       HSPA5	&	       HSPA8	&	       HSPB1	&	       HSPE1	\\
       HSPH1	&	       HTRA1	&	        IAH1	&	        IARS	&	       IARS2	&	         ID1	\\
         ID2	&	         ID3	&	        IER2	&	        IER3	&	       IFI16	&	       IFI27	\\
        IFI6	&	      IFITM2	&	      IFITM3	&	      IGFBP2	&	      IGFBP3	&	      IGFBP4	\\
      IGFBP5	&	      IGFBP6	&	       IKBIP	&	     IL13RA1	&	        IL1B	&	        IL32	\\
        IL7R	&	        ILF2	&	        IMP4	&	       IMPA1	&	       IMPA2	&	        IPO7	\\
      IQGAP1	&	     IRF2BPL	&	        IRS2	&	        IRX3	&	        ISCU	&	       ITGA3	\\
       ITGAE	&	       ITGAV	&	       ITM2B	&	         JTB	&	        KARS	&	      KDELR2	\\
      KDELR3	&	     KHDRBS3	&	    KIAA0101	&	    KIAA1191	&	    KIAA1598	&	      KIF21B	\\
        KLF5	&	       KPNA2	&	       KRT10	&	       KRT17	&	       KRT18	&	       KRT19	\\
        KRT5	&	       KRT6A	&	       KRT80	&	        KTN1	&	       LAMB1	&	       LAMC1	\\
       LAMP2	&	     LAMTOR1	&	        LAP3	&	     LAPTM4A	&	     LAPTM4B	&	      LAPTM5	\\
       LASP1	&	         LBR	&	        LDHA	&	        LDHB	&	       LDOC1	&	      LEPRE1	\\
      LGALS1	&	      LGALS3	&	    LGALS3BP	&	        LGMN	&	   LINC00493	&	LOC100129361	\\
LOC100288911	&	LOC100289026	&	LOC100505937	&	LOC100506377	&	LOC100507246	&	   LOC344887	\\
         LOX	&	       LRP11	&	        LSM1	&	        LSM7	&	       LTA4H	&	     LURAP1L	\\
         LXN	&	         LYN	&	      LYPLA1	&	      MAD2L1	&	     MAGEA12	&	      MAGEA3	\\
      MAGEA6	&	      MAGED1	&	      MAGEH1	&	        MAL2	&	      MALAT1	&	        MALL	\\
        MANF	&	      MANSC1	&	       MAP1B	&	    MAP1LC3B	&	       MAPK6	&	      MAPRE1	\\
      MARCKS	&	       MATN2	&	        MEA1	&	         MET	&	     METTL23	&	     METTL7B	\\
       MFSD1	&	      MGAT4B	&	        MGLL	&	       MGST1	&	       MGST2	&	       MIEN1	\\
         MIF	&	     MIR22HG	&	        MLF2	&	        MLH1	&	      MLLT11	&	        MLPH	\\
      MMADHC	&	         MOK	&	       MORC4	&	     MORF4L1	&	      MRFAP1	&	      MRPL13	\\
      MRPL14	&	      MRPL15	&	      MRPL17	&	      MRPL18	&	      MRPL21	&	       MRPL3	\\
      MRPL32	&	      MRPL33	&	      MRPL36	&	      MRPL49	&	      MRPL51	&	      MRPS21	\\
      MRPS23	&	      MRPS24	&	      MRPS30	&	      MRPS33	&	       MRPS6	&	       MSMO1	\\
         MSN	&	        MT1E	&	       MT1P2	&	        MT1X	&	        MT2A	&	       MTCH1	\\
      MTHFD1	&	      MTHFD2	&	       MTUS1	&	         MVP	&	         MX1	&	       MYH10	\\
      MYL12B	&	        MYL9	&	       MYO5C	&	        MYO6	&	        MYOF	&	       MZT2A	\\
       NAA20	&	        NACA	&	      NACAP1	&	        NAE1	&	       NAMPT	&	      NAP1L1	\\
        NARS	&	       NCEH1	&	       NCOA4	&	         ND2	&	       NDRG1	&	      NDUFA1	\\
     NDUFA12	&	     NDUFA13	&	      NDUFA3	&	      NDUFA4	&	      NDUFA8	&	      NDUFA9	\\
     NDUFAB1	&	     NDUFB11	&	      NDUFB3	&	      NDUFB5	&	      NDUFB9	&	      NDUFS3	\\
      NDUFS6	&	      NDUFV2	&	       NEDD8	&	        NEK7	&	       NETO2	&	        NEXN	\\
      NFKBIA	&	     NGFRAP1	&	        NGRN	&	        NHP2	&	       NIPA2	&	        NME1	\\
        NNMT	&	       NOL11	&	        NONO	&	       NOP10	&	       NOP58	&	        NPC2	\\
       NPDC1	&	        NPM1	&	        NPTN	&	        NQO1	&	       NR3C1	&	        NSA2	\\
        NT5E	&	        NTN4	&	       NUAK1	&	      NUDT19	&	       NUP37	&	       NUPR1	\\
      NUSAP1	&	         OAT	&	        OAZ1	&	      OCIAD2	&	        ODC1	&	        ODZ2	\\
        ORC6	&	      ORMDL2	&	        OST4	&	        OSTC	&	       OXA1L	&	       P2RY8	\\
        P4HB	&	      PABPC3	&	      PABPC4	&	         PAM	&	      PAPSS1	&	      PAPSS2	\\
       PARK7	&	         PBK	&	        PBX1	&	       PCBD1	&	       PCBP1	&	       PCMT1	\\
        PCNA	&	      PDCD10	&	        PDHB	&	       PDIA6	&	      PDLIM1	&	        PDP1	\\
      PDZD11	&	       PDZK1	&	       PEA15	&	       PEBP1	&	       PEG10	&	       PFDN2	\\
       PFDN5	&	        PFKP	&	        PFN1	&	        PFN2	&	       PGAM1	&	        PGM1	\\
      PGRMC1	&	        PHB2	&	      PHLDA1	&	        PIGP	&	         PIR	&	      PITPNB	\\
      PKD1P1	&	        PKIG	&	        PKM2	&	     PLA2G16	&	        PLAT	&	        PLAU	\\
       PLCB4	&	     PLEKHA1	&	     PLEKHH1	&	       PLIN3	&	        PLK2	&	       PLOD2	\\
       PLOD3	&	        PLP1	&	        PLP2	&	        PLS1	&	        PLS3	&	      PMEPA1	\\
       PMP22	&	       POLE3	&	      POLR2G	&	      POLR2J	&	      POPDC3	&	        PPA1	\\
      PPAP2B	&	      PPAP2C	&	        PPIB	&	        PPIC	&	       PPIL1	&	      PPP1CA	\\
      PPP1CB	&	      PPP1CC	&	     PPP1R18	&	      PPP3CA	&	        PPT1	&	        PRC1	\\
       PRDX1	&	       PRDX4	&	       PRDX5	&	       PRDX6	&	     PRELID1	&	    PRICKLE2	\\
     PRKCDBP	&	        PRNP	&	       PROCR	&	       PRPS1	&	       PRR11	&	       PRR13	\\
      PRSS23	&	        PSAP	&	       PSMA1	&	       PSMA2	&	       PSMA4	&	       PSMA6	\\
       PSMA7	&	       PSMB3	&	       PSMB4	&	       PSMB5	&	       PSMB6	&	       PSMB8	\\
       PSMB9	&	       PSMC1	&	       PSMC3	&	       PSMC4	&	       PSMC5	&	       PSMC6	\\
      PSMD10	&	      PSMD14	&	       PSMD2	&	       PSMD8	&	       PSME1	&	       PSME2	\\
       PSMG1	&	       PSMG2	&	      PTDSS1	&	      PTGES3	&	      PTGFRN	&	       PTGR1	\\
        PTMA	&	      PTP4A2	&	     PTPLAD1	&	         PTS	&	       PTTG1	&	     PTTG1IP	\\
        PXDN	&	        PYGL	&	        QARS	&	        QPCT	&	       RAB10	&	       RAB13	\\
       RAB31	&	       RAB38	&	       RAB8A	&	      RABAC1	&	        RAC1	&	        RAC2	\\
     RACGAP1	&	       RAD21	&	       RAI14	&	         RAN	&	       RAP1B	&	     RARRES3	\\
        RARS	&	       RBBP7	&	       RBM24	&	        RBX1	&	        RCN2	&	       RCSD1	\\
        RDBP	&	       REEP5	&	        RFC4	&	       RHPN2	&	      RNASEK	&	        RND3	\\
      RNF128	&	      RNF135	&	       ROMO1	&	        RPA3	&	        RPF2	&	       RPL11	\\
       RPL12	&	      RPL13A	&	       RPL14	&	       RPL17	&	       RPL19	&	       RPL21	\\
       RPL22	&	     RPL22L1	&	      RPL23A	&	       RPL24	&	       RPL26	&	     RPL26L1	\\
       RPL27	&	       RPL28	&	       RPL29	&	        RPL3	&	       RPL30	&	       RPL31	\\
       RPL32	&	       RPL34	&	       RPL35	&	       RPL36	&	      RPL36A	&	     RPL36AL	\\
       RPL38	&	       RPL39	&	        RPL4	&	       RPL41	&	        RPL5	&	        RPL6	\\
       RPL7A	&	      RPL7L1	&	        RPL8	&	        RPL9	&	       RPLP0	&	       RPLP1	\\
        RPN1	&	        RPN2	&	       RPS10	&	       RPS11	&	       RPS13	&	     RPS14P3	\\
       RPS16	&	       RPS17	&	       RPS18	&	        RPS2	&	       RPS20	&	       RPS21	\\
       RPS23	&	       RPS24	&	       RPS25	&	       RPS26	&	       RPS29	&	        RPS3	\\
       RPS3A	&	       RPS4X	&	        RPS5	&	        RPS6	&	        RPS7	&	        RPSA	\\
       RRAGD	&	        RRAS	&	       RRAS2	&	        RRM1	&	        RRM2	&	     RSL24D1	\\
        RTN4	&	     S100A10	&	     S100A11	&	     S100A16	&	      S100A2	&	       S100P	\\
        SACS	&	       SARNP	&	        SAT1	&	         SCD	&	        SCG5	&	        SCP2	\\
       SCRN1	&	        SDC1	&	        SDC2	&	        SDC4	&	       SDCBP	&	        SDHA	\\
      SEC11A	&	      SEC11C	&	       SEC13	&	      SEC31A	&	      SEC61G	&	        SELK	\\
        SELM	&	        SELS	&	      SEMA3C	&	       SEP15	&	      SEPHS2	&	      SEPT10	\\
       SEPW1	&	       SERF2	&	     SERINC5	&	    SERPINE1	&	         SET	&	       SF3B1	\\
       SF3B5	&	         SFN	&	        SGCE	&	        SGK1	&	      SGK223	&	       SH2B3	\\
     SH3BGRL	&	    SH3BGRL3	&	     SH3KBP1	&	      SHCBP1	&	       SHFM1	&	      SHISA5	\\
        SKP1	&	        SLBP	&	     SLC16A4	&	    SLC22A18	&	     SLC25A3	&	     SLC25A5	\\
     SLC25A6	&	     SLC2A10	&	     SLC38A2	&	      SLC3A2	&	     SLC7A11	&	      SLC7A5	\\
    SLC9A3R1	&	      SLFN11	&	       SLIRP	&	       SMAGP	&	       SNAI2	&	       SNHG5	\\
       SNHG6	&	       SNHG8	&	       SNRPA	&	       SNRPB	&	      SNRPD2	&	      SNRPD3	\\
       SNRPF	&	       SNRPG	&	       SNX10	&	        SNX3	&	        SNX7	&	        SOD1	\\
      SOWAHC	&	        SOX9	&	       SPARC	&	       SPCS1	&	      SPINK1	&	      SPINT2	\\
      SPOCK1	&	        SPP1	&	       SQRDL	&	        SRGN	&	       SRP14	&	       SRP19	\\
       SRP68	&	        SRP9	&	        SRPX	&	       SRSF2	&	       SRSF9	&	       SRXN1	\\
         SSB	&	        SSR2	&	        SSR4	&	        ST13	&	  ST6GALNAC2	&	      STARD7	\\
       STAU1	&	      STEAP1	&	       STUB1	&	      STXBP1	&	       SUMO2	&	       SUMO3	\\
       SURF4	&	        SVIP	&	        SYNC	&	       SYPL1	&	       SYT13	&	       SYTL2	\\
        TAF7	&	        TAF9	&	      TAGLN2	&	      TALDO1	&	      TATDN1	&	     TAX1BP1	\\
     TAX1BP3	&	        TBCA	&	        TBCB	&	      TCEAL3	&	      TCEAL4	&	        TCF4	\\
        TCP1	&	    TCTEX1D2	&	        TDP2	&	       TEAD1	&	        TFF3	&	        TFPI	\\
     TGFB1I1	&	       TGFBI	&	        TH1L	&	     TIMMDC1	&	       TIMP1	&	       TIMP2	\\
       TIMP3	&	        TJP1	&	         TK1	&	      TM4SF1	&	     TM4SF18	&	      TM9SF2	\\
      TMBIM4	&	      TMBIM6	&	       TMED2	&	     TMEM123	&	    TMEM126A	&	     TMEM139	\\
     TMEM147	&	     TMEM14A	&	     TMEM14B	&	     TMEM14C	&	     TMEM158	&	    TMEM167A	\\
    TMEM200A	&	      TMEM47	&	      TMEM85	&	      TMEM93	&	      TMEM97	&	      TMSB10	\\
        TMX2	&	   TNFRSF11B	&	   TNFRSF12A	&	    TNFRSF21	&	        TOB1	&	      TOMM20	\\
       TOMM5	&	        TOP1	&	       TOP2B	&	     TPD52L1	&	        TPM1	&	        TPT1	\\
        TPX2	&	       TRAM1	&	      TRIM16	&	      TRIM59	&	      TRIP13	&	     TRMT112	\\
      TSG101	&	       TSHZ1	&	     TSPAN13	&	      TSPAN4	&	      TSPAN6	&	      TSPAN8	\\
        TSPO	&	      TSPYL5	&	       TSTD1	&	      TUBA1A	&	      TUBA1B	&	      TUBA1C	\\
        TUBB	&	      TUBB2A	&	       TUBB3	&	      TUBB4B	&	       TUBB6	&	       TUFT1	\\
       TUSC1	&	         TXN	&	     TXNDC12	&	       TXNIP	&	       TYRP1	&	        UAP1	\\
        UBA2	&	       UBA52	&	         UBB	&	         UBC	&	       UBE2C	&	      UBE2E2	\\
      UBE2E3	&	       UBE2S	&	      UBE2V2	&	        UBL3	&	        UBL5	&	       UCHL1	\\
       UCHL3	&	        UCP2	&	        UFC1	&	       UFD1L	&	        UGCG	&	        UGDH	\\
        UPP1	&	      UQCRC1	&	     UQCRFS1	&	       UQCRH	&	       UQCRQ	&	       USMG5	\\
        USP1	&	         UXT	&	       VAMP3	&	       VAMP7	&	       VAMP8	&	        VBP1	\\
        VCAN	&	       VDAC2	&	         VIM	&	      VKORC1	&	        WBP5	&	       WDR82	\\
     WDR83OS	&	       WIPI1	&	       WNT5A	&	         WRB	&	        WWC3	&	       WWTR1	\\
        XPOT	&	        YAP1	&	       YPEL5	&	       YWHAB	&	       YWHAE	&	       YWHAG	\\
       YWHAQ	&	       YWHAZ	&	     ZC3H11A	&	       ZCRB1	&	        ZEB1	&	    ZMPSTE24	\\
      ZNF721	&	   ZNFX1-AS1	&	       ZWINT	&			&			&			\\


==> tables/holdout_2percent.tex <==
\begin{ThreePartTable}
    \begin{TableNotes}[flushleft]  %%% This should come before longtable and it is not tablenotes but TableNotes
  \small
  \item
    \begin{footnotesize}
        \bgroup
%        \def\arraystretch{0.5}%       
        \setstretch{1}
		The columns corresponding to ``$l$'', ``$\alpha$'',
                ``$\beta$'', ``$\gamma$'', ``usim'', and ``$\sigma$'' have the
                latent dimension, weighting factor,
                latent vector regularization parameter,
                cell line similarity regularization parameter,
                cell line similarity function, and parameter for rbf cell line similarity,
                respectively, for \MTCRP.
	      \par
              \egroup
    \end{footnotesize}
  \end{TableNotes}
  \begin{longtable}{
      @{\hspace{5pt}}>{\raggedleft}p{0.04\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.04\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.04\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.04\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.07\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.04\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.04\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft\arraybackslash}p{0.10\textwidth}@{\hspace{6pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
    }
    \caption{\mbox{\MTCRP Performance on New Cell Lines ($\theta$ = 2)}}
    \label{supp:tbl:holdout:2percent}\\
  %
    \hline\hline
    n & $l$ & $\alpha$ & $\beta$ & $\gamma$ & usim & $\sigma$ & \small{AP@$5$} & \small{AP@$10$} & \small{\rCI} & \small{\CI} \\
    \hline
    \endfirsthead
  %
    \multicolumn{11}{c}{{\tablename\ \thetable{} -- continued from previous page}}\\
    \hline\hline
    n & $l$ & $\alpha$ & $\beta$ & $\gamma$ & usim & $\sigma$ & \small{AP@$5$} & \small{AP@$10$} & \small{\rCI} & \small{\CI} \\
    \hline
    \endhead
  %
    \hline
    %  \midrule
    \multicolumn{11}{c}{{Continued on next page}} \\
    \hline
    %\midrule
    \endfoot
    %
    \hline\hline
    %\bottomrule
    \insertTableNotes         %% this added
    \endlastfoot
    %
    \input{tables/holdout_2percent_data.tex}
	
    \hline
  \end{longtable}
\end{ThreePartTable}


==> tables/holdout_2percent_KRL.tex <==
\begin{ThreePartTable}
    \begin{TableNotes}[flushleft]  %%% This should come before longtable and it is not tablenotes but TableNotes
  \small
  \item
    \begin{footnotesize}
        \bgroup
%        \def\arraystretch{0.5}%       
        \setstretch{1}
                The columns corresponding to ``$k$'', ``$\lambda$'',
                ``usim'', and ``$\sigma$'' have the
                two hyperparameters, cell line similarity function,
                and parameter for {$\RBF$} cell line similarity, respectively, 
                for {\KRL}.
	      \par
              \egroup
    \end{footnotesize}
  \end{TableNotes}
  \begin{longtable}{
      @{\hspace{5pt}}>{\raggedleft}p{0.04\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.04\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft\arraybackslash}p{0.10\textwidth}@{\hspace{6pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
    }
    \caption{\mbox{\KRL Performance on New Cell Lines ($\theta$ = 2)}}
    \label{supp:tbl:holdout:2percent:KRL}\\
  %
    \hline\hline
    n & $k$ & $\lambda$ & usim & $\sigma$ & \small{AP@$5$} & \small{AP@$10$} & \small{\rCI} & \small{\CI} \\
    \hline
    \endfirsthead
  %
    \multicolumn{9}{c}{{\tablename\ \thetable{} -- continued from previous page}}\\
    \hline\hline
    n & $k$ & $\lambda$ & usim & $\sigma$ & \small{AP@$5$} & \small{AP@$10$} & \small{\rCI} & \small{\CI} \\
    \hline
    \endhead
  %
    \hline
    %  \midrule
    \multicolumn{9}{c}{{Continued on next page}} \\
    \hline
    %\midrule
    \endfoot
    %
    \hline\hline
    %\bottomrule
    \insertTableNotes         %% this added
    \endlastfoot
    %
    \input{tables/holdout_2percent_KRL_data.tex}
	
    \hline
  \end{longtable}
\end{ThreePartTable}


==> tables/holdout_2percent_KRL_data.tex <==
50	& 5	&   0.000001	&       \RBF	&     0.0001	& 0.322	& 0.330	& 0.541	& 0.747 \\
50	& 5	&   0.000001	&       \RBF	&      0.001	& 0.283	& 0.295	& 0.559	& 0.725 \\
50	& 5	&   0.000001	&       \RBF	&       0.01	& 0.138	& 0.170	& 0.534	& 0.604 \\
50	& 5	&    0.00001	&       \LIN	&          -	& 0.111	& 0.149	& 0.542	& 0.706 \\
50	& 5	&    0.00001	&       \RBF	&     0.0001	& 0.425	& 0.419	& 0.550	& 0.755 \\
50	& 5	&    0.00001	&       \RBF	&       0.01	& 0.124	& 0.175	& 0.537	& 0.616 \\
50	& 5	&     0.0001	&       \LIN	&          -	& 0.189	& 0.217	& 0.509	& 0.717 \\
50	& 5	&     0.0001	&       \RBF	&     0.0001	& 0.436	& 0.423	& 0.557	& 0.764 \\
50	& 5	&     0.0001	&       \RBF	&      0.001	& 0.446	& 0.410	& 0.546	& 0.754 \\
50	& 5	&     0.0001	&       \RBF	&       0.01	& 0.132	& 0.184	& 0.543	& 0.576 \\
50	& 5	&      0.001	&       \LIN	&          -	& 0.195	& 0.238	& 0.511	& 0.698 \\
50	& 5	&      0.001	&       \RBF	&     0.0001	& 0.436	& 0.423	& 0.557	& 0.764 \\
50	& 5	&      0.001	&       \RBF	&      0.001	& 0.446	& 0.410	& 0.546	& 0.754 \\
50	& 5	&      0.001	&       \RBF	&       0.01	& 0.112	& 0.165	& 0.549	& 0.530 \\
50	& 5	&       0.01	&       \LIN	&          -	& 0.307	& 0.298	& 0.535	& 0.747 \\
50	& 5	&       0.01	&       \RBF	&     0.0001	& 0.436	& 0.423	& 0.557	& 0.764 \\
50	& 5	&       0.01	&       \RBF	&      0.001	& 0.446	& 0.410	& 0.546	& 0.754 \\
50	& 5	&       0.01	&       \RBF	&       0.01	& 0.106	& 0.147	& 0.516	& 0.490 \\
50	& 5	&        0.1	&       \LIN	&          -	& 0.421	& 0.424	& 0.555	& 0.760 \\
50	& 5	&        0.1	&       \RBF	&     0.0001	& 0.436	& 0.423	& 0.557	& 0.764 \\
50	& 5	&        0.1	&       \RBF	&      0.001	& 0.446	& 0.410	& 0.546	& 0.754 \\
50	& 5	&        0.1	&       \RBF	&       0.01	& 0.073	& 0.090	& 0.495	& 0.473 \\
50	& 5	&        0.2	&       \LIN	&          -	& 0.439	& 0.414	& 0.556	& 0.763 \\
50	& 5	&        0.2	&       \RBF	&     0.0001	& 0.436	& 0.423	& 0.557	& 0.764 \\
50	& 5	&        0.2	&       \RBF	&      0.001	& 0.446	& 0.410	& 0.546	& 0.754 \\
50	& 5	&        0.2	&       \RBF	&       0.01	& 0.072	& 0.093	& 0.495	& 0.471 \\
50	& 5	&        0.4	&       \LIN	&          -	& 0.445	& 0.399	& 0.559	& 0.770 \\
50	& 5	&        0.4	&       \RBF	&     0.0001	& 0.436	& 0.423	& 0.557	& 0.764 \\
50	& 5	&        0.4	&       \RBF	&      0.001	& 0.446	& 0.410	& 0.546	& 0.754 \\
50	& 5	&        0.4	&       \RBF	&       0.01	& 0.049	& 0.070	& 0.495	& 0.470 \\
50	& 5	&        0.6	&       \LIN	&          -	& 0.451	& 0.436	& 0.551	& 0.768 \\
50	& 5	&        0.6	&       \RBF	&     0.0001	& 0.436	& 0.423	& 0.557	& 0.764 \\
50	& 5	&        0.6	&       \RBF	&      0.001	& 0.446	& 0.410	& 0.546	& 0.754 \\
50	& 5	&        0.6	&       \RBF	&       0.01	& 0.049	& 0.070	& 0.496	& 0.469 \\
50	& 5	&        0.8	&       \LIN	&          -	& 0.433	& 0.413	& 0.553	& 0.771 \\
50	& 5	&        0.8	&       \RBF	&     0.0001	& 0.436	& 0.423	& 0.557	& 0.764 \\
50	& 5	&        0.8	&       \RBF	&      0.001	& 0.446	& 0.410	& 0.546	& 0.754 \\
50	& 5	&        0.8	&       \RBF	&       0.01	& 0.049	& 0.070	& 0.496	& 0.469 \\
50	& 5	&        1.0	&       \LIN	&          -	& 0.425	& 0.420	& 0.549	& 0.773 \\
50	& 5	&        1.0	&       \RBF	&     0.0001	& 0.436	& 0.423	& 0.557	& 0.764 \\
50	& 5	&        1.0	&       \RBF	&      0.001	& 0.446	& 0.410	& 0.546	& 0.754 \\
50	& 5	&        1.0	&       \RBF	&       0.01	& 0.029	& 0.050	& 0.496	& 0.469 \\
50	& 5	&         10	&       \LIN	&          -	& 0.442	& 0.416	& 0.555	& 0.759 \\
50	& 5	&         10	&       \RBF	&     0.0001	& 0.436	& 0.423	& 0.557	& 0.764 \\
50	& 5	&         10	&       \RBF	&      0.001	& 0.446	& 0.410	& 0.546	& 0.754 \\
50	& 5	&         10	&       \RBF	&       0.01	& 0.009	& 0.030	& 0.498	& 0.469 \\
50	& 5	&         50	&       \LIN	&          -	& 0.421	& 0.430	& 0.559	& 0.700 \\
50	& 5	&         50	&       \RBF	&     0.0001	& 0.436	& 0.423	& 0.557	& 0.764 \\
50	& 5	&         50	&       \RBF	&      0.001	& 0.446	& 0.410	& 0.546	& 0.754 \\
50	& 5	&         50	&       \RBF	&       0.01	& 0.009	& 0.030	& 0.498	& 0.468 \\
50	& 5	&        100	&       \LIN	&          -	& 0.421	& 0.430	& 0.559	& 0.700 \\
50	& 5	&        100	&       \RBF	&     0.0001	& 0.436	& 0.423	& 0.557	& 0.764 \\
50	& 5	&        100	&       \RBF	&      0.001	& 0.446	& 0.410	& 0.546	& 0.754 \\
50	& 5	&        100	&       \RBF	&       0.01	& 0.004	& 0.025	& 0.498	& 0.468 \\
50	& 10	&   0.000001	&       \RBF	&     0.0001	& 0.302	& 0.312	& 0.547	& 0.748 \\
50	& 10	&   0.000001	&       \RBF	&       0.01	& 0.126	& 0.158	& 0.541	& 0.598 \\
50	& 10	&      0.001	&       \LIN	&          -	& 0.186	& 0.221	& 0.523	& 0.689 \\
50	& 10	&      0.001	&       \RBF	&     0.0001	& 0.437	& 0.427	& 0.558	& 0.765 \\
50	& 10	&      0.001	&       \RBF	&      0.001	& 0.449	& 0.419	& 0.548	& 0.747 \\
50	& 10	&      0.001	&       \RBF	&       0.01	& 0.106	& 0.163	& 0.546	& 0.527 \\
50	& 10	&       0.01	&       \LIN	&          -	& 0.205	& 0.226	& 0.520	& 0.722 \\
50	& 10	&       0.01	&       \RBF	&     0.0001	& 0.437	& 0.427	& 0.558	& 0.765 \\
50	& 10	&       0.01	&       \RBF	&      0.001	& 0.449	& 0.419	& 0.548	& 0.747 \\
50	& 10	&       0.01	&       \RBF	&       0.01	& 0.115	& 0.148	& 0.516	& 0.491 \\
50	& 10	&        0.1	&       \LIN	&          -	& 0.376	& 0.368	& 0.551	& 0.755 \\
50	& 10	&        0.1	&       \RBF	&     0.0001	& 0.437	& 0.427	& 0.558	& 0.765 \\
50	& 10	&        0.1	&       \RBF	&      0.001	& 0.449	& 0.419	& 0.548	& 0.747 \\
50	& 10	&        0.1	&       \RBF	&       0.01	& 0.070	& 0.081	& 0.493	& 0.474 \\
50	& 10	&        0.2	&       \LIN	&          -	& 0.445	& 0.409	& 0.551	& 0.756 \\
50	& 10	&        0.2	&       \RBF	&     0.0001	& 0.437	& 0.427	& 0.558	& 0.765 \\
50	& 10	&        0.2	&       \RBF	&      0.001	& 0.449	& 0.419	& 0.548	& 0.747 \\
50	& 10	&        0.2	&       \RBF	&       0.01	& 0.050	& 0.074	& 0.495	& 0.471 \\
50	& 10	&        0.4	&       \LIN	&          -	& 0.432	& 0.415	& 0.556	& 0.757 \\
50	& 10	&        0.4	&       \RBF	&     0.0001	& 0.437	& 0.427	& 0.558	& 0.765 \\
50	& 10	&        0.4	&       \RBF	&      0.001	& 0.449	& 0.419	& 0.548	& 0.747 \\
50	& 10	&        0.4	&       \RBF	&       0.01	& 0.059	& 0.080	& 0.494	& 0.470 \\
50	& 10	&        0.6	&       \LIN	&          -	& 0.425	& 0.403	& 0.555	& 0.761 \\
50	& 10	&        0.6	&       \RBF	&     0.0001	& 0.437	& 0.427	& 0.558	& 0.765 \\
50	& 10	&        0.6	&       \RBF	&      0.001	& 0.449	& 0.419	& 0.548	& 0.747 \\
50	& 10	&        0.6	&       \RBF	&       0.01	& 0.039	& 0.060	& 0.496	& 0.469 \\
50	& 10	&        0.8	&       \LIN	&          -	& 0.419	& 0.407	& 0.559	& 0.762 \\
50	& 10	&        0.8	&       \RBF	&     0.0001	& 0.437	& 0.427	& 0.558	& 0.765 \\
50	& 10	&        0.8	&       \RBF	&      0.001	& 0.449	& 0.419	& 0.548	& 0.747 \\
50	& 10	&        0.8	&       \RBF	&       0.01	& 0.049	& 0.070	& 0.496	& 0.469 \\
50	& 10	&        1.0	&       \LIN	&          -	& 0.409	& 0.401	& 0.553	& 0.762 \\
50	& 10	&        1.0	&       \RBF	&     0.0001	& 0.437	& 0.427	& 0.558	& 0.765 \\
50	& 10	&        1.0	&       \RBF	&      0.001	& 0.449	& 0.419	& 0.548	& 0.747 \\
50	& 10	&        1.0	&       \RBF	&       0.01	& 0.029	& 0.050	& 0.496	& 0.469 \\
50	& 10	&         10	&       \LIN	&          -	& 0.445	& 0.425	& 0.552	& 0.773 \\
50	& 10	&         10	&       \RBF	&     0.0001	& 0.437	& 0.427	& 0.558	& 0.765 \\
50	& 10	&         10	&       \RBF	&      0.001	& 0.449	& 0.419	& 0.548	& 0.747 \\
50	& 10	&         10	&       \RBF	&       0.01	& 0.009	& 0.030	& 0.498	& 0.469 \\
50	& 10	&         50	&       \LIN	&          -	& 0.440	& 0.436	& 0.548	& 0.771 \\
50	& 10	&         50	&       \RBF	&     0.0001	& 0.437	& 0.427	& 0.558	& 0.765 \\
50	& 10	&         50	&       \RBF	&      0.001	& 0.449	& 0.419	& 0.548	& 0.747 \\
50	& 10	&         50	&       \RBF	&       0.01	& 0.011	& 0.032	& 0.498	& 0.468 \\
50	& 10	&        100	&       \LIN	&          -	& 0.442	& 0.424	& 0.545	& 0.768 \\
50	& 10	&        100	&       \RBF	&     0.0001	& 0.437	& 0.427	& 0.558	& 0.765 \\
50	& 10	&        100	&       \RBF	&      0.001	& 0.449	& 0.419	& 0.548	& 0.747 \\
50	& 10	&        100	&       \RBF	&       0.01	& 0.004	& 0.025	& 0.498	& 0.468 \\
50	& 15	&      0.001	&       \RBF	&     0.0001	& 0.442	& 0.436	& 0.552	& 0.764 \\
50	& 15	&      0.001	&       \RBF	&      0.001	& 0.441	& 0.423	& 0.548	& 0.746 \\
50	& 15	&      0.001	&       \RBF	&       0.01	& 0.119	& 0.160	& 0.547	& 0.525 \\
50	& 15	&       0.01	&       \LIN	&          -	& 0.434	& 0.383	& 0.548	& 0.738 \\
50	& 15	&       0.01	&       \RBF	&     0.0001	& 0.442	& 0.436	& 0.552	& 0.764 \\
50	& 15	&       0.01	&       \RBF	&      0.001	& 0.441	& 0.423	& 0.548	& 0.746 \\
50	& 15	&       0.01	&       \RBF	&       0.01	& 0.100	& 0.131	& 0.518	& 0.490 \\
50	& 15	&        0.1	&       \LIN	&          -	& 0.404	& 0.386	& 0.543	& 0.738 \\
50	& 15	&        0.1	&       \RBF	&     0.0001	& 0.442	& 0.436	& 0.552	& 0.764 \\
50	& 15	&        0.1	&       \RBF	&      0.001	& 0.441	& 0.423	& 0.548	& 0.746 \\
50	& 15	&        0.1	&       \RBF	&       0.01	& 0.079	& 0.094	& 0.498	& 0.474 \\
50	& 15	&        0.2	&       \LIN	&          -	& 0.389	& 0.375	& 0.547	& 0.744 \\
50	& 15	&        0.2	&       \RBF	&     0.0001	& 0.442	& 0.436	& 0.552	& 0.764 \\
50	& 15	&        0.2	&       \RBF	&      0.001	& 0.441	& 0.423	& 0.548	& 0.746 \\
50	& 15	&        0.2	&       \RBF	&       0.01	& 0.051	& 0.075	& 0.498	& 0.471 \\
50	& 15	&        0.4	&       \LIN	&          -	& 0.429	& 0.430	& 0.532	& 0.732 \\
50	& 15	&        0.4	&       \RBF	&     0.0001	& 0.442	& 0.436	& 0.552	& 0.764 \\
50	& 15	&        0.4	&       \RBF	&      0.001	& 0.441	& 0.423	& 0.548	& 0.746 \\
50	& 15	&        0.4	&       \RBF	&       0.01	& 0.056	& 0.077	& 0.496	& 0.470 \\
50	& 15	&        0.6	&       \LIN	&          -	& 0.377	& 0.369	& 0.539	& 0.741 \\
50	& 15	&        0.6	&       \RBF	&     0.0001	& 0.442	& 0.436	& 0.552	& 0.764 \\
50	& 15	&        0.6	&       \RBF	&      0.001	& 0.441	& 0.423	& 0.548	& 0.746 \\
50	& 15	&        0.6	&       \RBF	&       0.01	& 0.039	& 0.060	& 0.496	& 0.469 \\
50	& 15	&        0.8	&       \LIN	&          -	& 0.425	& 0.424	& 0.505	& 0.738 \\
50	& 15	&        0.8	&       \RBF	&     0.0001	& 0.442	& 0.436	& 0.552	& 0.764 \\
50	& 15	&        0.8	&       \RBF	&      0.001	& 0.441	& 0.423	& 0.548	& 0.746 \\
50	& 15	&        0.8	&       \RBF	&       0.01	& 0.039	& 0.060	& 0.496	& 0.469 \\
50	& 15	&        1.0	&       \LIN	&          -	& 0.434	& 0.431	& 0.528	& 0.741 \\
50	& 15	&        1.0	&       \RBF	&     0.0001	& 0.442	& 0.436	& 0.552	& 0.764 \\
50	& 15	&        1.0	&       \RBF	&      0.001	& 0.441	& 0.423	& 0.548	& 0.746 \\
50	& 15	&        1.0	&       \RBF	&       0.01	& 0.019	& 0.040	& 0.496	& 0.469 \\
50	& 15	&         10	&       \LIN	&          -	& 0.439	& 0.429	& 0.558	& 0.718 \\
50	& 15	&         10	&       \RBF	&     0.0001	& 0.442	& 0.436	& 0.552	& 0.764 \\
50	& 15	&         10	&       \RBF	&      0.001	& 0.441	& 0.423	& 0.548	& 0.746 \\
50	& 15	&         10	&       \RBF	&       0.01	& 0.009	& 0.030	& 0.498	& 0.469 \\
50	& 15	&         50	&       \LIN	&          -	& 0.440	& 0.423	& 0.545	& 0.756 \\
50	& 15	&         50	&       \RBF	&     0.0001	& 0.442	& 0.436	& 0.552	& 0.764 \\
50	& 15	&         50	&       \RBF	&      0.001	& 0.441	& 0.423	& 0.549	& 0.746 \\
50	& 15	&         50	&       \RBF	&       0.01	& 0.009	& 0.030	& 0.498	& 0.468 \\
50	& 15	&        100	&       \LIN	&          -	& 0.440	& 0.428	& 0.548	& 0.766 \\
50	& 15	&        100	&       \RBF	&     0.0001	& 0.442	& 0.436	& 0.552	& 0.764 \\
50	& 15	&        100	&       \RBF	&      0.001	& 0.441	& 0.423	& 0.549	& 0.746 \\
50	& 15	&        100	&       \RBF	&       0.01	& 0.004	& 0.025	& 0.498	& 0.468 \\
100	& 5	&   0.000001	&       \RBF	&     0.0001	& 0.353	& 0.353	& 0.512	& 0.718 \\
100	& 5	&   0.000001	&       \RBF	&      0.001	& 0.291	& 0.303	& 0.539	& 0.715 \\
100	& 5	&   0.000001	&       \RBF	&       0.01	& 0.133	& 0.162	& 0.522	& 0.585 \\
100	& 5	&    0.00001	&       \LIN	&          -	& 0.136	& 0.163	& 0.536	& 0.703 \\
100	& 5	&    0.00001	&       \RBF	&      0.001	& 0.365	& 0.347	& 0.551	& 0.748 \\
100	& 5	&    0.00001	&       \RBF	&       0.01	& 0.117	& 0.140	& 0.519	& 0.589 \\
100	& 5	&     0.0001	&       \RBF	&     0.0001	& 0.378	& 0.353	& 0.558	& 0.763 \\
100	& 5	&     0.0001	&       \RBF	&      0.001	& 0.365	& 0.347	& 0.551	& 0.748 \\
100	& 5	&     0.0001	&       \RBF	&       0.01	& 0.122	& 0.145	& 0.525	& 0.552 \\
100	& 5	&      0.001	&       \LIN	&          -	& 0.267	& 0.263	& 0.523	& 0.701 \\
100	& 5	&      0.001	&       \RBF	&     0.0001	& 0.378	& 0.353	& 0.558	& 0.763 \\
100	& 5	&      0.001	&       \RBF	&      0.001	& 0.365	& 0.347	& 0.551	& 0.748 \\
100	& 5	&      0.001	&       \RBF	&       0.01	& 0.111	& 0.138	& 0.521	& 0.518 \\
100	& 5	&       0.01	&       \LIN	&          -	& 0.312	& 0.305	& 0.516	& 0.712 \\
100	& 5	&       0.01	&       \RBF	&     0.0001	& 0.378	& 0.353	& 0.558	& 0.763 \\
100	& 5	&       0.01	&       \RBF	&      0.001	& 0.365	& 0.347	& 0.551	& 0.748 \\
100	& 5	&       0.01	&       \RBF	&       0.01	& 0.084	& 0.103	& 0.505	& 0.491 \\
100	& 5	&        0.1	&       \LIN	&          -	& 0.392	& 0.369	& 0.538	& 0.754 \\
100	& 5	&        0.1	&       \RBF	&     0.0001	& 0.378	& 0.353	& 0.558	& 0.763 \\
100	& 5	&        0.1	&       \RBF	&      0.001	& 0.365	& 0.347	& 0.551	& 0.748 \\
100	& 5	&        0.1	&       \RBF	&       0.01	& 0.063	& 0.080	& 0.505	& 0.475 \\
100	& 5	&        0.2	&       \LIN	&          -	& 0.343	& 0.334	& 0.547	& 0.759 \\
100	& 5	&        0.2	&       \RBF	&     0.0001	& 0.378	& 0.353	& 0.558	& 0.763 \\
100	& 5	&        0.2	&       \RBF	&      0.001	& 0.365	& 0.347	& 0.551	& 0.748 \\
100	& 5	&        0.2	&       \RBF	&       0.01	& 0.050	& 0.068	& 0.501	& 0.473 \\
100	& 5	&        0.4	&       \LIN	&          -	& 0.399	& 0.393	& 0.545	& 0.763 \\
100	& 5	&        0.4	&       \RBF	&     0.0001	& 0.378	& 0.353	& 0.558	& 0.763 \\
100	& 5	&        0.4	&       \RBF	&      0.001	& 0.365	& 0.347	& 0.551	& 0.748 \\
100	& 5	&        0.4	&       \RBF	&       0.01	& 0.040	& 0.058	& 0.501	& 0.471 \\
100	& 5	&        0.6	&       \LIN	&          -	& 0.369	& 0.355	& 0.544	& 0.763 \\
100	& 5	&        0.6	&       \RBF	&     0.0001	& 0.378	& 0.353	& 0.558	& 0.763 \\
100	& 5	&        0.6	&       \RBF	&      0.001	& 0.365	& 0.347	& 0.551	& 0.748 \\
100	& 5	&        0.6	&       \RBF	&       0.01	& 0.034	& 0.052	& 0.502	& 0.470 \\
100	& 5	&        0.8	&       \LIN	&          -	& 0.400	& 0.394	& 0.546	& 0.763 \\
100	& 5	&        0.8	&       \RBF	&     0.0001	& 0.378	& 0.353	& 0.558	& 0.763 \\
100	& 5	&        0.8	&       \RBF	&      0.001	& 0.365	& 0.347	& 0.551	& 0.748 \\
100	& 5	&        0.8	&       \RBF	&       0.01	& 0.037	& 0.056	& 0.497	& 0.469 \\
100	& 5	&        1.0	&       \LIN	&          -	& 0.336	& 0.337	& 0.542	& 0.768 \\
100	& 5	&        1.0	&       \RBF	&     0.0001	& 0.378	& 0.353	& 0.558	& 0.763 \\
100	& 5	&        1.0	&       \RBF	&      0.001	& 0.365	& 0.347	& 0.551	& 0.748 \\
100	& 5	&        1.0	&       \RBF	&       0.01	& 0.021	& 0.039	& 0.497	& 0.469 \\
100	& 5	&         10	&       \LIN	&          -	& 0.368	& 0.359	& 0.544	& 0.759 \\
100	& 5	&         10	&       \RBF	&     0.0001	& 0.378	& 0.353	& 0.558	& 0.763 \\
100	& 5	&         10	&       \RBF	&      0.001	& 0.365	& 0.347	& 0.551	& 0.748 \\
100	& 5	&         10	&       \RBF	&       0.01	& 0.007	& 0.025	& 0.500	& 0.468 \\
100	& 5	&         50	&       \LIN	&          -	& 0.378	& 0.364	& 0.559	& 0.698 \\
100	& 5	&         50	&       \RBF	&     0.0001	& 0.378	& 0.353	& 0.558	& 0.763 \\
100	& 5	&         50	&       \RBF	&      0.001	& 0.365	& 0.347	& 0.551	& 0.748 \\
100	& 5	&         50	&       \RBF	&       0.01	& 0.005	& 0.023	& 0.499	& 0.467 \\
100	& 5	&        100	&       \LIN	&          -	& 0.378	& 0.364	& 0.559	& 0.698 \\
100	& 5	&        100	&       \RBF	&     0.0001	& 0.378	& 0.353	& 0.558	& 0.763 \\
100	& 5	&        100	&       \RBF	&      0.001	& 0.365	& 0.347	& 0.551	& 0.748 \\
100	& 5	&        100	&       \RBF	&       0.01	& 0.005	& 0.023	& 0.499	& 0.467 \\
100	& 10	&   0.000001	&       \RBF	&       0.01	& 0.134	& 0.159	& 0.522	& 0.581 \\
100	& 10	&      0.001	&       \LIN	&          -	& 0.187	& 0.199	& 0.527	& 0.709 \\
100	& 10	&      0.001	&       \RBF	&     0.0001	& 0.380	& 0.380	& 0.552	& 0.763 \\
100	& 10	&      0.001	&       \RBF	&      0.001	& 0.367	& 0.364	& 0.548	& 0.741 \\
100	& 10	&      0.001	&       \RBF	&       0.01	& 0.114	& 0.140	& 0.518	& 0.517 \\
100	& 10	&       0.01	&       \LIN	&          -	& 0.144	& 0.179	& 0.487	& 0.712 \\
100	& 10	&       0.01	&       \RBF	&     0.0001	& 0.380	& 0.380	& 0.552	& 0.763 \\
100	& 10	&       0.01	&       \RBF	&      0.001	& 0.367	& 0.364	& 0.548	& 0.741 \\
100	& 10	&       0.01	&       \RBF	&       0.01	& 0.117	& 0.133	& 0.502	& 0.491 \\
100	& 10	&        0.1	&       \LIN	&          -	& 0.206	& 0.246	& 0.535	& 0.731 \\
100	& 10	&        0.1	&       \RBF	&     0.0001	& 0.380	& 0.380	& 0.552	& 0.763 \\
100	& 10	&        0.1	&       \RBF	&      0.001	& 0.367	& 0.364	& 0.548	& 0.741 \\
100	& 10	&        0.1	&       \RBF	&       0.01	& 0.082	& 0.093	& 0.504	& 0.476 \\
100	& 10	&        0.2	&       \LIN	&          -	& 0.360	& 0.359	& 0.544	& 0.754 \\
100	& 10	&        0.2	&       \RBF	&     0.0001	& 0.380	& 0.380	& 0.552	& 0.763 \\
100	& 10	&        0.2	&       \RBF	&      0.001	& 0.367	& 0.364	& 0.548	& 0.741 \\
100	& 10	&        0.2	&       \RBF	&       0.01	& 0.064	& 0.080	& 0.503	& 0.473 \\
100	& 10	&        0.4	&       \LIN	&          -	& 0.408	& 0.398	& 0.543	& 0.758 \\
100	& 10	&        0.4	&       \RBF	&     0.0001	& 0.380	& 0.380	& 0.552	& 0.763 \\
100	& 10	&        0.4	&       \RBF	&      0.001	& 0.367	& 0.364	& 0.548	& 0.741 \\
100	& 10	&        0.4	&       \RBF	&       0.01	& 0.045	& 0.062	& 0.501	& 0.471 \\
100	& 10	&        0.6	&       \LIN	&          -	& 0.409	& 0.403	& 0.544	& 0.758 \\
100	& 10	&        0.6	&       \RBF	&     0.0001	& 0.380	& 0.380	& 0.552	& 0.763 \\
100	& 10	&        0.6	&       \RBF	&      0.001	& 0.367	& 0.364	& 0.548	& 0.741 \\
100	& 10	&        0.6	&       \RBF	&       0.01	& 0.040	& 0.057	& 0.501	& 0.470 \\
100	& 10	&        0.8	&       \LIN	&          -	& 0.393	& 0.376	& 0.548	& 0.759 \\
100	& 10	&        0.8	&       \RBF	&     0.0001	& 0.380	& 0.380	& 0.552	& 0.763 \\
100	& 10	&        0.8	&       \RBF	&      0.001	& 0.367	& 0.364	& 0.548	& 0.741 \\
100	& 10	&        0.8	&       \RBF	&       0.01	& 0.036	& 0.052	& 0.499	& 0.470 \\
100	& 10	&        1.0	&       \LIN	&          -	& 0.399	& 0.377	& 0.544	& 0.759 \\
100	& 10	&        1.0	&       \RBF	&     0.0001	& 0.380	& 0.380	& 0.552	& 0.763 \\
100	& 10	&        1.0	&       \RBF	&      0.001	& 0.367	& 0.364	& 0.548	& 0.741 \\
100	& 10	&        1.0	&       \RBF	&       0.01	& 0.027	& 0.042	& 0.499	& 0.469 \\
100	& 10	&         10	&       \LIN	&          -	& 0.339	& 0.334	& 0.545	& 0.768 \\
100	& 10	&         10	&       \RBF	&     0.0001	& 0.380	& 0.380	& 0.552	& 0.763 \\
100	& 10	&         10	&       \RBF	&      0.001	& 0.367	& 0.364	& 0.548	& 0.741 \\
100	& 10	&         10	&       \RBF	&       0.01	& 0.007	& 0.027	& 0.501	& 0.468 \\
100	& 10	&         50	&       \LIN	&          -	& 0.369	& 0.380	& 0.541	& 0.770 \\
100	& 10	&         50	&       \RBF	&     0.0001	& 0.380	& 0.380	& 0.552	& 0.763 \\
100	& 10	&         50	&       \RBF	&      0.001	& 0.367	& 0.364	& 0.548	& 0.741 \\
100	& 10	&         50	&       \RBF	&       0.01	& 0.008	& 0.026	& 0.500	& 0.467 \\
100	& 10	&        100	&       \LIN	&          -	& 0.369	& 0.379	& 0.542	& 0.768 \\
100	& 10	&        100	&       \RBF	&     0.0001	& 0.380	& 0.380	& 0.552	& 0.763 \\
100	& 10	&        100	&       \RBF	&      0.001	& 0.367	& 0.364	& 0.548	& 0.741 \\
100	& 10	&        100	&       \RBF	&       0.01	& 0.005	& 0.023	& 0.499	& 0.467 \\
100	& 15	&      0.001	&       \LIN	&          -	& 0.179	& 0.208	& 0.536	& 0.714 \\
100	& 15	&      0.001	&       \RBF	&     0.0001	& 0.372	& 0.381	& 0.550	& 0.763 \\
100	& 15	&      0.001	&       \RBF	&      0.001	& 0.371	& 0.363	& 0.546	& 0.740 \\
100	& 15	&      0.001	&       \RBF	&       0.01	& 0.110	& 0.141	& 0.520	& 0.516 \\
100	& 15	&       0.01	&       \LIN	&          -	& 0.197	& 0.222	& 0.527	& 0.718 \\
100	& 15	&       0.01	&       \RBF	&     0.0001	& 0.372	& 0.381	& 0.550	& 0.763 \\
100	& 15	&       0.01	&       \RBF	&      0.001	& 0.371	& 0.363	& 0.546	& 0.740 \\
100	& 15	&       0.01	&       \RBF	&       0.01	& 0.100	& 0.124	& 0.508	& 0.490 \\
100	& 15	&        0.1	&       \LIN	&          -	& 0.217	& 0.232	& 0.544	& 0.731 \\
100	& 15	&        0.1	&       \RBF	&     0.0001	& 0.372	& 0.381	& 0.550	& 0.763 \\
100	& 15	&        0.1	&       \RBF	&      0.001	& 0.371	& 0.363	& 0.546	& 0.740 \\
100	& 15	&        0.1	&       \RBF	&       0.01	& 0.077	& 0.087	& 0.504	& 0.476 \\
100	& 15	&        0.2	&       \LIN	&          -	& 0.276	& 0.287	& 0.525	& 0.723 \\
100	& 15	&        0.2	&       \RBF	&     0.0001	& 0.372	& 0.381	& 0.550	& 0.763 \\
100	& 15	&        0.2	&       \RBF	&      0.001	& 0.371	& 0.363	& 0.546	& 0.740 \\
100	& 15	&        0.2	&       \RBF	&       0.01	& 0.066	& 0.081	& 0.504	& 0.473 \\
100	& 15	&        0.4	&       \LIN	&          -	& 0.346	& 0.343	& 0.534	& 0.731 \\
100	& 15	&        0.4	&       \RBF	&     0.0001	& 0.372	& 0.381	& 0.550	& 0.763 \\
100	& 15	&        0.4	&       \RBF	&      0.001	& 0.371	& 0.363	& 0.546	& 0.740 \\
100	& 15	&        0.4	&       \RBF	&       0.01	& 0.050	& 0.067	& 0.502	& 0.471 \\
100	& 15	&        0.6	&       \LIN	&          -	& 0.260	& 0.283	& 0.528	& 0.736 \\
100	& 15	&        0.6	&       \RBF	&     0.0001	& 0.372	& 0.381	& 0.550	& 0.763 \\
100	& 15	&        0.6	&       \RBF	&      0.001	& 0.371	& 0.363	& 0.546	& 0.740 \\
100	& 15	&        0.6	&       \RBF	&       0.01	& 0.042	& 0.058	& 0.501	& 0.470 \\
100	& 15	&        0.8	&       \LIN	&          -	& 0.301	& 0.282	& 0.524	& 0.734 \\
100	& 15	&        0.8	&       \RBF	&     0.0001	& 0.372	& 0.381	& 0.550	& 0.763 \\
100	& 15	&        0.8	&       \RBF	&      0.001	& 0.371	& 0.363	& 0.546	& 0.740 \\
100	& 15	&        0.8	&       \RBF	&       0.01	& 0.046	& 0.062	& 0.500	& 0.469 \\
100	& 15	&        1.0	&       \LIN	&          -	& 0.276	& 0.286	& 0.523	& 0.729 \\
100	& 15	&        1.0	&       \RBF	&     0.0001	& 0.372	& 0.381	& 0.550	& 0.763 \\
100	& 15	&        1.0	&       \RBF	&      0.001	& 0.371	& 0.363	& 0.546	& 0.740 \\
100	& 15	&        1.0	&       \RBF	&       0.01	& 0.030	& 0.045	& 0.499	& 0.469 \\
100	& 15	&         10	&       \LIN	&          -	& 0.381	& 0.378	& 0.557	& 0.703 \\
100	& 15	&         10	&       \RBF	&     0.0001	& 0.372	& 0.381	& 0.550	& 0.763 \\
100	& 15	&         10	&       \RBF	&      0.001	& 0.371	& 0.363	& 0.546	& 0.740 \\
100	& 15	&         10	&       \RBF	&       0.01	& 0.010	& 0.028	& 0.501	& 0.468 \\
100	& 15	&         50	&       \LIN	&          -	& 0.369	& 0.382	& 0.542	& 0.769 \\
100	& 15	&         50	&       \RBF	&     0.0001	& 0.372	& 0.381	& 0.550	& 0.763 \\
100	& 15	&         50	&       \RBF	&      0.001	& 0.371	& 0.363	& 0.546	& 0.740 \\
100	& 15	&         50	&       \RBF	&       0.01	& 0.010	& 0.028	& 0.500	& 0.467 \\
100	& 15	&        100	&       \LIN	&          -	& 0.369	& 0.379	& 0.544	& 0.768 \\
100	& 15	&        100	&       \RBF	&     0.0001	& 0.372	& 0.381	& 0.550	& 0.763 \\
100	& 15	&        100	&       \RBF	&      0.001	& 0.371	& 0.363	& 0.546	& 0.740 \\
100	& 15	&        100	&       \RBF	&       0.01	& 0.015	& 0.033	& 0.500	& 0.467 \\
150	& 5	&   0.000001	&       \RBF	&     0.0001	& 0.343	& 0.334	& 0.568	& 0.732 \\
150	& 5	&   0.000001	&       \RBF	&      0.001	& 0.267	& 0.278	& 0.558	& 0.703 \\
150	& 5	&   0.000001	&       \RBF	&       0.01	& 0.143	& 0.166	& 0.529	& 0.576 \\
150	& 5	&    0.00001	&       \RBF	&      0.001	& 0.382	& 0.367	& 0.563	& 0.740 \\
150	& 5	&    0.00001	&       \RBF	&       0.01	& 0.135	& 0.164	& 0.517	& 0.579 \\
150	& 5	&     0.0001	&       \RBF	&     0.0001	& 0.395	& 0.381	& 0.567	& 0.757 \\
150	& 5	&     0.0001	&       \RBF	&      0.001	& 0.382	& 0.367	& 0.563	& 0.740 \\
150	& 5	&     0.0001	&       \RBF	&       0.01	& 0.141	& 0.156	& 0.525	& 0.544 \\
150	& 5	&      0.001	&       \LIN	&          -	& 0.212	& 0.235	& 0.561	& 0.707 \\
150	& 5	&      0.001	&       \RBF	&     0.0001	& 0.395	& 0.381	& 0.567	& 0.757 \\
150	& 5	&      0.001	&       \RBF	&      0.001	& 0.382	& 0.367	& 0.563	& 0.740 \\
150	& 5	&      0.001	&       \RBF	&       0.01	& 0.122	& 0.148	& 0.524	& 0.512 \\
150	& 5	&       0.01	&       \LIN	&          -	& 0.253	& 0.282	& 0.555	& 0.721 \\
150	& 5	&       0.01	&       \RBF	&     0.0001	& 0.395	& 0.381	& 0.567	& 0.757 \\
150	& 5	&       0.01	&       \RBF	&      0.001	& 0.382	& 0.367	& 0.563	& 0.740 \\
150	& 5	&       0.01	&       \RBF	&       0.01	& 0.107	& 0.124	& 0.511	& 0.488 \\
150	& 5	&        0.1	&       \LIN	&          -	& 0.294	& 0.294	& 0.567	& 0.750 \\
150	& 5	&        0.1	&       \RBF	&     0.0001	& 0.395	& 0.381	& 0.567	& 0.757 \\
150	& 5	&        0.1	&       \RBF	&      0.001	& 0.382	& 0.367	& 0.563	& 0.740 \\
150	& 5	&        0.1	&       \RBF	&       0.01	& 0.083	& 0.094	& 0.502	& 0.475 \\
150	& 5	&        0.2	&       \LIN	&          -	& 0.367	& 0.349	& 0.568	& 0.702 \\
150	& 5	&        0.2	&       \RBF	&     0.0001	& 0.395	& 0.381	& 0.567	& 0.757 \\
150	& 5	&        0.2	&       \RBF	&      0.001	& 0.382	& 0.367	& 0.563	& 0.740 \\
150	& 5	&        0.2	&       \RBF	&       0.01	& 0.076	& 0.090	& 0.497	& 0.473 \\
150	& 5	&        0.4	&       \LIN	&          -	& 0.391	& 0.377	& 0.566	& 0.757 \\
150	& 5	&        0.4	&       \RBF	&     0.0001	& 0.395	& 0.381	& 0.567	& 0.757 \\
150	& 5	&        0.4	&       \RBF	&      0.001	& 0.382	& 0.367	& 0.563	& 0.740 \\
150	& 5	&        0.4	&       \RBF	&       0.01	& 0.060	& 0.072	& 0.497	& 0.471 \\
150	& 5	&        0.6	&       \LIN	&          -	& 0.397	& 0.361	& 0.564	& 0.764 \\
150	& 5	&        0.6	&       \RBF	&     0.0001	& 0.395	& 0.381	& 0.567	& 0.757 \\
150	& 5	&        0.6	&       \RBF	&      0.001	& 0.382	& 0.367	& 0.563	& 0.740 \\
150	& 5	&        0.6	&       \RBF	&       0.01	& 0.050	& 0.066	& 0.496	& 0.470 \\
150	& 5	&        0.8	&       \LIN	&          -	& 0.350	& 0.324	& 0.564	& 0.757 \\
150	& 5	&        0.8	&       \RBF	&     0.0001	& 0.395	& 0.381	& 0.567	& 0.757 \\
150	& 5	&        0.8	&       \RBF	&      0.001	& 0.382	& 0.367	& 0.563	& 0.740 \\
150	& 5	&        0.8	&       \RBF	&       0.01	& 0.039	& 0.054	& 0.495	& 0.470 \\
150	& 5	&        1.0	&       \LIN	&          -	& 0.337	& 0.332	& 0.561	& 0.762 \\
150	& 5	&        1.0	&       \RBF	&     0.0001	& 0.395	& 0.381	& 0.567	& 0.757 \\
150	& 5	&        1.0	&       \RBF	&      0.001	& 0.382	& 0.367	& 0.563	& 0.740 \\
150	& 5	&        1.0	&       \RBF	&       0.01	& 0.039	& 0.054	& 0.495	& 0.469 \\
150	& 5	&         10	&       \LIN	&          -	& 0.369	& 0.358	& 0.561	& 0.755 \\
150	& 5	&         10	&       \RBF	&     0.0001	& 0.395	& 0.381	& 0.567	& 0.757 \\
150	& 5	&         10	&       \RBF	&      0.001	& 0.382	& 0.367	& 0.563	& 0.740 \\
150	& 5	&         10	&       \RBF	&       0.01	& 0.026	& 0.043	& 0.497	& 0.468 \\
150	& 5	&         50	&       \LIN	&          -	& 0.387	& 0.371	& 0.570	& 0.692 \\
150	& 5	&         50	&       \RBF	&     0.0001	& 0.395	& 0.381	& 0.567	& 0.757 \\
150	& 5	&         50	&       \RBF	&      0.001	& 0.382	& 0.367	& 0.563	& 0.740 \\
150	& 5	&         50	&       \RBF	&       0.01	& 0.025	& 0.040	& 0.496	& 0.467 \\
150	& 5	&        100	&       \LIN	&          -	& 0.387	& 0.371	& 0.570	& 0.692 \\
150	& 5	&        100	&       \RBF	&     0.0001	& 0.395	& 0.381	& 0.567	& 0.757 \\
150	& 5	&        100	&       \RBF	&      0.001	& 0.382	& 0.367	& 0.563	& 0.740 \\
150	& 5	&        100	&       \RBF	&       0.01	& 0.025	& 0.040	& 0.496	& 0.467 \\
150	& 10	&   0.000001	&       \RBF	&       0.01	& 0.153	& 0.177	& 0.528	& 0.570 \\
150	& 10	&      0.001	&       \LIN	&          -	& 0.208	& 0.221	& 0.553	& 0.715 \\
150	& 10	&      0.001	&       \RBF	&     0.0001	& 0.393	& 0.377	& 0.564	& 0.757 \\
150	& 10	&      0.001	&       \RBF	&      0.001	& 0.385	& 0.363	& 0.564	& 0.732 \\
150	& 10	&      0.001	&       \RBF	&       0.01	& 0.141	& 0.160	& 0.528	& 0.508 \\
150	& 10	&       0.01	&       \LIN	&          -	& 0.287	& 0.289	& 0.547	& 0.710 \\
150	& 10	&       0.01	&       \RBF	&     0.0001	& 0.393	& 0.377	& 0.564	& 0.757 \\
150	& 10	&       0.01	&       \RBF	&      0.001	& 0.385	& 0.363	& 0.564	& 0.732 \\
150	& 10	&       0.01	&       \RBF	&       0.01	& 0.120	& 0.135	& 0.509	& 0.488 \\
150	& 10	&        0.1	&       \LIN	&          -	& 0.357	& 0.347	& 0.516	& 0.707 \\
150	& 10	&        0.1	&       \RBF	&     0.0001	& 0.393	& 0.377	& 0.564	& 0.757 \\
150	& 10	&        0.1	&       \RBF	&      0.001	& 0.385	& 0.363	& 0.564	& 0.732 \\
150	& 10	&        0.1	&       \RBF	&       0.01	& 0.085	& 0.096	& 0.500	& 0.475 \\
150	& 10	&        0.2	&       \LIN	&          -	& 0.245	& 0.257	& 0.553	& 0.658 \\
150	& 10	&        0.2	&       \RBF	&     0.0001	& 0.393	& 0.377	& 0.564	& 0.757 \\
150	& 10	&        0.2	&       \RBF	&      0.001	& 0.385	& 0.363	& 0.564	& 0.732 \\
150	& 10	&        0.2	&       \RBF	&       0.01	& 0.073	& 0.086	& 0.497	& 0.473 \\
150	& 10	&        0.4	&       \LIN	&          -	& 0.397	& 0.385	& 0.571	& 0.750 \\
150	& 10	&        0.4	&       \RBF	&     0.0001	& 0.393	& 0.377	& 0.564	& 0.757 \\
150	& 10	&        0.4	&       \RBF	&      0.001	& 0.385	& 0.363	& 0.564	& 0.732 \\
150	& 10	&        0.4	&       \RBF	&       0.01	& 0.059	& 0.072	& 0.496	& 0.471 \\
150	& 10	&        0.6	&       \LIN	&          -	& 0.399	& 0.390	& 0.568	& 0.751 \\
150	& 10	&        0.6	&       \RBF	&     0.0001	& 0.393	& 0.377	& 0.564	& 0.757 \\
150	& 10	&        0.6	&       \RBF	&      0.001	& 0.385	& 0.363	& 0.564	& 0.732 \\
150	& 10	&        0.6	&       \RBF	&       0.01	& 0.052	& 0.065	& 0.495	& 0.470 \\
150	& 10	&        0.8	&       \LIN	&          -	& 0.370	& 0.355	& 0.572	& 0.752 \\
150	& 10	&        0.8	&       \RBF	&     0.0001	& 0.393	& 0.377	& 0.564	& 0.757 \\
150	& 10	&        0.8	&       \RBF	&      0.001	& 0.385	& 0.363	& 0.564	& 0.732 \\
150	& 10	&        0.8	&       \RBF	&       0.01	& 0.045	& 0.057	& 0.494	& 0.470 \\
150	& 10	&        1.0	&       \LIN	&          -	& 0.386	& 0.357	& 0.568	& 0.753 \\
150	& 10	&        1.0	&       \RBF	&     0.0001	& 0.393	& 0.377	& 0.564	& 0.757 \\
150	& 10	&        1.0	&       \RBF	&      0.001	& 0.385	& 0.363	& 0.564	& 0.732 \\
150	& 10	&        1.0	&       \RBF	&       0.01	& 0.045	& 0.057	& 0.494	& 0.469 \\
150	& 10	&         10	&       \LIN	&          -	& 0.374	& 0.368	& 0.562	& 0.764 \\
150	& 10	&         10	&       \RBF	&     0.0001	& 0.393	& 0.377	& 0.564	& 0.757 \\
150	& 10	&         10	&       \RBF	&      0.001	& 0.385	& 0.363	& 0.564	& 0.732 \\
150	& 10	&         10	&       \RBF	&       0.01	& 0.028	& 0.043	& 0.497	& 0.468 \\
150	& 10	&         50	&       \LIN	&          -	& 0.386	& 0.389	& 0.557	& 0.756 \\
150	& 10	&         50	&       \RBF	&     0.0001	& 0.393	& 0.377	& 0.564	& 0.757 \\
150	& 10	&         50	&       \RBF	&      0.001	& 0.385	& 0.363	& 0.564	& 0.732 \\
150	& 10	&         50	&       \RBF	&       0.01	& 0.028	& 0.044	& 0.497	& 0.467 \\
150	& 10	&        100	&       \LIN	&          -	& 0.386	& 0.388	& 0.559	& 0.760 \\
150	& 10	&        100	&       \RBF	&     0.0001	& 0.393	& 0.377	& 0.564	& 0.757 \\
150	& 10	&        100	&       \RBF	&      0.001	& 0.385	& 0.363	& 0.564	& 0.732 \\
150	& 10	&        100	&       \RBF	&       0.01	& 0.025	& 0.040	& 0.496	& 0.467 \\
150	& 15	&      0.001	&       \LIN	&          -	& 0.141	& 0.173	& 0.510	& 0.717 \\
150	& 15	&      0.001	&       \RBF	&     0.0001	& 0.389	& 0.389	& 0.562	& 0.756 \\
150	& 15	&      0.001	&       \RBF	&      0.001	& 0.386	& 0.368	& 0.565	& 0.731 \\
150	& 15	&      0.001	&       \RBF	&       0.01	& 0.132	& 0.150	& 0.525	& 0.508 \\
150	& 15	&       0.01	&       \LIN	&          -	& 0.187	& 0.214	& 0.529	& 0.723 \\
150	& 15	&       0.01	&       \RBF	&     0.0001	& 0.389	& 0.389	& 0.562	& 0.756 \\
150	& 15	&       0.01	&       \RBF	&      0.001	& 0.386	& 0.368	& 0.565	& 0.731 \\
150	& 15	&       0.01	&       \RBF	&       0.01	& 0.108	& 0.124	& 0.512	& 0.488 \\
150	& 15	&        0.1	&       \LIN	&          -	& 0.366	& 0.359	& 0.540	& 0.733 \\
150	& 15	&        0.1	&       \RBF	&     0.0001	& 0.389	& 0.389	& 0.562	& 0.756 \\
150	& 15	&        0.1	&       \RBF	&      0.001	& 0.386	& 0.368	& 0.565	& 0.731 \\
150	& 15	&        0.1	&       \RBF	&       0.01	& 0.083	& 0.092	& 0.501	& 0.475 \\
150	& 15	&        0.2	&       \LIN	&          -	& 0.277	& 0.283	& 0.538	& 0.728 \\
150	& 15	&        0.2	&       \RBF	&     0.0001	& 0.389	& 0.389	& 0.562	& 0.756 \\
150	& 15	&        0.2	&       \RBF	&      0.001	& 0.386	& 0.368	& 0.565	& 0.731 \\
150	& 15	&        0.2	&       \RBF	&       0.01	& 0.067	& 0.083	& 0.499	& 0.473 \\
150	& 15	&        0.4	&       \LIN	&          -	& 0.392	& 0.369	& 0.572	& 0.735 \\
150	& 15	&        0.4	&       \RBF	&     0.0001	& 0.389	& 0.389	& 0.562	& 0.756 \\
150	& 15	&        0.4	&       \RBF	&      0.001	& 0.386	& 0.368	& 0.565	& 0.731 \\
150	& 15	&        0.4	&       \RBF	&       0.01	& 0.060	& 0.073	& 0.496	& 0.471 \\
150	& 15	&        0.6	&       \LIN	&          -	& 0.391	& 0.372	& 0.571	& 0.732 \\
150	& 15	&        0.6	&       \RBF	&     0.0001	& 0.389	& 0.389	& 0.562	& 0.756 \\
150	& 15	&        0.6	&       \RBF	&      0.001	& 0.386	& 0.368	& 0.565	& 0.731 \\
150	& 15	&        0.6	&       \RBF	&       0.01	& 0.051	& 0.064	& 0.496	& 0.470 \\
150	& 15	&        0.8	&       \LIN	&          -	& 0.392	& 0.376	& 0.571	& 0.729 \\
150	& 15	&        0.8	&       \RBF	&     0.0001	& 0.389	& 0.389	& 0.562	& 0.756 \\
150	& 15	&        0.8	&       \RBF	&      0.001	& 0.386	& 0.368	& 0.565	& 0.731 \\
150	& 15	&        0.8	&       \RBF	&       0.01	& 0.052	& 0.066	& 0.494	& 0.469 \\
150	& 15	&        1.0	&       \LIN	&          -	& 0.393	& 0.382	& 0.573	& 0.725 \\
150	& 15	&        1.0	&       \RBF	&     0.0001	& 0.389	& 0.389	& 0.562	& 0.756 \\
150	& 15	&        1.0	&       \RBF	&      0.001	& 0.386	& 0.368	& 0.565	& 0.731 \\
150	& 15	&        1.0	&       \RBF	&       0.01	& 0.041	& 0.054	& 0.494	& 0.469 \\
150	& 15	&         10	&       \LIN	&          -	& 0.391	& 0.376	& 0.569	& 0.700 \\
150	& 15	&         10	&       \RBF	&     0.0001	& 0.389	& 0.389	& 0.562	& 0.756 \\
150	& 15	&         10	&       \RBF	&      0.001	& 0.386	& 0.368	& 0.565	& 0.731 \\
150	& 15	&         10	&       \RBF	&       0.01	& 0.029	& 0.044	& 0.497	& 0.468 \\
150	& 15	&         50	&       \LIN	&          -	& 0.387	& 0.388	& 0.557	& 0.756 \\
150	& 15	&         50	&       \RBF	&     0.0001	& 0.389	& 0.389	& 0.562	& 0.756 \\
150	& 15	&         50	&       \RBF	&      0.001	& 0.386	& 0.368	& 0.565	& 0.731 \\
150	& 15	&         50	&       \RBF	&       0.01	& 0.030	& 0.044	& 0.497	& 0.467 \\
150	& 15	&        100	&       \LIN	&          -	& 0.382	& 0.384	& 0.556	& 0.761 \\
150	& 15	&        100	&       \RBF	&     0.0001	& 0.389	& 0.389	& 0.563	& 0.756 \\
150	& 15	&        100	&       \RBF	&      0.001	& 0.386	& 0.368	& 0.565	& 0.731 \\
150	& 15	&        100	&       \RBF	&       0.01	& 0.032	& 0.046	& 0.497	& 0.467 \\
200	& 5	&   0.000001	&       \RBF	&     0.0001	& 0.293	& 0.290	& 0.551	& 0.724 \\
200	& 5	&   0.000001	&       \RBF	&      0.001	& 0.305	& 0.315	& 0.554	& 0.698 \\
200	& 5	&   0.000001	&       \RBF	&       0.01	& 0.156	& 0.171	& 0.524	& 0.564 \\
200	& 5	&    0.00001	&       \LIN	&          -	& 0.144	& 0.175	& 0.531	& 0.704 \\
200	& 5	&    0.00001	&       \RBF	&      0.001	& 0.373	& 0.358	& 0.554	& 0.734 \\
200	& 5	&    0.00001	&       \RBF	&       0.01	& 0.148	& 0.172	& 0.519	& 0.566 \\
200	& 5	&     0.0001	&       \RBF	&     0.0001	& 0.394	& 0.387	& 0.557	& 0.752 \\
200	& 5	&     0.0001	&       \RBF	&      0.001	& 0.373	& 0.358	& 0.554	& 0.734 \\
200	& 5	&     0.0001	&       \RBF	&       0.01	& 0.141	& 0.162	& 0.522	& 0.535 \\
200	& 5	&      0.001	&       \LIN	&          -	& 0.216	& 0.235	& 0.541	& 0.710 \\
200	& 5	&      0.001	&       \RBF	&     0.0001	& 0.394	& 0.387	& 0.557	& 0.752 \\
200	& 5	&      0.001	&       \RBF	&      0.001	& 0.373	& 0.358	& 0.554	& 0.734 \\
200	& 5	&      0.001	&       \RBF	&       0.01	& 0.117	& 0.135	& 0.528	& 0.508 \\
200	& 5	&       0.01	&       \LIN	&          -	& 0.312	& 0.310	& 0.504	& 0.697 \\
200	& 5	&       0.01	&       \RBF	&     0.0001	& 0.394	& 0.387	& 0.557	& 0.752 \\
200	& 5	&       0.01	&       \RBF	&      0.001	& 0.373	& 0.358	& 0.554	& 0.734 \\
200	& 5	&       0.01	&       \RBF	&       0.01	& 0.091	& 0.108	& 0.509	& 0.486 \\
200	& 5	&        0.1	&       \LIN	&          -	& 0.391	& 0.360	& 0.553	& 0.750 \\
200	& 5	&        0.1	&       \RBF	&     0.0001	& 0.394	& 0.387	& 0.557	& 0.752 \\
200	& 5	&        0.1	&       \RBF	&      0.001	& 0.373	& 0.358	& 0.554	& 0.734 \\
200	& 5	&        0.1	&       \RBF	&       0.01	& 0.063	& 0.076	& 0.501	& 0.475 \\
200	& 5	&        0.2	&       \LIN	&          -	& 0.400	& 0.374	& 0.553	& 0.753 \\
200	& 5	&        0.2	&       \RBF	&     0.0001	& 0.394	& 0.387	& 0.557	& 0.752 \\
200	& 5	&        0.2	&       \RBF	&      0.001	& 0.373	& 0.358	& 0.554	& 0.734 \\
200	& 5	&        0.2	&       \RBF	&       0.01	& 0.057	& 0.072	& 0.500	& 0.473 \\
200	& 5	&        0.4	&       \LIN	&          -	& 0.405	& 0.379	& 0.552	& 0.759 \\
200	& 5	&        0.4	&       \RBF	&     0.0001	& 0.394	& 0.387	& 0.557	& 0.752 \\
200	& 5	&        0.4	&       \RBF	&      0.001	& 0.373	& 0.358	& 0.554	& 0.734 \\
200	& 5	&        0.4	&       \RBF	&       0.01	& 0.044	& 0.060	& 0.498	& 0.472 \\
200	& 5	&        0.6	&       \LIN	&          -	& 0.347	& 0.318	& 0.552	& 0.754 \\
200	& 5	&        0.6	&       \RBF	&     0.0001	& 0.394	& 0.387	& 0.557	& 0.752 \\
200	& 5	&        0.6	&       \RBF	&      0.001	& 0.373	& 0.358	& 0.554	& 0.734 \\
200	& 5	&        0.6	&       \RBF	&       0.01	& 0.041	& 0.056	& 0.498	& 0.471 \\
200	& 5	&        0.8	&       \LIN	&          -	& 0.432	& 0.398	& 0.551	& 0.749 \\
200	& 5	&        0.8	&       \RBF	&     0.0001	& 0.394	& 0.387	& 0.557	& 0.752 \\
200	& 5	&        0.8	&       \RBF	&      0.001	& 0.373	& 0.358	& 0.554	& 0.734 \\
200	& 5	&        0.8	&       \RBF	&       0.01	& 0.039	& 0.053	& 0.497	& 0.470 \\
200	& 5	&        1.0	&       \LIN	&          -	& 0.345	& 0.332	& 0.552	& 0.760 \\
200	& 5	&        1.0	&       \RBF	&     0.0001	& 0.394	& 0.387	& 0.557	& 0.752 \\
200	& 5	&        1.0	&       \RBF	&      0.001	& 0.373	& 0.358	& 0.554	& 0.734 \\
200	& 5	&        1.0	&       \RBF	&       0.01	& 0.036	& 0.050	& 0.498	& 0.470 \\
200	& 5	&         10	&       \LIN	&          -	& 0.393	& 0.382	& 0.552	& 0.750 \\
200	& 5	&         10	&       \RBF	&     0.0001	& 0.394	& 0.387	& 0.557	& 0.752 \\
200	& 5	&         10	&       \RBF	&      0.001	& 0.373	& 0.358	& 0.554	& 0.734 \\
200	& 5	&         10	&       \RBF	&       0.01	& 0.024	& 0.039	& 0.499	& 0.468 \\
200	& 5	&         50	&       \LIN	&          -	& 0.390	& 0.374	& 0.561	& 0.690 \\
200	& 5	&         50	&       \RBF	&     0.0001	& 0.394	& 0.387	& 0.557	& 0.752 \\
200	& 5	&         50	&       \RBF	&      0.001	& 0.376	& 0.359	& 0.554	& 0.734 \\
200	& 5	&         50	&       \RBF	&       0.01	& 0.018	& 0.033	& 0.498	& 0.468 \\
200	& 5	&        100	&       \LIN	&          -	& 0.390	& 0.374	& 0.561	& 0.690 \\
200	& 5	&        100	&       \RBF	&     0.0001	& 0.394	& 0.387	& 0.557	& 0.752 \\
200	& 5	&        100	&       \RBF	&      0.001	& 0.376	& 0.359	& 0.554	& 0.734 \\
200	& 5	&        100	&       \RBF	&       0.01	& 0.017	& 0.032	& 0.498	& 0.468 \\
200	& 10	&   0.000001	&       \LIN	&          -	& 0.101	& 0.122	& 0.527	& 0.703 \\
200	& 10	&   0.000001	&       \RBF	&       0.01	& 0.163	& 0.173	& 0.527	& 0.560 \\
200	& 10	&      0.001	&       \LIN	&          -	& 0.182	& 0.204	& 0.544	& 0.713 \\
200	& 10	&      0.001	&       \RBF	&     0.0001	& 0.392	& 0.388	& 0.556	& 0.751 \\
200	& 10	&      0.001	&       \RBF	&      0.001	& 0.373	& 0.365	& 0.558	& 0.725 \\
200	& 10	&      0.001	&       \RBF	&       0.01	& 0.123	& 0.134	& 0.527	& 0.505 \\
200	& 10	&       0.01	&       \LIN	&          -	& 0.273	& 0.281	& 0.530	& 0.718 \\
200	& 10	&       0.01	&       \RBF	&     0.0001	& 0.392	& 0.388	& 0.556	& 0.751 \\
200	& 10	&       0.01	&       \RBF	&      0.001	& 0.373	& 0.365	& 0.558	& 0.725 \\
200	& 10	&       0.01	&       \RBF	&       0.01	& 0.094	& 0.108	& 0.509	& 0.485 \\
200	& 10	&        0.1	&       \LIN	&          -	& 0.394	& 0.375	& 0.559	& 0.745 \\
200	& 10	&        0.1	&       \RBF	&     0.0001	& 0.392	& 0.388	& 0.556	& 0.751 \\
200	& 10	&        0.1	&       \RBF	&      0.001	& 0.373	& 0.365	& 0.558	& 0.725 \\
200	& 10	&        0.1	&       \RBF	&       0.01	& 0.065	& 0.075	& 0.502	& 0.475 \\
200	& 10	&        0.2	&       \LIN	&          -	& 0.407	& 0.382	& 0.556	& 0.747 \\
200	& 10	&        0.2	&       \RBF	&     0.0001	& 0.392	& 0.388	& 0.556	& 0.751 \\
200	& 10	&        0.2	&       \RBF	&      0.001	& 0.373	& 0.365	& 0.558	& 0.725 \\
200	& 10	&        0.2	&       \RBF	&       0.01	& 0.056	& 0.071	& 0.500	& 0.473 \\
200	& 10	&        0.4	&       \LIN	&          -	& 0.342	& 0.332	& 0.554	& 0.749 \\
200	& 10	&        0.4	&       \RBF	&     0.0001	& 0.392	& 0.388	& 0.556	& 0.751 \\
200	& 10	&        0.4	&       \RBF	&      0.001	& 0.373	& 0.365	& 0.558	& 0.725 \\
200	& 10	&        0.4	&       \RBF	&       0.01	& 0.043	& 0.057	& 0.497	& 0.471 \\
200	& 10	&        0.6	&       \LIN	&          -	& 0.324	& 0.321	& 0.556	& 0.751 \\
200	& 10	&        0.6	&       \RBF	&     0.0001	& 0.392	& 0.388	& 0.556	& 0.751 \\
200	& 10	&        0.6	&       \RBF	&      0.001	& 0.373	& 0.365	& 0.558	& 0.725 \\
200	& 10	&        0.6	&       \RBF	&       0.01	& 0.040	& 0.053	& 0.498	& 0.471 \\
200	& 10	&        0.8	&       \LIN	&          -	& 0.404	& 0.373	& 0.553	& 0.751 \\
200	& 10	&        0.8	&       \RBF	&     0.0001	& 0.392	& 0.388	& 0.556	& 0.751 \\
200	& 10	&        0.8	&       \RBF	&      0.001	& 0.373	& 0.365	& 0.558	& 0.725 \\
200	& 10	&        0.8	&       \RBF	&       0.01	& 0.035	& 0.049	& 0.497	& 0.470 \\
200	& 10	&        1.0	&       \LIN	&          -	& 0.358	& 0.360	& 0.550	& 0.751 \\
200	& 10	&        1.0	&       \RBF	&     0.0001	& 0.392	& 0.388	& 0.556	& 0.751 \\
200	& 10	&        1.0	&       \RBF	&      0.001	& 0.373	& 0.365	& 0.558	& 0.725 \\
200	& 10	&        1.0	&       \RBF	&       0.01	& 0.035	& 0.050	& 0.497	& 0.470 \\
200	& 10	&         10	&       \LIN	&          -	& 0.385	& 0.381	& 0.550	& 0.756 \\
200	& 10	&         10	&       \RBF	&     0.0001	& 0.392	& 0.388	& 0.556	& 0.751 \\
200	& 10	&         10	&       \RBF	&      0.001	& 0.373	& 0.365	& 0.558	& 0.725 \\
200	& 10	&         10	&       \RBF	&       0.01	& 0.022	& 0.038	& 0.499	& 0.468 \\
200	& 10	&         50	&       \LIN	&          -	& 0.392	& 0.383	& 0.550	& 0.755 \\
200	& 10	&         50	&       \RBF	&     0.0001	& 0.392	& 0.388	& 0.556	& 0.751 \\
200	& 10	&         50	&       \RBF	&      0.001	& 0.373	& 0.365	& 0.558	& 0.725 \\
200	& 10	&         50	&       \RBF	&       0.01	& 0.025	& 0.040	& 0.498	& 0.468 \\
200	& 10	&        100	&       \LIN	&          -	& 0.390	& 0.390	& 0.552	& 0.756 \\
200	& 10	&        100	&       \RBF	&     0.0001	& 0.392	& 0.388	& 0.556	& 0.751 \\
200	& 10	&        100	&       \RBF	&      0.001	& 0.373	& 0.365	& 0.558	& 0.725 \\
200	& 10	&        100	&       \RBF	&       0.01	& 0.017	& 0.032	& 0.498	& 0.468 \\
200	& 15	&      0.001	&       \LIN	&          -	& 0.186	& 0.208	& 0.521	& 0.708 \\
200	& 15	&      0.001	&       \RBF	&     0.0001	& 0.396	& 0.388	& 0.555	& 0.750 \\
200	& 15	&      0.001	&       \RBF	&      0.001	& 0.371	& 0.365	& 0.556	& 0.724 \\
200	& 15	&      0.001	&       \RBF	&       0.01	& 0.118	& 0.131	& 0.529	& 0.504 \\
200	& 15	&       0.01	&       \LIN	&          -	& 0.239	& 0.254	& 0.531	& 0.721 \\
200	& 15	&       0.01	&       \RBF	&     0.0001	& 0.396	& 0.388	& 0.555	& 0.750 \\
200	& 15	&       0.01	&       \RBF	&      0.001	& 0.371	& 0.365	& 0.556	& 0.724 \\
200	& 15	&       0.01	&       \RBF	&       0.01	& 0.093	& 0.108	& 0.507	& 0.485 \\
200	& 15	&        0.1	&       \LIN	&          -	& 0.242	& 0.234	& 0.531	& 0.721 \\
200	& 15	&        0.1	&       \RBF	&     0.0001	& 0.396	& 0.388	& 0.555	& 0.750 \\
200	& 15	&        0.1	&       \RBF	&      0.001	& 0.371	& 0.365	& 0.556	& 0.724 \\
200	& 15	&        0.1	&       \RBF	&       0.01	& 0.065	& 0.075	& 0.503	& 0.475 \\
200	& 15	&        0.2	&       \LIN	&          -	& 0.314	& 0.308	& 0.509	& 0.721 \\
200	& 15	&        0.2	&       \RBF	&     0.0001	& 0.396	& 0.388	& 0.555	& 0.750 \\
200	& 15	&        0.2	&       \RBF	&      0.001	& 0.371	& 0.365	& 0.556	& 0.724 \\
200	& 15	&        0.2	&       \RBF	&       0.01	& 0.060	& 0.073	& 0.500	& 0.473 \\
200	& 15	&        0.4	&       \LIN	&          -	& 0.312	& 0.316	& 0.541	& 0.704 \\
200	& 15	&        0.4	&       \RBF	&     0.0001	& 0.396	& 0.388	& 0.555	& 0.750 \\
200	& 15	&        0.4	&       \RBF	&      0.001	& 0.371	& 0.365	& 0.556	& 0.724 \\
200	& 15	&        0.4	&       \RBF	&       0.01	& 0.049	& 0.062	& 0.498	& 0.471 \\
200	& 15	&        0.6	&       \LIN	&          -	& 0.344	& 0.322	& 0.550	& 0.706 \\
200	& 15	&        0.6	&       \RBF	&     0.0001	& 0.396	& 0.388	& 0.555	& 0.750 \\
200	& 15	&        0.6	&       \RBF	&      0.001	& 0.371	& 0.365	& 0.556	& 0.724 \\
200	& 15	&        0.6	&       \RBF	&       0.01	& 0.041	& 0.055	& 0.498	& 0.470 \\
200	& 15	&        0.8	&       \LIN	&          -	& 0.294	& 0.297	& 0.534	& 0.692 \\
200	& 15	&        0.8	&       \RBF	&     0.0001	& 0.396	& 0.388	& 0.555	& 0.750 \\
200	& 15	&        0.8	&       \RBF	&      0.001	& 0.371	& 0.365	& 0.556	& 0.724 \\
200	& 15	&        0.8	&       \RBF	&       0.01	& 0.042	& 0.054	& 0.497	& 0.470 \\
200	& 15	&        1.0	&       \LIN	&          -	& 0.289	& 0.305	& 0.553	& 0.698 \\
200	& 15	&        1.0	&       \RBF	&     0.0001	& 0.396	& 0.388	& 0.555	& 0.750 \\
200	& 15	&        1.0	&       \RBF	&      0.001	& 0.371	& 0.365	& 0.556	& 0.724 \\
200	& 15	&        1.0	&       \RBF	&       0.01	& 0.034	& 0.049	& 0.496	& 0.470 \\
200	& 15	&         10	&       \LIN	&          -	& 0.285	& 0.304	& 0.493	& 0.677 \\
200	& 15	&         10	&       \RBF	&     0.0001	& 0.396	& 0.388	& 0.555	& 0.750 \\
200	& 15	&         10	&       \RBF	&      0.001	& 0.371	& 0.365	& 0.556	& 0.724 \\
200	& 15	&         10	&       \RBF	&       0.01	& 0.023	& 0.038	& 0.498	& 0.468 \\
200	& 15	&         50	&       \LIN	&          -	& 0.389	& 0.379	& 0.548	& 0.751 \\
200	& 15	&         50	&       \RBF	&     0.0001	& 0.396	& 0.388	& 0.555	& 0.750 \\
200	& 15	&         50	&       \RBF	&      0.001	& 0.371	& 0.365	& 0.556	& 0.724 \\
200	& 15	&         50	&       \RBF	&       0.01	& 0.025	& 0.040	& 0.498	& 0.468 \\
200	& 15	&        100	&       \LIN	&          -	& 0.392	& 0.379	& 0.549	& 0.753 \\
200	& 15	&        100	&       \RBF	&     0.0001	& 0.396	& 0.388	& 0.555	& 0.750 \\
200	& 15	&        100	&       \RBF	&      0.001	& 0.371	& 0.365	& 0.556	& 0.724 \\
200	& 15	&        100	&       \RBF	&       0.01	& 0.025	& 0.040	& 0.498	& 0.468 \\
250	& 5	&   0.000001	&       \LIN	&          -	& 0.165	& 0.188	& 0.541	& 0.698 \\
250	& 5	&   0.000001	&       \RBF	&     0.0001	& 0.281	& 0.282	& 0.554	& 0.728 \\
250	& 5	&   0.000001	&       \RBF	&      0.001	& 0.320	& 0.315	& 0.555	& 0.699 \\
250	& 5	&   0.000001	&       \RBF	&       0.01	& 0.172	& 0.190	& 0.525	& 0.563 \\
250	& 5	&    0.00001	&       \RBF	&     0.0001	& 0.395	& 0.373	& 0.555	& 0.766 \\
250	& 5	&    0.00001	&       \RBF	&      0.001	& 0.395	& 0.375	& 0.561	& 0.736 \\
250	& 5	&    0.00001	&       \RBF	&       0.01	& 0.161	& 0.182	& 0.518	& 0.561 \\
250	& 5	&     0.0001	&       \RBF	&     0.0001	& 0.396	& 0.384	& 0.557	& 0.756 \\
250	& 5	&     0.0001	&       \RBF	&      0.001	& 0.395	& 0.375	& 0.561	& 0.736 \\
250	& 5	&     0.0001	&       \RBF	&       0.01	& 0.141	& 0.159	& 0.524	& 0.531 \\
250	& 5	&      0.001	&       \LIN	&          -	& 0.200	& 0.223	& 0.535	& 0.711 \\
250	& 5	&      0.001	&       \RBF	&     0.0001	& 0.396	& 0.384	& 0.557	& 0.756 \\
250	& 5	&      0.001	&       \RBF	&      0.001	& 0.395	& 0.375	& 0.561	& 0.736 \\
250	& 5	&      0.001	&       \RBF	&       0.01	& 0.123	& 0.140	& 0.520	& 0.506 \\
250	& 5	&       0.01	&       \LIN	&          -	& 0.317	& 0.325	& 0.537	& 0.703 \\
250	& 5	&       0.01	&       \RBF	&     0.0001	& 0.396	& 0.384	& 0.557	& 0.756 \\
250	& 5	&       0.01	&       \RBF	&      0.001	& 0.395	& 0.375	& 0.561	& 0.736 \\
250	& 5	&       0.01	&       \RBF	&       0.01	& 0.094	& 0.108	& 0.504	& 0.487 \\
250	& 5	&        0.1	&       \LIN	&          -	& 0.381	& 0.373	& 0.544	& 0.728 \\
250	& 5	&        0.1	&       \RBF	&     0.0001	& 0.396	& 0.384	& 0.557	& 0.756 \\
250	& 5	&        0.1	&       \RBF	&      0.001	& 0.395	& 0.375	& 0.561	& 0.736 \\
250	& 5	&        0.1	&       \RBF	&       0.01	& 0.065	& 0.074	& 0.503	& 0.476 \\
250	& 5	&        0.2	&       \LIN	&          -	& 0.381	& 0.365	& 0.558	& 0.752 \\
250	& 5	&        0.2	&       \RBF	&     0.0001	& 0.396	& 0.384	& 0.557	& 0.756 \\
250	& 5	&        0.2	&       \RBF	&      0.001	& 0.395	& 0.375	& 0.561	& 0.736 \\
250	& 5	&        0.2	&       \RBF	&       0.01	& 0.050	& 0.064	& 0.502	& 0.474 \\
250	& 5	&        0.4	&       \LIN	&          -	& 0.393	& 0.377	& 0.554	& 0.757 \\
250	& 5	&        0.4	&       \RBF	&     0.0001	& 0.396	& 0.384	& 0.557	& 0.756 \\
250	& 5	&        0.4	&       \RBF	&      0.001	& 0.395	& 0.375	& 0.561	& 0.736 \\
250	& 5	&        0.4	&       \RBF	&       0.01	& 0.041	& 0.057	& 0.500	& 0.473 \\
250	& 5	&        0.6	&       \LIN	&          -	& 0.394	& 0.384	& 0.550	& 0.761 \\
250	& 5	&        0.6	&       \RBF	&     0.0001	& 0.396	& 0.384	& 0.557	& 0.756 \\
250	& 5	&        0.6	&       \RBF	&      0.001	& 0.395	& 0.375	& 0.561	& 0.736 \\
250	& 5	&        0.6	&       \RBF	&       0.01	& 0.043	& 0.058	& 0.500	& 0.472 \\
250	& 5	&        0.8	&       \LIN	&          -	& 0.398	& 0.374	& 0.551	& 0.759 \\
250	& 5	&        0.8	&       \RBF	&     0.0001	& 0.396	& 0.384	& 0.557	& 0.756 \\
250	& 5	&        0.8	&       \RBF	&      0.001	& 0.395	& 0.375	& 0.561	& 0.736 \\
250	& 5	&        0.8	&       \RBF	&       0.01	& 0.038	& 0.052	& 0.499	& 0.471 \\
250	& 5	&        1.0	&       \LIN	&          -	& 0.430	& 0.404	& 0.551	& 0.758 \\
250	& 5	&        1.0	&       \RBF	&     0.0001	& 0.396	& 0.384	& 0.557	& 0.756 \\
250	& 5	&        1.0	&       \RBF	&      0.001	& 0.395	& 0.375	& 0.561	& 0.736 \\
250	& 5	&        1.0	&       \RBF	&       0.01	& 0.032	& 0.047	& 0.499	& 0.471 \\
250	& 5	&         10	&       \LIN	&          -	& 0.381	& 0.374	& 0.553	& 0.752 \\
250	& 5	&         10	&       \RBF	&     0.0001	& 0.396	& 0.384	& 0.557	& 0.756 \\
250	& 5	&         10	&       \RBF	&      0.001	& 0.395	& 0.375	& 0.561	& 0.736 \\
250	& 5	&         10	&       \RBF	&       0.01	& 0.019	& 0.035	& 0.502	& 0.469 \\
250	& 5	&         50	&       \LIN	&          -	& 0.391	& 0.383	& 0.556	& 0.699 \\
250	& 5	&         50	&       \RBF	&     0.0001	& 0.396	& 0.384	& 0.557	& 0.756 \\
250	& 5	&         50	&       \RBF	&      0.001	& 0.395	& 0.375	& 0.562	& 0.736 \\
250	& 5	&         50	&       \RBF	&       0.01	& 0.018	& 0.033	& 0.502	& 0.469 \\
250	& 5	&        100	&       \LIN	&          -	& 0.391	& 0.383	& 0.556	& 0.699 \\
250	& 5	&        100	&       \RBF	&     0.0001	& 0.396	& 0.384	& 0.557	& 0.756 \\
250	& 5	&        100	&       \RBF	&      0.001	& 0.395	& 0.375	& 0.561	& 0.736 \\
250	& 5	&        100	&       \RBF	&       0.01	& 0.016	& 0.030	& 0.502	& 0.468 \\
250	& 10	&   0.000001	&       \LIN	&          -	& 0.142	& 0.171	& 0.529	& 0.701 \\
250	& 10	&   0.000001	&       \RBF	&       0.01	& 0.175	& 0.186	& 0.526	& 0.560 \\
250	& 10	&      0.001	&       \LIN	&          -	& 0.277	& 0.269	& 0.533	& 0.693 \\
250	& 10	&      0.001	&       \RBF	&     0.0001	& 0.397	& 0.385	& 0.555	& 0.755 \\
250	& 10	&      0.001	&       \RBF	&      0.001	& 0.376	& 0.362	& 0.557	& 0.729 \\
250	& 10	&      0.001	&       \RBF	&       0.01	& 0.129	& 0.144	& 0.527	& 0.504 \\
250	& 10	&       0.01	&       \LIN	&          -	& 0.178	& 0.199	& 0.542	& 0.724 \\
250	& 10	&       0.01	&       \RBF	&     0.0001	& 0.397	& 0.385	& 0.555	& 0.755 \\
250	& 10	&       0.01	&       \RBF	&      0.001	& 0.376	& 0.362	& 0.557	& 0.729 \\
250	& 10	&       0.01	&       \RBF	&       0.01	& 0.092	& 0.107	& 0.506	& 0.486 \\
250	& 10	&        0.1	&       \LIN	&          -	& 0.229	& 0.260	& 0.537	& 0.730 \\
250	& 10	&        0.1	&       \RBF	&     0.0001	& 0.397	& 0.385	& 0.555	& 0.755 \\
250	& 10	&        0.1	&       \RBF	&      0.001	& 0.376	& 0.362	& 0.557	& 0.729 \\
250	& 10	&        0.1	&       \RBF	&       0.01	& 0.065	& 0.077	& 0.502	& 0.476 \\
250	& 10	&        0.2	&       \LIN	&          -	& 0.420	& 0.388	& 0.558	& 0.749 \\
250	& 10	&        0.2	&       \RBF	&     0.0001	& 0.397	& 0.385	& 0.555	& 0.755 \\
250	& 10	&        0.2	&       \RBF	&      0.001	& 0.376	& 0.362	& 0.557	& 0.729 \\
250	& 10	&        0.2	&       \RBF	&       0.01	& 0.058	& 0.074	& 0.502	& 0.474 \\
250	& 10	&        0.4	&       \LIN	&          -	& 0.419	& 0.386	& 0.558	& 0.749 \\
250	& 10	&        0.4	&       \RBF	&     0.0001	& 0.397	& 0.385	& 0.555	& 0.755 \\
250	& 10	&        0.4	&       \RBF	&      0.001	& 0.376	& 0.362	& 0.557	& 0.729 \\
250	& 10	&        0.4	&       \RBF	&       0.01	& 0.044	& 0.060	& 0.500	& 0.472 \\
250	& 10	&        0.6	&       \LIN	&          -	& 0.422	& 0.387	& 0.558	& 0.750 \\
250	& 10	&        0.6	&       \RBF	&     0.0001	& 0.397	& 0.385	& 0.555	& 0.755 \\
250	& 10	&        0.6	&       \RBF	&      0.001	& 0.376	& 0.362	& 0.557	& 0.729 \\
250	& 10	&        0.6	&       \RBF	&       0.01	& 0.043	& 0.058	& 0.499	& 0.472 \\
250	& 10	&        0.8	&       \LIN	&          -	& 0.376	& 0.361	& 0.554	& 0.751 \\
250	& 10	&        0.8	&       \RBF	&     0.0001	& 0.397	& 0.385	& 0.555	& 0.755 \\
250	& 10	&        0.8	&       \RBF	&      0.001	& 0.376	& 0.362	& 0.557	& 0.729 \\
250	& 10	&        0.8	&       \RBF	&       0.01	& 0.040	& 0.054	& 0.499	& 0.471 \\
250	& 10	&        1.0	&       \LIN	&          -	& 0.384	& 0.373	& 0.555	& 0.750 \\
250	& 10	&        1.0	&       \RBF	&     0.0001	& 0.397	& 0.385	& 0.555	& 0.755 \\
250	& 10	&        1.0	&       \RBF	&      0.001	& 0.376	& 0.362	& 0.557	& 0.729 \\
250	& 10	&        1.0	&       \RBF	&       0.01	& 0.036	& 0.051	& 0.500	& 0.471 \\
250	& 10	&         10	&       \LIN	&          -	& 0.392	& 0.383	& 0.553	& 0.761 \\
250	& 10	&         10	&       \RBF	&     0.0001	& 0.397	& 0.385	& 0.555	& 0.755 \\
250	& 10	&         10	&       \RBF	&      0.001	& 0.376	& 0.362	& 0.557	& 0.729 \\
250	& 10	&         10	&       \RBF	&       0.01	& 0.022	& 0.038	& 0.501	& 0.469 \\
250	& 10	&         50	&       \LIN	&          -	& 0.392	& 0.383	& 0.551	& 0.758 \\
250	& 10	&         50	&       \RBF	&     0.0001	& 0.397	& 0.385	& 0.555	& 0.755 \\
250	& 10	&         50	&       \RBF	&      0.001	& 0.376	& 0.362	& 0.557	& 0.729 \\
250	& 10	&         50	&       \RBF	&       0.01	& 0.019	& 0.035	& 0.502	& 0.469 \\
250	& 10	&        100	&       \LIN	&          -	& 0.393	& 0.386	& 0.551	& 0.759 \\
250	& 10	&        100	&       \RBF	&     0.0001	& 0.397	& 0.385	& 0.555	& 0.755 \\
250	& 10	&        100	&       \RBF	&      0.001	& 0.376	& 0.362	& 0.557	& 0.729 \\
250	& 10	&        100	&       \RBF	&       0.01	& 0.018	& 0.034	& 0.502	& 0.468 \\
250	& 15	&      0.001	&       \LIN	&          -	& 0.236	& 0.252	& 0.533	& 0.724 \\
250	& 15	&      0.001	&       \RBF	&     0.0001	& 0.399	& 0.385	& 0.553	& 0.755 \\
250	& 15	&      0.001	&       \RBF	&      0.001	& 0.374	& 0.362	& 0.557	& 0.728 \\
250	& 15	&      0.001	&       \RBF	&       0.01	& 0.137	& 0.148	& 0.527	& 0.503 \\
250	& 15	&       0.01	&       \LIN	&          -	& 0.238	& 0.252	& 0.512	& 0.721 \\
250	& 15	&       0.01	&       \RBF	&     0.0001	& 0.399	& 0.385	& 0.553	& 0.755 \\
250	& 15	&       0.01	&       \RBF	&      0.001	& 0.374	& 0.362	& 0.557	& 0.728 \\
250	& 15	&       0.01	&       \RBF	&       0.01	& 0.099	& 0.114	& 0.509	& 0.486 \\
250	& 15	&        0.1	&       \LIN	&          -	& 0.293	& 0.294	& 0.522	& 0.726 \\
250	& 15	&        0.1	&       \RBF	&     0.0001	& 0.399	& 0.385	& 0.553	& 0.755 \\
250	& 15	&        0.1	&       \RBF	&      0.001	& 0.374	& 0.362	& 0.557	& 0.728 \\
250	& 15	&        0.1	&       \RBF	&       0.01	& 0.071	& 0.083	& 0.503	& 0.476 \\
250	& 15	&        0.2	&       \LIN	&          -	& 0.339	& 0.315	& 0.498	& 0.722 \\
250	& 15	&        0.2	&       \RBF	&     0.0001	& 0.399	& 0.385	& 0.553	& 0.755 \\
250	& 15	&        0.2	&       \RBF	&      0.001	& 0.374	& 0.362	& 0.557	& 0.728 \\
250	& 15	&        0.2	&       \RBF	&       0.01	& 0.060	& 0.075	& 0.503	& 0.474 \\
250	& 15	&        0.4	&       \LIN	&          -	& 0.354	& 0.357	& 0.510	& 0.711 \\
250	& 15	&        0.4	&       \RBF	&     0.0001	& 0.399	& 0.385	& 0.553	& 0.755 \\
250	& 15	&        0.4	&       \RBF	&      0.001	& 0.374	& 0.362	& 0.557	& 0.728 \\
250	& 15	&        0.4	&       \RBF	&       0.01	& 0.046	& 0.061	& 0.499	& 0.472 \\
250	& 15	&        0.6	&       \LIN	&          -	& 0.390	& 0.383	& 0.558	& 0.732 \\
250	& 15	&        0.6	&       \RBF	&     0.0001	& 0.399	& 0.385	& 0.553	& 0.755 \\
250	& 15	&        0.6	&       \RBF	&      0.001	& 0.374	& 0.362	& 0.557	& 0.728 \\
250	& 15	&        0.6	&       \RBF	&       0.01	& 0.044	& 0.059	& 0.500	& 0.472 \\
250	& 15	&        0.8	&       \LIN	&          -	& 0.390	& 0.380	& 0.558	& 0.729 \\
250	& 15	&        0.8	&       \RBF	&     0.0001	& 0.399	& 0.385	& 0.553	& 0.755 \\
250	& 15	&        0.8	&       \RBF	&      0.001	& 0.374	& 0.362	& 0.557	& 0.728 \\
250	& 15	&        0.8	&       \RBF	&       0.01	& 0.041	& 0.054	& 0.501	& 0.471 \\
250	& 15	&        1.0	&       \LIN	&          -	& 0.385	& 0.371	& 0.559	& 0.726 \\
250	& 15	&        1.0	&       \RBF	&     0.0001	& 0.399	& 0.385	& 0.553	& 0.755 \\
250	& 15	&        1.0	&       \RBF	&      0.001	& 0.374	& 0.362	& 0.557	& 0.728 \\
250	& 15	&        1.0	&       \RBF	&       0.01	& 0.037	& 0.051	& 0.500	& 0.471 \\
250	& 15	&         10	&       \LIN	&          -	& 0.374	& 0.354	& 0.554	& 0.747 \\
250	& 15	&         10	&       \RBF	&     0.0001	& 0.399	& 0.385	& 0.553	& 0.755 \\
250	& 15	&         10	&       \RBF	&      0.001	& 0.374	& 0.362	& 0.557	& 0.728 \\
250	& 15	&         10	&       \RBF	&       0.01	& 0.024	& 0.039	& 0.502	& 0.469 \\
250	& 15	&         50	&       \LIN	&          -	& 0.392	& 0.385	& 0.551	& 0.757 \\
250	& 15	&         50	&       \RBF	&     0.0001	& 0.399	& 0.385	& 0.553	& 0.755 \\
250	& 15	&         50	&       \RBF	&      0.001	& 0.374	& 0.362	& 0.557	& 0.728 \\
250	& 15	&         50	&       \RBF	&       0.01	& 0.019	& 0.035	& 0.501	& 0.469 \\
250	& 15	&        100	&       \LIN	&          -	& 0.393	& 0.386	& 0.551	& 0.757 \\
250	& 15	&        100	&       \RBF	&     0.0001	& 0.399	& 0.385	& 0.553	& 0.755 \\
250	& 15	&        100	&       \RBF	&      0.001	& 0.374	& 0.362	& 0.557	& 0.728 \\
250	& 15	&        100	&       \RBF	&       0.01	& 0.019	& 0.035	& 0.501	& 0.468 \\
300	& 5	&   0.000001	&       \RBF	&     0.0001	& 0.306	& 0.313	& 0.550	& 0.735 \\
300	& 5	&   0.000001	&       \RBF	&      0.001	& 0.320	& 0.322	& 0.551	& 0.692 \\
300	& 5	&   0.000001	&       \RBF	&       0.01	& 0.179	& 0.190	& 0.525	& 0.553 \\
300	& 5	&    0.00001	&       \RBF	&     0.0001	& 0.365	& 0.351	& 0.552	& 0.753 \\
300	& 5	&    0.00001	&       \RBF	&      0.001	& 0.357	& 0.353	& 0.552	& 0.729 \\
300	& 5	&    0.00001	&       \RBF	&       0.01	& 0.168	& 0.185	& 0.528	& 0.550 \\
300	& 5	&     0.0001	&       \RBF	&     0.0001	& 0.384	& 0.375	& 0.557	& 0.752 \\
300	& 5	&     0.0001	&       \RBF	&      0.001	& 0.357	& 0.353	& 0.552	& 0.729 \\
300	& 5	&     0.0001	&       \RBF	&       0.01	& 0.147	& 0.162	& 0.530	& 0.524 \\
300	& 5	&      0.001	&       \LIN	&          -	& 0.222	& 0.231	& 0.537	& 0.702 \\
300	& 5	&      0.001	&       \RBF	&     0.0001	& 0.384	& 0.375	& 0.557	& 0.752 \\
300	& 5	&      0.001	&       \RBF	&      0.001	& 0.357	& 0.353	& 0.552	& 0.729 \\
300	& 5	&      0.001	&       \RBF	&       0.01	& 0.126	& 0.139	& 0.526	& 0.502 \\
300	& 5	&       0.01	&       \LIN	&          -	& 0.243	& 0.253	& 0.520	& 0.674 \\
300	& 5	&       0.01	&       \RBF	&     0.0001	& 0.384	& 0.375	& 0.557	& 0.752 \\
300	& 5	&       0.01	&       \RBF	&      0.001	& 0.357	& 0.353	& 0.552	& 0.729 \\
300	& 5	&       0.01	&       \RBF	&       0.01	& 0.100	& 0.108	& 0.511	& 0.486 \\
300	& 5	&        0.1	&       \LIN	&          -	& 0.296	& 0.299	& 0.552	& 0.747 \\
300	& 5	&        0.1	&       \RBF	&     0.0001	& 0.384	& 0.375	& 0.557	& 0.752 \\
300	& 5	&        0.1	&       \RBF	&      0.001	& 0.357	& 0.353	& 0.552	& 0.729 \\
300	& 5	&        0.1	&       \RBF	&       0.01	& 0.067	& 0.081	& 0.507	& 0.476 \\
300	& 5	&        0.2	&       \LIN	&          -	& 0.364	& 0.360	& 0.549	& 0.750 \\
300	& 5	&        0.2	&       \RBF	&     0.0001	& 0.384	& 0.375	& 0.557	& 0.752 \\
300	& 5	&        0.2	&       \RBF	&      0.001	& 0.357	& 0.353	& 0.552	& 0.729 \\
300	& 5	&        0.2	&       \RBF	&       0.01	& 0.061	& 0.073	& 0.505	& 0.474 \\
300	& 5	&        0.4	&       \LIN	&          -	& 0.365	& 0.341	& 0.552	& 0.755 \\
300	& 5	&        0.4	&       \RBF	&     0.0001	& 0.384	& 0.375	& 0.557	& 0.752 \\
300	& 5	&        0.4	&       \RBF	&      0.001	& 0.357	& 0.353	& 0.552	& 0.729 \\
300	& 5	&        0.4	&       \RBF	&       0.01	& 0.049	& 0.063	& 0.505	& 0.472 \\
300	& 5	&        0.6	&       \LIN	&          -	& 0.336	& 0.329	& 0.551	& 0.760 \\
300	& 5	&        0.6	&       \RBF	&     0.0001	& 0.384	& 0.375	& 0.557	& 0.752 \\
300	& 5	&        0.6	&       \RBF	&      0.001	& 0.357	& 0.353	& 0.552	& 0.729 \\
300	& 5	&        0.6	&       \RBF	&       0.01	& 0.041	& 0.056	& 0.504	& 0.471 \\
300	& 5	&        0.8	&       \LIN	&          -	& 0.381	& 0.373	& 0.553	& 0.759 \\
300	& 5	&        0.8	&       \RBF	&     0.0001	& 0.384	& 0.375	& 0.557	& 0.752 \\
300	& 5	&        0.8	&       \RBF	&      0.001	& 0.357	& 0.353	& 0.552	& 0.729 \\
300	& 5	&        0.8	&       \RBF	&       0.01	& 0.042	& 0.056	& 0.504	& 0.471 \\
300	& 5	&        1.0	&       \LIN	&          -	& 0.354	& 0.346	& 0.552	& 0.761 \\
300	& 5	&        1.0	&       \RBF	&     0.0001	& 0.384	& 0.375	& 0.557	& 0.752 \\
300	& 5	&        1.0	&       \RBF	&      0.001	& 0.357	& 0.353	& 0.552	& 0.729 \\
300	& 5	&        1.0	&       \RBF	&       0.01	& 0.036	& 0.049	& 0.505	& 0.470 \\
300	& 5	&         10	&       \LIN	&          -	& 0.366	& 0.349	& 0.552	& 0.750 \\
300	& 5	&         10	&       \RBF	&     0.0001	& 0.384	& 0.375	& 0.557	& 0.752 \\
300	& 5	&         10	&       \RBF	&      0.001	& 0.357	& 0.353	& 0.552	& 0.729 \\
300	& 5	&         10	&       \RBF	&       0.01	& 0.020	& 0.036	& 0.505	& 0.469 \\
300	& 5	&         50	&       \LIN	&          -	& 0.376	& 0.368	& 0.558	& 0.701 \\
300	& 5	&         50	&       \RBF	&     0.0001	& 0.384	& 0.375	& 0.557	& 0.752 \\
300	& 5	&         50	&       \RBF	&      0.001	& 0.357	& 0.353	& 0.552	& 0.729 \\
300	& 5	&         50	&       \RBF	&       0.01	& 0.018	& 0.034	& 0.505	& 0.468 \\
300	& 5	&        100	&       \LIN	&          -	& 0.376	& 0.368	& 0.558	& 0.701 \\
300	& 5	&        100	&       \RBF	&     0.0001	& 0.384	& 0.375	& 0.557	& 0.752 \\
300	& 5	&        100	&       \RBF	&      0.001	& 0.357	& 0.353	& 0.552	& 0.729 \\
300	& 5	&        100	&       \RBF	&       0.01	& 0.016	& 0.032	& 0.505	& 0.468 \\
300	& 10	&   0.000001	&       \LIN	&          -	& 0.129	& 0.157	& 0.534	& 0.710 \\
300	& 10	&   0.000001	&       \RBF	&       0.01	& 0.180	& 0.185	& 0.524	& 0.548 \\
300	& 10	&      0.001	&       \LIN	&          -	& 0.170	& 0.195	& 0.511	& 0.711 \\
300	& 10	&      0.001	&       \RBF	&     0.0001	& 0.387	& 0.371	& 0.556	& 0.750 \\
300	& 10	&      0.001	&       \RBF	&      0.001	& 0.360	& 0.354	& 0.554	& 0.722 \\
300	& 10	&      0.001	&       \RBF	&       0.01	& 0.129	& 0.141	& 0.525	& 0.500 \\
300	& 10	&       0.01	&       \LIN	&          -	& 0.255	& 0.264	& 0.509	& 0.660 \\
300	& 10	&       0.01	&       \RBF	&     0.0001	& 0.387	& 0.371	& 0.556	& 0.750 \\
300	& 10	&       0.01	&       \RBF	&      0.001	& 0.360	& 0.354	& 0.554	& 0.722 \\
300	& 10	&       0.01	&       \RBF	&       0.01	& 0.107	& 0.116	& 0.511	& 0.485 \\
300	& 10	&        0.1	&       \LIN	&          -	& 0.373	& 0.352	& 0.554	& 0.740 \\
300	& 10	&        0.1	&       \RBF	&     0.0001	& 0.387	& 0.371	& 0.556	& 0.750 \\
300	& 10	&        0.1	&       \RBF	&      0.001	& 0.360	& 0.354	& 0.554	& 0.722 \\
300	& 10	&        0.1	&       \RBF	&       0.01	& 0.073	& 0.086	& 0.508	& 0.476 \\
300	& 10	&        0.2	&       \LIN	&          -	& 0.381	& 0.378	& 0.553	& 0.744 \\
300	& 10	&        0.2	&       \RBF	&     0.0001	& 0.387	& 0.371	& 0.556	& 0.750 \\
300	& 10	&        0.2	&       \RBF	&      0.001	& 0.360	& 0.354	& 0.554	& 0.722 \\
300	& 10	&        0.2	&       \RBF	&       0.01	& 0.064	& 0.077	& 0.506	& 0.474 \\
300	& 10	&        0.4	&       \LIN	&          -	& 0.363	& 0.360	& 0.556	& 0.748 \\
300	& 10	&        0.4	&       \RBF	&     0.0001	& 0.387	& 0.371	& 0.556	& 0.750 \\
300	& 10	&        0.4	&       \RBF	&      0.001	& 0.360	& 0.354	& 0.554	& 0.722 \\
300	& 10	&        0.4	&       \RBF	&       0.01	& 0.047	& 0.062	& 0.504	& 0.472 \\
300	& 10	&        0.6	&       \LIN	&          -	& 0.368	& 0.358	& 0.554	& 0.750 \\
300	& 10	&        0.6	&       \RBF	&     0.0001	& 0.387	& 0.371	& 0.556	& 0.750 \\
300	& 10	&        0.6	&       \RBF	&      0.001	& 0.360	& 0.354	& 0.554	& 0.722 \\
300	& 10	&        0.6	&       \RBF	&       0.01	& 0.044	& 0.059	& 0.504	& 0.471 \\
300	& 10	&        0.8	&       \LIN	&          -	& 0.370	& 0.370	& 0.552	& 0.749 \\
300	& 10	&        0.8	&       \RBF	&     0.0001	& 0.387	& 0.371	& 0.556	& 0.750 \\
300	& 10	&        0.8	&       \RBF	&      0.001	& 0.360	& 0.354	& 0.554	& 0.722 \\
300	& 10	&        0.8	&       \RBF	&       0.01	& 0.043	& 0.057	& 0.504	& 0.471 \\
300	& 10	&        1.0	&       \LIN	&          -	& 0.378	& 0.373	& 0.552	& 0.749 \\
300	& 10	&        1.0	&       \RBF	&     0.0001	& 0.387	& 0.371	& 0.556	& 0.750 \\
300	& 10	&        1.0	&       \RBF	&      0.001	& 0.360	& 0.354	& 0.554	& 0.722 \\
300	& 10	&        1.0	&       \RBF	&       0.01	& 0.036	& 0.050	& 0.504	& 0.470 \\
300	& 10	&         10	&       \LIN	&          -	& 0.374	& 0.362	& 0.550	& 0.756 \\
300	& 10	&         10	&       \RBF	&     0.0001	& 0.387	& 0.371	& 0.556	& 0.750 \\
300	& 10	&         10	&       \RBF	&      0.001	& 0.360	& 0.354	& 0.554	& 0.722 \\
300	& 10	&         10	&       \RBF	&       0.01	& 0.022	& 0.038	& 0.506	& 0.469 \\
300	& 10	&         50	&       \LIN	&          -	& 0.385	& 0.375	& 0.551	& 0.756 \\
300	& 10	&         50	&       \RBF	&     0.0001	& 0.387	& 0.371	& 0.556	& 0.750 \\
300	& 10	&         50	&       \RBF	&      0.001	& 0.360	& 0.354	& 0.554	& 0.722 \\
300	& 10	&         50	&       \RBF	&       0.01	& 0.020	& 0.036	& 0.505	& 0.468 \\
300	& 10	&        100	&       \LIN	&          -	& 0.385	& 0.376	& 0.552	& 0.755 \\
300	& 10	&        100	&       \RBF	&     0.0001	& 0.387	& 0.371	& 0.556	& 0.750 \\
300	& 10	&        100	&       \RBF	&      0.001	& 0.360	& 0.354	& 0.555	& 0.722 \\
300	& 10	&        100	&       \RBF	&       0.01	& 0.016	& 0.032	& 0.505	& 0.468 \\
300	& 15	&      0.001	&       \LIN	&          -	& 0.206	& 0.227	& 0.535	& 0.712 \\
300	& 15	&      0.001	&       \RBF	&     0.0001	& 0.388	& 0.379	& 0.555	& 0.750 \\
300	& 15	&      0.001	&       \RBF	&      0.001	& 0.359	& 0.352	& 0.552	& 0.721 \\
300	& 15	&      0.001	&       \RBF	&       0.01	& 0.127	& 0.138	& 0.528	& 0.499 \\
300	& 15	&       0.01	&       \LIN	&          -	& 0.276	& 0.281	& 0.547	& 0.724 \\
300	& 15	&       0.01	&       \RBF	&     0.0001	& 0.388	& 0.379	& 0.555	& 0.750 \\
300	& 15	&       0.01	&       \RBF	&      0.001	& 0.359	& 0.352	& 0.552	& 0.721 \\
300	& 15	&       0.01	&       \RBF	&       0.01	& 0.099	& 0.111	& 0.511	& 0.484 \\
300	& 15	&        0.1	&       \LIN	&          -	& 0.382	& 0.372	& 0.556	& 0.737 \\
300	& 15	&        0.1	&       \RBF	&     0.0001	& 0.388	& 0.379	& 0.555	& 0.750 \\
300	& 15	&        0.1	&       \RBF	&      0.001	& 0.359	& 0.352	& 0.552	& 0.721 \\
300	& 15	&        0.1	&       \RBF	&       0.01	& 0.074	& 0.086	& 0.510	& 0.476 \\
300	& 15	&        0.2	&       \LIN	&          -	& 0.378	& 0.358	& 0.552	& 0.734 \\
300	& 15	&        0.2	&       \RBF	&     0.0001	& 0.388	& 0.379	& 0.555	& 0.750 \\
300	& 15	&        0.2	&       \RBF	&      0.001	& 0.359	& 0.352	& 0.552	& 0.721 \\
300	& 15	&        0.2	&       \RBF	&       0.01	& 0.066	& 0.078	& 0.507	& 0.474 \\
300	& 15	&        0.4	&       \LIN	&          -	& 0.366	& 0.358	& 0.558	& 0.729 \\
300	& 15	&        0.4	&       \RBF	&     0.0001	& 0.388	& 0.379	& 0.555	& 0.750 \\
300	& 15	&        0.4	&       \RBF	&      0.001	& 0.359	& 0.352	& 0.552	& 0.721 \\
300	& 15	&        0.4	&       \RBF	&       0.01	& 0.053	& 0.068	& 0.505	& 0.472 \\
300	& 15	&        0.6	&       \LIN	&          -	& 0.367	& 0.367	& 0.559	& 0.726 \\
300	& 15	&        0.6	&       \RBF	&     0.0001	& 0.388	& 0.379	& 0.555	& 0.750 \\
300	& 15	&        0.6	&       \RBF	&      0.001	& 0.359	& 0.352	& 0.552	& 0.721 \\
300	& 15	&        0.6	&       \RBF	&       0.01	& 0.043	& 0.058	& 0.504	& 0.471 \\
300	& 15	&        0.8	&       \LIN	&          -	& 0.365	& 0.356	& 0.559	& 0.723 \\
300	& 15	&        0.8	&       \RBF	&     0.0001	& 0.388	& 0.379	& 0.555	& 0.750 \\
300	& 15	&        0.8	&       \RBF	&      0.001	& 0.359	& 0.352	& 0.552	& 0.721 \\
300	& 15	&        0.8	&       \RBF	&       0.01	& 0.037	& 0.052	& 0.504	& 0.471 \\
300	& 15	&        1.0	&       \LIN	&          -	& 0.382	& 0.365	& 0.559	& 0.721 \\
300	& 15	&        1.0	&       \RBF	&     0.0001	& 0.388	& 0.379	& 0.555	& 0.750 \\
300	& 15	&        1.0	&       \RBF	&      0.001	& 0.359	& 0.352	& 0.552	& 0.721 \\
300	& 15	&        1.0	&       \RBF	&       0.01	& 0.037	& 0.052	& 0.505	& 0.470 \\
300	& 15	&         10	&       \LIN	&          -	& 0.385	& 0.370	& 0.557	& 0.704 \\
300	& 15	&         10	&       \RBF	&     0.0001	& 0.388	& 0.379	& 0.555	& 0.750 \\
300	& 15	&         10	&       \RBF	&      0.001	& 0.359	& 0.352	& 0.552	& 0.721 \\
300	& 15	&         10	&       \RBF	&       0.01	& 0.022	& 0.038	& 0.506	& 0.469 \\
300	& 15	&         50	&       \LIN	&          -	& 0.381	& 0.371	& 0.547	& 0.751 \\
300	& 15	&         50	&       \RBF	&     0.0001	& 0.388	& 0.379	& 0.555	& 0.750 \\
300	& 15	&         50	&       \RBF	&      0.001	& 0.359	& 0.353	& 0.552	& 0.721 \\
300	& 15	&         50	&       \RBF	&       0.01	& 0.020	& 0.036	& 0.505	& 0.468 \\
300	& 15	&        100	&       \LIN	&          -	& 0.381	& 0.370	& 0.550	& 0.752 \\
300	& 15	&        100	&       \RBF	&     0.0001	& 0.388	& 0.379	& 0.555	& 0.750 \\
300	& 15	&        100	&       \RBF	&      0.001	& 0.358	& 0.352	& 0.552	& 0.721 \\
300	& 15	&        100	&       \RBF	&       0.01	& 0.021	& 0.036	& 0.505	& 0.468 \\
350	& 5	&   0.000001	&       \LIN	&          -	& 0.134	& 0.155	& 0.548	& 0.712 \\
350	& 5	&   0.000001	&       \RBF	&     0.0001	& 0.306	& 0.310	& 0.556	& 0.737 \\
350	& 5	&   0.000001	&       \RBF	&      0.001	& 0.311	& 0.310	& 0.554	& 0.694 \\
350	& 5	&   0.000001	&       \RBF	&       0.01	& 0.181	& 0.190	& 0.525	& 0.549 \\
350	& 5	&    0.00001	&       \LIN	&          -	& 0.209	& 0.221	& 0.532	& 0.720 \\
350	& 5	&    0.00001	&       \RBF	&     0.0001	& 0.358	& 0.348	& 0.555	& 0.757 \\
350	& 5	&    0.00001	&       \RBF	&      0.001	& 0.348	& 0.341	& 0.555	& 0.728 \\
350	& 5	&    0.00001	&       \RBF	&       0.01	& 0.167	& 0.180	& 0.524	& 0.547 \\
350	& 5	&     0.0001	&       \RBF	&     0.0001	& 0.373	& 0.365	& 0.555	& 0.748 \\
350	& 5	&     0.0001	&       \RBF	&      0.001	& 0.348	& 0.341	& 0.555	& 0.728 \\
350	& 5	&     0.0001	&       \RBF	&       0.01	& 0.146	& 0.156	& 0.525	& 0.522 \\
350	& 5	&      0.001	&       \LIN	&          -	& 0.188	& 0.210	& 0.533	& 0.713 \\
350	& 5	&      0.001	&       \RBF	&     0.0001	& 0.373	& 0.365	& 0.555	& 0.748 \\
350	& 5	&      0.001	&       \RBF	&      0.001	& 0.348	& 0.341	& 0.555	& 0.728 \\
350	& 5	&      0.001	&       \RBF	&       0.01	& 0.127	& 0.139	& 0.519	& 0.502 \\
350	& 5	&       0.01	&       \LIN	&          -	& 0.281	& 0.286	& 0.554	& 0.741 \\
350	& 5	&       0.01	&       \RBF	&     0.0001	& 0.373	& 0.365	& 0.555	& 0.748 \\
350	& 5	&       0.01	&       \RBF	&      0.001	& 0.348	& 0.341	& 0.555	& 0.728 \\
350	& 5	&       0.01	&       \RBF	&       0.01	& 0.097	& 0.109	& 0.508	& 0.486 \\
350	& 5	&        0.1	&       \LIN	&          -	& 0.287	& 0.290	& 0.543	& 0.726 \\
350	& 5	&        0.1	&       \RBF	&     0.0001	& 0.373	& 0.365	& 0.555	& 0.748 \\
350	& 5	&        0.1	&       \RBF	&      0.001	& 0.348	& 0.341	& 0.555	& 0.728 \\
350	& 5	&        0.1	&       \RBF	&       0.01	& 0.071	& 0.081	& 0.504	& 0.476 \\
350	& 5	&        0.2	&       \LIN	&          -	& 0.377	& 0.352	& 0.553	& 0.747 \\
350	& 5	&        0.2	&       \RBF	&     0.0001	& 0.373	& 0.365	& 0.555	& 0.748 \\
350	& 5	&        0.2	&       \RBF	&      0.001	& 0.348	& 0.341	& 0.555	& 0.728 \\
350	& 5	&        0.2	&       \RBF	&       0.01	& 0.063	& 0.076	& 0.503	& 0.474 \\
350	& 5	&        0.4	&       \LIN	&          -	& 0.368	& 0.355	& 0.552	& 0.750 \\
350	& 5	&        0.4	&       \RBF	&     0.0001	& 0.373	& 0.365	& 0.555	& 0.748 \\
350	& 5	&        0.4	&       \RBF	&      0.001	& 0.348	& 0.341	& 0.555	& 0.728 \\
350	& 5	&        0.4	&       \RBF	&       0.01	& 0.055	& 0.068	& 0.501	& 0.472 \\
350	& 5	&        0.6	&       \LIN	&          -	& 0.356	& 0.340	& 0.555	& 0.743 \\
350	& 5	&        0.6	&       \RBF	&     0.0001	& 0.373	& 0.365	& 0.555	& 0.748 \\
350	& 5	&        0.6	&       \RBF	&      0.001	& 0.348	& 0.341	& 0.555	& 0.728 \\
350	& 5	&        0.6	&       \RBF	&       0.01	& 0.046	& 0.061	& 0.502	& 0.472 \\
350	& 5	&        0.8	&       \LIN	&          -	& 0.367	& 0.343	& 0.550	& 0.749 \\
350	& 5	&        0.8	&       \RBF	&     0.0001	& 0.373	& 0.365	& 0.555	& 0.748 \\
350	& 5	&        0.8	&       \RBF	&      0.001	& 0.348	& 0.341	& 0.555	& 0.728 \\
350	& 5	&        0.8	&       \RBF	&       0.01	& 0.043	& 0.057	& 0.502	& 0.471 \\
350	& 5	&        1.0	&       \LIN	&          -	& 0.374	& 0.354	& 0.551	& 0.756 \\
350	& 5	&        1.0	&       \RBF	&     0.0001	& 0.373	& 0.365	& 0.555	& 0.748 \\
350	& 5	&        1.0	&       \RBF	&      0.001	& 0.348	& 0.341	& 0.555	& 0.728 \\
350	& 5	&        1.0	&       \RBF	&       0.01	& 0.039	& 0.053	& 0.500	& 0.471 \\
350	& 5	&         10	&       \LIN	&          -	& 0.362	& 0.354	& 0.553	& 0.738 \\
350	& 5	&         10	&       \RBF	&     0.0001	& 0.373	& 0.365	& 0.555	& 0.748 \\
350	& 5	&         10	&       \RBF	&      0.001	& 0.348	& 0.341	& 0.555	& 0.728 \\
350	& 5	&         10	&       \RBF	&       0.01	& 0.026	& 0.042	& 0.501	& 0.469 \\
350	& 5	&         50	&       \LIN	&          -	& 0.369	& 0.364	& 0.559	& 0.697 \\
350	& 5	&         50	&       \RBF	&     0.0001	& 0.373	& 0.365	& 0.555	& 0.748 \\
350	& 5	&         50	&       \RBF	&      0.001	& 0.348	& 0.340	& 0.555	& 0.728 \\
350	& 5	&         50	&       \RBF	&       0.01	& 0.021	& 0.037	& 0.501	& 0.469 \\
350	& 5	&        100	&       \LIN	&          -	& 0.369	& 0.364	& 0.559	& 0.697 \\
350	& 5	&        100	&       \RBF	&     0.0001	& 0.373	& 0.365	& 0.555	& 0.748 \\
350	& 5	&        100	&       \RBF	&      0.001	& 0.348	& 0.340	& 0.555	& 0.728 \\
350	& 5	&        100	&       \RBF	&       0.01	& 0.019	& 0.035	& 0.501	& 0.469 \\
350	& 10	&   0.000001	&       \LIN	&          -	& 0.206	& 0.219	& 0.546	& 0.714 \\
350	& 10	&   0.000001	&       \RBF	&       0.01	& 0.186	& 0.191	& 0.527	& 0.546 \\
350	& 10	&      0.001	&       \LIN	&          -	& 0.193	& 0.214	& 0.531	& 0.704 \\
350	& 10	&      0.001	&       \RBF	&     0.0001	& 0.380	& 0.367	& 0.553	& 0.748 \\
350	& 10	&      0.001	&       \RBF	&      0.001	& 0.351	& 0.344	& 0.556	& 0.721 \\
350	& 10	&      0.001	&       \RBF	&       0.01	& 0.132	& 0.143	& 0.519	& 0.499 \\
350	& 10	&       0.01	&       \LIN	&          -	& 0.262	& 0.266	& 0.547	& 0.720 \\
350	& 10	&       0.01	&       \RBF	&     0.0001	& 0.380	& 0.367	& 0.553	& 0.748 \\
350	& 10	&       0.01	&       \RBF	&      0.001	& 0.351	& 0.344	& 0.556	& 0.721 \\
350	& 10	&       0.01	&       \RBF	&       0.01	& 0.102	& 0.113	& 0.507	& 0.486 \\
350	& 10	&        0.1	&       \LIN	&          -	& 0.276	& 0.285	& 0.551	& 0.711 \\
350	& 10	&        0.1	&       \RBF	&     0.0001	& 0.380	& 0.367	& 0.553	& 0.748 \\
350	& 10	&        0.1	&       \RBF	&      0.001	& 0.351	& 0.344	& 0.556	& 0.721 \\
350	& 10	&        0.1	&       \RBF	&       0.01	& 0.074	& 0.084	& 0.503	& 0.476 \\
350	& 10	&        0.2	&       \LIN	&          -	& 0.396	& 0.368	& 0.560	& 0.742 \\
350	& 10	&        0.2	&       \RBF	&     0.0001	& 0.380	& 0.367	& 0.553	& 0.748 \\
350	& 10	&        0.2	&       \RBF	&      0.001	& 0.351	& 0.344	& 0.556	& 0.721 \\
350	& 10	&        0.2	&       \RBF	&       0.01	& 0.070	& 0.083	& 0.502	& 0.474 \\
350	& 10	&        0.4	&       \LIN	&          -	& 0.397	& 0.377	& 0.554	& 0.743 \\
350	& 10	&        0.4	&       \RBF	&     0.0001	& 0.380	& 0.367	& 0.553	& 0.748 \\
350	& 10	&        0.4	&       \RBF	&      0.001	& 0.351	& 0.344	& 0.556	& 0.721 \\
350	& 10	&        0.4	&       \RBF	&       0.01	& 0.053	& 0.068	& 0.502	& 0.472 \\
350	& 10	&        0.6	&       \LIN	&          -	& 0.369	& 0.358	& 0.556	& 0.743 \\
350	& 10	&        0.6	&       \RBF	&     0.0001	& 0.380	& 0.367	& 0.553	& 0.748 \\
350	& 10	&        0.6	&       \RBF	&      0.001	& 0.351	& 0.344	& 0.556	& 0.721 \\
350	& 10	&        0.6	&       \RBF	&       0.01	& 0.049	& 0.063	& 0.500	& 0.472 \\
350	& 10	&        0.8	&       \LIN	&          -	& 0.386	& 0.352	& 0.555	& 0.745 \\
350	& 10	&        0.8	&       \RBF	&     0.0001	& 0.380	& 0.367	& 0.553	& 0.748 \\
350	& 10	&        0.8	&       \RBF	&      0.001	& 0.351	& 0.344	& 0.556	& 0.721 \\
350	& 10	&        0.8	&       \RBF	&       0.01	& 0.040	& 0.053	& 0.501	& 0.471 \\
350	& 10	&        1.0	&       \LIN	&          -	& 0.393	& 0.365	& 0.552	& 0.743 \\
350	& 10	&        1.0	&       \RBF	&     0.0001	& 0.380	& 0.367	& 0.553	& 0.748 \\
350	& 10	&        1.0	&       \RBF	&      0.001	& 0.351	& 0.344	& 0.556	& 0.721 \\
350	& 10	&        1.0	&       \RBF	&       0.01	& 0.038	& 0.053	& 0.501	& 0.471 \\
350	& 10	&         10	&       \LIN	&          -	& 0.349	& 0.349	& 0.547	& 0.757 \\
350	& 10	&         10	&       \RBF	&     0.0001	& 0.380	& 0.367	& 0.553	& 0.748 \\
350	& 10	&         10	&       \RBF	&      0.001	& 0.351	& 0.344	& 0.556	& 0.721 \\
350	& 10	&         10	&       \RBF	&       0.01	& 0.026	& 0.042	& 0.501	& 0.469 \\
350	& 10	&         50	&       \LIN	&          -	& 0.374	& 0.371	& 0.547	& 0.754 \\
350	& 10	&         50	&       \RBF	&     0.0001	& 0.380	& 0.367	& 0.553	& 0.748 \\
350	& 10	&         50	&       \RBF	&      0.001	& 0.351	& 0.345	& 0.556	& 0.721 \\
350	& 10	&         50	&       \RBF	&       0.01	& 0.021	& 0.037	& 0.501	& 0.469 \\
350	& 10	&        100	&       \LIN	&          -	& 0.382	& 0.376	& 0.548	& 0.752 \\
350	& 10	&        100	&       \RBF	&     0.0001	& 0.380	& 0.367	& 0.553	& 0.748 \\
350	& 10	&        100	&       \RBF	&      0.001	& 0.351	& 0.345	& 0.556	& 0.721 \\
350	& 10	&        100	&       \RBF	&       0.01	& 0.022	& 0.038	& 0.502	& 0.469 \\
350	& 15	&      0.001	&       \LIN	&          -	& 0.180	& 0.201	& 0.524	& 0.712 \\
350	& 15	&      0.001	&       \RBF	&     0.0001	& 0.381	& 0.370	& 0.550	& 0.747 \\
350	& 15	&      0.001	&       \RBF	&      0.001	& 0.353	& 0.348	& 0.555	& 0.721 \\
350	& 15	&      0.001	&       \RBF	&       0.01	& 0.125	& 0.137	& 0.518	& 0.499 \\
350	& 15	&       0.01	&       \LIN	&          -	& 0.179	& 0.190	& 0.515	& 0.707 \\
350	& 15	&       0.01	&       \RBF	&     0.0001	& 0.381	& 0.370	& 0.550	& 0.747 \\
350	& 15	&       0.01	&       \RBF	&      0.001	& 0.353	& 0.348	& 0.555	& 0.721 \\
350	& 15	&       0.01	&       \RBF	&       0.01	& 0.096	& 0.110	& 0.509	& 0.485 \\
350	& 15	&        0.1	&       \LIN	&          -	& 0.301	& 0.303	& 0.530	& 0.719 \\
350	& 15	&        0.1	&       \RBF	&     0.0001	& 0.381	& 0.370	& 0.550	& 0.747 \\
350	& 15	&        0.1	&       \RBF	&      0.001	& 0.353	& 0.348	& 0.555	& 0.721 \\
350	& 15	&        0.1	&       \RBF	&       0.01	& 0.073	& 0.084	& 0.504	& 0.476 \\
350	& 15	&        0.2	&       \LIN	&          -	& 0.143	& 0.173	& 0.526	& 0.712 \\
350	& 15	&        0.2	&       \RBF	&     0.0001	& 0.381	& 0.370	& 0.550	& 0.747 \\
350	& 15	&        0.2	&       \RBF	&      0.001	& 0.353	& 0.348	& 0.555	& 0.721 \\
350	& 15	&        0.2	&       \RBF	&       0.01	& 0.066	& 0.079	& 0.503	& 0.474 \\
350	& 15	&        0.4	&       \LIN	&          -	& 0.257	& 0.262	& 0.515	& 0.729 \\
350	& 15	&        0.4	&       \RBF	&     0.0001	& 0.381	& 0.370	& 0.550	& 0.747 \\
350	& 15	&        0.4	&       \RBF	&      0.001	& 0.353	& 0.348	& 0.555	& 0.721 \\
350	& 15	&        0.4	&       \RBF	&       0.01	& 0.057	& 0.071	& 0.502	& 0.472 \\
350	& 15	&        0.6	&       \LIN	&          -	& 0.320	& 0.321	& 0.529	& 0.717 \\
350	& 15	&        0.6	&       \RBF	&     0.0001	& 0.381	& 0.370	& 0.550	& 0.747 \\
350	& 15	&        0.6	&       \RBF	&      0.001	& 0.353	& 0.348	& 0.555	& 0.721 \\
350	& 15	&        0.6	&       \RBF	&       0.01	& 0.050	& 0.062	& 0.500	& 0.472 \\
350	& 15	&        0.8	&       \LIN	&          -	& 0.382	& 0.351	& 0.555	& 0.739 \\
350	& 15	&        0.8	&       \RBF	&     0.0001	& 0.381	& 0.370	& 0.550	& 0.747 \\
350	& 15	&        0.8	&       \RBF	&      0.001	& 0.353	& 0.348	& 0.555	& 0.721 \\
350	& 15	&        0.8	&       \RBF	&       0.01	& 0.043	& 0.057	& 0.500	& 0.471 \\
350	& 15	&        1.0	&       \LIN	&          -	& 0.380	& 0.361	& 0.554	& 0.740 \\
350	& 15	&        1.0	&       \RBF	&     0.0001	& 0.381	& 0.370	& 0.550	& 0.747 \\
350	& 15	&        1.0	&       \RBF	&      0.001	& 0.353	& 0.348	& 0.555	& 0.721 \\
350	& 15	&        1.0	&       \RBF	&       0.01	& 0.040	& 0.055	& 0.500	& 0.471 \\
350	& 15	&         10	&       \LIN	&          -	& 0.349	& 0.352	& 0.549	& 0.736 \\
350	& 15	&         10	&       \RBF	&     0.0001	& 0.381	& 0.370	& 0.550	& 0.747 \\
350	& 15	&         10	&       \RBF	&      0.001	& 0.353	& 0.348	& 0.555	& 0.721 \\
350	& 15	&         10	&       \RBF	&       0.01	& 0.025	& 0.041	& 0.501	& 0.469 \\
350	& 15	&         50	&       \LIN	&          -	& 0.374	& 0.367	& 0.546	& 0.751 \\
350	& 15	&         50	&       \RBF	&     0.0001	& 0.381	& 0.370	& 0.550	& 0.747 \\
350	& 15	&         50	&       \RBF	&      0.001	& 0.353	& 0.348	& 0.555	& 0.721 \\
350	& 15	&         50	&       \RBF	&       0.01	& 0.021	& 0.037	& 0.501	& 0.469 \\
350	& 15	&        100	&       \LIN	&          -	& 0.377	& 0.370	& 0.546	& 0.749 \\
350	& 15	&        100	&       \RBF	&     0.0001	& 0.381	& 0.370	& 0.550	& 0.747 \\
350	& 15	&        100	&       \RBF	&      0.001	& 0.352	& 0.348	& 0.555	& 0.721 \\
350	& 15	&        100	&       \RBF	&       0.01	& 0.022	& 0.038	& 0.502	& 0.469 \\
400	& 5	&   0.000001	&       \LIN	&          -	& 0.234	& 0.249	& 0.538	& 0.711 \\
400	& 5	&   0.000001	&       \RBF	&     0.0001	& 0.328	& 0.320	& 0.555	& 0.727 \\
400	& 5	&   0.000001	&       \RBF	&      0.001	& 0.316	& 0.314	& 0.556	& 0.680 \\
400	& 5	&   0.000001	&       \RBF	&       0.01	& 0.183	& 0.195	& 0.523	& 0.540 \\
400	& 5	&    0.00001	&       \LIN	&          -	& 0.123	& 0.155	& 0.528	& 0.705 \\
400	& 5	&    0.00001	&       \RBF	&     0.0001	& 0.357	& 0.347	& 0.551	& 0.757 \\
400	& 5	&    0.00001	&       \RBF	&      0.001	& 0.355	& 0.358	& 0.552	& 0.720 \\
400	& 5	&    0.00001	&       \RBF	&       0.01	& 0.178	& 0.186	& 0.527	& 0.538 \\
400	& 5	&     0.0001	&       \LIN	&          -	& 0.204	& 0.222	& 0.516	& 0.709 \\
400	& 5	&     0.0001	&       \RBF	&     0.0001	& 0.370	& 0.366	& 0.552	& 0.746 \\
400	& 5	&     0.0001	&       \RBF	&      0.001	& 0.355	& 0.358	& 0.552	& 0.720 \\
400	& 5	&     0.0001	&       \RBF	&       0.01	& 0.150	& 0.158	& 0.525	& 0.517 \\
400	& 5	&      0.001	&       \LIN	&          -	& 0.109	& 0.141	& 0.524	& 0.634 \\
400	& 5	&      0.001	&       \RBF	&     0.0001	& 0.370	& 0.366	& 0.552	& 0.746 \\
400	& 5	&      0.001	&       \RBF	&      0.001	& 0.355	& 0.358	& 0.552	& 0.720 \\
400	& 5	&      0.001	&       \RBF	&       0.01	& 0.134	& 0.148	& 0.519	& 0.498 \\
400	& 5	&       0.01	&       \LIN	&          -	& 0.286	& 0.292	& 0.511	& 0.660 \\
400	& 5	&       0.01	&       \RBF	&     0.0001	& 0.370	& 0.366	& 0.552	& 0.746 \\
400	& 5	&       0.01	&       \RBF	&      0.001	& 0.355	& 0.358	& 0.552	& 0.720 \\
400	& 5	&       0.01	&       \RBF	&       0.01	& 0.100	& 0.111	& 0.506	& 0.484 \\
400	& 5	&        0.1	&       \LIN	&          -	& 0.328	& 0.318	& 0.555	& 0.742 \\
400	& 5	&        0.1	&       \RBF	&     0.0001	& 0.370	& 0.366	& 0.552	& 0.746 \\
400	& 5	&        0.1	&       \RBF	&      0.001	& 0.355	& 0.358	& 0.552	& 0.720 \\
400	& 5	&        0.1	&       \RBF	&       0.01	& 0.074	& 0.087	& 0.502	& 0.476 \\
400	& 5	&        0.2	&       \LIN	&          -	& 0.359	& 0.353	& 0.555	& 0.746 \\
400	& 5	&        0.2	&       \RBF	&     0.0001	& 0.370	& 0.366	& 0.552	& 0.746 \\
400	& 5	&        0.2	&       \RBF	&      0.001	& 0.355	& 0.358	& 0.552	& 0.720 \\
400	& 5	&        0.2	&       \RBF	&       0.01	& 0.068	& 0.080	& 0.503	& 0.474 \\
400	& 5	&        0.4	&       \LIN	&          -	& 0.374	& 0.362	& 0.555	& 0.752 \\
400	& 5	&        0.4	&       \RBF	&     0.0001	& 0.370	& 0.366	& 0.552	& 0.746 \\
400	& 5	&        0.4	&       \RBF	&      0.001	& 0.355	& 0.358	& 0.552	& 0.720 \\
400	& 5	&        0.4	&       \RBF	&       0.01	& 0.058	& 0.071	& 0.500	& 0.472 \\
400	& 5	&        0.6	&       \LIN	&          -	& 0.324	& 0.329	& 0.554	& 0.749 \\
400	& 5	&        0.6	&       \RBF	&     0.0001	& 0.370	& 0.366	& 0.552	& 0.746 \\
400	& 5	&        0.6	&       \RBF	&      0.001	& 0.355	& 0.358	& 0.552	& 0.720 \\
400	& 5	&        0.6	&       \RBF	&       0.01	& 0.050	& 0.065	& 0.501	& 0.471 \\
400	& 5	&        0.8	&       \LIN	&          -	& 0.359	& 0.342	& 0.554	& 0.750 \\
400	& 5	&        0.8	&       \RBF	&     0.0001	& 0.370	& 0.366	& 0.552	& 0.746 \\
400	& 5	&        0.8	&       \RBF	&      0.001	& 0.355	& 0.358	& 0.552	& 0.720 \\
400	& 5	&        0.8	&       \RBF	&       0.01	& 0.046	& 0.060	& 0.501	& 0.471 \\
400	& 5	&        1.0	&       \LIN	&          -	& 0.381	& 0.364	& 0.550	& 0.754 \\
400	& 5	&        1.0	&       \RBF	&     0.0001	& 0.370	& 0.366	& 0.552	& 0.746 \\
400	& 5	&        1.0	&       \RBF	&      0.001	& 0.355	& 0.358	& 0.552	& 0.720 \\
400	& 5	&        1.0	&       \RBF	&       0.01	& 0.042	& 0.056	& 0.501	& 0.471 \\
400	& 5	&         10	&       \LIN	&          -	& 0.367	& 0.361	& 0.553	& 0.724 \\
400	& 5	&         10	&       \RBF	&     0.0001	& 0.370	& 0.366	& 0.552	& 0.746 \\
400	& 5	&         10	&       \RBF	&      0.001	& 0.355	& 0.358	& 0.551	& 0.720 \\
400	& 5	&         10	&       \RBF	&       0.01	& 0.026	& 0.043	& 0.501	& 0.469 \\
400	& 5	&         50	&       \LIN	&          -	& 0.366	& 0.362	& 0.554	& 0.695 \\
400	& 5	&         50	&       \RBF	&     0.0001	& 0.370	& 0.366	& 0.552	& 0.746 \\
400	& 5	&         50	&       \RBF	&      0.001	& 0.355	& 0.358	& 0.552	& 0.720 \\
400	& 5	&         50	&       \RBF	&       0.01	& 0.019	& 0.036	& 0.500	& 0.469 \\
400	& 5	&        100	&       \LIN	&          -	& 0.366	& 0.362	& 0.554	& 0.695 \\
400	& 5	&        100	&       \RBF	&     0.0001	& 0.370	& 0.366	& 0.552	& 0.746 \\
400	& 5	&        100	&       \RBF	&      0.001	& 0.355	& 0.358	& 0.552	& 0.720 \\
400	& 5	&        100	&       \RBF	&       0.01	& 0.020	& 0.037	& 0.501	& 0.469 \\
400	& 10	&   0.000001	&       \LIN	&          -	& 0.165	& 0.187	& 0.535	& 0.722 \\
400	& 10	&   0.000001	&       \RBF	&      0.001	& 0.331	& 0.334	& 0.557	& 0.664 \\
400	& 10	&   0.000001	&       \RBF	&       0.01	& 0.183	& 0.191	& 0.521	& 0.536 \\
400	& 10	&      0.001	&       \LIN	&          -	& 0.206	& 0.228	& 0.515	& 0.708 \\
400	& 10	&      0.001	&       \RBF	&     0.0001	& 0.374	& 0.370	& 0.552	& 0.743 \\
400	& 10	&      0.001	&       \RBF	&      0.001	& 0.354	& 0.350	& 0.552	& 0.710 \\
400	& 10	&      0.001	&       \RBF	&       0.01	& 0.138	& 0.153	& 0.519	& 0.497 \\
400	& 10	&       0.01	&       \LIN	&          -	& 0.228	& 0.233	& 0.525	& 0.687 \\
400	& 10	&       0.01	&       \RBF	&     0.0001	& 0.374	& 0.370	& 0.552	& 0.743 \\
400	& 10	&       0.01	&       \RBF	&      0.001	& 0.354	& 0.350	& 0.552	& 0.710 \\
400	& 10	&       0.01	&       \RBF	&       0.01	& 0.093	& 0.108	& 0.509	& 0.484 \\
400	& 10	&        0.1	&       \LIN	&          -	& 0.319	& 0.313	& 0.559	& 0.738 \\
400	& 10	&        0.1	&       \RBF	&     0.0001	& 0.374	& 0.370	& 0.552	& 0.743 \\
400	& 10	&        0.1	&       \RBF	&      0.001	& 0.354	& 0.350	& 0.552	& 0.710 \\
400	& 10	&        0.1	&       \RBF	&       0.01	& 0.076	& 0.089	& 0.503	& 0.476 \\
400	& 10	&        0.2	&       \LIN	&          -	& 0.332	& 0.327	& 0.557	& 0.739 \\
400	& 10	&        0.2	&       \RBF	&     0.0001	& 0.374	& 0.370	& 0.552	& 0.743 \\
400	& 10	&        0.2	&       \RBF	&      0.001	& 0.354	& 0.350	& 0.552	& 0.710 \\
400	& 10	&        0.2	&       \RBF	&       0.01	& 0.071	& 0.085	& 0.503	& 0.474 \\
400	& 10	&        0.4	&       \LIN	&          -	& 0.335	& 0.326	& 0.556	& 0.739 \\
400	& 10	&        0.4	&       \RBF	&     0.0001	& 0.374	& 0.370	& 0.552	& 0.743 \\
400	& 10	&        0.4	&       \RBF	&      0.001	& 0.354	& 0.350	& 0.552	& 0.710 \\
400	& 10	&        0.4	&       \RBF	&       0.01	& 0.059	& 0.074	& 0.501	& 0.472 \\
400	& 10	&        0.6	&       \LIN	&          -	& 0.381	& 0.357	& 0.560	& 0.739 \\
400	& 10	&        0.6	&       \RBF	&     0.0001	& 0.374	& 0.370	& 0.552	& 0.743 \\
400	& 10	&        0.6	&       \RBF	&      0.001	& 0.354	& 0.350	& 0.552	& 0.710 \\
400	& 10	&        0.6	&       \RBF	&       0.01	& 0.050	& 0.064	& 0.500	& 0.471 \\
400	& 10	&        0.8	&       \LIN	&          -	& 0.382	& 0.356	& 0.559	& 0.739 \\
400	& 10	&        0.8	&       \RBF	&     0.0001	& 0.374	& 0.370	& 0.552	& 0.743 \\
400	& 10	&        0.8	&       \RBF	&      0.001	& 0.354	& 0.350	& 0.552	& 0.710 \\
400	& 10	&        0.8	&       \RBF	&       0.01	& 0.047	& 0.062	& 0.501	& 0.471 \\
400	& 10	&        1.0	&       \LIN	&          -	& 0.338	& 0.310	& 0.558	& 0.738 \\
400	& 10	&        1.0	&       \RBF	&     0.0001	& 0.374	& 0.370	& 0.552	& 0.743 \\
400	& 10	&        1.0	&       \RBF	&      0.001	& 0.354	& 0.350	& 0.552	& 0.710 \\
400	& 10	&        1.0	&       \RBF	&       0.01	& 0.044	& 0.058	& 0.501	& 0.471 \\
400	& 10	&         10	&       \LIN	&          -	& 0.376	& 0.366	& 0.548	& 0.754 \\
400	& 10	&         10	&       \RBF	&     0.0001	& 0.374	& 0.370	& 0.552	& 0.743 \\
400	& 10	&         10	&       \RBF	&      0.001	& 0.354	& 0.350	& 0.552	& 0.710 \\
400	& 10	&         10	&       \RBF	&       0.01	& 0.029	& 0.045	& 0.502	& 0.469 \\
400	& 10	&         50	&       \LIN	&          -	& 0.379	& 0.370	& 0.549	& 0.745 \\
400	& 10	&         50	&       \RBF	&     0.0001	& 0.374	& 0.370	& 0.552	& 0.743 \\
400	& 10	&         50	&       \RBF	&      0.001	& 0.354	& 0.350	& 0.552	& 0.710 \\
400	& 10	&         50	&       \RBF	&       0.01	& 0.023	& 0.039	& 0.501	& 0.469 \\
400	& 10	&        100	&       \LIN	&          -	& 0.382	& 0.373	& 0.550	& 0.746 \\
400	& 10	&        100	&       \RBF	&     0.0001	& 0.374	& 0.370	& 0.552	& 0.743 \\
400	& 10	&        100	&       \RBF	&      0.001	& 0.354	& 0.350	& 0.552	& 0.710 \\
400	& 10	&        100	&       \RBF	&       0.01	& 0.019	& 0.036	& 0.501	& 0.469 \\
400	& 15	&      0.001	&       \LIN	&          -	& 0.154	& 0.178	& 0.515	& 0.694 \\
400	& 15	&      0.001	&       \RBF	&     0.0001	& 0.378	& 0.370	& 0.552	& 0.742 \\
400	& 15	&      0.001	&       \RBF	&      0.001	& 0.351	& 0.346	& 0.552	& 0.710 \\
400	& 15	&      0.001	&       \RBF	&       0.01	& 0.136	& 0.147	& 0.518	& 0.496 \\
400	& 15	&       0.01	&       \LIN	&          -	& 0.282	& 0.285	& 0.556	& 0.732 \\
400	& 15	&       0.01	&       \RBF	&     0.0001	& 0.378	& 0.370	& 0.552	& 0.742 \\
400	& 15	&       0.01	&       \RBF	&      0.001	& 0.351	& 0.346	& 0.552	& 0.710 \\
400	& 15	&       0.01	&       \RBF	&       0.01	& 0.097	& 0.112	& 0.509	& 0.484 \\
400	& 15	&        0.1	&       \LIN	&          -	& 0.339	& 0.341	& 0.558	& 0.730 \\
400	& 15	&        0.1	&       \RBF	&     0.0001	& 0.378	& 0.370	& 0.552	& 0.742 \\
400	& 15	&        0.1	&       \RBF	&      0.001	& 0.351	& 0.346	& 0.552	& 0.710 \\
400	& 15	&        0.1	&       \RBF	&       0.01	& 0.077	& 0.089	& 0.504	& 0.476 \\
400	& 15	&        0.2	&       \LIN	&          -	& 0.301	& 0.298	& 0.560	& 0.724 \\
400	& 15	&        0.2	&       \RBF	&     0.0001	& 0.378	& 0.370	& 0.552	& 0.742 \\
400	& 15	&        0.2	&       \RBF	&      0.001	& 0.351	& 0.346	& 0.552	& 0.710 \\
400	& 15	&        0.2	&       \RBF	&       0.01	& 0.068	& 0.082	& 0.503	& 0.474 \\
400	& 15	&        0.4	&       \LIN	&          -	& 0.359	& 0.344	& 0.554	& 0.719 \\
400	& 15	&        0.4	&       \RBF	&     0.0001	& 0.378	& 0.370	& 0.552	& 0.742 \\
400	& 15	&        0.4	&       \RBF	&      0.001	& 0.351	& 0.346	& 0.552	& 0.710 \\
400	& 15	&        0.4	&       \RBF	&       0.01	& 0.060	& 0.074	& 0.501	& 0.472 \\
400	& 15	&        0.6	&       \LIN	&          -	& 0.381	& 0.370	& 0.557	& 0.716 \\
400	& 15	&        0.6	&       \RBF	&     0.0001	& 0.378	& 0.370	& 0.552	& 0.742 \\
400	& 15	&        0.6	&       \RBF	&      0.001	& 0.351	& 0.346	& 0.552	& 0.710 \\
400	& 15	&        0.6	&       \RBF	&       0.01	& 0.051	& 0.065	& 0.500	& 0.471 \\
400	& 15	&        0.8	&       \LIN	&          -	& 0.358	& 0.354	& 0.558	& 0.712 \\
400	& 15	&        0.8	&       \RBF	&     0.0001	& 0.378	& 0.370	& 0.552	& 0.742 \\
400	& 15	&        0.8	&       \RBF	&      0.001	& 0.351	& 0.346	& 0.552	& 0.710 \\
400	& 15	&        0.8	&       \RBF	&       0.01	& 0.047	& 0.061	& 0.501	& 0.471 \\
400	& 15	&        1.0	&       \LIN	&          -	& 0.361	& 0.358	& 0.557	& 0.709 \\
400	& 15	&        1.0	&       \RBF	&     0.0001	& 0.378	& 0.370	& 0.552	& 0.742 \\
400	& 15	&        1.0	&       \RBF	&      0.001	& 0.351	& 0.346	& 0.552	& 0.710 \\
400	& 15	&        1.0	&       \RBF	&       0.01	& 0.044	& 0.058	& 0.501	& 0.471 \\
400	& 15	&         10	&       \LIN	&          -	& 0.362	& 0.361	& 0.551	& 0.732 \\
400	& 15	&         10	&       \RBF	&     0.0001	& 0.378	& 0.370	& 0.552	& 0.742 \\
400	& 15	&         10	&       \RBF	&      0.001	& 0.351	& 0.346	& 0.552	& 0.710 \\
400	& 15	&         10	&       \RBF	&       0.01	& 0.028	& 0.045	& 0.502	& 0.469 \\
400	& 15	&         50	&       \LIN	&          -	& 0.380	& 0.372	& 0.550	& 0.744 \\
400	& 15	&         50	&       \RBF	&     0.0001	& 0.378	& 0.370	& 0.552	& 0.742 \\
400	& 15	&         50	&       \RBF	&      0.001	& 0.351	& 0.346	& 0.552	& 0.710 \\
400	& 15	&         50	&       \RBF	&       0.01	& 0.021	& 0.038	& 0.501	& 0.469 \\
400	& 15	&        100	&       \LIN	&          -	& 0.380	& 0.372	& 0.550	& 0.744 \\
400	& 15	&        100	&       \RBF	&     0.0001	& 0.378	& 0.370	& 0.552	& 0.742 \\
400	& 15	&        100	&       \RBF	&      0.001	& 0.351	& 0.346	& 0.551	& 0.710 \\
400	& 15	&        100	&       \RBF	&       0.01	& 0.022	& 0.038	& 0.501	& 0.469 \\


==> tables/holdout_2percent_baseline.tex <==
\begin{ThreePartTable}
    \begin{TableNotes}[flushleft]  %%% This should come before longtable and it is not tablenotes but TableNotes
  \small
  \item
    \begin{footnotesize}
        \bgroup
%        \def\arraystretch{0.5}%       
        \setstretch{1}
                The columns corresponding to ``$\alpha_b$'', ``$\beta_b$'',
                ``usim'', and ``$\sigma$'' have the
                two hyperparameters, cell line similarity function,
                and parameter for \hl{$\RBF$} cell line similarity, respectively, for \BMTMKL.
	      \par
              \egroup
    \end{footnotesize}
  \end{TableNotes}
  \begin{longtable}{
      @{\hspace{5pt}}>{\raggedleft}p{0.04\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.04\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.04\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft\arraybackslash}p{0.10\textwidth}@{\hspace{6pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
    }
    \caption{\mbox{\BMTMKL Performance on New Cell Lines ($\theta$ = 2)}}
    \label{supp:tbl:holdout:2percent:BMTMKL}\\
  %
    \hline\hline
    n & $\alpha_b$ & $\beta_b$ & usim & $\sigma$ & \small{AP@$5$} & \small{AP@$10$} & \small{\rCI} & \small{\CI} \\
    \hline
    \endfirsthead
  %
    \multicolumn{9}{c}{{\tablename\ \thetable{} -- continued from previous page}}\\
    \hline\hline
    n & $\alpha_b$ & $\beta_b$ & usim & $\sigma$ & \small{AP@$5$} & \small{AP@$10$} & \small{\rCI} & \small{\CI} \\
    \hline
    \endhead
  %
    \hline
    %  \midrule
    \multicolumn{9}{c}{{Continued on next page}} \\
    \hline
    %\midrule
    \endfoot
    %
    \hline\hline
    %\bottomrule
    \insertTableNotes         %% this added
    \endlastfoot
    %
    \input{tables/holdout_2percent_baseline_data.tex}
	
    \hline
  \end{longtable}
\end{ThreePartTable}


==> tables/holdout_2percent_baseline_data.tex <==
100	& 1	& 1	& \RBF	& 10.0	& 0.838	& 0.782	& 0.613	& 0.800\\
100	& 1e-10	& 1e-10	& \RBF	& 10.0	& 0.842	& 0.783	& 0.612	& 0.800\\
100	& 1e-10	& 1e+10	& \RBF	& 10.0	& 0.837	& 0.782	& 0.613	& 0.800\\
150	& 1	& 1	& \RBF	& 10.0	& 0.844	& 0.783	& 0.619	& 0.800\\
150	& 1e-10	& 1e-10	& \RBF	& 10.0	& 0.840	& 0.783	& 0.619	& 0.800\\
150	& 1e-10	& 1e+10	& \RBF	& 10.0	& 0.844	& 0.783	& 0.619	& 0.800\\
200	& 1	& 1	& \RBF	& 10.0	& 0.834	& 0.778	& 0.625	& 0.800\\
200	& 1e-10	& 1e-10	& \RBF	& 10.0	& 0.833	& 0.777	& 0.626	& 0.800\\
200	& 1e-10	& 1e+10	& \RBF	& 10.0	& 0.834	& 0.778	& 0.625	& 0.800\\
250	& 1	& 1	& \RBF	& 10.0	& 0.833	& 0.774	& 0.622	& 0.802\\
250	& 1e-10	& 1e-10	& \RBF	& 10.0	& 0.833	& 0.774	& 0.621	& 0.802\\
250	& 1e-10	& 1e+10	& \RBF	& 10.0	& 0.831	& 0.774	& 0.621	& 0.802\\
300	& 1	& 1	& \RBF	& 10.0	& 0.829	& 0.768	& 0.621	& 0.801\\
300	& 1e-10	& 1e-10	& \RBF	& 10.0	& 0.829	& 0.768	& 0.621	& 0.802\\
300	& 1e-10	& 1e+10	& \RBF	& 10.0	& 0.829	& 0.768	& 0.621	& 0.801\\
350	& 1	& 1	& \RBF	& 10.0	& 0.823	& 0.763	& 0.621	& 0.800\\
350	& 1e-10	& 1e-10	& \RBF	& 10.0	& 0.823	& 0.763	& 0.621	& 0.799\\
350	& 1e-10	& 1e+10	& \RBF	& 10.0	& 0.823	& 0.763	& 0.621	& 0.800\\
400	& 1	& 1	& \RBF	& 10.0	& 0.829	& 0.768	& 0.626	& 0.800\\
400	& 1e-10	& 1e-10	& \RBF	& 10.0	& 0.828	& 0.769	& 0.626	& 0.800\\
400	& 1e-10	& 1e+10	& \RBF	& 10.0	& 0.828	& 0.769	& 0.627	& 0.800\\
50	& 1	& 1	& \RBF	& 10.0	& 0.855	& 0.792	& 0.617	& 0.804\\
50	& 1e-10	& 1e-10	& \RBF	& 10.0	& 0.855	& 0.792	& 0.616	& 0.804\\
50	& 1e-10	& 1e+10	& \RBF	& 10.0	& 0.855	& 0.792	& 0.617	& 0.804\\


==> tables/holdout_2percent_data.tex <==
50	& 5	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.866	& 0.776	& 0.628	& 0.740 \\ 
50	& 5	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.866	& 0.776	& 0.628	& 0.740 \\ 
50	& 5	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.868	& 0.807	& 0.619	& 0.630 \\ 
50	& 5	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.865	& 0.777	& 0.627	& 0.742 \\ 
50	& 5	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.865	& 0.804	& 0.618	& 0.634 \\ 
50	& 5	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.876	& 0.800	& 0.615	& 0.628 \\ 
50	& 5	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.864	& 0.776	& 0.632	& 0.761 \\ 
50	& 5	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.864	& 0.776	& 0.631	& 0.761 \\ 
50	& 5	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.857	& 0.783	& 0.638	& 0.791 \\ 
50	& 5	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.863	& 0.780	& 0.638	& 0.792 \\ 
50	& 10	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.865	& 0.796	& 0.626	& 0.669 \\ 
50	& 10	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.866	& 0.800	& 0.625	& 0.667 \\ 
50	& 10	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.864	& 0.796	& 0.623	& 0.674 \\ 
50	& 10	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.863	& 0.796	& 0.619	& 0.672 \\ 
50	& 10	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.861	& 0.804	& 0.613	& 0.788 \\ 
50	& 10	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.861	& 0.804	& 0.613	& 0.788 \\ 
50	& 10	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.859	& 0.780	& 0.617	& 0.769 \\ 
50	& 10	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.866	& 0.776	& 0.625	& 0.677 \\ 
50	& 10	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.853	& 0.791	& 0.611	& 0.792 \\ 
50	& 10	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.853	& 0.794	& 0.611	& 0.792 \\ 
50	& 15	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.863	& 0.785	& 0.618	& 0.755 \\ 
50	& 15	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.864	& 0.784	& 0.621	& 0.745 \\ 
50	& 15	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.869	& 0.802	& 0.623	& 0.682 \\ 
50	& 15	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.866	& 0.802	& 0.622	& 0.680 \\ 
50	& 15	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.865	& 0.800	& 0.618	& 0.628 \\ 
50	& 15	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.863	& 0.784	& 0.615	& 0.759 \\ 
50	& 15	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.858	& 0.796	& 0.618	& 0.640 \\ 
50	& 15	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.859	& 0.798	& 0.620	& 0.649 \\ 
50	& 15	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.847	& 0.780	& 0.613	& 0.792 \\ 
50	& 15	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.846	& 0.779	& 0.610	& 0.792 \\ 
100	& 5	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.853	& 0.770	& 0.615	& 0.772 \\ 
100	& 5	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.853	& 0.772	& 0.612	& 0.782 \\ 
100	& 5	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.856	& 0.763	& 0.622	& 0.741 \\ 
100	& 5	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.855	& 0.765	& 0.622	& 0.741 \\ 
100	& 5	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.858	& 0.764	& 0.623	& 0.743 \\ 
100	& 5	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.863	& 0.785	& 0.626	& 0.626 \\ 
100	& 5	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.855	& 0.764	& 0.628	& 0.760 \\ 
100	& 5	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.856	& 0.765	& 0.627	& 0.760 \\ 
100	& 5	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.846	& 0.764	& 0.626	& 0.788 \\ 
100	& 5	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.848	& 0.765	& 0.623	& 0.788 \\ 
100	& 10	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.853	& 0.768	& 0.621	& 0.746 \\ 
100	& 10	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.856	& 0.772	& 0.611	& 0.784 \\ 
100	& 10	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.856	& 0.769	& 0.619	& 0.750 \\ 
100	& 10	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.855	& 0.768	& 0.618	& 0.750 \\ 
100	& 10	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.857	& 0.770	& 0.618	& 0.752 \\ 
100	& 10	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.857	& 0.769	& 0.617	& 0.752 \\ 
100	& 10	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.858	& 0.783	& 0.623	& 0.645 \\ 
100	& 10	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.870	& 0.770	& 0.630	& 0.678 \\ 
100	& 10	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.851	& 0.763	& 0.610	& 0.788 \\ 
100	& 10	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.853	& 0.767	& 0.609	& 0.788 \\ 
100	& 15	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.853	& 0.765	& 0.621	& 0.754 \\ 
100	& 15	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.855	& 0.770	& 0.625	& 0.738 \\ 
100	& 15	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.854	& 0.764	& 0.620	& 0.755 \\ 
100	& 15	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.853	& 0.764	& 0.620	& 0.755 \\ 
100	& 15	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.856	& 0.766	& 0.620	& 0.756 \\ 
100	& 15	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.860	& 0.777	& 0.622	& 0.616 \\ 
100	& 15	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.856	& 0.779	& 0.628	& 0.647 \\ 
100	& 15	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.855	& 0.761	& 0.632	& 0.684 \\ 
100	& 15	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.848	& 0.741	& 0.632	& 0.763 \\ 
100	& 15	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.842	& 0.752	& 0.620	& 0.785 \\ 
150	& 5	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.860	& 0.785	& 0.619	& 0.774 \\ 
150	& 5	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.859	& 0.789	& 0.616	& 0.784 \\ 
150	& 5	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.858	& 0.789	& 0.617	& 0.784 \\ 
150	& 5	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.858	& 0.789	& 0.617	& 0.784 \\ 
150	& 5	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.860	& 0.794	& 0.637	& 0.639 \\ 
150	& 5	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.860	& 0.798	& 0.636	& 0.629 \\ 
150	& 5	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.869	& 0.789	& 0.647	& 0.666 \\ 
150	& 5	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.863	& 0.782	& 0.632	& 0.763 \\ 
150	& 5	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.859	& 0.775	& 0.633	& 0.789 \\ 
150	& 5	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.863	& 0.780	& 0.629	& 0.789 \\ 
150	& 10	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.860	& 0.780	& 0.624	& 0.750 \\ 
150	& 10	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.858	& 0.776	& 0.627	& 0.744 \\ 
150	& 10	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.860	& 0.780	& 0.623	& 0.754 \\ 
150	& 10	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.860	& 0.780	& 0.623	& 0.754 \\ 
150	& 10	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.860	& 0.781	& 0.623	& 0.755 \\ 
150	& 10	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.860	& 0.780	& 0.624	& 0.755 \\ 
150	& 10	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.867	& 0.788	& 0.633	& 0.645 \\ 
150	& 10	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.870	& 0.789	& 0.642	& 0.680 \\ 
150	& 10	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.852	& 0.771	& 0.620	& 0.789 \\ 
150	& 10	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.853	& 0.775	& 0.615	& 0.789 \\ 
150	& 15	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.865	& 0.784	& 0.619	& 0.780 \\ 
150	& 15	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.858	& 0.778	& 0.617	& 0.786 \\ 
150	& 15	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.860	& 0.782	& 0.625	& 0.758 \\ 
150	& 15	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.861	& 0.783	& 0.625	& 0.758 \\ 
150	& 15	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.861	& 0.782	& 0.625	& 0.760 \\ 
150	& 15	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.864	& 0.788	& 0.633	& 0.614 \\ 
150	& 15	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.857	& 0.789	& 0.637	& 0.633 \\ 
150	& 15	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.856	& 0.783	& 0.645	& 0.687 \\ 
150	& 15	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.851	& 0.779	& 0.618	& 0.788 \\ 
150	& 15	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.849	& 0.783	& 0.616	& 0.789 \\ 
200	& 5	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.845	& 0.778	& 0.623	& 0.777 \\ 
200	& 5	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.842	& 0.780	& 0.618	& 0.786 \\ 
200	& 5	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.843	& 0.789	& 0.643	& 0.665 \\ 
200	& 5	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.844	& 0.786	& 0.641	& 0.614 \\ 
200	& 5	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.847	& 0.772	& 0.633	& 0.750 \\ 
200	& 5	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.845	& 0.771	& 0.632	& 0.750 \\ 
200	& 5	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.848	& 0.780	& 0.645	& 0.659 \\ 
200	& 5	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.849	& 0.779	& 0.645	& 0.650 \\ 
200	& 5	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.848	& 0.776	& 0.630	& 0.790 \\ 
200	& 5	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.849	& 0.777	& 0.630	& 0.790 \\ 
200	& 10	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.846	& 0.770	& 0.629	& 0.753 \\ 
200	& 10	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.846	& 0.770	& 0.632	& 0.740 \\ 
200	& 10	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.847	& 0.771	& 0.629	& 0.757 \\ 
200	& 10	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.847	& 0.771	& 0.629	& 0.757 \\ 
200	& 10	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.849	& 0.771	& 0.629	& 0.758 \\ 
200	& 10	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.849	& 0.770	& 0.629	& 0.759 \\ 
200	& 10	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.847	& 0.776	& 0.637	& 0.651 \\ 
200	& 10	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.847	& 0.777	& 0.644	& 0.683 \\ 
200	& 10	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.841	& 0.768	& 0.622	& 0.790 \\ 
200	& 10	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.837	& 0.769	& 0.621	& 0.790 \\ 
200	& 15	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.852	& 0.777	& 0.624	& 0.784 \\ 
200	& 15	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.848	& 0.771	& 0.632	& 0.728 \\ 
200	& 15	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.851	& 0.776	& 0.628	& 0.762 \\ 
200	& 15	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.851	& 0.776	& 0.628	& 0.762 \\ 
200	& 15	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.852	& 0.776	& 0.629	& 0.763 \\ 
200	& 15	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.851	& 0.776	& 0.629	& 0.763 \\ 
200	& 15	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.846	& 0.771	& 0.621	& 0.788 \\ 
200	& 15	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.849	& 0.782	& 0.641	& 0.652 \\ 
200	& 15	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.839	& 0.772	& 0.621	& 0.790 \\ 
200	& 15	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.837	& 0.769	& 0.619	& 0.790 \\ 
250	& 5	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.847	& 0.781	& 0.622	& 0.778 \\ 
250	& 5	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.847	& 0.783	& 0.616	& 0.787 \\ 
250	& 5	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.847	& 0.783	& 0.616	& 0.787 \\ 
250	& 5	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.847	& 0.783	& 0.616	& 0.787 \\ 
250	& 5	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.847	& 0.784	& 0.615	& 0.788 \\ 
250	& 5	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.848	& 0.795	& 0.640	& 0.612 \\ 
250	& 5	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.861	& 0.798	& 0.644	& 0.661 \\ 
250	& 5	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.853	& 0.779	& 0.635	& 0.768 \\ 
250	& 5	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.853	& 0.777	& 0.628	& 0.791 \\ 
250	& 5	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.852	& 0.777	& 0.627	& 0.791 \\ 
250	& 10	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.855	& 0.782	& 0.618	& 0.784 \\ 
250	& 10	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.852	& 0.782	& 0.618	& 0.788 \\ 
250	& 10	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.853	& 0.777	& 0.627	& 0.760 \\ 
250	& 10	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.852	& 0.783	& 0.618	& 0.789 \\ 
250	& 10	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.853	& 0.778	& 0.627	& 0.761 \\ 
250	& 10	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.853	& 0.778	& 0.627	& 0.761 \\ 
250	& 10	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.853	& 0.782	& 0.618	& 0.790 \\ 
250	& 10	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.853	& 0.782	& 0.618	& 0.790 \\ 
250	& 10	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.850	& 0.773	& 0.622	& 0.791 \\ 
250	& 10	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.850	& 0.776	& 0.620	& 0.792 \\ 
250	& 15	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.856	& 0.781	& 0.621	& 0.785 \\ 
250	& 15	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.852	& 0.780	& 0.618	& 0.789 \\ 
250	& 15	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.852	& 0.781	& 0.627	& 0.765 \\ 
250	& 15	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.853	& 0.781	& 0.628	& 0.756 \\ 
250	& 15	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.853	& 0.781	& 0.627	& 0.766 \\ 
250	& 15	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.858	& 0.794	& 0.632	& 0.616 \\ 
250	& 15	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.849	& 0.787	& 0.638	& 0.639 \\ 
250	& 15	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.853	& 0.783	& 0.641	& 0.633 \\ 
250	& 15	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.847	& 0.775	& 0.620	& 0.791 \\ 
250	& 15	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.846	& 0.776	& 0.618	& 0.791 \\ 
300	& 5	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.845	& 0.778	& 0.623	& 0.780 \\ 
300	& 5	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.847	& 0.780	& 0.618	& 0.788 \\ 
300	& 5	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.848	& 0.780	& 0.619	& 0.788 \\ 
300	& 5	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.848	& 0.780	& 0.619	& 0.788 \\ 
300	& 5	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.848	& 0.780	& 0.618	& 0.788 \\ 
300	& 5	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.852	& 0.787	& 0.638	& 0.613 \\ 
300	& 5	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.855	& 0.787	& 0.643	& 0.659 \\ 
300	& 5	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.852	& 0.785	& 0.645	& 0.650 \\ 
300	& 5	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.851	& 0.772	& 0.631	& 0.791 \\ 
300	& 5	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.852	& 0.773	& 0.629	& 0.792 \\ 
300	& 10	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.851	& 0.778	& 0.621	& 0.786 \\ 
300	& 10	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.851	& 0.779	& 0.621	& 0.789 \\ 
300	& 10	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.852	& 0.780	& 0.621	& 0.789 \\ 
300	& 10	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.851	& 0.779	& 0.621	& 0.789 \\ 
300	& 10	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.853	& 0.780	& 0.621	& 0.789 \\ 
300	& 10	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.853	& 0.780	& 0.621	& 0.789 \\ 
300	& 10	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.856	& 0.774	& 0.627	& 0.776 \\ 
300	& 10	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.852	& 0.779	& 0.622	& 0.791 \\ 
300	& 10	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.849	& 0.770	& 0.627	& 0.792 \\ 
300	& 10	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.846	& 0.773	& 0.625	& 0.792 \\ 
300	& 15	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.853	& 0.780	& 0.621	& 0.788 \\ 
300	& 15	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.853	& 0.780	& 0.622	& 0.789 \\ 
300	& 15	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.856	& 0.780	& 0.628	& 0.767 \\ 
300	& 15	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.853	& 0.780	& 0.622	& 0.790 \\ 
300	& 15	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.855	& 0.782	& 0.627	& 0.768 \\ 
300	& 15	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.856	& 0.779	& 0.629	& 0.761 \\ 
300	& 15	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.849	& 0.781	& 0.621	& 0.791 \\ 
300	& 15	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.850	& 0.781	& 0.621	& 0.791 \\ 
300	& 15	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.849	& 0.769	& 0.624	& 0.792 \\ 
300	& 15	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.847	& 0.776	& 0.623	& 0.792 \\ 
350	& 5	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.838	& 0.771	& 0.621	& 0.781 \\ 
350	& 5	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.839	& 0.771	& 0.620	& 0.786 \\ 
350	& 5	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.840	& 0.771	& 0.619	& 0.786 \\ 
350	& 5	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.840	& 0.771	& 0.620	& 0.786 \\ 
350	& 5	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.841	& 0.781	& 0.644	& 0.673 \\ 
350	& 5	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.840	& 0.771	& 0.619	& 0.786 \\ 
350	& 5	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.846	& 0.770	& 0.635	& 0.769 \\ 
350	& 5	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.845	& 0.771	& 0.635	& 0.769 \\ 
350	& 5	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.840	& 0.765	& 0.630	& 0.790 \\ 
350	& 5	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.841	& 0.764	& 0.628	& 0.790 \\ 
350	& 10	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.842	& 0.771	& 0.621	& 0.786 \\ 
350	& 10	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.843	& 0.771	& 0.620	& 0.788 \\ 
350	& 10	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.845	& 0.767	& 0.628	& 0.762 \\ 
350	& 10	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.843	& 0.771	& 0.620	& 0.788 \\ 
350	& 10	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.845	& 0.770	& 0.620	& 0.788 \\ 
350	& 10	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.845	& 0.770	& 0.620	& 0.788 \\ 
350	& 10	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.844	& 0.769	& 0.621	& 0.789 \\ 
350	& 10	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.844	& 0.769	& 0.621	& 0.789 \\ 
350	& 10	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.842	& 0.763	& 0.626	& 0.790 \\ 
350	& 10	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.841	& 0.766	& 0.625	& 0.791 \\ 
350	& 15	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.848	& 0.771	& 0.629	& 0.764 \\ 
350	& 15	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.845	& 0.770	& 0.624	& 0.788 \\ 
350	& 15	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.846	& 0.771	& 0.629	& 0.767 \\ 
350	& 15	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.844	& 0.785	& 0.640	& 0.617 \\ 
350	& 15	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.844	& 0.771	& 0.629	& 0.769 \\ 
350	& 15	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.844	& 0.769	& 0.623	& 0.788 \\ 
350	& 15	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.844	& 0.770	& 0.623	& 0.789 \\ 
350	& 15	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.843	& 0.770	& 0.623	& 0.789 \\ 
350	& 15	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.842	& 0.768	& 0.627	& 0.790 \\ 
350	& 15	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.842	& 0.767	& 0.626	& 0.790 \\ 
400	& 5	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.845	& 0.773	& 0.635	& 0.754 \\ 
400	& 5	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.843	& 0.777	& 0.621	& 0.787 \\ 
400	& 5	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.846	& 0.773	& 0.635	& 0.756 \\ 
400	& 5	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.845	& 0.773	& 0.635	& 0.756 \\ 
400	& 5	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.846	& 0.788	& 0.650	& 0.674 \\ 
400	& 5	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.846	& 0.772	& 0.635	& 0.757 \\ 
400	& 5	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.850	& 0.780	& 0.651	& 0.659 \\ 
400	& 5	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.844	& 0.777	& 0.650	& 0.644 \\ 
400	& 5	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.843	& 0.763	& 0.631	& 0.791 \\ 
400	& 5	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.844	& 0.770	& 0.628	& 0.791 \\ 
400	& 10	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.847	& 0.773	& 0.623	& 0.789 \\ 
400	& 10	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.846	& 0.772	& 0.623	& 0.789 \\ 
400	& 10	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.847	& 0.773	& 0.631	& 0.765 \\ 
400	& 10	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.847	& 0.775	& 0.640	& 0.734 \\ 
400	& 10	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.847	& 0.774	& 0.631	& 0.766 \\ 
400	& 10	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.849	& 0.787	& 0.646	& 0.618 \\ 
400	& 10	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.849	& 0.773	& 0.629	& 0.777 \\ 
400	& 10	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.846	& 0.779	& 0.653	& 0.688 \\ 
400	& 10	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.844	& 0.767	& 0.626	& 0.792 \\ 
400	& 10	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.845	& 0.770	& 0.623	& 0.792 \\ 
400	& 15	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.847	& 0.773	& 0.625	& 0.790 \\ 
400	& 15	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.847	& 0.772	& 0.625	& 0.790 \\ 
400	& 15	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.848	& 0.776	& 0.632	& 0.770 \\ 
400	& 15	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.853	& 0.792	& 0.643	& 0.605 \\ 
400	& 15	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.849	& 0.776	& 0.630	& 0.771 \\ 
400	& 15	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.848	& 0.789	& 0.645	& 0.617 \\ 
400	& 15	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.850	& 0.780	& 0.649	& 0.644 \\ 
400	& 15	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.847	& 0.781	& 0.650	& 0.638 \\ 
400	& 15	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.843	& 0.768	& 0.628	& 0.792 \\ 
400	& 15	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.843	& 0.768	& 0.625	& 0.792 \\ 


==> tables/holdout_5percent.tex <==
\begin{ThreePartTable}
    \begin{TableNotes}[flushleft]  %%% This should come before longtable and it is not tablenotes but TableNotes
  \small
  \item
    \begin{footnotesize}
        \bgroup
%        \def\arraystretch{0.5}%       
        \setstretch{1}
		The columns corresponding to ``d'', ``$\alpha$'',
                ``$\beta$'', ``$\gamma$'', ``usim'', and ``$\sigma$'' have the
                latent dimension, weighting factor,
                latent vector regularization parameter,
                cell line similarity regularization parameter,
                cell line similarity function, and parameter for rbf cell line similarity,
                respectively, for \MTCRP.
	      \par
              \egroup
    \end{footnotesize}
  \end{TableNotes}
  \begin{longtable}{
      @{\hspace{5pt}}>{\raggedleft}p{0.04\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.04\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.04\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.04\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.07\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.04\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.04\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft\arraybackslash}p{0.10\textwidth}@{\hspace{6pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
    }
    \caption{\mbox{\MTCRP Performance on New Cell Lines ($\theta$ = 5)}}
    \label{supp:tbl:holdout:5percent}\\
  %
    \hline\hline
    n & d & $\alpha$ & $\beta$ & $\gamma$ & usim & $\sigma$ & \small{AP@$5$} & \small{AP@$10$} & \small{\rCI} & \small{\CI} \\
    \hline
    \endfirsthead
  %
    \multicolumn{11}{c}{{\tablename\ \thetable{} -- continued from previous page}}\\
    \hline\hline
    n & d & $\alpha$ & $\beta$ & $\gamma$ & usim & $\sigma$ & \small{AP@$5$} & \small{AP@$10$} & \small{\rCI} & \small{\CI} \\
    \hline
    \endhead
  %
    \hline
    %  \midrule
    \multicolumn{11}{c}{{Continued on next page}} \\
    \hline
    %\midrule
    \endfoot
    %
    \hline\hline
    %\bottomrule
    \insertTableNotes         %% this added
    \endlastfoot
    %
    \input{tables/holdout_5percent_data.tex}
	
    \hline
  \end{longtable}
\end{ThreePartTable}


==> tables/holdout_5percent_KRL.tex <==
\begin{ThreePartTable}
    \begin{TableNotes}[flushleft]  %%% This should come before longtable and it is not tablenotes but TableNotes
  \small
  \item
    \begin{footnotesize}
        \bgroup
%        \def\arraystretch{0.5}%       
        \setstretch{1}
                The columns corresponding to ``$k$'', ``$\lambda$'',
                ``usim'', and ``$\sigma$'' have the
                two hyperparameters, cell line similarity function,
                and parameter for {$\RBF$} cell line similarity, respectively, 
                for {\KRL}.
	      \par
              \egroup
    \end{footnotesize}
  \end{TableNotes}
  \begin{longtable}{
      @{\hspace{5pt}}>{\raggedleft}p{0.04\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.04\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft\arraybackslash}p{0.10\textwidth}@{\hspace{6pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
    }
    \caption{\mbox{\KRL Performance on New Cell Lines ($\theta$ = 5)}}
    \label{supp:tbl:holdout:5percent:KRL}\\
  %
    \hline\hline
    n & $k$ & $\lambda$ & usim & $\sigma$ & \small{AP@$5$} & \small{AP@$10$} & \small{\rCI} & \small{\CI} \\
    \hline
    \endfirsthead
  %
    \multicolumn{9}{c}{{\tablename\ \thetable{} -- continued from previous page}}\\
    \hline\hline
    n & $k$ & $\lambda$ & usim & $\sigma$ & \small{AP@$5$} & \small{AP@$10$} & \small{\rCI} & \small{\CI} \\
    \hline
    \endhead
  %
    \hline
    %  \midrule
    \multicolumn{9}{c}{{Continued on next page}} \\
    \hline
    %\midrule
    \endfoot
    %
    \hline\hline
    %\bottomrule
    \insertTableNotes         %% this added
    \endlastfoot
    %
    \input{tables/holdout_5percent_KRL_data.tex}
	
    \hline
  \end{longtable}
\end{ThreePartTable}


==> tables/holdout_5percent_KRL_data.tex <==
50	& 5	&   0.000001	&       \RBF	&     0.0001	& 0.511	& 0.463	& 0.538	& 0.729 \\
50	& 5	&   0.000001	&       \RBF	&      0.001	& 0.474	& 0.438	& 0.570	& 0.736 \\
50	& 5	&   0.000001	&       \RBF	&       0.01	& 0.261	& 0.267	& 0.550	& 0.620 \\
50	& 5	&    0.00001	&       \RBF	&       0.01	& 0.275	& 0.306	& 0.533	& 0.635 \\
50	& 5	&     0.0001	&       \RBF	&     0.0001	& 0.478	& 0.450	& 0.552	& 0.783 \\
50	& 5	&     0.0001	&       \RBF	&      0.001	& 0.602	& 0.530	& 0.560	& 0.764 \\
50	& 5	&     0.0001	&       \RBF	&       0.01	& 0.295	& 0.319	& 0.527	& 0.604 \\
50	& 5	&      0.001	&       \LIN	&          -	& 0.422	& 0.400	& 0.551	& 0.723 \\
50	& 5	&      0.001	&       \RBF	&     0.0001	& 0.571	& 0.529	& 0.559	& 0.734 \\
50	& 5	&      0.001	&       \RBF	&      0.001	& 0.602	& 0.530	& 0.560	& 0.764 \\
50	& 5	&      0.001	&       \RBF	&       0.01	& 0.288	& 0.304	& 0.528	& 0.558 \\
50	& 5	&       0.01	&       \LIN	&          -	& 0.499	& 0.438	& 0.545	& 0.738 \\
50	& 5	&       0.01	&       \RBF	&     0.0001	& 0.571	& 0.529	& 0.559	& 0.734 \\
50	& 5	&       0.01	&       \RBF	&      0.001	& 0.602	& 0.530	& 0.560	& 0.764 \\
50	& 5	&       0.01	&       \RBF	&       0.01	& 0.204	& 0.249	& 0.512	& 0.506 \\
50	& 5	&        0.1	&       \LIN	&          -	& 0.570	& 0.506	& 0.535	& 0.767 \\
50	& 5	&        0.1	&       \RBF	&     0.0001	& 0.571	& 0.529	& 0.559	& 0.734 \\
50	& 5	&        0.1	&       \RBF	&      0.001	& 0.602	& 0.530	& 0.560	& 0.764 \\
50	& 5	&        0.1	&       \RBF	&       0.01	& 0.144	& 0.173	& 0.508	& 0.477 \\
50	& 5	&        0.2	&       \LIN	&          -	& 0.516	& 0.483	& 0.553	& 0.766 \\
50	& 5	&        0.2	&       \RBF	&     0.0001	& 0.571	& 0.529	& 0.559	& 0.734 \\
50	& 5	&        0.2	&       \RBF	&      0.001	& 0.602	& 0.530	& 0.560	& 0.764 \\
50	& 5	&        0.2	&       \RBF	&       0.01	& 0.071	& 0.099	& 0.512	& 0.473 \\
50	& 5	&        0.4	&       \LIN	&          -	& 0.454	& 0.430	& 0.535	& 0.780 \\
50	& 5	&        0.4	&       \RBF	&     0.0001	& 0.571	& 0.529	& 0.559	& 0.734 \\
50	& 5	&        0.4	&       \RBF	&      0.001	& 0.602	& 0.530	& 0.560	& 0.764 \\
50	& 5	&        0.4	&       \RBF	&       0.01	& 0.067	& 0.093	& 0.509	& 0.471 \\
50	& 5	&        0.6	&       \LIN	&          -	& 0.438	& 0.417	& 0.548	& 0.761 \\
50	& 5	&        0.6	&       \RBF	&     0.0001	& 0.571	& 0.529	& 0.559	& 0.734 \\
50	& 5	&        0.6	&       \RBF	&      0.001	& 0.602	& 0.530	& 0.560	& 0.764 \\
50	& 5	&        0.6	&       \RBF	&       0.01	& 0.037	& 0.069	& 0.508	& 0.470 \\
50	& 5	&        0.8	&       \LIN	&          -	& 0.594	& 0.559	& 0.548	& 0.760 \\
50	& 5	&        0.8	&       \RBF	&     0.0001	& 0.571	& 0.529	& 0.559	& 0.734 \\
50	& 5	&        0.8	&       \RBF	&      0.001	& 0.602	& 0.530	& 0.560	& 0.764 \\
50	& 5	&        0.8	&       \RBF	&       0.01	& 0.046	& 0.077	& 0.508	& 0.469 \\
50	& 5	&        1.0	&       \LIN	&          -	& 0.573	& 0.536	& 0.547	& 0.774 \\
50	& 5	&        1.0	&       \RBF	&     0.0001	& 0.571	& 0.529	& 0.559	& 0.734 \\
50	& 5	&        1.0	&       \RBF	&      0.001	& 0.602	& 0.530	& 0.560	& 0.764 \\
50	& 5	&        1.0	&       \RBF	&       0.01	& 0.046	& 0.077	& 0.508	& 0.469 \\
50	& 5	&         10	&       \LIN	&          -	& 0.567	& 0.520	& 0.531	& 0.789 \\
50	& 5	&         10	&       \RBF	&     0.0001	& 0.571	& 0.529	& 0.559	& 0.734 \\
50	& 5	&         10	&       \RBF	&      0.001	& 0.602	& 0.530	& 0.560	& 0.764 \\
50	& 5	&         10	&       \RBF	&       0.01	& 0.021	& 0.051	& 0.510	& 0.469 \\
50	& 5	&         50	&       \LIN	&          -	& 0.586	& 0.560	& 0.561	& 0.752 \\
50	& 5	&         50	&       \RBF	&     0.0001	& 0.571	& 0.529	& 0.559	& 0.734 \\
50	& 5	&         50	&       \RBF	&      0.001	& 0.602	& 0.530	& 0.560	& 0.764 \\
50	& 5	&         50	&       \RBF	&       0.01	& 0.018	& 0.050	& 0.509	& 0.468 \\
50	& 5	&        100	&       \LIN	&          -	& 0.590	& 0.530	& 0.561	& 0.707 \\
50	& 5	&        100	&       \RBF	&     0.0001	& 0.571	& 0.529	& 0.559	& 0.734 \\
50	& 5	&        100	&       \RBF	&      0.001	& 0.602	& 0.530	& 0.560	& 0.764 \\
50	& 5	&        100	&       \RBF	&       0.01	& 0.021	& 0.053	& 0.509	& 0.468 \\
50	& 10	&   0.000001	&       \LIN	&          -	& 0.347	& 0.355	& 0.534	& 0.700 \\
50	& 10	&   0.000001	&       \RBF	&       0.01	& 0.288	& 0.281	& 0.548	& 0.610 \\
50	& 10	&      0.001	&       \LIN	&          -	& 0.401	& 0.352	& 0.535	& 0.700 \\
50	& 10	&      0.001	&       \RBF	&     0.0001	& 0.571	& 0.534	& 0.563	& 0.774 \\
50	& 10	&      0.001	&       \RBF	&      0.001	& 0.609	& 0.535	& 0.564	& 0.777 \\
50	& 10	&      0.001	&       \RBF	&       0.01	& 0.260	& 0.287	& 0.535	& 0.570 \\
50	& 10	&       0.01	&       \LIN	&          -	& 0.461	& 0.450	& 0.551	& 0.768 \\
50	& 10	&       0.01	&       \RBF	&     0.0001	& 0.571	& 0.534	& 0.563	& 0.774 \\
50	& 10	&       0.01	&       \RBF	&      0.001	& 0.609	& 0.535	& 0.564	& 0.777 \\
50	& 10	&       0.01	&       \RBF	&       0.01	& 0.215	& 0.251	& 0.516	& 0.512 \\
50	& 10	&        0.1	&       \LIN	&          -	& 0.583	& 0.526	& 0.545	& 0.783 \\
50	& 10	&        0.1	&       \RBF	&     0.0001	& 0.571	& 0.534	& 0.563	& 0.774 \\
50	& 10	&        0.1	&       \RBF	&      0.001	& 0.609	& 0.535	& 0.564	& 0.777 \\
50	& 10	&        0.1	&       \RBF	&       0.01	& 0.145	& 0.174	& 0.509	& 0.479 \\
50	& 10	&        0.2	&       \LIN	&          -	& 0.528	& 0.479	& 0.550	& 0.782 \\
50	& 10	&        0.2	&       \RBF	&     0.0001	& 0.571	& 0.534	& 0.563	& 0.774 \\
50	& 10	&        0.2	&       \RBF	&      0.001	& 0.609	& 0.535	& 0.564	& 0.777 \\
50	& 10	&        0.2	&       \RBF	&       0.01	& 0.069	& 0.098	& 0.512	& 0.474 \\
50	& 10	&        0.4	&       \LIN	&          -	& 0.600	& 0.546	& 0.551	& 0.786 \\
50	& 10	&        0.4	&       \RBF	&     0.0001	& 0.571	& 0.534	& 0.563	& 0.774 \\
50	& 10	&        0.4	&       \RBF	&      0.001	& 0.609	& 0.535	& 0.564	& 0.777 \\
50	& 10	&        0.4	&       \RBF	&       0.01	& 0.077	& 0.104	& 0.510	& 0.472 \\
50	& 10	&        0.6	&       \LIN	&          -	& 0.597	& 0.556	& 0.549	& 0.783 \\
50	& 10	&        0.6	&       \RBF	&     0.0001	& 0.571	& 0.534	& 0.563	& 0.774 \\
50	& 10	&        0.6	&       \RBF	&      0.001	& 0.609	& 0.535	& 0.564	& 0.777 \\
50	& 10	&        0.6	&       \RBF	&       0.01	& 0.049	& 0.081	& 0.509	& 0.470 \\
50	& 10	&        0.8	&       \LIN	&          -	& 0.587	& 0.559	& 0.545	& 0.785 \\
50	& 10	&        0.8	&       \RBF	&     0.0001	& 0.571	& 0.534	& 0.563	& 0.774 \\
50	& 10	&        0.8	&       \RBF	&      0.001	& 0.609	& 0.535	& 0.564	& 0.777 \\
50	& 10	&        0.8	&       \RBF	&       0.01	& 0.046	& 0.078	& 0.510	& 0.470 \\
50	& 10	&        1.0	&       \LIN	&          -	& 0.594	& 0.539	& 0.545	& 0.785 \\
50	& 10	&        1.0	&       \RBF	&     0.0001	& 0.571	& 0.534	& 0.563	& 0.774 \\
50	& 10	&        1.0	&       \RBF	&      0.001	& 0.609	& 0.535	& 0.564	& 0.777 \\
50	& 10	&        1.0	&       \RBF	&       0.01	& 0.049	& 0.081	& 0.510	& 0.470 \\
50	& 10	&         10	&       \LIN	&          -	& 0.582	& 0.545	& 0.547	& 0.791 \\
50	& 10	&         10	&       \RBF	&     0.0001	& 0.571	& 0.534	& 0.563	& 0.774 \\
50	& 10	&         10	&       \RBF	&      0.001	& 0.609	& 0.535	& 0.564	& 0.777 \\
50	& 10	&         10	&       \RBF	&       0.01	& 0.019	& 0.051	& 0.510	& 0.469 \\
50	& 10	&         50	&       \LIN	&          -	& 0.586	& 0.555	& 0.553	& 0.768 \\
50	& 10	&         50	&       \RBF	&     0.0001	& 0.571	& 0.534	& 0.563	& 0.774 \\
50	& 10	&         50	&       \RBF	&      0.001	& 0.609	& 0.535	& 0.564	& 0.777 \\
50	& 10	&         50	&       \RBF	&       0.01	& 0.024	& 0.054	& 0.510	& 0.469 \\
50	& 10	&        100	&       \LIN	&          -	& 0.572	& 0.535	& 0.561	& 0.720 \\
50	& 10	&        100	&       \RBF	&     0.0001	& 0.571	& 0.534	& 0.563	& 0.774 \\
50	& 10	&        100	&       \RBF	&      0.001	& 0.609	& 0.535	& 0.564	& 0.777 \\
50	& 10	&        100	&       \RBF	&       0.01	& 0.021	& 0.053	& 0.509	& 0.468 \\
50	& 15	&      0.001	&       \LIN	&          -	& 0.374	& 0.362	& 0.534	& 0.717 \\
50	& 15	&      0.001	&       \RBF	&     0.0001	& 0.577	& 0.522	& 0.562	& 0.781 \\
50	& 15	&      0.001	&       \RBF	&      0.001	& 0.608	& 0.538	& 0.566	& 0.776 \\
50	& 15	&      0.001	&       \RBF	&       0.01	& 0.277	& 0.303	& 0.538	& 0.574 \\
50	& 15	&       0.01	&       \LIN	&          -	& 0.473	& 0.436	& 0.555	& 0.768 \\
50	& 15	&       0.01	&       \RBF	&     0.0001	& 0.577	& 0.522	& 0.562	& 0.781 \\
50	& 15	&       0.01	&       \RBF	&      0.001	& 0.608	& 0.538	& 0.566	& 0.776 \\
50	& 15	&       0.01	&       \RBF	&       0.01	& 0.228	& 0.260	& 0.518	& 0.515 \\
50	& 15	&        0.1	&       \LIN	&          -	& 0.347	& 0.339	& 0.515	& 0.743 \\
50	& 15	&        0.1	&       \RBF	&     0.0001	& 0.577	& 0.522	& 0.562	& 0.781 \\
50	& 15	&        0.1	&       \RBF	&      0.001	& 0.608	& 0.538	& 0.566	& 0.776 \\
50	& 15	&        0.1	&       \RBF	&       0.01	& 0.141	& 0.171	& 0.513	& 0.480 \\
50	& 15	&        0.2	&       \LIN	&          -	& 0.621	& 0.573	& 0.548	& 0.780 \\
50	& 15	&        0.2	&       \RBF	&     0.0001	& 0.577	& 0.522	& 0.562	& 0.781 \\
50	& 15	&        0.2	&       \RBF	&      0.001	& 0.608	& 0.538	& 0.566	& 0.776 \\
50	& 15	&        0.2	&       \RBF	&       0.01	& 0.076	& 0.106	& 0.513	& 0.474 \\
50	& 15	&        0.4	&       \LIN	&          -	& 0.605	& 0.555	& 0.551	& 0.783 \\
50	& 15	&        0.4	&       \RBF	&     0.0001	& 0.577	& 0.522	& 0.562	& 0.781 \\
50	& 15	&        0.4	&       \RBF	&      0.001	& 0.608	& 0.538	& 0.566	& 0.776 \\
50	& 15	&        0.4	&       \RBF	&       0.01	& 0.081	& 0.108	& 0.512	& 0.471 \\
50	& 15	&        0.6	&       \LIN	&          -	& 0.602	& 0.563	& 0.550	& 0.783 \\
50	& 15	&        0.6	&       \RBF	&     0.0001	& 0.577	& 0.522	& 0.562	& 0.781 \\
50	& 15	&        0.6	&       \RBF	&      0.001	& 0.608	& 0.538	& 0.566	& 0.776 \\
50	& 15	&        0.6	&       \RBF	&       0.01	& 0.049	& 0.082	& 0.510	& 0.470 \\
50	& 15	&        0.8	&       \LIN	&          -	& 0.303	& 0.332	& 0.510	& 0.758 \\
50	& 15	&        0.8	&       \RBF	&     0.0001	& 0.577	& 0.522	& 0.562	& 0.781 \\
50	& 15	&        0.8	&       \RBF	&      0.001	& 0.608	& 0.538	& 0.566	& 0.776 \\
50	& 15	&        0.8	&       \RBF	&       0.01	& 0.046	& 0.078	& 0.511	& 0.470 \\
50	& 15	&        1.0	&       \LIN	&          -	& 0.466	& 0.445	& 0.532	& 0.757 \\
50	& 15	&        1.0	&       \RBF	&     0.0001	& 0.577	& 0.522	& 0.562	& 0.781 \\
50	& 15	&        1.0	&       \RBF	&      0.001	& 0.608	& 0.538	& 0.566	& 0.776 \\
50	& 15	&        1.0	&       \RBF	&       0.01	& 0.046	& 0.078	& 0.512	& 0.470 \\
50	& 15	&         10	&       \LIN	&          -	& 0.547	& 0.529	& 0.551	& 0.786 \\
50	& 15	&         10	&       \RBF	&     0.0001	& 0.577	& 0.522	& 0.562	& 0.781 \\
50	& 15	&         10	&       \RBF	&      0.001	& 0.608	& 0.538	& 0.566	& 0.776 \\
50	& 15	&         10	&       \RBF	&       0.01	& 0.019	& 0.051	& 0.511	& 0.469 \\
50	& 15	&         50	&       \LIN	&          -	& 0.593	& 0.560	& 0.546	& 0.785 \\
50	& 15	&         50	&       \RBF	&     0.0001	& 0.577	& 0.522	& 0.562	& 0.781 \\
50	& 15	&         50	&       \RBF	&      0.001	& 0.608	& 0.538	& 0.566	& 0.776 \\
50	& 15	&         50	&       \RBF	&       0.01	& 0.024	& 0.054	& 0.510	& 0.469 \\
50	& 15	&        100	&       \LIN	&          -	& 0.567	& 0.520	& 0.557	& 0.748 \\
50	& 15	&        100	&       \RBF	&     0.0001	& 0.577	& 0.522	& 0.562	& 0.781 \\
50	& 15	&        100	&       \RBF	&      0.001	& 0.608	& 0.538	& 0.566	& 0.776 \\
50	& 15	&        100	&       \RBF	&       0.01	& 0.019	& 0.051	& 0.509	& 0.469 \\
100	& 5	&   0.000001	&       \RBF	&     0.0001	& 0.503	& 0.474	& 0.541	& 0.726 \\
100	& 5	&   0.000001	&       \RBF	&      0.001	& 0.562	& 0.481	& 0.550	& 0.732 \\
100	& 5	&   0.000001	&       \RBF	&       0.01	& 0.278	& 0.272	& 0.526	& 0.614 \\
100	& 5	&    0.00001	&       \LIN	&          -	& 0.350	& 0.333	& 0.521	& 0.692 \\
100	& 5	&    0.00001	&       \RBF	&       0.01	& 0.264	& 0.277	& 0.517	& 0.618 \\
100	& 5	&     0.0001	&       \RBF	&     0.0001	& 0.495	& 0.439	& 0.545	& 0.779 \\
100	& 5	&     0.0001	&       \RBF	&      0.001	& 0.568	& 0.497	& 0.568	& 0.761 \\
100	& 5	&     0.0001	&       \RBF	&       0.01	& 0.238	& 0.259	& 0.520	& 0.586 \\
100	& 5	&      0.001	&       \LIN	&          -	& 0.417	& 0.408	& 0.539	& 0.721 \\
100	& 5	&      0.001	&       \RBF	&     0.0001	& 0.512	& 0.470	& 0.557	& 0.733 \\
100	& 5	&      0.001	&       \RBF	&      0.001	& 0.568	& 0.497	& 0.568	& 0.761 \\
100	& 5	&      0.001	&       \RBF	&       0.01	& 0.227	& 0.248	& 0.512	& 0.546 \\
100	& 5	&       0.01	&       \LIN	&          -	& 0.463	& 0.446	& 0.534	& 0.743 \\
100	& 5	&       0.01	&       \RBF	&     0.0001	& 0.512	& 0.470	& 0.557	& 0.733 \\
100	& 5	&       0.01	&       \RBF	&      0.001	& 0.568	& 0.497	& 0.568	& 0.761 \\
100	& 5	&       0.01	&       \RBF	&       0.01	& 0.182	& 0.209	& 0.509	& 0.508 \\
100	& 5	&        0.1	&       \LIN	&          -	& 0.479	& 0.444	& 0.543	& 0.768 \\
100	& 5	&        0.1	&       \RBF	&     0.0001	& 0.512	& 0.470	& 0.557	& 0.733 \\
100	& 5	&        0.1	&       \RBF	&      0.001	& 0.568	& 0.497	& 0.568	& 0.761 \\
100	& 5	&        0.1	&       \RBF	&       0.01	& 0.140	& 0.164	& 0.510	& 0.483 \\
100	& 5	&        0.2	&       \LIN	&          -	& 0.458	& 0.429	& 0.544	& 0.763 \\
100	& 5	&        0.2	&       \RBF	&     0.0001	& 0.512	& 0.470	& 0.557	& 0.733 \\
100	& 5	&        0.2	&       \RBF	&      0.001	& 0.568	& 0.497	& 0.568	& 0.761 \\
100	& 5	&        0.2	&       \RBF	&       0.01	& 0.074	& 0.102	& 0.512	& 0.478 \\
100	& 5	&        0.4	&       \LIN	&          -	& 0.495	& 0.485	& 0.546	& 0.769 \\
100	& 5	&        0.4	&       \RBF	&     0.0001	& 0.512	& 0.470	& 0.557	& 0.733 \\
100	& 5	&        0.4	&       \RBF	&      0.001	& 0.568	& 0.497	& 0.568	& 0.761 \\
100	& 5	&        0.4	&       \RBF	&       0.01	& 0.075	& 0.106	& 0.509	& 0.475 \\
100	& 5	&        0.6	&       \LIN	&          -	& 0.524	& 0.493	& 0.551	& 0.762 \\
100	& 5	&        0.6	&       \RBF	&     0.0001	& 0.512	& 0.470	& 0.557	& 0.733 \\
100	& 5	&        0.6	&       \RBF	&      0.001	& 0.568	& 0.497	& 0.568	& 0.761 \\
100	& 5	&        0.6	&       \RBF	&       0.01	& 0.064	& 0.099	& 0.509	& 0.473 \\
100	& 5	&        0.8	&       \LIN	&          -	& 0.524	& 0.488	& 0.549	& 0.761 \\
100	& 5	&        0.8	&       \RBF	&     0.0001	& 0.512	& 0.470	& 0.557	& 0.733 \\
100	& 5	&        0.8	&       \RBF	&      0.001	& 0.568	& 0.497	& 0.568	& 0.761 \\
100	& 5	&        0.8	&       \RBF	&       0.01	& 0.053	& 0.089	& 0.509	& 0.472 \\
100	& 5	&        1.0	&       \LIN	&          -	& 0.555	& 0.503	& 0.549	& 0.775 \\
100	& 5	&        1.0	&       \RBF	&     0.0001	& 0.512	& 0.470	& 0.557	& 0.733 \\
100	& 5	&        1.0	&       \RBF	&      0.001	& 0.568	& 0.497	& 0.568	& 0.761 \\
100	& 5	&        1.0	&       \RBF	&       0.01	& 0.043	& 0.077	& 0.508	& 0.472 \\
100	& 5	&         10	&       \LIN	&          -	& 0.504	& 0.477	& 0.535	& 0.782 \\
100	& 5	&         10	&       \RBF	&     0.0001	& 0.512	& 0.470	& 0.557	& 0.733 \\
100	& 5	&         10	&       \RBF	&      0.001	& 0.568	& 0.497	& 0.568	& 0.761 \\
100	& 5	&         10	&       \RBF	&       0.01	& 0.026	& 0.064	& 0.506	& 0.469 \\
100	& 5	&         50	&       \LIN	&          -	& 0.515	& 0.500	& 0.558	& 0.752 \\
100	& 5	&         50	&       \RBF	&     0.0001	& 0.512	& 0.470	& 0.557	& 0.733 \\
100	& 5	&         50	&       \RBF	&      0.001	& 0.568	& 0.497	& 0.568	& 0.761 \\
100	& 5	&         50	&       \RBF	&       0.01	& 0.026	& 0.066	& 0.505	& 0.468 \\
100	& 5	&        100	&       \LIN	&          -	& 0.508	& 0.469	& 0.557	& 0.699 \\
100	& 5	&        100	&       \RBF	&     0.0001	& 0.512	& 0.470	& 0.557	& 0.733 \\
100	& 5	&        100	&       \RBF	&      0.001	& 0.568	& 0.497	& 0.568	& 0.761 \\
100	& 5	&        100	&       \RBF	&       0.01	& 0.026	& 0.067	& 0.505	& 0.468 \\
100	& 10	&   0.000001	&       \LIN	&          -	& 0.160	& 0.203	& 0.520	& 0.694 \\
100	& 10	&   0.000001	&       \RBF	&       0.01	& 0.280	& 0.284	& 0.531	& 0.605 \\
100	& 10	&      0.001	&       \RBF	&     0.0001	& 0.523	& 0.485	& 0.559	& 0.773 \\
100	& 10	&      0.001	&       \RBF	&      0.001	& 0.560	& 0.496	& 0.566	& 0.774 \\
100	& 10	&      0.001	&       \RBF	&       0.01	& 0.210	& 0.247	& 0.512	& 0.557 \\
100	& 10	&       0.01	&       \LIN	&          -	& 0.484	& 0.454	& 0.547	& 0.765 \\
100	& 10	&       0.01	&       \RBF	&     0.0001	& 0.523	& 0.485	& 0.559	& 0.773 \\
100	& 10	&       0.01	&       \RBF	&      0.001	& 0.560	& 0.496	& 0.566	& 0.774 \\
100	& 10	&       0.01	&       \RBF	&       0.01	& 0.188	& 0.218	& 0.509	& 0.514 \\
100	& 10	&        0.1	&       \LIN	&          -	& 0.513	& 0.458	& 0.553	& 0.781 \\
100	& 10	&        0.1	&       \RBF	&     0.0001	& 0.523	& 0.485	& 0.559	& 0.773 \\
100	& 10	&        0.1	&       \RBF	&      0.001	& 0.560	& 0.496	& 0.566	& 0.774 \\
100	& 10	&        0.1	&       \RBF	&       0.01	& 0.138	& 0.165	& 0.511	& 0.485 \\
100	& 10	&        0.2	&       \LIN	&          -	& 0.525	& 0.480	& 0.550	& 0.774 \\
100	& 10	&        0.2	&       \RBF	&     0.0001	& 0.523	& 0.485	& 0.559	& 0.773 \\
100	& 10	&        0.2	&       \RBF	&      0.001	& 0.560	& 0.496	& 0.566	& 0.774 \\
100	& 10	&        0.2	&       \RBF	&       0.01	& 0.087	& 0.115	& 0.513	& 0.479 \\
100	& 10	&        0.4	&       \LIN	&          -	& 0.538	& 0.496	& 0.547	& 0.781 \\
100	& 10	&        0.4	&       \RBF	&     0.0001	& 0.523	& 0.485	& 0.559	& 0.773 \\
100	& 10	&        0.4	&       \RBF	&      0.001	& 0.560	& 0.496	& 0.566	& 0.774 \\
100	& 10	&        0.4	&       \RBF	&       0.01	& 0.077	& 0.108	& 0.510	& 0.475 \\
100	& 10	&        0.6	&       \LIN	&          -	& 0.547	& 0.488	& 0.547	& 0.784 \\
100	& 10	&        0.6	&       \RBF	&     0.0001	& 0.523	& 0.485	& 0.559	& 0.773 \\
100	& 10	&        0.6	&       \RBF	&      0.001	& 0.560	& 0.496	& 0.566	& 0.774 \\
100	& 10	&        0.6	&       \RBF	&       0.01	& 0.068	& 0.105	& 0.509	& 0.473 \\
100	& 10	&        0.8	&       \LIN	&          -	& 0.481	& 0.466	& 0.552	& 0.781 \\
100	& 10	&        0.8	&       \RBF	&     0.0001	& 0.523	& 0.485	& 0.559	& 0.773 \\
100	& 10	&        0.8	&       \RBF	&      0.001	& 0.560	& 0.496	& 0.566	& 0.774 \\
100	& 10	&        0.8	&       \RBF	&       0.01	& 0.057	& 0.094	& 0.509	& 0.472 \\
100	& 10	&        1.0	&       \LIN	&          -	& 0.542	& 0.498	& 0.545	& 0.784 \\
100	& 10	&        1.0	&       \RBF	&     0.0001	& 0.523	& 0.485	& 0.559	& 0.773 \\
100	& 10	&        1.0	&       \RBF	&      0.001	& 0.560	& 0.496	& 0.566	& 0.774 \\
100	& 10	&        1.0	&       \RBF	&       0.01	& 0.056	& 0.092	& 0.509	& 0.472 \\
100	& 10	&         10	&       \LIN	&          -	& 0.493	& 0.466	& 0.543	& 0.774 \\
100	& 10	&         10	&       \RBF	&     0.0001	& 0.523	& 0.485	& 0.559	& 0.773 \\
100	& 10	&         10	&       \RBF	&      0.001	& 0.560	& 0.496	& 0.566	& 0.774 \\
100	& 10	&         10	&       \RBF	&       0.01	& 0.028	& 0.067	& 0.506	& 0.469 \\
100	& 10	&         50	&       \LIN	&          -	& 0.525	& 0.499	& 0.550	& 0.771 \\
100	& 10	&         50	&       \RBF	&     0.0001	& 0.523	& 0.485	& 0.559	& 0.773 \\
100	& 10	&         50	&       \RBF	&      0.001	& 0.560	& 0.496	& 0.566	& 0.774 \\
100	& 10	&         50	&       \RBF	&       0.01	& 0.032	& 0.071	& 0.506	& 0.468 \\
100	& 10	&        100	&       \LIN	&          -	& 0.510	& 0.481	& 0.558	& 0.723 \\
100	& 10	&        100	&       \RBF	&     0.0001	& 0.523	& 0.485	& 0.559	& 0.773 \\
100	& 10	&        100	&       \RBF	&      0.001	& 0.560	& 0.496	& 0.566	& 0.774 \\
100	& 10	&        100	&       \RBF	&       0.01	& 0.029	& 0.067	& 0.505	& 0.468 \\
100	& 15	&      0.001	&       \LIN	&          -	& 0.353	& 0.335	& 0.535	& 0.703 \\
100	& 15	&      0.001	&       \RBF	&     0.0001	& 0.528	& 0.490	& 0.559	& 0.781 \\
100	& 15	&      0.001	&       \RBF	&      0.001	& 0.554	& 0.494	& 0.562	& 0.773 \\
100	& 15	&      0.001	&       \RBF	&       0.01	& 0.212	& 0.249	& 0.514	& 0.561 \\
100	& 15	&       0.01	&       \RBF	&     0.0001	& 0.528	& 0.490	& 0.559	& 0.781 \\
100	& 15	&       0.01	&       \RBF	&      0.001	& 0.554	& 0.494	& 0.562	& 0.773 \\
100	& 15	&       0.01	&       \RBF	&       0.01	& 0.188	& 0.220	& 0.512	& 0.517 \\
100	& 15	&        0.1	&       \LIN	&          -	& 0.507	& 0.460	& 0.555	& 0.777 \\
100	& 15	&        0.1	&       \RBF	&     0.0001	& 0.528	& 0.490	& 0.559	& 0.781 \\
100	& 15	&        0.1	&       \RBF	&      0.001	& 0.554	& 0.494	& 0.562	& 0.773 \\
100	& 15	&        0.1	&       \RBF	&       0.01	& 0.142	& 0.167	& 0.511	& 0.486 \\
100	& 15	&        0.2	&       \LIN	&          -	& 0.539	& 0.503	& 0.554	& 0.779 \\
100	& 15	&        0.2	&       \RBF	&     0.0001	& 0.528	& 0.490	& 0.559	& 0.781 \\
100	& 15	&        0.2	&       \RBF	&      0.001	& 0.554	& 0.494	& 0.562	& 0.773 \\
100	& 15	&        0.2	&       \RBF	&       0.01	& 0.092	& 0.119	& 0.515	& 0.480 \\
100	& 15	&        0.4	&       \LIN	&          -	& 0.538	& 0.503	& 0.554	& 0.781 \\
100	& 15	&        0.4	&       \RBF	&     0.0001	& 0.528	& 0.490	& 0.559	& 0.781 \\
100	& 15	&        0.4	&       \RBF	&      0.001	& 0.554	& 0.494	& 0.562	& 0.773 \\
100	& 15	&        0.4	&       \RBF	&       0.01	& 0.080	& 0.112	& 0.510	& 0.476 \\
100	& 15	&        0.6	&       \LIN	&          -	& 0.535	& 0.497	& 0.554	& 0.782 \\
100	& 15	&        0.6	&       \RBF	&     0.0001	& 0.528	& 0.490	& 0.559	& 0.781 \\
100	& 15	&        0.6	&       \RBF	&      0.001	& 0.554	& 0.494	& 0.562	& 0.773 \\
100	& 15	&        0.6	&       \RBF	&       0.01	& 0.067	& 0.104	& 0.509	& 0.473 \\
100	& 15	&        0.8	&       \LIN	&          -	& 0.533	& 0.504	& 0.551	& 0.782 \\
100	& 15	&        0.8	&       \RBF	&     0.0001	& 0.528	& 0.490	& 0.559	& 0.781 \\
100	& 15	&        0.8	&       \RBF	&      0.001	& 0.554	& 0.494	& 0.562	& 0.773 \\
100	& 15	&        0.8	&       \RBF	&       0.01	& 0.058	& 0.096	& 0.509	& 0.473 \\
100	& 15	&        1.0	&       \LIN	&          -	& 0.511	& 0.494	& 0.553	& 0.783 \\
100	& 15	&        1.0	&       \RBF	&     0.0001	& 0.528	& 0.490	& 0.559	& 0.781 \\
100	& 15	&        1.0	&       \RBF	&      0.001	& 0.554	& 0.494	& 0.562	& 0.773 \\
100	& 15	&        1.0	&       \RBF	&       0.01	& 0.044	& 0.079	& 0.507	& 0.472 \\
100	& 15	&         10	&       \LIN	&          -	& 0.508	& 0.494	& 0.547	& 0.784 \\
100	& 15	&         10	&       \RBF	&     0.0001	& 0.528	& 0.490	& 0.559	& 0.781 \\
100	& 15	&         10	&       \RBF	&      0.001	& 0.554	& 0.494	& 0.562	& 0.773 \\
100	& 15	&         10	&       \RBF	&       0.01	& 0.030	& 0.068	& 0.506	& 0.469 \\
100	& 15	&         50	&       \LIN	&          -	& 0.528	& 0.498	& 0.547	& 0.786 \\
100	& 15	&         50	&       \RBF	&     0.0001	& 0.528	& 0.490	& 0.559	& 0.781 \\
100	& 15	&         50	&       \RBF	&      0.001	& 0.554	& 0.494	& 0.562	& 0.773 \\
100	& 15	&         50	&       \RBF	&       0.01	& 0.031	& 0.069	& 0.506	& 0.468 \\
100	& 15	&        100	&       \LIN	&          -	& 0.511	& 0.486	& 0.555	& 0.749 \\
100	& 15	&        100	&       \RBF	&     0.0001	& 0.528	& 0.490	& 0.559	& 0.781 \\
100	& 15	&        100	&       \RBF	&      0.001	& 0.554	& 0.494	& 0.562	& 0.773 \\
100	& 15	&        100	&       \RBF	&       0.01	& 0.034	& 0.072	& 0.505	& 0.468 \\
150	& 5	&   0.000001	&       \LIN	&          -	& 0.330	& 0.312	& 0.534	& 0.688 \\
150	& 5	&   0.000001	&       \RBF	&     0.0001	& 0.460	& 0.444	& 0.543	& 0.728 \\
150	& 5	&   0.000001	&       \RBF	&      0.001	& 0.481	& 0.431	& 0.548	& 0.729 \\
150	& 5	&   0.000001	&       \RBF	&       0.01	& 0.277	& 0.280	& 0.529	& 0.605 \\
150	& 5	&    0.00001	&       \RBF	&      0.001	& 0.534	& 0.496	& 0.565	& 0.758 \\
150	& 5	&    0.00001	&       \RBF	&       0.01	& 0.249	& 0.273	& 0.524	& 0.608 \\
150	& 5	&     0.0001	&       \RBF	&     0.0001	& 0.459	& 0.429	& 0.551	& 0.773 \\
150	& 5	&     0.0001	&       \RBF	&      0.001	& 0.534	& 0.496	& 0.565	& 0.758 \\
150	& 5	&     0.0001	&       \RBF	&       0.01	& 0.250	& 0.272	& 0.522	& 0.573 \\
150	& 5	&      0.001	&       \LIN	&          -	& 0.407	& 0.393	& 0.535	& 0.727 \\
150	& 5	&      0.001	&       \RBF	&     0.0001	& 0.543	& 0.496	& 0.556	& 0.727 \\
150	& 5	&      0.001	&       \RBF	&      0.001	& 0.534	& 0.496	& 0.565	& 0.758 \\
150	& 5	&      0.001	&       \RBF	&       0.01	& 0.240	& 0.261	& 0.525	& 0.535 \\
150	& 5	&       0.01	&       \LIN	&          -	& 0.484	& 0.458	& 0.548	& 0.750 \\
150	& 5	&       0.01	&       \RBF	&     0.0001	& 0.543	& 0.496	& 0.556	& 0.727 \\
150	& 5	&       0.01	&       \RBF	&      0.001	& 0.534	& 0.496	& 0.565	& 0.758 \\
150	& 5	&       0.01	&       \RBF	&       0.01	& 0.200	& 0.223	& 0.524	& 0.503 \\
150	& 5	&        0.1	&       \LIN	&          -	& 0.488	& 0.432	& 0.543	& 0.749 \\
150	& 5	&        0.1	&       \RBF	&     0.0001	& 0.543	& 0.496	& 0.556	& 0.727 \\
150	& 5	&        0.1	&       \RBF	&      0.001	& 0.534	& 0.496	& 0.565	& 0.758 \\
150	& 5	&        0.1	&       \RBF	&       0.01	& 0.135	& 0.158	& 0.519	& 0.482 \\
150	& 5	&        0.2	&       \LIN	&          -	& 0.510	& 0.473	& 0.547	& 0.761 \\
150	& 5	&        0.2	&       \RBF	&     0.0001	& 0.543	& 0.496	& 0.556	& 0.727 \\
150	& 5	&        0.2	&       \RBF	&      0.001	& 0.534	& 0.496	& 0.565	& 0.758 \\
150	& 5	&        0.2	&       \RBF	&       0.01	& 0.110	& 0.134	& 0.520	& 0.478 \\
150	& 5	&        0.4	&       \LIN	&          -	& 0.519	& 0.466	& 0.546	& 0.759 \\
150	& 5	&        0.4	&       \RBF	&     0.0001	& 0.543	& 0.496	& 0.556	& 0.727 \\
150	& 5	&        0.4	&       \RBF	&      0.001	& 0.534	& 0.496	& 0.565	& 0.758 \\
150	& 5	&        0.4	&       \RBF	&       0.01	& 0.095	& 0.126	& 0.516	& 0.475 \\
150	& 5	&        0.6	&       \LIN	&          -	& 0.434	& 0.405	& 0.549	& 0.777 \\
150	& 5	&        0.6	&       \RBF	&     0.0001	& 0.543	& 0.496	& 0.556	& 0.727 \\
150	& 5	&        0.6	&       \RBF	&      0.001	& 0.534	& 0.496	& 0.565	& 0.758 \\
150	& 5	&        0.6	&       \RBF	&       0.01	& 0.088	& 0.119	& 0.516	& 0.473 \\
150	& 5	&        0.8	&       \LIN	&          -	& 0.526	& 0.474	& 0.549	& 0.772 \\
150	& 5	&        0.8	&       \RBF	&     0.0001	& 0.543	& 0.496	& 0.556	& 0.727 \\
150	& 5	&        0.8	&       \RBF	&      0.001	& 0.534	& 0.496	& 0.565	& 0.758 \\
150	& 5	&        0.8	&       \RBF	&       0.01	& 0.072	& 0.100	& 0.514	& 0.472 \\
150	& 5	&        1.0	&       \LIN	&          -	& 0.523	& 0.475	& 0.550	& 0.776 \\
150	& 5	&        1.0	&       \RBF	&     0.0001	& 0.543	& 0.496	& 0.556	& 0.727 \\
150	& 5	&        1.0	&       \RBF	&      0.001	& 0.534	& 0.496	& 0.565	& 0.758 \\
150	& 5	&        1.0	&       \RBF	&       0.01	& 0.079	& 0.107	& 0.514	& 0.472 \\
150	& 5	&         10	&       \LIN	&          -	& 0.537	& 0.504	& 0.543	& 0.779 \\
150	& 5	&         10	&       \RBF	&     0.0001	& 0.543	& 0.496	& 0.556	& 0.727 \\
150	& 5	&         10	&       \RBF	&      0.001	& 0.534	& 0.496	& 0.565	& 0.758 \\
150	& 5	&         10	&       \RBF	&       0.01	& 0.055	& 0.087	& 0.513	& 0.469 \\
150	& 5	&         50	&       \LIN	&          -	& 0.521	& 0.497	& 0.558	& 0.748 \\
150	& 5	&         50	&       \RBF	&     0.0001	& 0.543	& 0.496	& 0.556	& 0.727 \\
150	& 5	&         50	&       \RBF	&      0.001	& 0.534	& 0.496	& 0.565	& 0.758 \\
150	& 5	&         50	&       \RBF	&       0.01	& 0.056	& 0.088	& 0.512	& 0.468 \\
150	& 5	&        100	&       \LIN	&          -	& 0.513	& 0.478	& 0.555	& 0.683 \\
150	& 5	&        100	&       \RBF	&     0.0001	& 0.543	& 0.496	& 0.556	& 0.727 \\
150	& 5	&        100	&       \RBF	&      0.001	& 0.534	& 0.496	& 0.565	& 0.758 \\
150	& 5	&        100	&       \RBF	&       0.01	& 0.055	& 0.087	& 0.512	& 0.467 \\
150	& 10	&   0.000001	&       \LIN	&          -	& 0.367	& 0.341	& 0.526	& 0.700 \\
150	& 10	&   0.000001	&       \RBF	&       0.01	& 0.292	& 0.285	& 0.526	& 0.598 \\
150	& 10	&      0.001	&       \RBF	&     0.0001	& 0.542	& 0.500	& 0.557	& 0.771 \\
150	& 10	&      0.001	&       \RBF	&      0.001	& 0.537	& 0.495	& 0.564	& 0.773 \\
150	& 10	&      0.001	&       \RBF	&       0.01	& 0.234	& 0.262	& 0.523	& 0.546 \\
150	& 10	&       0.01	&       \LIN	&          -	& 0.454	& 0.428	& 0.548	& 0.760 \\
150	& 10	&       0.01	&       \RBF	&     0.0001	& 0.542	& 0.500	& 0.557	& 0.771 \\
150	& 10	&       0.01	&       \RBF	&      0.001	& 0.537	& 0.495	& 0.564	& 0.773 \\
150	& 10	&       0.01	&       \RBF	&       0.01	& 0.195	& 0.217	& 0.522	& 0.508 \\
150	& 10	&        0.1	&       \LIN	&          -	& 0.512	& 0.462	& 0.557	& 0.777 \\
150	& 10	&        0.1	&       \RBF	&     0.0001	& 0.542	& 0.500	& 0.557	& 0.771 \\
150	& 10	&        0.1	&       \RBF	&      0.001	& 0.537	& 0.495	& 0.564	& 0.773 \\
150	& 10	&        0.1	&       \RBF	&       0.01	& 0.146	& 0.166	& 0.518	& 0.484 \\
150	& 10	&        0.2	&       \LIN	&          -	& 0.553	& 0.498	& 0.558	& 0.773 \\
150	& 10	&        0.2	&       \RBF	&     0.0001	& 0.542	& 0.500	& 0.557	& 0.771 \\
150	& 10	&        0.2	&       \RBF	&      0.001	& 0.537	& 0.495	& 0.564	& 0.773 \\
150	& 10	&        0.2	&       \RBF	&       0.01	& 0.109	& 0.129	& 0.519	& 0.480 \\
150	& 10	&        0.4	&       \LIN	&          -	& 0.516	& 0.468	& 0.551	& 0.777 \\
150	& 10	&        0.4	&       \RBF	&     0.0001	& 0.542	& 0.500	& 0.557	& 0.771 \\
150	& 10	&        0.4	&       \RBF	&      0.001	& 0.537	& 0.495	& 0.564	& 0.773 \\
150	& 10	&        0.4	&       \RBF	&       0.01	& 0.102	& 0.131	& 0.517	& 0.476 \\
150	& 10	&        0.6	&       \LIN	&          -	& 0.518	& 0.485	& 0.553	& 0.777 \\
150	& 10	&        0.6	&       \RBF	&     0.0001	& 0.542	& 0.500	& 0.557	& 0.771 \\
150	& 10	&        0.6	&       \RBF	&      0.001	& 0.537	& 0.495	& 0.564	& 0.773 \\
150	& 10	&        0.6	&       \RBF	&       0.01	& 0.085	& 0.116	& 0.516	& 0.474 \\
150	& 10	&        0.8	&       \LIN	&          -	& 0.529	& 0.508	& 0.549	& 0.778 \\
150	& 10	&        0.8	&       \RBF	&     0.0001	& 0.542	& 0.500	& 0.557	& 0.771 \\
150	& 10	&        0.8	&       \RBF	&      0.001	& 0.537	& 0.495	& 0.564	& 0.773 \\
150	& 10	&        0.8	&       \RBF	&       0.01	& 0.070	& 0.102	& 0.515	& 0.473 \\
150	& 10	&        1.0	&       \LIN	&          -	& 0.565	& 0.524	& 0.550	& 0.782 \\
150	& 10	&        1.0	&       \RBF	&     0.0001	& 0.542	& 0.500	& 0.557	& 0.771 \\
150	& 10	&        1.0	&       \RBF	&      0.001	& 0.537	& 0.495	& 0.564	& 0.773 \\
150	& 10	&        1.0	&       \RBF	&       0.01	& 0.071	& 0.101	& 0.513	& 0.472 \\
150	& 10	&         10	&       \LIN	&          -	& 0.527	& 0.501	& 0.546	& 0.779 \\
150	& 10	&         10	&       \RBF	&     0.0001	& 0.542	& 0.500	& 0.557	& 0.771 \\
150	& 10	&         10	&       \RBF	&      0.001	& 0.537	& 0.495	& 0.564	& 0.773 \\
150	& 10	&         10	&       \RBF	&       0.01	& 0.058	& 0.091	& 0.513	& 0.469 \\
150	& 10	&         50	&       \LIN	&          -	& 0.511	& 0.493	& 0.555	& 0.764 \\
150	& 10	&         50	&       \RBF	&     0.0001	& 0.542	& 0.500	& 0.557	& 0.771 \\
150	& 10	&         50	&       \RBF	&      0.001	& 0.537	& 0.495	& 0.564	& 0.773 \\
150	& 10	&         50	&       \RBF	&       0.01	& 0.057	& 0.089	& 0.512	& 0.468 \\
150	& 10	&        100	&       \LIN	&          -	& 0.529	& 0.487	& 0.555	& 0.695 \\
150	& 10	&        100	&       \RBF	&     0.0001	& 0.542	& 0.500	& 0.557	& 0.771 \\
150	& 10	&        100	&       \RBF	&      0.001	& 0.537	& 0.495	& 0.564	& 0.773 \\
150	& 10	&        100	&       \RBF	&       0.01	& 0.056	& 0.088	& 0.512	& 0.467 \\
150	& 15	&      0.001	&       \LIN	&          -	& 0.398	& 0.407	& 0.547	& 0.719 \\
150	& 15	&      0.001	&       \RBF	&     0.0001	& 0.538	& 0.492	& 0.557	& 0.779 \\
150	& 15	&      0.001	&       \RBF	&      0.001	& 0.539	& 0.493	& 0.561	& 0.772 \\
150	& 15	&      0.001	&       \RBF	&       0.01	& 0.259	& 0.278	& 0.522	& 0.549 \\
150	& 15	&       0.01	&       \LIN	&          -	& 0.444	& 0.416	& 0.556	& 0.764 \\
150	& 15	&       0.01	&       \RBF	&     0.0001	& 0.538	& 0.492	& 0.557	& 0.779 \\
150	& 15	&       0.01	&       \RBF	&      0.001	& 0.539	& 0.493	& 0.561	& 0.772 \\
150	& 15	&       0.01	&       \RBF	&       0.01	& 0.201	& 0.218	& 0.521	& 0.510 \\
150	& 15	&        0.1	&       \LIN	&          -	& 0.550	& 0.498	& 0.559	& 0.776 \\
150	& 15	&        0.1	&       \RBF	&     0.0001	& 0.538	& 0.492	& 0.557	& 0.779 \\
150	& 15	&        0.1	&       \RBF	&      0.001	& 0.539	& 0.493	& 0.561	& 0.772 \\
150	& 15	&        0.1	&       \RBF	&       0.01	& 0.147	& 0.164	& 0.518	& 0.485 \\
150	& 15	&        0.2	&       \LIN	&          -	& 0.540	& 0.505	& 0.556	& 0.777 \\
150	& 15	&        0.2	&       \RBF	&     0.0001	& 0.538	& 0.492	& 0.557	& 0.779 \\
150	& 15	&        0.2	&       \RBF	&      0.001	& 0.539	& 0.493	& 0.561	& 0.772 \\
150	& 15	&        0.2	&       \RBF	&       0.01	& 0.116	& 0.139	& 0.519	& 0.480 \\
150	& 15	&        0.4	&       \LIN	&          -	& 0.540	& 0.509	& 0.556	& 0.777 \\
150	& 15	&        0.4	&       \RBF	&     0.0001	& 0.538	& 0.492	& 0.557	& 0.779 \\
150	& 15	&        0.4	&       \RBF	&      0.001	& 0.539	& 0.493	& 0.561	& 0.772 \\
150	& 15	&        0.4	&       \RBF	&       0.01	& 0.108	& 0.134	& 0.516	& 0.476 \\
150	& 15	&        0.6	&       \LIN	&          -	& 0.544	& 0.508	& 0.554	& 0.780 \\
150	& 15	&        0.6	&       \RBF	&     0.0001	& 0.538	& 0.492	& 0.557	& 0.779 \\
150	& 15	&        0.6	&       \RBF	&      0.001	& 0.539	& 0.493	& 0.561	& 0.772 \\
150	& 15	&        0.6	&       \RBF	&       0.01	& 0.087	& 0.119	& 0.516	& 0.474 \\
150	& 15	&        0.8	&       \LIN	&          -	& 0.558	& 0.522	& 0.553	& 0.781 \\
150	& 15	&        0.8	&       \RBF	&     0.0001	& 0.538	& 0.492	& 0.557	& 0.779 \\
150	& 15	&        0.8	&       \RBF	&      0.001	& 0.539	& 0.493	& 0.561	& 0.772 \\
150	& 15	&        0.8	&       \RBF	&       0.01	& 0.078	& 0.108	& 0.515	& 0.473 \\
150	& 15	&        1.0	&       \LIN	&          -	& 0.544	& 0.506	& 0.555	& 0.782 \\
150	& 15	&        1.0	&       \RBF	&     0.0001	& 0.538	& 0.492	& 0.557	& 0.779 \\
150	& 15	&        1.0	&       \RBF	&      0.001	& 0.539	& 0.493	& 0.561	& 0.772 \\
150	& 15	&        1.0	&       \RBF	&       0.01	& 0.073	& 0.101	& 0.514	& 0.473 \\
150	& 15	&         10	&       \LIN	&          -	& 0.530	& 0.485	& 0.549	& 0.783 \\
150	& 15	&         10	&       \RBF	&     0.0001	& 0.538	& 0.492	& 0.557	& 0.779 \\
150	& 15	&         10	&       \RBF	&      0.001	& 0.539	& 0.493	& 0.561	& 0.772 \\
150	& 15	&         10	&       \RBF	&       0.01	& 0.058	& 0.091	& 0.513	& 0.469 \\
150	& 15	&         50	&       \LIN	&          -	& 0.521	& 0.494	& 0.553	& 0.770 \\
150	& 15	&         50	&       \RBF	&     0.0001	& 0.538	& 0.492	& 0.557	& 0.779 \\
150	& 15	&         50	&       \RBF	&      0.001	& 0.539	& 0.493	& 0.561	& 0.772 \\
150	& 15	&         50	&       \RBF	&       0.01	& 0.055	& 0.087	& 0.512	& 0.468 \\
150	& 15	&        100	&       \LIN	&          -	& 0.525	& 0.486	& 0.553	& 0.730 \\
150	& 15	&        100	&       \RBF	&     0.0001	& 0.538	& 0.492	& 0.557	& 0.779 \\
150	& 15	&        100	&       \RBF	&      0.001	& 0.539	& 0.493	& 0.561	& 0.772 \\
150	& 15	&        100	&       \RBF	&       0.01	& 0.058	& 0.089	& 0.512	& 0.468 \\
200	& 5	&   0.000001	&       \LIN	&          -	& 0.322	& 0.328	& 0.521	& 0.703 \\
200	& 5	&   0.000001	&       \RBF	&     0.0001	& 0.490	& 0.458	& 0.532	& 0.729 \\
200	& 5	&   0.000001	&       \RBF	&      0.001	& 0.464	& 0.445	& 0.546	& 0.728 \\
200	& 5	&   0.000001	&       \RBF	&       0.01	& 0.299	& 0.300	& 0.528	& 0.597 \\
200	& 5	&    0.00001	&       \RBF	&      0.001	& 0.520	& 0.488	& 0.557	& 0.756 \\
200	& 5	&    0.00001	&       \RBF	&       0.01	& 0.271	& 0.295	& 0.524	& 0.596 \\
200	& 5	&     0.0001	&       \RBF	&     0.0001	& 0.515	& 0.475	& 0.550	& 0.774 \\
200	& 5	&     0.0001	&       \RBF	&      0.001	& 0.520	& 0.488	& 0.557	& 0.756 \\
200	& 5	&     0.0001	&       \RBF	&       0.01	& 0.262	& 0.284	& 0.526	& 0.564 \\
200	& 5	&      0.001	&       \LIN	&          -	& 0.440	& 0.420	& 0.535	& 0.722 \\
200	& 5	&      0.001	&       \RBF	&     0.0001	& 0.528	& 0.495	& 0.551	& 0.729 \\
200	& 5	&      0.001	&       \RBF	&      0.001	& 0.520	& 0.488	& 0.557	& 0.756 \\
200	& 5	&      0.001	&       \RBF	&       0.01	& 0.241	& 0.261	& 0.527	& 0.530 \\
200	& 5	&       0.01	&       \LIN	&          -	& 0.469	& 0.457	& 0.542	& 0.746 \\
200	& 5	&       0.01	&       \RBF	&     0.0001	& 0.528	& 0.495	& 0.551	& 0.729 \\
200	& 5	&       0.01	&       \RBF	&      0.001	& 0.520	& 0.488	& 0.557	& 0.756 \\
200	& 5	&       0.01	&       \RBF	&       0.01	& 0.185	& 0.206	& 0.522	& 0.500 \\
200	& 5	&        0.1	&       \LIN	&          -	& 0.487	& 0.466	& 0.544	& 0.756 \\
200	& 5	&        0.1	&       \RBF	&     0.0001	& 0.528	& 0.495	& 0.551	& 0.729 \\
200	& 5	&        0.1	&       \RBF	&      0.001	& 0.520	& 0.488	& 0.557	& 0.756 \\
200	& 5	&        0.1	&       \RBF	&       0.01	& 0.124	& 0.149	& 0.521	& 0.481 \\
200	& 5	&        0.2	&       \LIN	&          -	& 0.520	& 0.463	& 0.543	& 0.769 \\
200	& 5	&        0.2	&       \RBF	&     0.0001	& 0.528	& 0.495	& 0.551	& 0.729 \\
200	& 5	&        0.2	&       \RBF	&      0.001	& 0.520	& 0.488	& 0.557	& 0.756 \\
200	& 5	&        0.2	&       \RBF	&       0.01	& 0.106	& 0.135	& 0.518	& 0.477 \\
200	& 5	&        0.4	&       \LIN	&          -	& 0.499	& 0.475	& 0.546	& 0.767 \\
200	& 5	&        0.4	&       \RBF	&     0.0001	& 0.528	& 0.495	& 0.551	& 0.729 \\
200	& 5	&        0.4	&       \RBF	&      0.001	& 0.520	& 0.488	& 0.557	& 0.756 \\
200	& 5	&        0.4	&       \RBF	&       0.01	& 0.094	& 0.126	& 0.516	& 0.475 \\
200	& 5	&        0.6	&       \LIN	&          -	& 0.530	& 0.487	& 0.544	& 0.754 \\
200	& 5	&        0.6	&       \RBF	&     0.0001	& 0.528	& 0.495	& 0.551	& 0.729 \\
200	& 5	&        0.6	&       \RBF	&      0.001	& 0.520	& 0.488	& 0.557	& 0.756 \\
200	& 5	&        0.6	&       \RBF	&       0.01	& 0.075	& 0.108	& 0.516	& 0.473 \\
200	& 5	&        0.8	&       \LIN	&          -	& 0.497	& 0.460	& 0.547	& 0.761 \\
200	& 5	&        0.8	&       \RBF	&     0.0001	& 0.528	& 0.495	& 0.551	& 0.729 \\
200	& 5	&        0.8	&       \RBF	&      0.001	& 0.520	& 0.488	& 0.557	& 0.756 \\
200	& 5	&        0.8	&       \RBF	&       0.01	& 0.079	& 0.110	& 0.514	& 0.472 \\
200	& 5	&        1.0	&       \LIN	&          -	& 0.518	& 0.472	& 0.543	& 0.757 \\
200	& 5	&        1.0	&       \RBF	&     0.0001	& 0.528	& 0.495	& 0.551	& 0.729 \\
200	& 5	&        1.0	&       \RBF	&      0.001	& 0.520	& 0.488	& 0.557	& 0.756 \\
200	& 5	&        1.0	&       \RBF	&       0.01	& 0.068	& 0.100	& 0.514	& 0.472 \\
200	& 5	&         10	&       \LIN	&          -	& 0.533	& 0.500	& 0.543	& 0.779 \\
200	& 5	&         10	&       \RBF	&     0.0001	& 0.528	& 0.495	& 0.551	& 0.729 \\
200	& 5	&         10	&       \RBF	&      0.001	& 0.520	& 0.488	& 0.557	& 0.756 \\
200	& 5	&         10	&       \RBF	&       0.01	& 0.055	& 0.088	& 0.514	& 0.469 \\
200	& 5	&         50	&       \LIN	&          -	& 0.533	& 0.505	& 0.554	& 0.744 \\
200	& 5	&         50	&       \RBF	&     0.0001	& 0.528	& 0.495	& 0.551	& 0.729 \\
200	& 5	&         50	&       \RBF	&      0.001	& 0.520	& 0.487	& 0.557	& 0.756 \\
200	& 5	&         50	&       \RBF	&       0.01	& 0.051	& 0.084	& 0.513	& 0.468 \\
200	& 5	&        100	&       \LIN	&          -	& 0.529	& 0.491	& 0.550	& 0.668 \\
200	& 5	&        100	&       \RBF	&     0.0001	& 0.528	& 0.495	& 0.551	& 0.729 \\
200	& 5	&        100	&       \RBF	&      0.001	& 0.520	& 0.487	& 0.557	& 0.756 \\
200	& 5	&        100	&       \RBF	&       0.01	& 0.055	& 0.088	& 0.513	& 0.468 \\
200	& 10	&   0.000001	&       \LIN	&          -	& 0.233	& 0.249	& 0.518	& 0.703 \\
200	& 10	&   0.000001	&       \RBF	&       0.01	& 0.297	& 0.299	& 0.526	& 0.590 \\
200	& 10	&      0.001	&       \RBF	&     0.0001	& 0.533	& 0.495	& 0.552	& 0.769 \\
200	& 10	&      0.001	&       \RBF	&      0.001	& 0.522	& 0.493	& 0.556	& 0.770 \\
200	& 10	&      0.001	&       \RBF	&       0.01	& 0.233	& 0.254	& 0.522	& 0.539 \\
200	& 10	&       0.01	&       \LIN	&          -	& 0.439	& 0.418	& 0.543	& 0.764 \\
200	& 10	&       0.01	&       \RBF	&     0.0001	& 0.533	& 0.495	& 0.552	& 0.769 \\
200	& 10	&       0.01	&       \RBF	&      0.001	& 0.522	& 0.493	& 0.556	& 0.770 \\
200	& 10	&       0.01	&       \RBF	&       0.01	& 0.194	& 0.211	& 0.521	& 0.506 \\
200	& 10	&        0.1	&       \LIN	&          -	& 0.500	& 0.471	& 0.548	& 0.773 \\
200	& 10	&        0.1	&       \RBF	&     0.0001	& 0.533	& 0.495	& 0.552	& 0.769 \\
200	& 10	&        0.1	&       \RBF	&      0.001	& 0.522	& 0.493	& 0.556	& 0.770 \\
200	& 10	&        0.1	&       \RBF	&       0.01	& 0.127	& 0.151	& 0.519	& 0.483 \\
200	& 10	&        0.2	&       \LIN	&          -	& 0.523	& 0.486	& 0.554	& 0.773 \\
200	& 10	&        0.2	&       \RBF	&     0.0001	& 0.533	& 0.495	& 0.552	& 0.769 \\
200	& 10	&        0.2	&       \RBF	&      0.001	& 0.522	& 0.493	& 0.556	& 0.770 \\
200	& 10	&        0.2	&       \RBF	&       0.01	& 0.115	& 0.141	& 0.518	& 0.479 \\
200	& 10	&        0.4	&       \LIN	&          -	& 0.502	& 0.473	& 0.548	& 0.782 \\
200	& 10	&        0.4	&       \RBF	&     0.0001	& 0.533	& 0.495	& 0.552	& 0.769 \\
200	& 10	&        0.4	&       \RBF	&      0.001	& 0.522	& 0.493	& 0.556	& 0.770 \\
200	& 10	&        0.4	&       \RBF	&       0.01	& 0.095	& 0.127	& 0.516	& 0.476 \\
200	& 10	&        0.6	&       \LIN	&          -	& 0.484	& 0.458	& 0.547	& 0.779 \\
200	& 10	&        0.6	&       \RBF	&     0.0001	& 0.533	& 0.495	& 0.552	& 0.769 \\
200	& 10	&        0.6	&       \RBF	&      0.001	& 0.522	& 0.493	& 0.556	& 0.770 \\
200	& 10	&        0.6	&       \RBF	&       0.01	& 0.079	& 0.109	& 0.515	& 0.474 \\
200	& 10	&        0.8	&       \LIN	&          -	& 0.495	& 0.474	& 0.548	& 0.783 \\
200	& 10	&        0.8	&       \RBF	&     0.0001	& 0.533	& 0.495	& 0.552	& 0.769 \\
200	& 10	&        0.8	&       \RBF	&      0.001	& 0.522	& 0.493	& 0.556	& 0.770 \\
200	& 10	&        0.8	&       \RBF	&       0.01	& 0.078	& 0.110	& 0.515	& 0.473 \\
200	& 10	&        1.0	&       \LIN	&          -	& 0.514	& 0.488	& 0.547	& 0.781 \\
200	& 10	&        1.0	&       \RBF	&     0.0001	& 0.533	& 0.495	& 0.552	& 0.769 \\
200	& 10	&        1.0	&       \RBF	&      0.001	& 0.522	& 0.493	& 0.556	& 0.770 \\
200	& 10	&        1.0	&       \RBF	&       0.01	& 0.070	& 0.099	& 0.515	& 0.473 \\
200	& 10	&         10	&       \LIN	&          -	& 0.536	& 0.503	& 0.546	& 0.762 \\
200	& 10	&         10	&       \RBF	&     0.0001	& 0.533	& 0.495	& 0.552	& 0.769 \\
200	& 10	&         10	&       \RBF	&      0.001	& 0.522	& 0.493	& 0.556	& 0.770 \\
200	& 10	&         10	&       \RBF	&       0.01	& 0.055	& 0.088	& 0.514	& 0.469 \\
200	& 10	&         50	&       \LIN	&          -	& 0.542	& 0.511	& 0.551	& 0.760 \\
200	& 10	&         50	&       \RBF	&     0.0001	& 0.533	& 0.495	& 0.552	& 0.769 \\
200	& 10	&         50	&       \RBF	&      0.001	& 0.522	& 0.493	& 0.556	& 0.770 \\
200	& 10	&         50	&       \RBF	&       0.01	& 0.052	& 0.086	& 0.513	& 0.468 \\
200	& 10	&        100	&       \LIN	&          -	& 0.529	& 0.491	& 0.550	& 0.686 \\
200	& 10	&        100	&       \RBF	&     0.0001	& 0.533	& 0.495	& 0.552	& 0.769 \\
200	& 10	&        100	&       \RBF	&      0.001	& 0.522	& 0.493	& 0.556	& 0.770 \\
200	& 10	&        100	&       \RBF	&       0.01	& 0.056	& 0.088	& 0.513	& 0.468 \\
200	& 15	&      0.001	&       \LIN	&          -	& 0.373	& 0.361	& 0.532	& 0.703 \\
200	& 15	&      0.001	&       \RBF	&     0.0001	& 0.537	& 0.496	& 0.552	& 0.777 \\
200	& 15	&      0.001	&       \RBF	&      0.001	& 0.540	& 0.506	& 0.554	& 0.770 \\
200	& 15	&      0.001	&       \RBF	&       0.01	& 0.240	& 0.259	& 0.522	& 0.543 \\
200	& 15	&       0.01	&       \RBF	&     0.0001	& 0.537	& 0.496	& 0.552	& 0.777 \\
200	& 15	&       0.01	&       \RBF	&      0.001	& 0.540	& 0.506	& 0.554	& 0.770 \\
200	& 15	&       0.01	&       \RBF	&       0.01	& 0.188	& 0.206	& 0.520	& 0.508 \\
200	& 15	&        0.1	&       \LIN	&          -	& 0.505	& 0.478	& 0.553	& 0.775 \\
200	& 15	&        0.1	&       \RBF	&     0.0001	& 0.537	& 0.496	& 0.552	& 0.777 \\
200	& 15	&        0.1	&       \RBF	&      0.001	& 0.540	& 0.506	& 0.554	& 0.770 \\
200	& 15	&        0.1	&       \RBF	&       0.01	& 0.129	& 0.157	& 0.518	& 0.485 \\
200	& 15	&        0.2	&       \LIN	&          -	& 0.534	& 0.503	& 0.553	& 0.775 \\
200	& 15	&        0.2	&       \RBF	&     0.0001	& 0.537	& 0.496	& 0.552	& 0.777 \\
200	& 15	&        0.2	&       \RBF	&      0.001	& 0.540	& 0.506	& 0.554	& 0.770 \\
200	& 15	&        0.2	&       \RBF	&       0.01	& 0.115	& 0.140	& 0.519	& 0.480 \\
200	& 15	&        0.4	&       \LIN	&          -	& 0.515	& 0.494	& 0.553	& 0.777 \\
200	& 15	&        0.4	&       \RBF	&     0.0001	& 0.537	& 0.496	& 0.552	& 0.777 \\
200	& 15	&        0.4	&       \RBF	&      0.001	& 0.540	& 0.506	& 0.554	& 0.770 \\
200	& 15	&        0.4	&       \RBF	&       0.01	& 0.103	& 0.130	& 0.516	& 0.477 \\
200	& 15	&        0.6	&       \LIN	&          -	& 0.527	& 0.507	& 0.553	& 0.779 \\
200	& 15	&        0.6	&       \RBF	&     0.0001	& 0.537	& 0.496	& 0.552	& 0.777 \\
200	& 15	&        0.6	&       \RBF	&      0.001	& 0.540	& 0.506	& 0.554	& 0.770 \\
200	& 15	&        0.6	&       \RBF	&       0.01	& 0.084	& 0.113	& 0.515	& 0.475 \\
200	& 15	&        0.8	&       \LIN	&          -	& 0.511	& 0.489	& 0.552	& 0.780 \\
200	& 15	&        0.8	&       \RBF	&     0.0001	& 0.537	& 0.496	& 0.552	& 0.777 \\
200	& 15	&        0.8	&       \RBF	&      0.001	& 0.540	& 0.506	& 0.554	& 0.770 \\
200	& 15	&        0.8	&       \RBF	&       0.01	& 0.079	& 0.110	& 0.515	& 0.474 \\
200	& 15	&        1.0	&       \LIN	&          -	& 0.545	& 0.501	& 0.553	& 0.780 \\
200	& 15	&        1.0	&       \RBF	&     0.0001	& 0.537	& 0.496	& 0.552	& 0.777 \\
200	& 15	&        1.0	&       \RBF	&      0.001	& 0.540	& 0.506	& 0.554	& 0.770 \\
200	& 15	&        1.0	&       \RBF	&       0.01	& 0.074	& 0.102	& 0.514	& 0.473 \\
200	& 15	&         10	&       \LIN	&          -	& 0.536	& 0.514	& 0.548	& 0.785 \\
200	& 15	&         10	&       \RBF	&     0.0001	& 0.537	& 0.496	& 0.552	& 0.777 \\
200	& 15	&         10	&       \RBF	&      0.001	& 0.540	& 0.506	& 0.554	& 0.770 \\
200	& 15	&         10	&       \RBF	&       0.01	& 0.057	& 0.089	& 0.514	& 0.470 \\
200	& 15	&         50	&       \LIN	&          -	& 0.535	& 0.514	& 0.550	& 0.768 \\
200	& 15	&         50	&       \RBF	&     0.0001	& 0.537	& 0.496	& 0.552	& 0.777 \\
200	& 15	&         50	&       \RBF	&      0.001	& 0.540	& 0.506	& 0.554	& 0.770 \\
200	& 15	&         50	&       \RBF	&       0.01	& 0.052	& 0.086	& 0.513	& 0.468 \\
200	& 15	&        100	&       \LIN	&          -	& 0.528	& 0.492	& 0.550	& 0.724 \\
200	& 15	&        100	&       \RBF	&     0.0001	& 0.537	& 0.496	& 0.552	& 0.777 \\
200	& 15	&        100	&       \RBF	&      0.001	& 0.540	& 0.506	& 0.554	& 0.770 \\
200	& 15	&        100	&       \RBF	&       0.01	& 0.062	& 0.093	& 0.513	& 0.468 \\
250	& 5	&   0.000001	&       \RBF	&     0.0001	& 0.473	& 0.442	& 0.538	& 0.728 \\
250	& 5	&   0.000001	&       \RBF	&      0.001	& 0.499	& 0.467	& 0.549	& 0.722 \\
250	& 5	&   0.000001	&       \RBF	&       0.01	& 0.317	& 0.320	& 0.525	& 0.590 \\
250	& 5	&    0.00001	&       \LIN	&          -	& 0.195	& 0.231	& 0.538	& 0.671 \\
250	& 5	&    0.00001	&       \RBF	&     0.0001	& 0.523	& 0.489	& 0.535	& 0.757 \\
250	& 5	&    0.00001	&       \RBF	&      0.001	& 0.553	& 0.516	& 0.560	& 0.758 \\
250	& 5	&    0.00001	&       \RBF	&       0.01	& 0.294	& 0.302	& 0.527	& 0.587 \\
250	& 5	&     0.0001	&       \RBF	&     0.0001	& 0.513	& 0.467	& 0.550	& 0.775 \\
250	& 5	&     0.0001	&       \RBF	&      0.001	& 0.553	& 0.516	& 0.560	& 0.758 \\
250	& 5	&     0.0001	&       \RBF	&       0.01	& 0.269	& 0.277	& 0.523	& 0.556 \\
250	& 5	&      0.001	&       \LIN	&          -	& 0.393	& 0.380	& 0.542	& 0.723 \\
250	& 5	&      0.001	&       \RBF	&     0.0001	& 0.536	& 0.501	& 0.552	& 0.730 \\
250	& 5	&      0.001	&       \RBF	&      0.001	& 0.553	& 0.516	& 0.560	& 0.758 \\
250	& 5	&      0.001	&       \RBF	&       0.01	& 0.241	& 0.254	& 0.520	& 0.525 \\
250	& 5	&       0.01	&       \LIN	&          -	& 0.493	& 0.466	& 0.549	& 0.749 \\
250	& 5	&       0.01	&       \RBF	&     0.0001	& 0.536	& 0.501	& 0.552	& 0.730 \\
250	& 5	&       0.01	&       \RBF	&      0.001	& 0.553	& 0.516	& 0.560	& 0.758 \\
250	& 5	&       0.01	&       \RBF	&       0.01	& 0.180	& 0.201	& 0.517	& 0.498 \\
250	& 5	&        0.1	&       \LIN	&          -	& 0.475	& 0.447	& 0.541	& 0.764 \\
250	& 5	&        0.1	&       \RBF	&     0.0001	& 0.536	& 0.501	& 0.552	& 0.730 \\
250	& 5	&        0.1	&       \RBF	&      0.001	& 0.553	& 0.516	& 0.560	& 0.758 \\
250	& 5	&        0.1	&       \RBF	&       0.01	& 0.138	& 0.163	& 0.516	& 0.482 \\
250	& 5	&        0.2	&       \LIN	&          -	& 0.460	& 0.431	& 0.546	& 0.771 \\
250	& 5	&        0.2	&       \RBF	&     0.0001	& 0.536	& 0.501	& 0.552	& 0.730 \\
250	& 5	&        0.2	&       \RBF	&      0.001	& 0.553	& 0.516	& 0.560	& 0.758 \\
250	& 5	&        0.2	&       \RBF	&       0.01	& 0.114	& 0.140	& 0.514	& 0.479 \\
250	& 5	&        0.4	&       \LIN	&          -	& 0.512	& 0.472	& 0.545	& 0.772 \\
250	& 5	&        0.4	&       \RBF	&     0.0001	& 0.536	& 0.501	& 0.552	& 0.730 \\
250	& 5	&        0.4	&       \RBF	&      0.001	& 0.553	& 0.516	& 0.560	& 0.758 \\
250	& 5	&        0.4	&       \RBF	&       0.01	& 0.106	& 0.134	& 0.513	& 0.475 \\
250	& 5	&        0.6	&       \LIN	&          -	& 0.518	& 0.484	& 0.543	& 0.767 \\
250	& 5	&        0.6	&       \RBF	&     0.0001	& 0.536	& 0.501	& 0.552	& 0.730 \\
250	& 5	&        0.6	&       \RBF	&      0.001	& 0.553	& 0.516	& 0.560	& 0.758 \\
250	& 5	&        0.6	&       \RBF	&       0.01	& 0.092	& 0.122	& 0.512	& 0.474 \\
250	& 5	&        0.8	&       \LIN	&          -	& 0.514	& 0.472	& 0.549	& 0.766 \\
250	& 5	&        0.8	&       \RBF	&     0.0001	& 0.536	& 0.501	& 0.552	& 0.730 \\
250	& 5	&        0.8	&       \RBF	&      0.001	& 0.553	& 0.516	& 0.560	& 0.758 \\
250	& 5	&        0.8	&       \RBF	&       0.01	& 0.078	& 0.111	& 0.512	& 0.473 \\
250	& 5	&        1.0	&       \LIN	&          -	& 0.506	& 0.475	& 0.547	& 0.760 \\
250	& 5	&        1.0	&       \RBF	&     0.0001	& 0.536	& 0.501	& 0.552	& 0.730 \\
250	& 5	&        1.0	&       \RBF	&      0.001	& 0.553	& 0.516	& 0.560	& 0.758 \\
250	& 5	&        1.0	&       \RBF	&       0.01	& 0.080	& 0.110	& 0.511	& 0.473 \\
250	& 5	&         10	&       \LIN	&          -	& 0.561	& 0.520	& 0.547	& 0.777 \\
250	& 5	&         10	&       \RBF	&     0.0001	& 0.536	& 0.501	& 0.552	& 0.730 \\
250	& 5	&         10	&       \RBF	&      0.001	& 0.553	& 0.516	& 0.560	& 0.758 \\
250	& 5	&         10	&       \RBF	&       0.01	& 0.058	& 0.092	& 0.510	& 0.470 \\
250	& 5	&         50	&       \LIN	&          -	& 0.534	& 0.502	& 0.554	& 0.737 \\
250	& 5	&         50	&       \RBF	&     0.0001	& 0.536	& 0.501	& 0.552	& 0.730 \\
250	& 5	&         50	&       \RBF	&      0.001	& 0.553	& 0.516	& 0.560	& 0.758 \\
250	& 5	&         50	&       \RBF	&       0.01	& 0.051	& 0.086	& 0.509	& 0.469 \\
250	& 5	&        100	&       \LIN	&          -	& 0.527	& 0.493	& 0.552	& 0.656 \\
250	& 5	&        100	&       \RBF	&     0.0001	& 0.536	& 0.501	& 0.552	& 0.730 \\
250	& 5	&        100	&       \RBF	&      0.001	& 0.553	& 0.516	& 0.560	& 0.758 \\
250	& 5	&        100	&       \RBF	&       0.01	& 0.045	& 0.079	& 0.510	& 0.469 \\
250	& 10	&   0.000001	&       \LIN	&          -	& 0.334	& 0.325	& 0.516	& 0.685 \\
250	& 10	&   0.000001	&       \RBF	&       0.01	& 0.311	& 0.317	& 0.525	& 0.583 \\
250	& 10	&      0.001	&       \LIN	&          -	& 0.371	& 0.365	& 0.544	& 0.719 \\
250	& 10	&      0.001	&       \RBF	&     0.0001	& 0.537	& 0.506	& 0.554	& 0.769 \\
250	& 10	&      0.001	&       \RBF	&      0.001	& 0.554	& 0.514	& 0.557	& 0.770 \\
250	& 10	&      0.001	&       \RBF	&       0.01	& 0.238	& 0.253	& 0.521	& 0.533 \\
250	& 10	&       0.01	&       \LIN	&          -	& 0.419	& 0.397	& 0.546	& 0.762 \\
250	& 10	&       0.01	&       \RBF	&     0.0001	& 0.537	& 0.506	& 0.554	& 0.769 \\
250	& 10	&       0.01	&       \RBF	&      0.001	& 0.554	& 0.514	& 0.557	& 0.770 \\
250	& 10	&       0.01	&       \RBF	&       0.01	& 0.177	& 0.197	& 0.518	& 0.503 \\
250	& 10	&        0.1	&       \LIN	&          -	& 0.519	& 0.474	& 0.551	& 0.777 \\
250	& 10	&        0.1	&       \RBF	&     0.0001	& 0.537	& 0.506	& 0.554	& 0.769 \\
250	& 10	&        0.1	&       \RBF	&      0.001	& 0.554	& 0.514	& 0.557	& 0.770 \\
250	& 10	&        0.1	&       \RBF	&       0.01	& 0.148	& 0.170	& 0.515	& 0.485 \\
250	& 10	&        0.2	&       \LIN	&          -	& 0.481	& 0.442	& 0.553	& 0.778 \\
250	& 10	&        0.2	&       \RBF	&     0.0001	& 0.537	& 0.506	& 0.554	& 0.769 \\
250	& 10	&        0.2	&       \RBF	&      0.001	& 0.554	& 0.514	& 0.557	& 0.770 \\
250	& 10	&        0.2	&       \RBF	&       0.01	& 0.122	& 0.149	& 0.515	& 0.481 \\
250	& 10	&        0.4	&       \LIN	&          -	& 0.562	& 0.505	& 0.552	& 0.778 \\
250	& 10	&        0.4	&       \RBF	&     0.0001	& 0.537	& 0.506	& 0.554	& 0.769 \\
250	& 10	&        0.4	&       \RBF	&      0.001	& 0.554	& 0.514	& 0.557	& 0.770 \\
250	& 10	&        0.4	&       \RBF	&       0.01	& 0.104	& 0.133	& 0.513	& 0.477 \\
250	& 10	&        0.6	&       \LIN	&          -	& 0.497	& 0.456	& 0.554	& 0.780 \\
250	& 10	&        0.6	&       \RBF	&     0.0001	& 0.537	& 0.506	& 0.554	& 0.769 \\
250	& 10	&        0.6	&       \RBF	&      0.001	& 0.554	& 0.514	& 0.557	& 0.770 \\
250	& 10	&        0.6	&       \RBF	&       0.01	& 0.095	& 0.122	& 0.512	& 0.475 \\
250	& 10	&        0.8	&       \LIN	&          -	& 0.511	& 0.486	& 0.553	& 0.782 \\
250	& 10	&        0.8	&       \RBF	&     0.0001	& 0.537	& 0.506	& 0.554	& 0.769 \\
250	& 10	&        0.8	&       \RBF	&      0.001	& 0.554	& 0.514	& 0.557	& 0.770 \\
250	& 10	&        0.8	&       \RBF	&       0.01	& 0.091	& 0.119	& 0.512	& 0.474 \\
250	& 10	&        1.0	&       \LIN	&          -	& 0.547	& 0.484	& 0.550	& 0.779 \\
250	& 10	&        1.0	&       \RBF	&     0.0001	& 0.537	& 0.506	& 0.554	& 0.769 \\
250	& 10	&        1.0	&       \RBF	&      0.001	& 0.554	& 0.514	& 0.557	& 0.770 \\
250	& 10	&        1.0	&       \RBF	&       0.01	& 0.075	& 0.108	& 0.512	& 0.474 \\
250	& 10	&         10	&       \LIN	&          -	& 0.560	& 0.537	& 0.548	& 0.784 \\
250	& 10	&         10	&       \RBF	&     0.0001	& 0.537	& 0.506	& 0.554	& 0.769 \\
250	& 10	&         10	&       \RBF	&      0.001	& 0.554	& 0.514	& 0.557	& 0.770 \\
250	& 10	&         10	&       \RBF	&       0.01	& 0.058	& 0.092	& 0.510	& 0.470 \\
250	& 10	&         50	&       \LIN	&          -	& 0.537	& 0.508	& 0.552	& 0.753 \\
250	& 10	&         50	&       \RBF	&     0.0001	& 0.537	& 0.506	& 0.554	& 0.769 \\
250	& 10	&         50	&       \RBF	&      0.001	& 0.554	& 0.514	& 0.557	& 0.770 \\
250	& 10	&         50	&       \RBF	&       0.01	& 0.051	& 0.085	& 0.510	& 0.469 \\
250	& 10	&        100	&       \LIN	&          -	& 0.532	& 0.496	& 0.555	& 0.687 \\
250	& 10	&        100	&       \RBF	&     0.0001	& 0.537	& 0.506	& 0.554	& 0.769 \\
250	& 10	&        100	&       \RBF	&      0.001	& 0.554	& 0.514	& 0.557	& 0.770 \\
250	& 10	&        100	&       \RBF	&       0.01	& 0.045	& 0.078	& 0.510	& 0.469 \\
250	& 15	&      0.001	&       \LIN	&          -	& 0.358	& 0.353	& 0.534	& 0.702 \\
250	& 15	&      0.001	&       \RBF	&     0.0001	& 0.546	& 0.509	& 0.553	& 0.776 \\
250	& 15	&      0.001	&       \RBF	&      0.001	& 0.551	& 0.512	& 0.555	& 0.769 \\
250	& 15	&      0.001	&       \RBF	&       0.01	& 0.234	& 0.250	& 0.519	& 0.536 \\
250	& 15	&       0.01	&       \LIN	&          -	& 0.382	& 0.374	& 0.519	& 0.675 \\
250	& 15	&       0.01	&       \RBF	&     0.0001	& 0.546	& 0.509	& 0.553	& 0.776 \\
250	& 15	&       0.01	&       \RBF	&      0.001	& 0.551	& 0.512	& 0.555	& 0.769 \\
250	& 15	&       0.01	&       \RBF	&       0.01	& 0.183	& 0.203	& 0.515	& 0.505 \\
250	& 15	&        0.1	&       \LIN	&          -	& 0.516	& 0.470	& 0.556	& 0.774 \\
250	& 15	&        0.1	&       \RBF	&     0.0001	& 0.546	& 0.509	& 0.553	& 0.776 \\
250	& 15	&        0.1	&       \RBF	&      0.001	& 0.551	& 0.512	& 0.555	& 0.769 \\
250	& 15	&        0.1	&       \RBF	&       0.01	& 0.139	& 0.163	& 0.515	& 0.485 \\
250	& 15	&        0.2	&       \LIN	&          -	& 0.538	& 0.501	& 0.559	& 0.775 \\
250	& 15	&        0.2	&       \RBF	&     0.0001	& 0.546	& 0.509	& 0.553	& 0.776 \\
250	& 15	&        0.2	&       \RBF	&      0.001	& 0.551	& 0.512	& 0.555	& 0.769 \\
250	& 15	&        0.2	&       \RBF	&       0.01	& 0.118	& 0.148	& 0.516	& 0.481 \\
250	& 15	&        0.4	&       \LIN	&          -	& 0.551	& 0.514	& 0.558	& 0.776 \\
250	& 15	&        0.4	&       \RBF	&     0.0001	& 0.546	& 0.509	& 0.553	& 0.776 \\
250	& 15	&        0.4	&       \RBF	&      0.001	& 0.551	& 0.512	& 0.555	& 0.769 \\
250	& 15	&        0.4	&       \RBF	&       0.01	& 0.100	& 0.130	& 0.513	& 0.477 \\
250	& 15	&        0.6	&       \LIN	&          -	& 0.522	& 0.483	& 0.559	& 0.776 \\
250	& 15	&        0.6	&       \RBF	&     0.0001	& 0.546	& 0.509	& 0.553	& 0.776 \\
250	& 15	&        0.6	&       \RBF	&      0.001	& 0.551	& 0.512	& 0.555	& 0.769 \\
250	& 15	&        0.6	&       \RBF	&       0.01	& 0.095	& 0.123	& 0.513	& 0.476 \\
250	& 15	&        0.8	&       \LIN	&          -	& 0.554	& 0.508	& 0.556	& 0.777 \\
250	& 15	&        0.8	&       \RBF	&     0.0001	& 0.546	& 0.509	& 0.553	& 0.776 \\
250	& 15	&        0.8	&       \RBF	&      0.001	& 0.551	& 0.512	& 0.555	& 0.769 \\
250	& 15	&        0.8	&       \RBF	&       0.01	& 0.089	& 0.120	& 0.512	& 0.475 \\
250	& 15	&        1.0	&       \LIN	&          -	& 0.525	& 0.490	& 0.556	& 0.778 \\
250	& 15	&        1.0	&       \RBF	&     0.0001	& 0.546	& 0.509	& 0.553	& 0.776 \\
250	& 15	&        1.0	&       \RBF	&      0.001	& 0.551	& 0.512	& 0.555	& 0.769 \\
250	& 15	&        1.0	&       \RBF	&       0.01	& 0.077	& 0.108	& 0.512	& 0.474 \\
250	& 15	&         10	&       \LIN	&          -	& 0.565	& 0.520	& 0.552	& 0.778 \\
250	& 15	&         10	&       \RBF	&     0.0001	& 0.546	& 0.509	& 0.553	& 0.776 \\
250	& 15	&         10	&       \RBF	&      0.001	& 0.551	& 0.512	& 0.555	& 0.769 \\
250	& 15	&         10	&       \RBF	&       0.01	& 0.059	& 0.092	& 0.510	& 0.470 \\
250	& 15	&         50	&       \LIN	&          -	& 0.543	& 0.520	& 0.553	& 0.766 \\
250	& 15	&         50	&       \RBF	&     0.0001	& 0.546	& 0.509	& 0.553	& 0.776 \\
250	& 15	&         50	&       \RBF	&      0.001	& 0.551	& 0.512	& 0.555	& 0.769 \\
250	& 15	&         50	&       \RBF	&       0.01	& 0.051	& 0.085	& 0.510	& 0.469 \\
250	& 15	&        100	&       \LIN	&          -	& 0.537	& 0.501	& 0.554	& 0.712 \\
250	& 15	&        100	&       \RBF	&     0.0001	& 0.546	& 0.509	& 0.553	& 0.776 \\
250	& 15	&        100	&       \RBF	&      0.001	& 0.551	& 0.512	& 0.555	& 0.769 \\
250	& 15	&        100	&       \RBF	&       0.01	& 0.047	& 0.079	& 0.509	& 0.469 \\
300	& 5	&   0.000001	&       \LIN	&          -	& 0.291	& 0.309	& 0.527	& 0.693 \\
300	& 5	&   0.000001	&       \RBF	&     0.0001	& 0.414	& 0.409	& 0.539	& 0.718 \\
300	& 5	&   0.000001	&       \RBF	&      0.001	& 0.453	& 0.429	& 0.553	& 0.719 \\
300	& 5	&   0.000001	&       \RBF	&       0.01	& 0.311	& 0.315	& 0.528	& 0.580 \\
300	& 5	&    0.00001	&       \RBF	&     0.0001	& 0.512	& 0.479	& 0.539	& 0.751 \\
300	& 5	&    0.00001	&       \RBF	&      0.001	& 0.519	& 0.487	& 0.561	& 0.754 \\
300	& 5	&    0.00001	&       \RBF	&       0.01	& 0.309	& 0.315	& 0.524	& 0.579 \\
300	& 5	&     0.0001	&       \RBF	&     0.0001	& 0.482	& 0.459	& 0.559	& 0.776 \\
300	& 5	&     0.0001	&       \RBF	&      0.001	& 0.519	& 0.487	& 0.561	& 0.754 \\
300	& 5	&     0.0001	&       \RBF	&       0.01	& 0.277	& 0.287	& 0.520	& 0.551 \\
300	& 5	&      0.001	&       \LIN	&          -	& 0.385	& 0.361	& 0.545	& 0.725 \\
300	& 5	&      0.001	&       \RBF	&     0.0001	& 0.534	& 0.497	& 0.550	& 0.729 \\
300	& 5	&      0.001	&       \RBF	&      0.001	& 0.519	& 0.487	& 0.561	& 0.754 \\
300	& 5	&      0.001	&       \RBF	&       0.01	& 0.247	& 0.263	& 0.520	& 0.522 \\
300	& 5	&       0.01	&       \LIN	&          -	& 0.469	& 0.449	& 0.549	& 0.747 \\
300	& 5	&       0.01	&       \RBF	&     0.0001	& 0.534	& 0.497	& 0.550	& 0.729 \\
300	& 5	&       0.01	&       \RBF	&      0.001	& 0.519	& 0.487	& 0.561	& 0.754 \\
300	& 5	&       0.01	&       \RBF	&       0.01	& 0.182	& 0.198	& 0.514	& 0.497 \\
300	& 5	&        0.1	&       \LIN	&          -	& 0.483	& 0.460	& 0.543	& 0.755 \\
300	& 5	&        0.1	&       \RBF	&     0.0001	& 0.534	& 0.497	& 0.550	& 0.729 \\
300	& 5	&        0.1	&       \RBF	&      0.001	& 0.519	& 0.487	& 0.561	& 0.754 \\
300	& 5	&        0.1	&       \RBF	&       0.01	& 0.133	& 0.159	& 0.515	& 0.482 \\
300	& 5	&        0.2	&       \LIN	&          -	& 0.533	& 0.486	& 0.550	& 0.762 \\
300	& 5	&        0.2	&       \RBF	&     0.0001	& 0.534	& 0.497	& 0.550	& 0.729 \\
300	& 5	&        0.2	&       \RBF	&      0.001	& 0.519	& 0.487	& 0.561	& 0.754 \\
300	& 5	&        0.2	&       \RBF	&       0.01	& 0.124	& 0.151	& 0.511	& 0.478 \\
300	& 5	&        0.4	&       \LIN	&          -	& 0.427	& 0.426	& 0.551	& 0.772 \\
300	& 5	&        0.4	&       \RBF	&     0.0001	& 0.534	& 0.497	& 0.550	& 0.729 \\
300	& 5	&        0.4	&       \RBF	&      0.001	& 0.519	& 0.487	& 0.561	& 0.754 \\
300	& 5	&        0.4	&       \RBF	&       0.01	& 0.102	& 0.129	& 0.510	& 0.475 \\
300	& 5	&        0.6	&       \LIN	&          -	& 0.545	& 0.488	& 0.551	& 0.765 \\
300	& 5	&        0.6	&       \RBF	&     0.0001	& 0.534	& 0.497	& 0.550	& 0.729 \\
300	& 5	&        0.6	&       \RBF	&      0.001	& 0.519	& 0.487	& 0.561	& 0.754 \\
300	& 5	&        0.6	&       \RBF	&       0.01	& 0.088	& 0.117	& 0.510	& 0.474 \\
300	& 5	&        0.8	&       \LIN	&          -	& 0.507	& 0.477	& 0.550	& 0.770 \\
300	& 5	&        0.8	&       \RBF	&     0.0001	& 0.534	& 0.497	& 0.550	& 0.729 \\
300	& 5	&        0.8	&       \RBF	&      0.001	& 0.519	& 0.487	& 0.561	& 0.754 \\
300	& 5	&        0.8	&       \RBF	&       0.01	& 0.077	& 0.107	& 0.509	& 0.473 \\
300	& 5	&        1.0	&       \LIN	&          -	& 0.519	& 0.490	& 0.553	& 0.770 \\
300	& 5	&        1.0	&       \RBF	&     0.0001	& 0.534	& 0.497	& 0.550	& 0.729 \\
300	& 5	&        1.0	&       \RBF	&      0.001	& 0.519	& 0.487	& 0.561	& 0.754 \\
300	& 5	&        1.0	&       \RBF	&       0.01	& 0.078	& 0.105	& 0.509	& 0.472 \\
300	& 5	&         10	&       \LIN	&          -	& 0.570	& 0.503	& 0.549	& 0.773 \\
300	& 5	&         10	&       \RBF	&     0.0001	& 0.534	& 0.497	& 0.550	& 0.729 \\
300	& 5	&         10	&       \RBF	&      0.001	& 0.519	& 0.487	& 0.561	& 0.754 \\
300	& 5	&         10	&       \RBF	&       0.01	& 0.052	& 0.086	& 0.508	& 0.470 \\
300	& 5	&         50	&       \LIN	&          -	& 0.540	& 0.502	& 0.555	& 0.742 \\
300	& 5	&         50	&       \RBF	&     0.0001	& 0.534	& 0.497	& 0.550	& 0.729 \\
300	& 5	&         50	&       \RBF	&      0.001	& 0.519	& 0.487	& 0.561	& 0.754 \\
300	& 5	&         50	&       \RBF	&       0.01	& 0.044	& 0.079	& 0.508	& 0.469 \\
300	& 5	&        100	&       \LIN	&          -	& 0.532	& 0.495	& 0.550	& 0.664 \\
300	& 5	&        100	&       \RBF	&     0.0001	& 0.534	& 0.497	& 0.550	& 0.729 \\
300	& 5	&        100	&       \RBF	&      0.001	& 0.519	& 0.487	& 0.561	& 0.754 \\
300	& 5	&        100	&       \RBF	&       0.01	& 0.044	& 0.077	& 0.508	& 0.468 \\
300	& 10	&   0.000001	&       \LIN	&          -	& 0.252	& 0.267	& 0.516	& 0.693 \\
300	& 10	&   0.000001	&       \RBF	&       0.01	& 0.318	& 0.320	& 0.527	& 0.572 \\
300	& 10	&      0.001	&       \LIN	&          -	& 0.376	& 0.367	& 0.536	& 0.708 \\
300	& 10	&      0.001	&       \RBF	&     0.0001	& 0.534	& 0.499	& 0.552	& 0.770 \\
300	& 10	&      0.001	&       \RBF	&      0.001	& 0.525	& 0.491	& 0.560	& 0.767 \\
300	& 10	&      0.001	&       \RBF	&       0.01	& 0.250	& 0.265	& 0.520	& 0.530 \\
300	& 10	&       0.01	&       \LIN	&          -	& 0.438	& 0.417	& 0.550	& 0.757 \\
300	& 10	&       0.01	&       \RBF	&     0.0001	& 0.534	& 0.499	& 0.552	& 0.770 \\
300	& 10	&       0.01	&       \RBF	&      0.001	& 0.525	& 0.491	& 0.560	& 0.767 \\
300	& 10	&       0.01	&       \RBF	&       0.01	& 0.188	& 0.203	& 0.514	& 0.502 \\
300	& 10	&        0.1	&       \LIN	&          -	& 0.482	& 0.459	& 0.552	& 0.776 \\
300	& 10	&        0.1	&       \RBF	&     0.0001	& 0.534	& 0.499	& 0.552	& 0.770 \\
300	& 10	&        0.1	&       \RBF	&      0.001	& 0.525	& 0.491	& 0.560	& 0.767 \\
300	& 10	&        0.1	&       \RBF	&       0.01	& 0.138	& 0.163	& 0.513	& 0.484 \\
300	& 10	&        0.2	&       \LIN	&          -	& 0.489	& 0.463	& 0.552	& 0.776 \\
300	& 10	&        0.2	&       \RBF	&     0.0001	& 0.534	& 0.499	& 0.552	& 0.770 \\
300	& 10	&        0.2	&       \RBF	&      0.001	& 0.525	& 0.491	& 0.560	& 0.767 \\
300	& 10	&        0.2	&       \RBF	&       0.01	& 0.130	& 0.154	& 0.511	& 0.480 \\
300	& 10	&        0.4	&       \LIN	&          -	& 0.518	& 0.470	& 0.551	& 0.776 \\
300	& 10	&        0.4	&       \RBF	&     0.0001	& 0.534	& 0.499	& 0.552	& 0.770 \\
300	& 10	&        0.4	&       \RBF	&      0.001	& 0.525	& 0.491	& 0.560	& 0.767 \\
300	& 10	&        0.4	&       \RBF	&       0.01	& 0.113	& 0.137	& 0.511	& 0.476 \\
300	& 10	&        0.6	&       \LIN	&          -	& 0.519	& 0.476	& 0.554	& 0.779 \\
300	& 10	&        0.6	&       \RBF	&     0.0001	& 0.534	& 0.499	& 0.552	& 0.770 \\
300	& 10	&        0.6	&       \RBF	&      0.001	& 0.525	& 0.491	& 0.560	& 0.767 \\
300	& 10	&        0.6	&       \RBF	&       0.01	& 0.091	& 0.119	& 0.509	& 0.475 \\
300	& 10	&        0.8	&       \LIN	&          -	& 0.549	& 0.499	& 0.552	& 0.780 \\
300	& 10	&        0.8	&       \RBF	&     0.0001	& 0.534	& 0.499	& 0.552	& 0.770 \\
300	& 10	&        0.8	&       \RBF	&      0.001	& 0.525	& 0.491	& 0.560	& 0.767 \\
300	& 10	&        0.8	&       \RBF	&       0.01	& 0.081	& 0.112	& 0.509	& 0.474 \\
300	& 10	&        1.0	&       \LIN	&          -	& 0.561	& 0.508	& 0.548	& 0.775 \\
300	& 10	&        1.0	&       \RBF	&     0.0001	& 0.534	& 0.499	& 0.552	& 0.770 \\
300	& 10	&        1.0	&       \RBF	&      0.001	& 0.525	& 0.491	& 0.560	& 0.767 \\
300	& 10	&        1.0	&       \RBF	&       0.01	& 0.080	& 0.108	& 0.509	& 0.473 \\
300	& 10	&         10	&       \LIN	&          -	& 0.546	& 0.517	& 0.549	& 0.788 \\
300	& 10	&         10	&       \RBF	&     0.0001	& 0.534	& 0.499	& 0.552	& 0.770 \\
300	& 10	&         10	&       \RBF	&      0.001	& 0.525	& 0.491	& 0.560	& 0.767 \\
300	& 10	&         10	&       \RBF	&       0.01	& 0.053	& 0.088	& 0.508	& 0.470 \\
300	& 10	&         50	&       \LIN	&          -	& 0.536	& 0.500	& 0.554	& 0.754 \\
300	& 10	&         50	&       \RBF	&     0.0001	& 0.534	& 0.499	& 0.552	& 0.770 \\
300	& 10	&         50	&       \RBF	&      0.001	& 0.525	& 0.491	& 0.560	& 0.767 \\
300	& 10	&         50	&       \RBF	&       0.01	& 0.046	& 0.081	& 0.508	& 0.469 \\
300	& 10	&        100	&       \LIN	&          -	& 0.533	& 0.495	& 0.551	& 0.691 \\
300	& 10	&        100	&       \RBF	&     0.0001	& 0.534	& 0.499	& 0.552	& 0.770 \\
300	& 10	&        100	&       \RBF	&      0.001	& 0.525	& 0.491	& 0.560	& 0.767 \\
300	& 10	&        100	&       \RBF	&       0.01	& 0.046	& 0.081	& 0.508	& 0.469 \\
300	& 15	&      0.001	&       \LIN	&          -	& 0.298	& 0.301	& 0.534	& 0.691 \\
300	& 15	&      0.001	&       \RBF	&     0.0001	& 0.538	& 0.504	& 0.556	& 0.776 \\
300	& 15	&      0.001	&       \RBF	&      0.001	& 0.527	& 0.497	& 0.558	& 0.765 \\
300	& 15	&      0.001	&       \RBF	&       0.01	& 0.252	& 0.266	& 0.520	& 0.532 \\
300	& 15	&       0.01	&       \LIN	&          -	& 0.359	& 0.353	& 0.535	& 0.699 \\
300	& 15	&       0.01	&       \RBF	&     0.0001	& 0.538	& 0.504	& 0.556	& 0.776 \\
300	& 15	&       0.01	&       \RBF	&      0.001	& 0.527	& 0.497	& 0.558	& 0.765 \\
300	& 15	&       0.01	&       \RBF	&       0.01	& 0.192	& 0.208	& 0.515	& 0.503 \\
300	& 15	&        0.1	&       \LIN	&          -	& 0.480	& 0.458	& 0.558	& 0.774 \\
300	& 15	&        0.1	&       \RBF	&     0.0001	& 0.538	& 0.504	& 0.556	& 0.776 \\
300	& 15	&        0.1	&       \RBF	&      0.001	& 0.527	& 0.497	& 0.558	& 0.765 \\
300	& 15	&        0.1	&       \RBF	&       0.01	& 0.136	& 0.162	& 0.513	& 0.485 \\
300	& 15	&        0.2	&       \LIN	&          -	& 0.525	& 0.485	& 0.557	& 0.774 \\
300	& 15	&        0.2	&       \RBF	&     0.0001	& 0.538	& 0.504	& 0.556	& 0.776 \\
300	& 15	&        0.2	&       \RBF	&      0.001	& 0.527	& 0.497	& 0.558	& 0.765 \\
300	& 15	&        0.2	&       \RBF	&       0.01	& 0.132	& 0.155	& 0.511	& 0.480 \\
300	& 15	&        0.4	&       \LIN	&          -	& 0.522	& 0.484	& 0.557	& 0.776 \\
300	& 15	&        0.4	&       \RBF	&     0.0001	& 0.538	& 0.504	& 0.556	& 0.776 \\
300	& 15	&        0.4	&       \RBF	&      0.001	& 0.527	& 0.497	& 0.558	& 0.765 \\
300	& 15	&        0.4	&       \RBF	&       0.01	& 0.118	& 0.143	& 0.509	& 0.477 \\
300	& 15	&        0.6	&       \LIN	&          -	& 0.542	& 0.496	& 0.555	& 0.775 \\
300	& 15	&        0.6	&       \RBF	&     0.0001	& 0.538	& 0.504	& 0.556	& 0.776 \\
300	& 15	&        0.6	&       \RBF	&      0.001	& 0.527	& 0.497	& 0.558	& 0.765 \\
300	& 15	&        0.6	&       \RBF	&       0.01	& 0.093	& 0.119	& 0.508	& 0.475 \\
300	& 15	&        0.8	&       \LIN	&          -	& 0.536	& 0.506	& 0.556	& 0.779 \\
300	& 15	&        0.8	&       \RBF	&     0.0001	& 0.538	& 0.504	& 0.556	& 0.776 \\
300	& 15	&        0.8	&       \RBF	&      0.001	& 0.527	& 0.497	& 0.558	& 0.765 \\
300	& 15	&        0.8	&       \RBF	&       0.01	& 0.081	& 0.113	& 0.509	& 0.474 \\
300	& 15	&        1.0	&       \LIN	&          -	& 0.560	& 0.514	& 0.556	& 0.779 \\
300	& 15	&        1.0	&       \RBF	&     0.0001	& 0.538	& 0.504	& 0.556	& 0.776 \\
300	& 15	&        1.0	&       \RBF	&      0.001	& 0.527	& 0.497	& 0.558	& 0.765 \\
300	& 15	&        1.0	&       \RBF	&       0.01	& 0.075	& 0.105	& 0.508	& 0.473 \\
300	& 15	&         10	&       \LIN	&          -	& 0.555	& 0.515	& 0.551	& 0.780 \\
300	& 15	&         10	&       \RBF	&     0.0001	& 0.538	& 0.504	& 0.556	& 0.776 \\
300	& 15	&         10	&       \RBF	&      0.001	& 0.527	& 0.497	& 0.558	& 0.765 \\
300	& 15	&         10	&       \RBF	&       0.01	& 0.054	& 0.088	& 0.508	& 0.470 \\
300	& 15	&         50	&       \LIN	&          -	& 0.534	& 0.506	& 0.555	& 0.764 \\
300	& 15	&         50	&       \RBF	&     0.0001	& 0.538	& 0.504	& 0.556	& 0.776 \\
300	& 15	&         50	&       \RBF	&      0.001	& 0.527	& 0.498	& 0.558	& 0.765 \\
300	& 15	&         50	&       \RBF	&       0.01	& 0.045	& 0.081	& 0.508	& 0.469 \\
300	& 15	&        100	&       \LIN	&          -	& 0.536	& 0.500	& 0.553	& 0.705 \\
300	& 15	&        100	&       \RBF	&     0.0001	& 0.538	& 0.504	& 0.556	& 0.776 \\
300	& 15	&        100	&       \RBF	&      0.001	& 0.527	& 0.498	& 0.558	& 0.765 \\
300	& 15	&        100	&       \RBF	&       0.01	& 0.047	& 0.081	& 0.508	& 0.469 \\
350	& 5	&   0.000001	&       \LIN	&          -	& 0.247	& 0.264	& 0.534	& 0.691 \\
350	& 5	&   0.000001	&       \RBF	&     0.0001	& 0.426	& 0.406	& 0.533	& 0.730 \\
350	& 5	&   0.000001	&       \RBF	&      0.001	& 0.463	& 0.431	& 0.549	& 0.714 \\
350	& 5	&   0.000001	&       \RBF	&       0.01	& 0.314	& 0.314	& 0.524	& 0.574 \\
350	& 5	&    0.00001	&       \RBF	&     0.0001	& 0.476	& 0.442	& 0.539	& 0.758 \\
350	& 5	&    0.00001	&       \RBF	&      0.001	& 0.513	& 0.482	& 0.555	& 0.748 \\
350	& 5	&    0.00001	&       \RBF	&       0.01	& 0.295	& 0.303	& 0.520	& 0.570 \\
350	& 5	&     0.0001	&       \RBF	&     0.0001	& 0.527	& 0.493	& 0.553	& 0.774 \\
350	& 5	&     0.0001	&       \RBF	&      0.001	& 0.513	& 0.482	& 0.555	& 0.748 \\
350	& 5	&     0.0001	&       \RBF	&       0.01	& 0.262	& 0.276	& 0.517	& 0.543 \\
350	& 5	&      0.001	&       \LIN	&          -	& 0.329	& 0.324	& 0.523	& 0.684 \\
350	& 5	&      0.001	&       \RBF	&     0.0001	& 0.528	& 0.488	& 0.551	& 0.724 \\
350	& 5	&      0.001	&       \RBF	&      0.001	& 0.513	& 0.482	& 0.555	& 0.748 \\
350	& 5	&      0.001	&       \RBF	&       0.01	& 0.236	& 0.252	& 0.515	& 0.518 \\
350	& 5	&       0.01	&       \LIN	&          -	& 0.461	& 0.432	& 0.545	& 0.744 \\
350	& 5	&       0.01	&       \RBF	&     0.0001	& 0.528	& 0.488	& 0.551	& 0.724 \\
350	& 5	&       0.01	&       \RBF	&      0.001	& 0.513	& 0.482	& 0.555	& 0.748 \\
350	& 5	&       0.01	&       \RBF	&       0.01	& 0.178	& 0.197	& 0.513	& 0.496 \\
350	& 5	&        0.1	&       \LIN	&          -	& 0.465	& 0.440	& 0.546	& 0.763 \\
350	& 5	&        0.1	&       \RBF	&     0.0001	& 0.528	& 0.488	& 0.551	& 0.724 \\
350	& 5	&        0.1	&       \RBF	&      0.001	& 0.513	& 0.482	& 0.555	& 0.748 \\
350	& 5	&        0.1	&       \RBF	&       0.01	& 0.138	& 0.164	& 0.510	& 0.482 \\
350	& 5	&        0.2	&       \LIN	&          -	& 0.460	& 0.438	& 0.545	& 0.761 \\
350	& 5	&        0.2	&       \RBF	&     0.0001	& 0.528	& 0.488	& 0.551	& 0.724 \\
350	& 5	&        0.2	&       \RBF	&      0.001	& 0.513	& 0.482	& 0.555	& 0.748 \\
350	& 5	&        0.2	&       \RBF	&       0.01	& 0.121	& 0.144	& 0.510	& 0.479 \\
350	& 5	&        0.4	&       \LIN	&          -	& 0.488	& 0.452	& 0.549	& 0.769 \\
350	& 5	&        0.4	&       \RBF	&     0.0001	& 0.528	& 0.488	& 0.551	& 0.724 \\
350	& 5	&        0.4	&       \RBF	&      0.001	& 0.513	& 0.482	& 0.555	& 0.748 \\
350	& 5	&        0.4	&       \RBF	&       0.01	& 0.102	& 0.129	& 0.510	& 0.476 \\
350	& 5	&        0.6	&       \LIN	&          -	& 0.518	& 0.464	& 0.548	& 0.767 \\
350	& 5	&        0.6	&       \RBF	&     0.0001	& 0.528	& 0.488	& 0.551	& 0.724 \\
350	& 5	&        0.6	&       \RBF	&      0.001	& 0.513	& 0.482	& 0.555	& 0.748 \\
350	& 5	&        0.6	&       \RBF	&       0.01	& 0.094	& 0.120	& 0.509	& 0.474 \\
350	& 5	&        0.8	&       \LIN	&          -	& 0.493	& 0.459	& 0.550	& 0.774 \\
350	& 5	&        0.8	&       \RBF	&     0.0001	& 0.528	& 0.488	& 0.551	& 0.724 \\
350	& 5	&        0.8	&       \RBF	&      0.001	& 0.513	& 0.482	& 0.555	& 0.748 \\
350	& 5	&        0.8	&       \RBF	&       0.01	& 0.092	& 0.119	& 0.508	& 0.474 \\
350	& 5	&        1.0	&       \LIN	&          -	& 0.488	& 0.457	& 0.548	& 0.770 \\
350	& 5	&        1.0	&       \RBF	&     0.0001	& 0.528	& 0.488	& 0.551	& 0.724 \\
350	& 5	&        1.0	&       \RBF	&      0.001	& 0.513	& 0.482	& 0.555	& 0.748 \\
350	& 5	&        1.0	&       \RBF	&       0.01	& 0.085	& 0.112	& 0.508	& 0.473 \\
350	& 5	&         10	&       \LIN	&          -	& 0.541	& 0.491	& 0.542	& 0.762 \\
350	& 5	&         10	&       \RBF	&     0.0001	& 0.528	& 0.488	& 0.551	& 0.724 \\
350	& 5	&         10	&       \RBF	&      0.001	& 0.513	& 0.482	& 0.555	& 0.748 \\
350	& 5	&         10	&       \RBF	&       0.01	& 0.057	& 0.090	& 0.508	& 0.470 \\
350	& 5	&         50	&       \LIN	&          -	& 0.520	& 0.491	& 0.553	& 0.719 \\
350	& 5	&         50	&       \RBF	&     0.0001	& 0.528	& 0.488	& 0.551	& 0.724 \\
350	& 5	&         50	&       \RBF	&      0.001	& 0.513	& 0.482	& 0.555	& 0.748 \\
350	& 5	&         50	&       \RBF	&       0.01	& 0.053	& 0.088	& 0.507	& 0.469 \\
350	& 5	&        100	&       \LIN	&          -	& 0.509	& 0.473	& 0.549	& 0.647 \\
350	& 5	&        100	&       \RBF	&     0.0001	& 0.528	& 0.488	& 0.551	& 0.724 \\
350	& 5	&        100	&       \RBF	&      0.001	& 0.513	& 0.482	& 0.555	& 0.748 \\
350	& 5	&        100	&       \RBF	&       0.01	& 0.050	& 0.084	& 0.507	& 0.469 \\
350	& 10	&   0.000001	&       \LIN	&          -	& 0.291	& 0.304	& 0.517	& 0.706 \\
350	& 10	&   0.000001	&       \RBF	&       0.01	& 0.314	& 0.315	& 0.524	& 0.566 \\
350	& 10	&      0.001	&       \LIN	&          -	& 0.365	& 0.366	& 0.535	& 0.696 \\
350	& 10	&      0.001	&       \RBF	&     0.0001	& 0.528	& 0.498	& 0.552	& 0.765 \\
350	& 10	&      0.001	&       \RBF	&      0.001	& 0.515	& 0.484	& 0.554	& 0.762 \\
350	& 10	&      0.001	&       \RBF	&       0.01	& 0.247	& 0.258	& 0.515	& 0.526 \\
350	& 10	&       0.01	&       \LIN	&          -	& 0.367	& 0.367	& 0.529	& 0.704 \\
350	& 10	&       0.01	&       \RBF	&     0.0001	& 0.528	& 0.498	& 0.552	& 0.765 \\
350	& 10	&       0.01	&       \RBF	&      0.001	& 0.515	& 0.484	& 0.554	& 0.762 \\
350	& 10	&       0.01	&       \RBF	&       0.01	& 0.180	& 0.200	& 0.513	& 0.501 \\
350	& 10	&        0.1	&       \LIN	&          -	& 0.472	& 0.440	& 0.547	& 0.774 \\
350	& 10	&        0.1	&       \RBF	&     0.0001	& 0.528	& 0.498	& 0.552	& 0.765 \\
350	& 10	&        0.1	&       \RBF	&      0.001	& 0.515	& 0.484	& 0.554	& 0.762 \\
350	& 10	&        0.1	&       \RBF	&       0.01	& 0.141	& 0.166	& 0.509	& 0.485 \\
350	& 10	&        0.2	&       \LIN	&          -	& 0.518	& 0.481	& 0.546	& 0.773 \\
350	& 10	&        0.2	&       \RBF	&     0.0001	& 0.528	& 0.498	& 0.552	& 0.765 \\
350	& 10	&        0.2	&       \RBF	&      0.001	& 0.515	& 0.484	& 0.554	& 0.762 \\
350	& 10	&        0.2	&       \RBF	&       0.01	& 0.123	& 0.149	& 0.510	& 0.481 \\
350	& 10	&        0.4	&       \LIN	&          -	& 0.523	& 0.486	& 0.546	& 0.776 \\
350	& 10	&        0.4	&       \RBF	&     0.0001	& 0.528	& 0.498	& 0.552	& 0.765 \\
350	& 10	&        0.4	&       \RBF	&      0.001	& 0.515	& 0.484	& 0.554	& 0.762 \\
350	& 10	&        0.4	&       \RBF	&       0.01	& 0.102	& 0.129	& 0.510	& 0.477 \\
350	& 10	&        0.6	&       \LIN	&          -	& 0.523	& 0.477	& 0.544	& 0.773 \\
350	& 10	&        0.6	&       \RBF	&     0.0001	& 0.528	& 0.498	& 0.552	& 0.765 \\
350	& 10	&        0.6	&       \RBF	&      0.001	& 0.515	& 0.484	& 0.554	& 0.762 \\
350	& 10	&        0.6	&       \RBF	&       0.01	& 0.092	& 0.120	& 0.509	& 0.476 \\
350	& 10	&        0.8	&       \LIN	&          -	& 0.533	& 0.502	& 0.547	& 0.778 \\
350	& 10	&        0.8	&       \RBF	&     0.0001	& 0.528	& 0.498	& 0.552	& 0.765 \\
350	& 10	&        0.8	&       \RBF	&      0.001	& 0.515	& 0.484	& 0.554	& 0.762 \\
350	& 10	&        0.8	&       \RBF	&       0.01	& 0.100	& 0.125	& 0.508	& 0.475 \\
350	& 10	&        1.0	&       \LIN	&          -	& 0.526	& 0.489	& 0.547	& 0.774 \\
350	& 10	&        1.0	&       \RBF	&     0.0001	& 0.528	& 0.498	& 0.552	& 0.765 \\
350	& 10	&        1.0	&       \RBF	&      0.001	& 0.515	& 0.484	& 0.554	& 0.762 \\
350	& 10	&        1.0	&       \RBF	&       0.01	& 0.080	& 0.108	& 0.508	& 0.474 \\
350	& 10	&         10	&       \LIN	&          -	& 0.549	& 0.515	& 0.544	& 0.782 \\
350	& 10	&         10	&       \RBF	&     0.0001	& 0.528	& 0.498	& 0.552	& 0.765 \\
350	& 10	&         10	&       \RBF	&      0.001	& 0.515	& 0.484	& 0.554	& 0.762 \\
350	& 10	&         10	&       \RBF	&       0.01	& 0.056	& 0.089	& 0.508	& 0.471 \\
350	& 10	&         50	&       \LIN	&          -	& 0.532	& 0.509	& 0.553	& 0.737 \\
350	& 10	&         50	&       \RBF	&     0.0001	& 0.528	& 0.498	& 0.552	& 0.765 \\
350	& 10	&         50	&       \RBF	&      0.001	& 0.515	& 0.484	& 0.554	& 0.762 \\
350	& 10	&         50	&       \RBF	&       0.01	& 0.055	& 0.089	& 0.507	& 0.470 \\
350	& 10	&        100	&       \LIN	&          -	& 0.513	& 0.481	& 0.552	& 0.686 \\
350	& 10	&        100	&       \RBF	&     0.0001	& 0.528	& 0.498	& 0.552	& 0.765 \\
350	& 10	&        100	&       \RBF	&      0.001	& 0.515	& 0.484	& 0.554	& 0.762 \\
350	& 10	&        100	&       \RBF	&       0.01	& 0.050	& 0.084	& 0.507	& 0.469 \\
350	& 15	&      0.001	&       \LIN	&          -	& 0.361	& 0.350	& 0.517	& 0.704 \\
350	& 15	&      0.001	&       \RBF	&     0.0001	& 0.531	& 0.506	& 0.554	& 0.772 \\
350	& 15	&      0.001	&       \RBF	&      0.001	& 0.511	& 0.485	& 0.553	& 0.760 \\
350	& 15	&      0.001	&       \RBF	&       0.01	& 0.250	& 0.259	& 0.515	& 0.528 \\
350	& 15	&       0.01	&       \LIN	&          -	& 0.351	& 0.351	& 0.528	& 0.723 \\
350	& 15	&       0.01	&       \RBF	&     0.0001	& 0.531	& 0.506	& 0.554	& 0.772 \\
350	& 15	&       0.01	&       \RBF	&      0.001	& 0.511	& 0.485	& 0.553	& 0.760 \\
350	& 15	&       0.01	&       \RBF	&       0.01	& 0.182	& 0.200	& 0.513	& 0.502 \\
350	& 15	&        0.1	&       \LIN	&          -	& 0.447	& 0.431	& 0.513	& 0.709 \\
350	& 15	&        0.1	&       \RBF	&     0.0001	& 0.531	& 0.506	& 0.554	& 0.772 \\
350	& 15	&        0.1	&       \RBF	&      0.001	& 0.511	& 0.485	& 0.553	& 0.760 \\
350	& 15	&        0.1	&       \RBF	&       0.01	& 0.143	& 0.163	& 0.510	& 0.485 \\
350	& 15	&        0.2	&       \LIN	&          -	& 0.505	& 0.475	& 0.551	& 0.771 \\
350	& 15	&        0.2	&       \RBF	&     0.0001	& 0.531	& 0.506	& 0.554	& 0.772 \\
350	& 15	&        0.2	&       \RBF	&      0.001	& 0.511	& 0.485	& 0.553	& 0.760 \\
350	& 15	&        0.2	&       \RBF	&       0.01	& 0.127	& 0.151	& 0.510	& 0.482 \\
350	& 15	&        0.4	&       \LIN	&          -	& 0.477	& 0.448	& 0.551	& 0.771 \\
350	& 15	&        0.4	&       \RBF	&     0.0001	& 0.531	& 0.506	& 0.554	& 0.772 \\
350	& 15	&        0.4	&       \RBF	&      0.001	& 0.511	& 0.485	& 0.553	& 0.760 \\
350	& 15	&        0.4	&       \RBF	&       0.01	& 0.107	& 0.130	& 0.510	& 0.478 \\
350	& 15	&        0.6	&       \LIN	&          -	& 0.510	& 0.484	& 0.550	& 0.773 \\
350	& 15	&        0.6	&       \RBF	&     0.0001	& 0.531	& 0.506	& 0.554	& 0.772 \\
350	& 15	&        0.6	&       \RBF	&      0.001	& 0.511	& 0.485	& 0.553	& 0.760 \\
350	& 15	&        0.6	&       \RBF	&       0.01	& 0.094	& 0.122	& 0.509	& 0.476 \\
350	& 15	&        0.8	&       \LIN	&          -	& 0.532	& 0.498	& 0.552	& 0.774 \\
350	& 15	&        0.8	&       \RBF	&     0.0001	& 0.531	& 0.506	& 0.554	& 0.772 \\
350	& 15	&        0.8	&       \RBF	&      0.001	& 0.511	& 0.485	& 0.553	& 0.760 \\
350	& 15	&        0.8	&       \RBF	&       0.01	& 0.099	& 0.125	& 0.509	& 0.475 \\
350	& 15	&        1.0	&       \LIN	&          -	& 0.479	& 0.461	& 0.551	& 0.775 \\
350	& 15	&        1.0	&       \RBF	&     0.0001	& 0.531	& 0.506	& 0.554	& 0.772 \\
350	& 15	&        1.0	&       \RBF	&      0.001	& 0.511	& 0.485	& 0.553	& 0.760 \\
350	& 15	&        1.0	&       \RBF	&       0.01	& 0.086	& 0.112	& 0.508	& 0.474 \\
350	& 15	&         10	&       \LIN	&          -	& 0.536	& 0.502	& 0.547	& 0.776 \\
350	& 15	&         10	&       \RBF	&     0.0001	& 0.531	& 0.506	& 0.554	& 0.772 \\
350	& 15	&         10	&       \RBF	&      0.001	& 0.511	& 0.485	& 0.553	& 0.760 \\
350	& 15	&         10	&       \RBF	&       0.01	& 0.057	& 0.089	& 0.508	& 0.471 \\
350	& 15	&         50	&       \LIN	&          -	& 0.537	& 0.512	& 0.551	& 0.751 \\
350	& 15	&         50	&       \RBF	&     0.0001	& 0.531	& 0.506	& 0.554	& 0.772 \\
350	& 15	&         50	&       \RBF	&      0.001	& 0.511	& 0.485	& 0.553	& 0.760 \\
350	& 15	&         50	&       \RBF	&       0.01	& 0.052	& 0.087	& 0.507	& 0.470 \\
350	& 15	&        100	&       \LIN	&          -	& 0.533	& 0.490	& 0.553	& 0.698 \\
350	& 15	&        100	&       \RBF	&     0.0001	& 0.531	& 0.506	& 0.554	& 0.772 \\
350	& 15	&        100	&       \RBF	&      0.001	& 0.510	& 0.484	& 0.553	& 0.760 \\
350	& 15	&        100	&       \RBF	&       0.01	& 0.051	& 0.085	& 0.507	& 0.469 \\
400	& 5	&   0.000001	&       \LIN	&          -	& 0.238	& 0.251	& 0.528	& 0.699 \\
400	& 5	&   0.000001	&       \RBF	&     0.0001	& 0.433	& 0.413	& 0.539	& 0.714 \\
400	& 5	&   0.000001	&       \RBF	&      0.001	& 0.456	& 0.434	& 0.551	& 0.712 \\
400	& 5	&   0.000001	&       \RBF	&       0.01	& 0.314	& 0.317	& 0.521	& 0.571 \\
400	& 5	&    0.00001	&       \RBF	&     0.0001	& 0.472	& 0.446	& 0.543	& 0.766 \\
400	& 5	&    0.00001	&       \RBF	&      0.001	& 0.530	& 0.491	& 0.556	& 0.747 \\
400	& 5	&    0.00001	&       \RBF	&       0.01	& 0.314	& 0.316	& 0.521	& 0.566 \\
400	& 5	&     0.0001	&       \LIN	&          -	& 0.376	& 0.359	& 0.523	& 0.680 \\
400	& 5	&     0.0001	&       \RBF	&     0.0001	& 0.535	& 0.497	& 0.555	& 0.770 \\
400	& 5	&     0.0001	&       \RBF	&      0.001	& 0.530	& 0.491	& 0.556	& 0.747 \\
400	& 5	&     0.0001	&       \RBF	&       0.01	& 0.279	& 0.286	& 0.515	& 0.541 \\
400	& 5	&      0.001	&       \LIN	&          -	& 0.371	& 0.366	& 0.544	& 0.723 \\
400	& 5	&      0.001	&       \RBF	&     0.0001	& 0.515	& 0.479	& 0.550	& 0.724 \\
400	& 5	&      0.001	&       \RBF	&      0.001	& 0.530	& 0.491	& 0.556	& 0.747 \\
400	& 5	&      0.001	&       \RBF	&       0.01	& 0.229	& 0.244	& 0.514	& 0.517 \\
400	& 5	&       0.01	&       \LIN	&          -	& 0.444	& 0.429	& 0.549	& 0.746 \\
400	& 5	&       0.01	&       \RBF	&     0.0001	& 0.515	& 0.479	& 0.550	& 0.724 \\
400	& 5	&       0.01	&       \RBF	&      0.001	& 0.530	& 0.491	& 0.556	& 0.747 \\
400	& 5	&       0.01	&       \RBF	&       0.01	& 0.175	& 0.194	& 0.511	& 0.496 \\
400	& 5	&        0.1	&       \LIN	&          -	& 0.441	& 0.417	& 0.535	& 0.766 \\
400	& 5	&        0.1	&       \RBF	&     0.0001	& 0.515	& 0.479	& 0.550	& 0.724 \\
400	& 5	&        0.1	&       \RBF	&      0.001	& 0.530	& 0.491	& 0.556	& 0.747 \\
400	& 5	&        0.1	&       \RBF	&       0.01	& 0.134	& 0.160	& 0.509	& 0.482 \\
400	& 5	&        0.2	&       \LIN	&          -	& 0.479	& 0.436	& 0.548	& 0.766 \\
400	& 5	&        0.2	&       \RBF	&     0.0001	& 0.515	& 0.479	& 0.550	& 0.724 \\
400	& 5	&        0.2	&       \RBF	&      0.001	& 0.530	& 0.491	& 0.556	& 0.747 \\
400	& 5	&        0.2	&       \RBF	&       0.01	& 0.126	& 0.149	& 0.508	& 0.479 \\
400	& 5	&        0.4	&       \LIN	&          -	& 0.451	& 0.442	& 0.548	& 0.768 \\
400	& 5	&        0.4	&       \RBF	&     0.0001	& 0.515	& 0.479	& 0.550	& 0.724 \\
400	& 5	&        0.4	&       \RBF	&      0.001	& 0.530	& 0.491	& 0.556	& 0.747 \\
400	& 5	&        0.4	&       \RBF	&       0.01	& 0.106	& 0.130	& 0.507	& 0.476 \\
400	& 5	&        0.6	&       \LIN	&          -	& 0.498	& 0.463	& 0.546	& 0.768 \\
400	& 5	&        0.6	&       \RBF	&     0.0001	& 0.515	& 0.479	& 0.550	& 0.724 \\
400	& 5	&        0.6	&       \RBF	&      0.001	& 0.530	& 0.491	& 0.556	& 0.747 \\
400	& 5	&        0.6	&       \RBF	&       0.01	& 0.098	& 0.125	& 0.508	& 0.474 \\
400	& 5	&        0.8	&       \LIN	&          -	& 0.443	& 0.436	& 0.549	& 0.763 \\
400	& 5	&        0.8	&       \RBF	&     0.0001	& 0.515	& 0.479	& 0.550	& 0.724 \\
400	& 5	&        0.8	&       \RBF	&      0.001	& 0.530	& 0.491	& 0.556	& 0.747 \\
400	& 5	&        0.8	&       \RBF	&       0.01	& 0.089	& 0.115	& 0.507	& 0.474 \\
400	& 5	&        1.0	&       \LIN	&          -	& 0.532	& 0.499	& 0.550	& 0.774 \\
400	& 5	&        1.0	&       \RBF	&     0.0001	& 0.515	& 0.479	& 0.550	& 0.724 \\
400	& 5	&        1.0	&       \RBF	&      0.001	& 0.530	& 0.491	& 0.556	& 0.747 \\
400	& 5	&        1.0	&       \RBF	&       0.01	& 0.084	& 0.109	& 0.507	& 0.473 \\
400	& 5	&         10	&       \LIN	&          -	& 0.474	& 0.444	& 0.548	& 0.762 \\
400	& 5	&         10	&       \RBF	&     0.0001	& 0.515	& 0.479	& 0.550	& 0.724 \\
400	& 5	&         10	&       \RBF	&      0.001	& 0.530	& 0.491	& 0.556	& 0.747 \\
400	& 5	&         10	&       \RBF	&       0.01	& 0.058	& 0.091	& 0.507	& 0.470 \\
400	& 5	&         50	&       \LIN	&          -	& 0.505	& 0.474	& 0.553	& 0.705 \\
400	& 5	&         50	&       \RBF	&     0.0001	& 0.515	& 0.479	& 0.550	& 0.724 \\
400	& 5	&         50	&       \RBF	&      0.001	& 0.530	& 0.491	& 0.556	& 0.747 \\
400	& 5	&         50	&       \RBF	&       0.01	& 0.049	& 0.084	& 0.505	& 0.469 \\
400	& 5	&        100	&       \LIN	&          -	& 0.510	& 0.476	& 0.549	& 0.649 \\
400	& 5	&        100	&       \RBF	&     0.0001	& 0.515	& 0.479	& 0.550	& 0.724 \\
400	& 5	&        100	&       \RBF	&      0.001	& 0.529	& 0.491	& 0.556	& 0.747 \\
400	& 5	&        100	&       \RBF	&       0.01	& 0.049	& 0.083	& 0.505	& 0.469 \\
400	& 10	&   0.000001	&       \LIN	&          -	& 0.281	& 0.284	& 0.534	& 0.691 \\
400	& 10	&   0.000001	&       \RBF	&      0.001	& 0.454	& 0.428	& 0.553	& 0.701 \\
400	& 10	&   0.000001	&       \RBF	&       0.01	& 0.312	& 0.318	& 0.520	& 0.564 \\
400	& 10	&      0.001	&       \LIN	&          -	& 0.381	& 0.372	& 0.520	& 0.706 \\
400	& 10	&      0.001	&       \RBF	&     0.0001	& 0.516	& 0.487	& 0.551	& 0.764 \\
400	& 10	&      0.001	&       \RBF	&      0.001	& 0.530	& 0.491	& 0.555	& 0.762 \\
400	& 10	&      0.001	&       \RBF	&       0.01	& 0.230	& 0.247	& 0.515	& 0.525 \\
400	& 10	&       0.01	&       \LIN	&          -	& 0.405	& 0.394	& 0.549	& 0.762 \\
400	& 10	&       0.01	&       \RBF	&     0.0001	& 0.516	& 0.487	& 0.551	& 0.764 \\
400	& 10	&       0.01	&       \RBF	&      0.001	& 0.530	& 0.491	& 0.555	& 0.762 \\
400	& 10	&       0.01	&       \RBF	&       0.01	& 0.181	& 0.197	& 0.511	& 0.501 \\
400	& 10	&        0.1	&       \LIN	&          -	& 0.459	& 0.435	& 0.551	& 0.769 \\
400	& 10	&        0.1	&       \RBF	&     0.0001	& 0.516	& 0.487	& 0.551	& 0.764 \\
400	& 10	&        0.1	&       \RBF	&      0.001	& 0.530	& 0.491	& 0.555	& 0.762 \\
400	& 10	&        0.1	&       \RBF	&       0.01	& 0.136	& 0.158	& 0.509	& 0.484 \\
400	& 10	&        0.2	&       \LIN	&          -	& 0.503	& 0.469	& 0.552	& 0.775 \\
400	& 10	&        0.2	&       \RBF	&     0.0001	& 0.516	& 0.487	& 0.551	& 0.764 \\
400	& 10	&        0.2	&       \RBF	&      0.001	& 0.530	& 0.491	& 0.555	& 0.762 \\
400	& 10	&        0.2	&       \RBF	&       0.01	& 0.129	& 0.149	& 0.508	& 0.481 \\
400	& 10	&        0.4	&       \LIN	&          -	& 0.506	& 0.471	& 0.551	& 0.776 \\
400	& 10	&        0.4	&       \RBF	&     0.0001	& 0.516	& 0.487	& 0.551	& 0.764 \\
400	& 10	&        0.4	&       \RBF	&      0.001	& 0.530	& 0.491	& 0.555	& 0.762 \\
400	& 10	&        0.4	&       \RBF	&       0.01	& 0.109	& 0.131	& 0.508	& 0.477 \\
400	& 10	&        0.6	&       \LIN	&          -	& 0.525	& 0.473	& 0.550	& 0.779 \\
400	& 10	&        0.6	&       \RBF	&     0.0001	& 0.516	& 0.487	& 0.551	& 0.764 \\
400	& 10	&        0.6	&       \RBF	&      0.001	& 0.530	& 0.491	& 0.555	& 0.762 \\
400	& 10	&        0.6	&       \RBF	&       0.01	& 0.096	& 0.121	& 0.508	& 0.476 \\
400	& 10	&        0.8	&       \LIN	&          -	& 0.543	& 0.502	& 0.549	& 0.778 \\
400	& 10	&        0.8	&       \RBF	&     0.0001	& 0.516	& 0.487	& 0.551	& 0.764 \\
400	& 10	&        0.8	&       \RBF	&      0.001	& 0.530	& 0.491	& 0.555	& 0.762 \\
400	& 10	&        0.8	&       \RBF	&       0.01	& 0.095	& 0.121	& 0.508	& 0.475 \\
400	& 10	&        1.0	&       \LIN	&          -	& 0.515	& 0.477	& 0.545	& 0.777 \\
400	& 10	&        1.0	&       \RBF	&     0.0001	& 0.516	& 0.487	& 0.551	& 0.764 \\
400	& 10	&        1.0	&       \RBF	&      0.001	& 0.530	& 0.491	& 0.555	& 0.762 \\
400	& 10	&        1.0	&       \RBF	&       0.01	& 0.084	& 0.111	& 0.507	& 0.474 \\
400	& 10	&         10	&       \LIN	&          -	& 0.528	& 0.500	& 0.547	& 0.785 \\
400	& 10	&         10	&       \RBF	&     0.0001	& 0.516	& 0.487	& 0.551	& 0.764 \\
400	& 10	&         10	&       \RBF	&      0.001	& 0.530	& 0.491	& 0.555	& 0.762 \\
400	& 10	&         10	&       \RBF	&       0.01	& 0.058	& 0.091	& 0.507	& 0.471 \\
400	& 10	&         50	&       \LIN	&          -	& 0.509	& 0.482	& 0.552	& 0.721 \\
400	& 10	&         50	&       \RBF	&     0.0001	& 0.516	& 0.487	& 0.551	& 0.764 \\
400	& 10	&         50	&       \RBF	&      0.001	& 0.530	& 0.491	& 0.555	& 0.762 \\
400	& 10	&         50	&       \RBF	&       0.01	& 0.049	& 0.084	& 0.505	& 0.469 \\
400	& 10	&        100	&       \LIN	&          -	& 0.509	& 0.475	& 0.552	& 0.688 \\
400	& 10	&        100	&       \RBF	&     0.0001	& 0.516	& 0.487	& 0.551	& 0.764 \\
400	& 10	&        100	&       \RBF	&      0.001	& 0.530	& 0.491	& 0.555	& 0.762 \\
400	& 10	&        100	&       \RBF	&       0.01	& 0.047	& 0.083	& 0.505	& 0.469 \\
400	& 15	&      0.001	&       \LIN	&          -	& 0.336	& 0.333	& 0.531	& 0.706 \\
400	& 15	&      0.001	&       \RBF	&     0.0001	& 0.520	& 0.491	& 0.552	& 0.771 \\
400	& 15	&      0.001	&       \RBF	&      0.001	& 0.527	& 0.490	& 0.554	& 0.760 \\
400	& 15	&      0.001	&       \RBF	&       0.01	& 0.235	& 0.249	& 0.512	& 0.528 \\
400	& 15	&       0.01	&       \LIN	&          -	& 0.421	& 0.409	& 0.550	& 0.762 \\
400	& 15	&       0.01	&       \RBF	&     0.0001	& 0.520	& 0.491	& 0.552	& 0.771 \\
400	& 15	&       0.01	&       \RBF	&      0.001	& 0.527	& 0.490	& 0.554	& 0.760 \\
400	& 15	&       0.01	&       \RBF	&       0.01	& 0.183	& 0.201	& 0.509	& 0.503 \\
400	& 15	&        0.1	&       \LIN	&          -	& 0.510	& 0.472	& 0.558	& 0.769 \\
400	& 15	&        0.1	&       \RBF	&     0.0001	& 0.520	& 0.491	& 0.552	& 0.771 \\
400	& 15	&        0.1	&       \RBF	&      0.001	& 0.527	& 0.490	& 0.554	& 0.760 \\
400	& 15	&        0.1	&       \RBF	&       0.01	& 0.135	& 0.158	& 0.509	& 0.485 \\
400	& 15	&        0.2	&       \LIN	&          -	& 0.497	& 0.464	& 0.555	& 0.769 \\
400	& 15	&        0.2	&       \RBF	&     0.0001	& 0.520	& 0.491	& 0.552	& 0.771 \\
400	& 15	&        0.2	&       \RBF	&      0.001	& 0.527	& 0.490	& 0.554	& 0.760 \\
400	& 15	&        0.2	&       \RBF	&       0.01	& 0.122	& 0.147	& 0.509	& 0.481 \\
400	& 15	&        0.4	&       \LIN	&          -	& 0.519	& 0.483	& 0.557	& 0.772 \\
400	& 15	&        0.4	&       \RBF	&     0.0001	& 0.520	& 0.491	& 0.552	& 0.771 \\
400	& 15	&        0.4	&       \RBF	&      0.001	& 0.527	& 0.490	& 0.554	& 0.760 \\
400	& 15	&        0.4	&       \RBF	&       0.01	& 0.108	& 0.133	& 0.508	& 0.478 \\
400	& 15	&        0.6	&       \LIN	&          -	& 0.491	& 0.469	& 0.557	& 0.773 \\
400	& 15	&        0.6	&       \RBF	&     0.0001	& 0.520	& 0.491	& 0.552	& 0.771 \\
400	& 15	&        0.6	&       \RBF	&      0.001	& 0.527	& 0.490	& 0.554	& 0.760 \\
400	& 15	&        0.6	&       \RBF	&       0.01	& 0.095	& 0.123	& 0.507	& 0.476 \\
400	& 15	&        0.8	&       \LIN	&          -	& 0.534	& 0.494	& 0.555	& 0.775 \\
400	& 15	&        0.8	&       \RBF	&     0.0001	& 0.520	& 0.491	& 0.552	& 0.771 \\
400	& 15	&        0.8	&       \RBF	&      0.001	& 0.527	& 0.490	& 0.554	& 0.760 \\
400	& 15	&        0.8	&       \RBF	&       0.01	& 0.093	& 0.120	& 0.508	& 0.475 \\
400	& 15	&        1.0	&       \LIN	&          -	& 0.512	& 0.472	& 0.555	& 0.774 \\
400	& 15	&        1.0	&       \RBF	&     0.0001	& 0.520	& 0.491	& 0.552	& 0.771 \\
400	& 15	&        1.0	&       \RBF	&      0.001	& 0.527	& 0.490	& 0.554	& 0.760 \\
400	& 15	&        1.0	&       \RBF	&       0.01	& 0.083	& 0.110	& 0.507	& 0.474 \\
400	& 15	&         10	&       \LIN	&          -	& 0.523	& 0.482	& 0.547	& 0.778 \\
400	& 15	&         10	&       \RBF	&     0.0001	& 0.520	& 0.491	& 0.552	& 0.771 \\
400	& 15	&         10	&       \RBF	&      0.001	& 0.527	& 0.490	& 0.554	& 0.760 \\
400	& 15	&         10	&       \RBF	&       0.01	& 0.057	& 0.091	& 0.506	& 0.471 \\
400	& 15	&         50	&       \LIN	&          -	& 0.532	& 0.501	& 0.552	& 0.743 \\
400	& 15	&         50	&       \RBF	&     0.0001	& 0.520	& 0.491	& 0.552	& 0.771 \\
400	& 15	&         50	&       \RBF	&      0.001	& 0.527	& 0.490	& 0.554	& 0.760 \\
400	& 15	&         50	&       \RBF	&       0.01	& 0.050	& 0.085	& 0.505	& 0.470 \\
400	& 15	&        100	&       \LIN	&          -	& 0.515	& 0.485	& 0.552	& 0.702 \\
400	& 15	&        100	&       \RBF	&     0.0001	& 0.520	& 0.491	& 0.552	& 0.771 \\
400	& 15	&        100	&       \RBF	&      0.001	& 0.527	& 0.490	& 0.554	& 0.760 \\
400	& 15	&        100	&       \RBF	&       0.01	& 0.049	& 0.084	& 0.504	& 0.469 \\


==> tables/holdout_5percent_baseline.tex <==
\begin{ThreePartTable}
    \begin{TableNotes}[flushleft]  %%% This should come before longtable and it is not tablenotes but TableNotes
  \small
  \item
    \begin{footnotesize}
        \bgroup
%        \def\arraystretch{0.5}%       
        \setstretch{1}
                The columns corresponding to ``$\alpha_b$'', ``$\beta_b$'',
                ``usim'', and ``$\sigma$'' have the
                two hyperparameters, cell line similarity function,
                and parameter for \hl{$\RBF$} cell line similarity, respectively, for \BMTMKL.
	      \par
              \egroup
    \end{footnotesize}
  \end{TableNotes}
  \begin{longtable}{
      @{\hspace{5pt}}>{\raggedleft}p{0.04\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.04\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.04\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{6pt}}
      @{\hspace{5pt}}>{\raggedleft\arraybackslash}p{0.10\textwidth}@{\hspace{6pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
    }
    \caption{\mbox{\BMTMKL Performance on New Cell Lines ($\theta$ = 5)}}
    \label{supp:tbl:holdout:5percent:BMTMKL}\\
  %
    \hline\hline
    n & $\alpha_b$ & $\beta_b$ & usim & $\sigma$ & \small{AP@$5$} & \small{AP@$10$} & \small{\rCI} & \small{\CI} \\
    \hline
    \endfirsthead
  %
    \multicolumn{9}{c}{{\tablename\ \thetable{} -- continued from previous page}}\\
    \hline\hline
    n & $\alpha_b$ & $\beta_b$ & usim & $\sigma$ & \small{AP@$5$} & \small{AP@$10$} & \small{\rCI} & \small{\CI} \\
    \hline
    \endhead
  %
    \hline
    %  \midrule
    \multicolumn{9}{c}{{Continued on next page}} \\
    \hline
    %\midrule
    \endfoot
    %
    \hline\hline
    %\bottomrule
    \insertTableNotes         %% this added
    \endlastfoot
    %
    \input{tables/holdout_5percent_baseline_data.tex}
	
    \hline
  \end{longtable}
\end{ThreePartTable}


==> tables/holdout_5percent_baseline_data.tex <==
100	& 1	& 1	& \RBF	& 10.0	& 0.943	& 0.909	& 0.646	& 0.800\\
100	& 1e-10	& 1e-10	& \RBF	& 10.0	& 0.945	& 0.908	& 0.646	& 0.800\\
100	& 1e-10	& 1e+10	& \RBF	& 10.0	& 0.943	& 0.909	& 0.646	& 0.800\\
150	& 1	& 1	& \RBF	& 10.0	& 0.946	& 0.911	& 0.649	& 0.800\\
150	& 1e-10	& 1e-10	& \RBF	& 10.0	& 0.944	& 0.912	& 0.649	& 0.800\\
150	& 1e-10	& 1e+10	& \RBF	& 10.0	& 0.945	& 0.912	& 0.649	& 0.800\\
200	& 1	& 1	& \RBF	& 10.0	& 0.937	& 0.907	& 0.650	& 0.800\\
200	& 1e-10	& 1e-10	& \RBF	& 10.0	& 0.936	& 0.907	& 0.650	& 0.800\\
200	& 1e-10	& 1e+10	& \RBF	& 10.0	& 0.937	& 0.907	& 0.650	& 0.800\\
250	& 1	& 1	& \RBF	& 10.0	& 0.939	& 0.908	& 0.653	& 0.802\\
250	& 1e-10	& 1e-10	& \RBF	& 10.0	& 0.939	& 0.908	& 0.653	& 0.802\\
250	& 1e-10	& 1e+10	& \RBF	& 10.0	& 0.940	& 0.908	& 0.653	& 0.802\\
300	& 1	& 1	& \RBF	& 10.0	& 0.937	& 0.906	& 0.652	& 0.801\\
300	& 1e-10	& 1e-10	& \RBF	& 10.0	& 0.937	& 0.906	& 0.651	& 0.802\\
300	& 1e-10	& 1e+10	& \RBF	& 10.0	& 0.937	& 0.906	& 0.651	& 0.801\\
350	& 1	& 1	& \RBF	& 10.0	& 0.935	& 0.903	& 0.648	& 0.800\\
350	& 1e-10	& 1e-10	& \RBF	& 10.0	& 0.935	& 0.903	& 0.648	& 0.799\\
350	& 1e-10	& 1e+10	& \RBF	& 10.0	& 0.935	& 0.903	& 0.648	& 0.800\\
400	& 1	& 1	& \RBF	& 10.0	& 0.938	& 0.905	& 0.651	& 0.800\\
400	& 1e-10	& 1e-10	& \RBF	& 10.0	& 0.938	& 0.906	& 0.651	& 0.800\\
400	& 1e-10	& 1e+10	& \RBF	& 10.0	& 0.938	& 0.906	& 0.651	& 0.800\\
50	& 1	& 1	& \RBF	& 10.0	& 0.951	& 0.903	& 0.637	& 0.804\\
50	& 1e-10	& 1e-10	& \RBF	& 10.0	& 0.951	& 0.903	& 0.637	& 0.804\\
50	& 1e-10	& 1e+10	& \RBF	& 10.0	& 0.951	& 0.903	& 0.636	& 0.804\\


==> tables/holdout_5percent_data.tex <==
50	& 5	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.963	& 0.910	& 0.639	& 0.674 \\ 
50	& 5	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.961	& 0.907	& 0.643	& 0.645 \\ 
50	& 5	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.955	& 0.901	& 0.643	& 0.741 \\ 
50	& 5	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.955	& 0.902	& 0.644	& 0.741 \\ 
50	& 5	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.963	& 0.900	& 0.635	& 0.678 \\ 
50	& 5	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.955	& 0.902	& 0.644	& 0.742 \\ 
50	& 5	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.955	& 0.901	& 0.647	& 0.758 \\ 
50	& 5	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.955	& 0.901	& 0.647	& 0.758 \\ 
50	& 5	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.955	& 0.895	& 0.640	& 0.792 \\ 
50	& 5	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.952	& 0.894	& 0.637	& 0.792 \\ 
50	& 10	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.962	& 0.905	& 0.638	& 0.680 \\ 
50	& 10	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.960	& 0.901	& 0.638	& 0.747 \\ 
50	& 10	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.965	& 0.902	& 0.638	& 0.681 \\ 
50	& 10	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.962	& 0.892	& 0.633	& 0.666 \\ 
50	& 10	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.964	& 0.898	& 0.632	& 0.679 \\ 
50	& 10	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.960	& 0.902	& 0.639	& 0.750 \\ 
50	& 10	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.961	& 0.900	& 0.633	& 0.693 \\ 
50	& 10	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.964	& 0.905	& 0.640	& 0.677 \\ 
50	& 10	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.953	& 0.900	& 0.625	& 0.792 \\ 
50	& 10	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.953	& 0.899	& 0.626	& 0.792 \\ 
50	& 15	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.964	& 0.907	& 0.641	& 0.685 \\ 
50	& 15	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.964	& 0.907	& 0.641	& 0.683 \\ 
50	& 15	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.965	& 0.908	& 0.641	& 0.689 \\ 
50	& 15	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.965	& 0.902	& 0.640	& 0.662 \\ 
50	& 15	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.959	& 0.905	& 0.642	& 0.754 \\ 
50	& 15	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.959	& 0.904	& 0.641	& 0.754 \\ 
50	& 15	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.960	& 0.897	& 0.641	& 0.693 \\ 
50	& 15	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.964	& 0.904	& 0.644	& 0.686 \\ 
50	& 15	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.955	& 0.901	& 0.633	& 0.792 \\ 
50	& 15	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.955	& 0.901	& 0.633	& 0.792 \\ 
100	& 5	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.952	& 0.910	& 0.651	& 0.671 \\ 
100	& 5	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.953	& 0.909	& 0.652	& 0.654 \\ 
100	& 5	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.950	& 0.904	& 0.651	& 0.740 \\ 
100	& 5	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.950	& 0.904	& 0.651	& 0.740 \\ 
100	& 5	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.950	& 0.905	& 0.651	& 0.742 \\ 
100	& 5	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.950	& 0.905	& 0.651	& 0.742 \\ 
100	& 5	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.949	& 0.905	& 0.652	& 0.757 \\ 
100	& 5	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.951	& 0.901	& 0.657	& 0.669 \\ 
100	& 5	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.946	& 0.895	& 0.643	& 0.788 \\ 
100	& 5	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.944	& 0.899	& 0.640	& 0.788 \\ 
100	& 10	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.956	& 0.909	& 0.652	& 0.678 \\ 
100	& 10	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.957	& 0.910	& 0.651	& 0.656 \\ 
100	& 10	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.957	& 0.907	& 0.651	& 0.677 \\ 
100	& 10	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.957	& 0.907	& 0.650	& 0.747 \\ 
100	& 10	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.957	& 0.906	& 0.650	& 0.749 \\ 
100	& 10	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.957	& 0.907	& 0.650	& 0.749 \\ 
100	& 10	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.954	& 0.907	& 0.649	& 0.763 \\ 
100	& 10	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.954	& 0.907	& 0.649	& 0.763 \\ 
100	& 10	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.954	& 0.902	& 0.639	& 0.788 \\ 
100	& 10	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.954	& 0.902	& 0.639	& 0.788 \\ 
100	& 15	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.958	& 0.908	& 0.651	& 0.750 \\ 
100	& 15	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.958	& 0.908	& 0.651	& 0.750 \\ 
100	& 15	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.958	& 0.908	& 0.651	& 0.751 \\ 
100	& 15	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.958	& 0.908	& 0.651	& 0.751 \\ 
100	& 15	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.958	& 0.908	& 0.654	& 0.690 \\ 
100	& 15	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.958	& 0.908	& 0.651	& 0.753 \\ 
100	& 15	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.952	& 0.907	& 0.651	& 0.766 \\ 
100	& 15	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.952	& 0.906	& 0.650	& 0.766 \\ 
100	& 15	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.947	& 0.896	& 0.640	& 0.787 \\ 
100	& 15	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.947	& 0.896	& 0.640	& 0.787 \\ 
150	& 5	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.951	& 0.910	& 0.655	& 0.671 \\ 
150	& 5	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.950	& 0.911	& 0.656	& 0.670 \\ 
150	& 5	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.950	& 0.908	& 0.656	& 0.675 \\ 
150	& 5	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.948	& 0.905	& 0.654	& 0.743 \\ 
150	& 5	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.947	& 0.905	& 0.654	& 0.745 \\ 
150	& 5	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.950	& 0.906	& 0.659	& 0.644 \\ 
150	& 5	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.948	& 0.900	& 0.661	& 0.665 \\ 
150	& 5	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.947	& 0.896	& 0.664	& 0.670 \\ 
150	& 5	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.946	& 0.895	& 0.642	& 0.789 \\ 
150	& 5	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.947	& 0.900	& 0.640	& 0.789 \\ 
150	& 10	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.952	& 0.908	& 0.655	& 0.679 \\ 
150	& 10	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.951	& 0.909	& 0.655	& 0.677 \\ 
150	& 10	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.951	& 0.907	& 0.656	& 0.683 \\ 
150	& 10	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.953	& 0.903	& 0.657	& 0.659 \\ 
150	& 10	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.950	& 0.905	& 0.652	& 0.752 \\ 
150	& 10	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.950	& 0.905	& 0.653	& 0.752 \\ 
150	& 10	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.952	& 0.907	& 0.651	& 0.766 \\ 
150	& 10	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.952	& 0.907	& 0.651	& 0.766 \\ 
150	& 10	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.949	& 0.903	& 0.641	& 0.789 \\ 
150	& 10	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.949	& 0.903	& 0.641	& 0.789 \\ 
150	& 15	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.955	& 0.908	& 0.654	& 0.753 \\ 
150	& 15	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.954	& 0.907	& 0.653	& 0.753 \\ 
150	& 15	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.954	& 0.908	& 0.654	& 0.755 \\ 
150	& 15	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.953	& 0.908	& 0.654	& 0.755 \\ 
150	& 15	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.953	& 0.908	& 0.654	& 0.756 \\ 
150	& 15	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.954	& 0.908	& 0.654	& 0.756 \\ 
150	& 15	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.951	& 0.907	& 0.653	& 0.769 \\ 
150	& 15	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.951	& 0.907	& 0.652	& 0.769 \\ 
150	& 15	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.945	& 0.900	& 0.643	& 0.789 \\ 
150	& 15	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.945	& 0.900	& 0.643	& 0.789 \\ 
200	& 5	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.943	& 0.907	& 0.656	& 0.671 \\ 
200	& 5	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.942	& 0.904	& 0.657	& 0.648 \\ 
200	& 5	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.940	& 0.902	& 0.656	& 0.746 \\ 
200	& 5	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.940	& 0.902	& 0.656	& 0.746 \\ 
200	& 5	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.943	& 0.900	& 0.658	& 0.665 \\ 
200	& 5	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.940	& 0.902	& 0.656	& 0.748 \\ 
200	& 5	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.940	& 0.902	& 0.657	& 0.763 \\ 
200	& 5	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.942	& 0.896	& 0.668	& 0.668 \\ 
200	& 5	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.937	& 0.897	& 0.646	& 0.790 \\ 
200	& 5	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.937	& 0.898	& 0.644	& 0.790 \\ 
200	& 10	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.946	& 0.906	& 0.656	& 0.680 \\ 
200	& 10	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.946	& 0.905	& 0.656	& 0.678 \\ 
200	& 10	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.947	& 0.906	& 0.657	& 0.684 \\ 
200	& 10	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.945	& 0.906	& 0.657	& 0.683 \\ 
200	& 10	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.944	& 0.903	& 0.654	& 0.755 \\ 
200	& 10	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.944	& 0.903	& 0.654	& 0.755 \\ 
200	& 10	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.944	& 0.901	& 0.653	& 0.768 \\ 
200	& 10	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.944	& 0.901	& 0.653	& 0.769 \\ 
200	& 10	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.937	& 0.893	& 0.644	& 0.790 \\ 
200	& 10	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.937	& 0.893	& 0.644	& 0.790 \\ 
200	& 15	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.948	& 0.907	& 0.657	& 0.685 \\ 
200	& 15	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.949	& 0.906	& 0.657	& 0.683 \\ 
200	& 15	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.947	& 0.906	& 0.659	& 0.690 \\ 
200	& 15	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.947	& 0.906	& 0.658	& 0.688 \\ 
200	& 15	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.946	& 0.905	& 0.659	& 0.693 \\ 
200	& 15	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.946	& 0.902	& 0.655	& 0.759 \\ 
200	& 15	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.944	& 0.900	& 0.653	& 0.771 \\ 
200	& 15	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.944	& 0.900	& 0.653	& 0.772 \\ 
200	& 15	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.935	& 0.891	& 0.644	& 0.790 \\ 
200	& 15	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.935	& 0.890	& 0.644	& 0.790 \\ 
250	& 5	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.945	& 0.908	& 0.659	& 0.671 \\ 
250	& 5	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.945	& 0.909	& 0.659	& 0.670 \\ 
250	& 5	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.944	& 0.906	& 0.660	& 0.675 \\ 
250	& 5	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.941	& 0.904	& 0.658	& 0.749 \\ 
250	& 5	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.944	& 0.906	& 0.662	& 0.676 \\ 
250	& 5	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.944	& 0.902	& 0.662	& 0.660 \\ 
250	& 5	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.943	& 0.899	& 0.663	& 0.682 \\ 
250	& 5	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.942	& 0.903	& 0.660	& 0.765 \\ 
250	& 5	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.940	& 0.900	& 0.649	& 0.792 \\ 
250	& 5	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.940	& 0.898	& 0.646	& 0.792 \\ 
250	& 10	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.947	& 0.900	& 0.651	& 0.783 \\ 
250	& 10	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.946	& 0.901	& 0.648	& 0.788 \\ 
250	& 10	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.946	& 0.900	& 0.648	& 0.788 \\ 
250	& 10	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.946	& 0.900	& 0.648	& 0.788 \\ 
250	& 10	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.946	& 0.900	& 0.648	& 0.788 \\ 
250	& 10	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.946	& 0.900	& 0.648	& 0.788 \\ 
250	& 10	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.947	& 0.903	& 0.656	& 0.771 \\ 
250	& 10	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.947	& 0.903	& 0.656	& 0.771 \\ 
250	& 10	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.944	& 0.899	& 0.646	& 0.792 \\ 
250	& 10	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.944	& 0.899	& 0.646	& 0.792 \\ 
250	& 15	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.949	& 0.904	& 0.657	& 0.759 \\ 
250	& 15	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.948	& 0.905	& 0.657	& 0.752 \\ 
250	& 15	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.949	& 0.904	& 0.656	& 0.761 \\ 
250	& 15	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.949	& 0.904	& 0.656	& 0.761 \\ 
250	& 15	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.949	& 0.904	& 0.656	& 0.762 \\ 
250	& 15	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.949	& 0.904	& 0.656	& 0.762 \\ 
250	& 15	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.946	& 0.903	& 0.656	& 0.774 \\ 
250	& 15	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.947	& 0.903	& 0.656	& 0.774 \\ 
250	& 15	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.937	& 0.895	& 0.647	& 0.791 \\ 
250	& 15	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.937	& 0.895	& 0.647	& 0.791 \\ 
300	& 5	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.944	& 0.908	& 0.658	& 0.673 \\ 
300	& 5	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.944	& 0.908	& 0.658	& 0.672 \\ 
300	& 5	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.940	& 0.905	& 0.656	& 0.751 \\ 
300	& 5	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.940	& 0.905	& 0.656	& 0.751 \\ 
300	& 5	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.940	& 0.904	& 0.657	& 0.753 \\ 
300	& 5	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.940	& 0.904	& 0.657	& 0.753 \\ 
300	& 5	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.939	& 0.903	& 0.658	& 0.767 \\ 
300	& 5	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.940	& 0.903	& 0.658	& 0.767 \\ 
300	& 5	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.939	& 0.899	& 0.647	& 0.792 \\ 
300	& 5	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.939	& 0.898	& 0.645	& 0.792 \\ 
300	& 10	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.946	& 0.907	& 0.658	& 0.683 \\ 
300	& 10	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.945	& 0.902	& 0.647	& 0.788 \\ 
300	& 10	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.945	& 0.908	& 0.659	& 0.687 \\ 
300	& 10	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.946	& 0.907	& 0.656	& 0.759 \\ 
300	& 10	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.947	& 0.907	& 0.655	& 0.760 \\ 
300	& 10	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.946	& 0.907	& 0.655	& 0.760 \\ 
300	& 10	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.946	& 0.904	& 0.654	& 0.773 \\ 
300	& 10	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.946	& 0.905	& 0.654	& 0.773 \\ 
300	& 10	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.941	& 0.900	& 0.644	& 0.792 \\ 
300	& 10	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.941	& 0.900	& 0.644	& 0.792 \\ 
300	& 15	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.948	& 0.906	& 0.656	& 0.762 \\ 
300	& 15	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.944	& 0.905	& 0.657	& 0.741 \\ 
300	& 15	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.947	& 0.905	& 0.656	& 0.763 \\ 
300	& 15	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.947	& 0.906	& 0.656	& 0.763 \\ 
300	& 15	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.948	& 0.908	& 0.660	& 0.697 \\ 
300	& 15	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.947	& 0.905	& 0.656	& 0.765 \\ 
300	& 15	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.948	& 0.907	& 0.655	& 0.776 \\ 
300	& 15	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.949	& 0.906	& 0.655	& 0.776 \\ 
300	& 15	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.938	& 0.897	& 0.647	& 0.792 \\ 
300	& 15	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.938	& 0.897	& 0.647	& 0.792 \\ 
350	& 5	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.941	& 0.902	& 0.655	& 0.675 \\ 
350	& 5	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.940	& 0.902	& 0.654	& 0.674 \\ 
350	& 5	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.941	& 0.902	& 0.656	& 0.679 \\ 
350	& 5	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.941	& 0.903	& 0.656	& 0.673 \\ 
350	& 5	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.940	& 0.901	& 0.657	& 0.682 \\ 
350	& 5	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.938	& 0.899	& 0.653	& 0.753 \\ 
350	& 5	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.937	& 0.900	& 0.654	& 0.767 \\ 
350	& 5	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.938	& 0.895	& 0.664	& 0.661 \\ 
350	& 5	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.934	& 0.893	& 0.644	& 0.790 \\ 
350	& 5	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.934	& 0.892	& 0.644	& 0.790 \\ 
350	& 10	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.942	& 0.902	& 0.655	& 0.685 \\ 
350	& 10	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.943	& 0.901	& 0.653	& 0.746 \\ 
350	& 10	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.943	& 0.903	& 0.656	& 0.689 \\ 
350	& 10	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.943	& 0.903	& 0.656	& 0.687 \\ 
350	& 10	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.942	& 0.902	& 0.658	& 0.692 \\ 
350	& 10	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.942	& 0.901	& 0.653	& 0.760 \\ 
350	& 10	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.943	& 0.900	& 0.652	& 0.773 \\ 
350	& 10	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.943	& 0.900	& 0.652	& 0.773 \\ 
350	& 10	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.939	& 0.895	& 0.643	& 0.791 \\ 
350	& 10	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.939	& 0.895	& 0.643	& 0.791 \\ 
350	& 15	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.946	& 0.900	& 0.653	& 0.763 \\ 
350	& 15	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.944	& 0.902	& 0.654	& 0.730 \\ 
350	& 15	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.945	& 0.904	& 0.656	& 0.695 \\ 
350	& 15	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.947	& 0.901	& 0.654	& 0.757 \\ 
350	& 15	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.945	& 0.903	& 0.657	& 0.699 \\ 
350	& 15	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.944	& 0.900	& 0.653	& 0.765 \\ 
350	& 15	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.942	& 0.900	& 0.654	& 0.776 \\ 
350	& 15	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.942	& 0.900	& 0.654	& 0.776 \\ 
350	& 15	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.936	& 0.892	& 0.646	& 0.790 \\ 
350	& 15	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.936	& 0.892	& 0.646	& 0.791 \\ 
400	& 5	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.943	& 0.904	& 0.658	& 0.676 \\ 
400	& 5	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.940	& 0.902	& 0.658	& 0.675 \\ 
400	& 5	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.943	& 0.904	& 0.660	& 0.680 \\ 
400	& 5	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.944	& 0.904	& 0.659	& 0.679 \\ 
400	& 5	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.942	& 0.904	& 0.661	& 0.681 \\ 
400	& 5	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.940	& 0.902	& 0.656	& 0.755 \\ 
400	& 5	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.938	& 0.898	& 0.649	& 0.789 \\ 
400	& 5	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.938	& 0.900	& 0.657	& 0.769 \\ 
400	& 5	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.938	& 0.897	& 0.647	& 0.791 \\ 
400	& 5	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.938	& 0.897	& 0.647	& 0.791 \\ 
400	& 10	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.944	& 0.904	& 0.655	& 0.760 \\ 
400	& 10	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.946	& 0.905	& 0.656	& 0.736 \\ 
400	& 10	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.944	& 0.905	& 0.660	& 0.690 \\ 
400	& 10	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.944	& 0.904	& 0.655	& 0.762 \\ 
400	& 10	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.945	& 0.905	& 0.655	& 0.763 \\ 
400	& 10	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.945	& 0.904	& 0.655	& 0.763 \\ 
400	& 10	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.945	& 0.902	& 0.655	& 0.775 \\ 
400	& 10	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.945	& 0.903	& 0.655	& 0.775 \\ 
400	& 10	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.941	& 0.898	& 0.647	& 0.792 \\ 
400	& 10	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.941	& 0.898	& 0.647	& 0.792 \\ 
400	& 15	& 0.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.944	& 0.905	& 0.659	& 0.694 \\ 
400	& 15	& 0.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.946	& 0.907	& 0.661	& 0.657 \\ 
400	& 15	& 0.05	& 0.1	&   10.0	& \RBF	& 10.0	& 0.946	& 0.906	& 0.660	& 0.697 \\ 
400	& 15	& 0.05	& 0.1	&  100.0	& \RBF	& 10.0	& 0.942	& 0.902	& 0.657	& 0.743 \\ 
400	& 15	& 0.10	& 0.1	&   10.0	& \RBF	& 10.0	& 0.947	& 0.906	& 0.661	& 0.701 \\ 
400	& 15	& 0.10	& 0.1	&  100.0	& \RBF	& 10.0	& 0.945	& 0.903	& 0.656	& 0.760 \\ 
400	& 15	& 0.50	& 0.1	&   10.0	& \RBF	& 10.0	& 0.944	& 0.901	& 0.656	& 0.778 \\ 
400	& 15	& 0.50	& 0.1	&  100.0	& \RBF	& 10.0	& 0.943	& 0.901	& 0.656	& 0.778 \\ 
400	& 15	& 1.00	& 0.1	&   10.0	& \RBF	& 10.0	& 0.937	& 0.893	& 0.649	& 0.792 \\ 
400	& 15	& 1.00	& 0.1	&  100.0	& \RBF	& 10.0	& 0.937	& 0.893	& 0.649	& 0.792 \\ 


==> tables/known_2percent.tex <==
\begin{ThreePartTable}
    \begin{TableNotes}[flushleft]  %%% This should come before longtable and it is not tablenotes but TableNotes
  \small
  \item
    \begin{footnotesize}
        \bgroup
%        \def\arraystretch{0.5}%       
        \setstretch{1}
		The columns corresponding to ``$l$'', ``$\alpha$'',
                ``$\beta$'', ``$\gamma$'', ``usim'', and ``$\sigma$'' have the
                latent dimension, weighting factor,
                latent vector regularization parameter,
                cell line similarity regularization parameter,
                cell line similarity function, and parameter for rbf cell line similarity,
                respectively, for \MTCRP.
	      \par
              \egroup
   \end{footnotesize}
  \end{TableNotes}
  \begin{longtable}{
      @{\hspace{5pt}}>{\raggedleft}p{0.03\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.03\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.03\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.04\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.03\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.03\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft\arraybackslash}p{0.06\textwidth}@{\hspace{7pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
    }
    \caption{\mbox{\MTCRP Performance on New and Known Drugs ($\theta$ = 2)}}
    \label{supp:tbl:transductive:2percent}\\
  %
    \hline\hline
    $l$	& $\alpha$	& $\beta$	& $\gamma$	& usim	& $\sigma$	& AP@$5$	& AH@$5$	& AP@$10$	& AH@$10$	& AT@$5$\% 	& AT@$10$\% 	& NT@$5$\% 	& NT@$10$\% \\
    \hline
    \endfirsthead
  %
    \multicolumn{14}{c}{{\tablename\ \thetable{} -- continued from previous page}}\\
    \hline\hline
    $l$ & $\alpha$      & $\beta$       & $\gamma$      & usim  & $\sigma$      & AP@$5$        & AH@$5$        & AP@$10$       & AH@$10$       & AT@$5$\%      & AT@$10$\%     & NT@$5$\%      & NT@$10$\% \\
    \hline
    \endhead
  %
    \hline
    %  \midrule
    \multicolumn{14}{c}{{Continued on next page}} \\
    \hline
    %\midrule
    \endfoot
    %
    \hline\hline
    %\bottomrule
    \insertTableNotes         %% this added
    \endlastfoot
    %
    \input{tables/known_2percent_data.tex}
	
    \hline
  \end{longtable}
\end{ThreePartTable}


==> tables/known_2percent_KRL.tex <==
\begin{ThreePartTable}
    \begin{TableNotes}[flushleft]  %%% This should come before longtable and it is not tablenotes but TableNotes
  \small
  \item
    \begin{footnotesize}
        \bgroup
%        \def\arraystretch{0.5}%       
        \setstretch{1}
                The columns corresponding to ``$k$'', ``$\lambda$'',
                ``usim'', and ``$\sigma$'' have the
                two hyperparameters, cell line similarity function,
                and parameter for {$\RBF$} cell line similarity, respectively, 
                for {\KRL}.
	      \par
              \egroup
   \end{footnotesize}
  \end{TableNotes}
  \begin{longtable}{
      @{\hspace{5pt}}>{\raggedleft}p{0.03\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.07\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.03\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft\arraybackslash}p{0.06\textwidth}@{\hspace{7pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
    }
    \caption{\mbox{\KRL Performance on New and Known Drugs ($\theta$ = 2)}}
    \label{supp:tbl:transductive:2percent:KRL}\\
  %
    \hline\hline
    $k$	& $\lambda$	& usim	& $\sigma$	& AP@$5$	& AH@$5$	& AP@$10$	& AH@$10$	& AT@$5$\% 	& AT@$10$\% 	& NT@$5$\% 	& NT@$10$\% \\
    \hline
    \endfirsthead
  %
    \multicolumn{12}{c}{{\tablename\ \thetable{} -- continued from previous page}}\\
    \hline\hline
    $k$ & $\lambda$     & usim  & $\sigma$      & AP@$5$        & AH@$5$        & AP@$10$       & AH@$10$       & AT@$5$\%      & AT@$10$\%     & NT@$5$\%      & NT@$10$\% \\
    \hline
    \endhead
  %
    \hline
    %  \midrule
    \multicolumn{12}{c}{{Continued on next page}} \\
    \hline
    %\midrule
    \endfoot
    %
    \hline\hline
    %\bottomrule
    \insertTableNotes         %% this added
    \endlastfoot
    %
    \input{tables/known_2percent_KRL_data.tex}
	
    \hline
  \end{longtable}
\end{ThreePartTable}


==> tables/known_2percent_KRL_data.tex <==
10	&   0.000001	&       \LIN	&          -	& 0.667	& 2.229	& 0.606	& 3.779	& 41.174	& 40.814	& 34.874	& 42.071 \\
10	&   0.000001	&       \RBF	&     0.0001	& 0.839	& 3.206	& 0.770	& 4.940	& 45.632	& 51.881	& 45.546	& 52.282 \\
10	&   0.000001	&       \RBF	&      0.001	& 0.879	& 3.591	& 0.813	& 5.745	& 55.059	& 59.932	& 43.333	& 51.916 \\
10	&   0.000001	&       \RBF	&       0.01	& 1.000	& 4.907	& 0.997	& 7.976	& 78.879	& 78.239	&  3.426	& 28.513 \\
10	&    0.00001	&       \LIN	&          -	& 0.714	& 2.579	& 0.647	& 4.370	& 43.566	& 46.358	& 40.638	& 46.850 \\
10	&    0.00001	&       \RBF	&     0.0001	& 0.839	& 3.206	& 0.770	& 4.940	& 45.632	& 51.881	& 45.546	& 52.282 \\
10	&    0.00001	&       \RBF	&      0.001	& 0.879	& 3.591	& 0.813	& 5.745	& 55.059	& 59.932	& 43.333	& 51.916 \\
10	&    0.00001	&       \RBF	&       0.01	& 1.000	& 4.906	& 0.997	& 7.957	& 78.821	& 77.973	&  3.339	& 27.476 \\
10	&     0.0001	&       \LIN	&          -	& 0.725	& 2.653	& 0.656	& 4.760	& 41.354	& 50.168	& 41.232	& 51.010 \\
10	&     0.0001	&       \RBF	&     0.0001	& 0.839	& 3.206	& 0.770	& 4.940	& 45.632	& 51.881	& 45.546	& 52.282 \\
10	&     0.0001	&       \RBF	&      0.001	& 0.879	& 3.591	& 0.813	& 5.745	& 55.059	& 59.932	& 43.333	& 51.916 \\
10	&     0.0001	&       \RBF	&       0.01	& 1.000	& 4.906	& 0.997	& 7.918	& 78.840	& 77.464	&  3.353	& 25.385 \\
10	&      0.001	&       \LIN	&          -	& 0.759	& 2.499	& 0.657	& 4.792	& 37.666	& 50.417	& 37.735	& 51.150 \\
10	&      0.001	&       \RBF	&     0.0001	& 0.839	& 3.206	& 0.770	& 4.940	& 45.632	& 51.881	& 45.546	& 52.282 \\
10	&      0.001	&       \RBF	&      0.001	& 0.879	& 3.591	& 0.813	& 5.745	& 55.059	& 59.932	& 43.333	& 51.916 \\
10	&      0.001	&       \RBF	&       0.01	& 1.000	& 4.905	& 0.998	& 7.860	& 78.801	& 76.673	&  3.280	& 22.605 \\
10	&       0.01	&       \LIN	&          -	& 0.783	& 2.664	& 0.686	& 4.831	& 39.669	& 50.853	& 40.088	& 51.364 \\
10	&       0.01	&       \RBF	&     0.0001	& 0.839	& 3.206	& 0.770	& 4.940	& 45.632	& 51.881	& 45.546	& 52.282 \\
10	&       0.01	&       \RBF	&      0.001	& 0.879	& 3.591	& 0.813	& 5.745	& 55.059	& 59.932	& 43.333	& 51.916 \\
10	&       0.01	&       \RBF	&       0.01	& 1.000	& 4.904	& 0.998	& 7.778	& 78.733	& 75.613	&  3.135	& 18.388 \\
10	&        0.1	&       \LIN	&          -	& 0.834	& 3.188	& 0.766	& 4.900	& 45.549	& 51.508	& 45.911	& 51.949 \\
10	&        0.1	&       \RBF	&     0.0001	& 0.839	& 3.206	& 0.770	& 4.940	& 45.632	& 51.881	& 45.546	& 52.282 \\
10	&        0.1	&       \RBF	&      0.001	& 0.879	& 3.591	& 0.813	& 5.745	& 55.059	& 59.932	& 43.333	& 51.916 \\
10	&        0.1	&       \RBF	&       0.01	& 1.000	& 4.904	& 0.999	& 7.700	& 78.684	& 74.512	&  3.013	& 14.353 \\
10	&        0.2	&       \LIN	&          -	& 0.834	& 3.188	& 0.764	& 4.914	& 45.559	& 51.605	& 45.947	& 51.899 \\
10	&        0.2	&       \RBF	&     0.0001	& 0.839	& 3.206	& 0.770	& 4.940	& 45.632	& 51.881	& 45.546	& 52.282 \\
10	&        0.2	&       \RBF	&      0.001	& 0.879	& 3.591	& 0.813	& 5.745	& 55.059	& 59.932	& 43.333	& 51.916 \\
10	&        0.2	&       \RBF	&       0.01	& 1.000	& 4.904	& 0.999	& 7.670	& 78.675	& 74.112	&  3.007	& 12.668 \\
10	&        0.4	&       \LIN	&          -	& 0.834	& 3.188	& 0.764	& 4.914	& 45.559	& 51.605	& 45.947	& 51.899 \\
10	&        0.4	&       \RBF	&     0.0001	& 0.839	& 3.206	& 0.770	& 4.940	& 45.632	& 51.881	& 45.546	& 52.282 \\
10	&        0.4	&       \RBF	&      0.001	& 0.879	& 3.591	& 0.813	& 5.745	& 55.059	& 59.932	& 43.333	& 51.916 \\
10	&        0.4	&       \RBF	&       0.01	& 1.000	& 4.903	& 0.999	& 7.637	& 78.650	& 73.664	&  2.927	& 11.007 \\
10	&        0.6	&       \LIN	&          -	& 0.834	& 3.188	& 0.764	& 4.914	& 45.559	& 51.605	& 45.947	& 51.899 \\
10	&        0.6	&       \RBF	&     0.0001	& 0.839	& 3.206	& 0.770	& 4.940	& 45.632	& 51.881	& 45.546	& 52.282 \\
10	&        0.6	&       \RBF	&      0.001	& 0.879	& 3.591	& 0.813	& 5.745	& 55.059	& 59.932	& 43.333	& 51.916 \\
10	&        0.6	&       \RBF	&       0.01	& 1.000	& 4.903	& 0.999	& 7.622	& 78.631	& 73.462	&  2.816	& 10.211 \\
10	&        0.8	&       \LIN	&          -	& 0.834	& 3.188	& 0.764	& 4.914	& 45.559	& 51.605	& 45.947	& 51.899 \\
10	&        0.8	&       \RBF	&     0.0001	& 0.839	& 3.206	& 0.770	& 4.940	& 45.632	& 51.881	& 45.546	& 52.282 \\
10	&        0.8	&       \RBF	&      0.001	& 0.879	& 3.591	& 0.813	& 5.745	& 55.059	& 59.932	& 43.333	& 51.916 \\
10	&        0.8	&       \RBF	&       0.01	& 1.000	& 4.902	& 0.999	& 7.614	& 78.616	& 73.320	&  2.779	&  9.660 \\
10	&        1.0	&       \LIN	&          -	& 0.834	& 3.188	& 0.764	& 4.914	& 45.559	& 51.605	& 45.947	& 51.899 \\
10	&        1.0	&       \RBF	&     0.0001	& 0.839	& 3.206	& 0.770	& 4.940	& 45.632	& 51.881	& 45.546	& 52.282 \\
10	&        1.0	&       \RBF	&      0.001	& 0.879	& 3.591	& 0.813	& 5.745	& 55.059	& 59.932	& 43.333	& 51.916 \\
10	&        1.0	&       \RBF	&       0.01	& 1.000	& 4.902	& 0.999	& 7.602	& 78.616	& 73.199	&  2.757	&  9.093 \\
10	&         10	&       \LIN	&          -	& 0.834	& 3.190	& 0.768	& 4.903	& 45.617	& 51.496	& 45.939	& 51.779 \\
10	&         10	&       \RBF	&     0.0001	& 0.839	& 3.206	& 0.770	& 4.940	& 45.632	& 51.881	& 45.546	& 52.282 \\
10	&         10	&       \RBF	&      0.001	& 0.879	& 3.591	& 0.813	& 5.745	& 55.059	& 59.932	& 43.333	& 51.916 \\
10	&         10	&       \RBF	&       0.01	& 1.000	& 4.900	& 0.999	& 7.551	& 78.533	& 72.512	&  2.500	&  6.188 \\
10	&         50	&       \LIN	&          -	& 0.835	& 3.190	& 0.770	& 4.896	& 45.637	& 51.440	& 45.993	& 51.818 \\
10	&         50	&       \RBF	&     0.0001	& 0.839	& 3.206	& 0.770	& 4.940	& 45.632	& 51.881	& 45.546	& 52.282 \\
10	&         50	&       \RBF	&      0.001	& 0.879	& 3.591	& 0.813	& 5.745	& 55.059	& 59.937	& 43.333	& 51.916 \\
10	&         50	&       \RBF	&       0.01	& 1.000	& 4.900	& 0.999	& 7.530	& 78.514	& 72.249	&  2.495	&  5.103 \\
10	&        100	&       \LIN	&          -	& 0.835	& 3.190	& 0.770	& 4.896	& 45.637	& 51.440	& 45.993	& 51.809 \\
10	&        100	&       \RBF	&     0.0001	& 0.839	& 3.206	& 0.770	& 4.940	& 45.632	& 51.881	& 45.546	& 52.282 \\
10	&        100	&       \RBF	&      0.001	& 0.879	& 3.591	& 0.813	& 5.745	& 55.059	& 59.932	& 43.333	& 51.916 \\
10	&        100	&       \RBF	&       0.01	& 1.000	& 4.901	& 0.999	& 7.524	& 78.524	& 72.173	&  2.507	&  4.812 \\


==> tables/known_2percent_baseline.tex <==
\begin{ThreePartTable}
    \begin{TableNotes}[flushleft]  %%% This should come before longtable and it is not tablenotes but TableNotes
  \small
  \item
    \begin{footnotesize}
        \bgroup
%        \def\arraystretch{0.5}%       
        \setstretch{1}
                The columns corresponding to ``$\alpha_b$'', ``$\beta_b$'',
                ``usim'', and ``$\sigma$'' have the
                two hyperparameters, cell line similarity function,
                and parameter for \hl{$\RBF$} cell line similarity, respectively, for \BMTMKL.
	      \par
              \egroup
   \end{footnotesize}
  \end{TableNotes}
  \begin{longtable}{
      @{\hspace{5pt}}>{\raggedleft}p{0.05\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.05\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.05\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.05\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft\arraybackslash}p{0.06\textwidth}@{\hspace{7pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
    }
    \caption{\mbox{\BMTMKL Performance on New and Known Drugs ($\theta$ = 2)}}
    \label{supp:tbl:transductive:2percent:baseline}\\
  %
    \hline\hline
    $\alpha_b$	& $\beta_b$	& usim	& $\sigma$	& AP@$5$	& AH@$5$	& AP@$10$	& AH@$10$	& AT@$5$\% 	& AT@$10$\% 	& NT@$5$\% 	& NT@$10$\% \\
    \hline
    \endfirsthead
  %
    \multicolumn{12}{c}{{\tablename\ \thetable{} -- continued from previous page}}\\
    \hline\hline
    $\alpha_b$  & $\beta_b$     & usim  & $\sigma$      & AP@$5$        & AH@$5$        & AP@$10$       & AH@$10$       & AT@$5$\%      & AT@$10$\%     & NT@$5$\%      & NT@$10$\% \\
    \hline
    \endhead
  %
    \hline
    %  \midrule
    \multicolumn{12}{c}{{Continued on next page}} \\
    \hline
    %\midrule
    \endfoot
    %
    \hline\hline
    %\bottomrule
    \insertTableNotes         %% this added
    \endlastfoot
    %
    \input{tables/known_2percent_baseline_data.tex}
	
    \hline
  \end{longtable}
\end{ThreePartTable}


==> tables/known_2percent_baseline_data.tex <==
1e0	& 1e0	& \RBF	& 10.0	& 0.850	& 0.789	& 3.346	& 5.175	& 48.03	& 54.57	& 47.57	& 54.00 \\
1e-10	& 1e10	& \RBF	& 10.0	& 0.850	& 0.789	& 3.347	& 5.174	& 48.03	& 54.55	& 47.61	& 54.00 \\
1e-10	& 1e-10	& \RBF	& 10.0	& 0.849	& 0.789	& 3.343	& 5.169	& 47.99	& 54.49	& 47.62	& 54.01 \\
1e0	& 1e0	& \COS	& - 	& 0.836	& 0.776	& 3.169	& 5.022	& 45.49	& 53.01	& 45.41	& 52.47 \\
1e-10	& 1e10	& \COS	& - 	& 0.836	& 0.776	& 3.183	& 5.051	& 45.74	& 53.31	& 45.71	& 52.76 \\
1e-10	& 1e-10	& \COS	& - 	& 0.834	& 0.777	& 3.176	& 5.033	& 45.54	& 53.17	& 45.65	& 52.69 \\


==> tables/known_2percent_data.tex <==
5 & 0.0 & 0.1 & 0.0 & \COS & - & 0.861 & 3.407 & 0.794 & 5.538 & 49.466 & 58.356 & 46.393 & 55.579 \\
5 & 0.0 & 0.1 & 0.0 & \RBF & 10.0 & 0.861 & 3.407 & 0.794 & 5.538 & 49.466 & 58.356 & 46.393 & 55.579 \\
5 & 0.0 & 0.1 & 1.0 & \COS & - & 0.861 & 3.407 & 0.794 & 5.538 & 49.466 & 58.358 & 46.393 & 55.588 \\
5 & 0.0 & 0.1 & 1.0 & \RBF & 10.0 & 0.861 & 3.407 & 0.794 & 5.538 & 49.466 & 58.358 & 46.393 & 55.588 \\
5 & 0.0 & 0.1 & 10.0 & \COS & - & 0.861 & 3.407 & 0.794 & 5.539 & 49.457 & 58.368 & 46.393 & 55.601 \\
5 & 0.0 & 0.1 & 10.0 & \RBF & 10.0 & 0.861 & 3.407 & 0.794 & 5.539 & 49.457 & 58.368 & 46.393 & 55.601 \\
5 & 0.0 & 0.1 & 100.0 & \COS & - & 0.861 & 3.407 & 0.794 & 5.543 & 49.452 & 58.385 & 46.382 & 55.523 \\
5 & 0.0 & 0.1 & 100.0 & \RBF & 10.0 & 0.861 & 3.406 & 0.794 & 5.543 & 49.457 & 58.400 & 46.382 & 55.555 \\
5 & 0.0 & 1.0 & 0.0 & \COS & - & 0.861 & 3.408 & 0.794 & 5.545 & 49.486 & 58.419 & 46.340 & 55.551 \\
5 & 0.0 & 1.0 & 0.0 & \RBF & 10.0 & 0.861 & 3.408 & 0.794 & 5.545 & 49.486 & 58.419 & 46.340 & 55.551 \\
5 & 0.0 & 1.0 & 1.0 & \COS & - & 0.861 & 3.408 & 0.794 & 5.545 & 49.486 & 58.419 & 46.340 & 55.551 \\
5 & 0.0 & 1.0 & 1.0 & \RBF & 10.0 & 0.861 & 3.408 & 0.794 & 5.545 & 49.486 & 58.419 & 46.340 & 55.551 \\
5 & 0.0 & 1.0 & 10.0 & \COS & - & 0.904 & 3.747 & 0.844 & 5.813 & 54.616 & 61.174 & 28.122 & 34.103 \\
5 & 0.0 & 1.0 & 10.0 & \RBF & 10.0 & 0.904 & 3.747 & 0.844 & 5.813 & 54.616 & 61.174 & 28.122 & 34.103 \\
5 & 0.0 & 1.0 & 100.0 & \COS & - & 0.861 & 3.407 & 0.794 & 5.543 & 49.452 & 58.382 & 46.382 & 55.523 \\
5 & 0.0 & 1.0 & 100.0 & \RBF & 10.0 & 0.861 & 3.406 & 0.794 & 5.543 & 49.457 & 58.400 & 46.382 & 55.555 \\
5 & 0.05 & 0.1 & 0.0 & \COS & - & 0.896 & 3.646 & 0.830 & 5.718 & 58.329 & 60.875 & 29.102 & 36.774 \\
5 & 0.05 & 0.1 & 0.0 & \RBF & 10.0 & 0.896 & 3.646 & 0.830 & 5.718 & 58.329 & 60.875 & 29.102 & 36.774 \\
5 & 0.05 & 0.1 & 1.0 & \COS & - & 0.896 & 3.646 & 0.830 & 5.717 & 58.329 & 60.875 & 29.115 & 36.801 \\
5 & 0.05 & 0.1 & 1.0 & \RBF & 10.0 & 0.896 & 3.646 & 0.830 & 5.717 & 58.329 & 60.875 & 29.115 & 36.787 \\
5 & 0.05 & 0.1 & 10.0 & \COS & - & 0.895 & 3.644 & 0.830 & 5.717 & 58.295 & 60.862 & 29.152 & 36.910 \\
5 & 0.05 & 0.1 & 10.0 & \RBF & 10.0 & 0.896 & 3.644 & 0.830 & 5.717 & 58.300 & 60.870 & 29.152 & 36.910 \\
5 & 0.05 & 0.1 & 100.0 & \COS & - & 0.892 & 3.613 & 0.825 & 5.698 & 57.822 & 60.626 & 30.146 & 38.156 \\
5 & 0.05 & 0.1 & 100.0 & \RBF & 10.0 & 0.892 & 3.617 & 0.825 & 5.704 & 57.890 & 60.714 & 30.017 & 38.035 \\
5 & 0.05 & 1.0 & 0.0 & \COS & - & 0.896 & 3.651 & 0.831 & 5.727 & 58.197 & 60.977 & 28.814 & 36.231 \\
5 & 0.05 & 1.0 & 0.0 & \RBF & 10.0 & 0.896 & 3.651 & 0.831 & 5.727 & 58.197 & 60.977 & 28.814 & 36.231 \\
5 & 0.05 & 1.0 & 1.0 & \COS & - & 0.896 & 3.650 & 0.831 & 5.725 & 58.178 & 60.965 & 28.807 & 36.147 \\
5 & 0.05 & 1.0 & 1.0 & \RBF & 10.0 & 0.896 & 3.650 & 0.831 & 5.725 & 58.178 & 60.962 & 28.807 & 36.175 \\
5 & 0.05 & 1.0 & 10.0 & \COS & - & 0.897 & 3.654 & 0.831 & 5.727 & 58.076 & 60.958 & 28.708 & 35.768 \\
5 & 0.05 & 1.0 & 10.0 & \RBF & 10.0 & 0.896 & 3.654 & 0.831 & 5.728 & 58.085 & 60.962 & 28.708 & 35.823 \\
5 & 0.05 & 1.0 & 100.0 & \COS & - & 0.892 & 3.620 & 0.826 & 5.704 & 57.837 & 60.690 & 29.915 & 37.625 \\
5 & 0.05 & 1.0 & 100.0 & \RBF & 10.0 & 0.894 & 3.634 & 0.828 & 5.710 & 57.837 & 60.753 & 29.122 & 36.714 \\
5 & 0.1 & 0.1 & 0.0 & \COS & - & 0.861 & 3.415 & 0.795 & 5.550 & 49.842 & 58.499 & 46.536 & 55.614 \\
5 & 0.1 & 0.1 & 0.0 & \RBF & 10.0 & 0.861 & 3.415 & 0.795 & 5.550 & 49.842 & 58.499 & 46.536 & 55.614 \\
5 & 0.1 & 0.1 & 1.0 & \COS & - & 0.861 & 3.415 & 0.795 & 5.550 & 49.842 & 58.495 & 46.536 & 55.614 \\
5 & 0.1 & 0.1 & 1.0 & \RBF & 10.0 & 0.861 & 3.415 & 0.795 & 5.550 & 49.842 & 58.495 & 46.536 & 55.614 \\
5 & 0.1 & 0.1 & 10.0 & \COS & - & 0.861 & 3.414 & 0.795 & 5.550 & 49.842 & 58.504 & 46.554 & 55.614 \\
5 & 0.1 & 0.1 & 10.0 & \RBF & 10.0 & 0.861 & 3.414 & 0.795 & 5.550 & 49.837 & 58.502 & 46.536 & 55.614 \\
5 & 0.1 & 0.1 & 100.0 & \COS & - & 0.861 & 3.413 & 0.795 & 5.547 & 49.837 & 58.463 & 46.645 & 55.572 \\
5 & 0.1 & 0.1 & 100.0 & \RBF & 10.0 & 0.861 & 3.413 & 0.795 & 5.548 & 49.841 & 58.468 & 46.645 & 55.577 \\
5 & 0.1 & 1.0 & 0.0 & \COS & - & 0.861 & 3.415 & 0.795 & 5.550 & 49.842 & 58.499 & 46.536 & 55.614 \\
5 & 0.1 & 1.0 & 0.0 & \RBF & 10.0 & 0.861 & 3.415 & 0.795 & 5.550 & 49.842 & 58.499 & 46.536 & 55.614 \\
5 & 0.1 & 1.0 & 1.0 & \COS & - & 0.861 & 3.415 & 0.795 & 5.550 & 49.842 & 58.497 & 46.554 & 55.614 \\
5 & 0.1 & 1.0 & 1.0 & \RBF & 10.0 & 0.861 & 3.415 & 0.795 & 5.550 & 49.842 & 58.497 & 46.554 & 55.614 \\
5 & 0.1 & 1.0 & 10.0 & \COS & - & 0.861 & 3.414 & 0.795 & 5.550 & 49.842 & 58.504 & 46.554 & 55.614 \\
5 & 0.1 & 1.0 & 10.0 & \RBF & 10.0 & 0.861 & 3.414 & 0.795 & 5.550 & 49.837 & 58.502 & 46.536 & 55.614 \\
5 & 0.1 & 1.0 & 100.0 & \COS & - & 0.861 & 3.413 & 0.795 & 5.547 & 49.837 & 58.460 & 46.645 & 55.572 \\
5 & 0.1 & 1.0 & 100.0 & \RBF & 10.0 & 0.861 & 3.413 & 0.795 & 5.548 & 49.841 & 58.468 & 46.645 & 55.577 \\
5 & 0.5 & 0.1 & 0.0 & \COS & - & 0.861 & 3.427 & 0.796 & 5.554 & 50.996 & 58.573 & 45.824 & 55.035 \\
5 & 0.5 & 0.1 & 0.0 & \RBF & 10.0 & 0.861 & 3.427 & 0.796 & 5.554 & 50.996 & 58.573 & 45.824 & 55.035 \\
5 & 0.5 & 0.1 & 1.0 & \COS & - & 0.861 & 3.427 & 0.796 & 5.554 & 51.001 & 58.575 & 45.824 & 55.048 \\
5 & 0.5 & 0.1 & 1.0 & \RBF & 10.0 & 0.861 & 3.427 & 0.796 & 5.554 & 51.001 & 58.575 & 45.824 & 55.048 \\
5 & 0.5 & 0.1 & 10.0 & \COS & - & 0.861 & 3.426 & 0.796 & 5.555 & 51.001 & 58.580 & 45.861 & 55.051 \\
5 & 0.5 & 0.1 & 10.0 & \RBF & 10.0 & 0.861 & 3.426 & 0.796 & 5.555 & 50.996 & 58.577 & 45.861 & 55.051 \\
5 & 0.5 & 0.1 & 100.0 & \COS & - & 0.862 & 3.424 & 0.796 & 5.552 & 50.943 & 58.548 & 45.826 & 54.928 \\
5 & 0.5 & 0.1 & 100.0 & \RBF & 10.0 & 0.862 & 3.425 & 0.796 & 5.554 & 50.957 & 58.563 & 45.826 & 54.972 \\
5 & 0.5 & 1.0 & 0.0 & \COS & - & 0.861 & 3.427 & 0.796 & 5.554 & 51.001 & 58.575 & 45.824 & 55.048 \\
5 & 0.5 & 1.0 & 0.0 & \RBF & 10.0 & 0.861 & 3.427 & 0.796 & 5.554 & 51.001 & 58.575 & 45.824 & 55.048 \\
5 & 0.5 & 1.0 & 1.0 & \COS & - & 0.861 & 3.427 & 0.796 & 5.554 & 51.001 & 58.575 & 45.824 & 55.048 \\
5 & 0.5 & 1.0 & 1.0 & \RBF & 10.0 & 0.861 & 3.427 & 0.796 & 5.554 & 51.001 & 58.575 & 45.824 & 55.048 \\
5 & 0.5 & 1.0 & 10.0 & \COS & - & 0.861 & 3.426 & 0.796 & 5.555 & 51.001 & 58.580 & 45.861 & 55.051 \\
5 & 0.5 & 1.0 & 10.0 & \RBF & 10.0 & 0.861 & 3.426 & 0.796 & 5.555 & 50.996 & 58.582 & 45.861 & 55.051 \\
5 & 0.5 & 1.0 & 100.0 & \COS & - & 0.862 & 3.424 & 0.796 & 5.552 & 50.943 & 58.546 & 45.826 & 54.928 \\
5 & 0.5 & 1.0 & 100.0 & \RBF & 10.0 & 0.862 & 3.425 & 0.796 & 5.554 & 50.953 & 58.563 & 45.826 & 54.972 \\
5 & 1.0 & 0.1 & 0.0 & \COS & - & 0.619 & 2.042 & 0.573 & 3.189 & 37.998 & 34.319 & 31.936 & 33.519 \\
5 & 1.0 & 0.1 & 0.0 & \RBF & 10.0 & 0.619 & 2.042 & 0.573 & 3.189 & 37.998 & 34.319 & 31.936 & 33.519 \\
5 & 1.0 & 0.1 & 1.0 & \COS & - & 0.627 & 2.070 & 0.580 & 3.222 & 38.499 & 34.718 & 32.466 & 33.688 \\
5 & 1.0 & 0.1 & 1.0 & \RBF & 10.0 & 0.621 & 2.043 & 0.574 & 3.192 & 37.988 & 34.402 & 32.023 & 33.467 \\
5 & 1.0 & 0.1 & 10.0 & \COS & - & 0.640 & 2.146 & 0.592 & 3.317 & 39.956 & 35.727 & 32.980 & 34.300 \\
5 & 1.0 & 0.1 & 10.0 & \RBF & 10.0 & 0.640 & 2.139 & 0.590 & 3.311 & 39.849 & 35.656 & 32.944 & 34.190 \\
5 & 1.0 & 0.1 & 100.0 & \COS & - & 0.670 & 2.294 & 0.619 & 3.552 & 42.631 & 38.202 & 34.129 & 37.010 \\
5 & 1.0 & 0.1 & 100.0 & \RBF & 10.0 & 0.679 & 2.355 & 0.627 & 3.629 & 43.810 & 39.023 & 34.904 & 37.408 \\
5 & 1.0 & 1.0 & 0.0 & \COS & - & 0.629 & 2.082 & 0.582 & 3.244 & 38.748 & 34.938 & 32.490 & 33.864 \\
5 & 1.0 & 1.0 & 0.0 & \RBF & 10.0 & 0.629 & 2.082 & 0.582 & 3.244 & 38.748 & 34.938 & 32.490 & 33.864 \\
5 & 1.0 & 1.0 & 1.0 & \COS & - & 0.631 & 2.092 & 0.583 & 3.253 & 38.938 & 35.035 & 32.550 & 33.926 \\
5 & 1.0 & 1.0 & 1.0 & \RBF & 10.0 & 0.628 & 2.076 & 0.580 & 3.236 & 38.650 & 34.836 & 32.410 & 33.827 \\
5 & 1.0 & 1.0 & 10.0 & \COS & - & 0.646 & 2.166 & 0.596 & 3.355 & 40.365 & 36.127 & 33.062 & 34.737 \\
5 & 1.0 & 1.0 & 10.0 & \RBF & 10.0 & 0.642 & 2.149 & 0.593 & 3.322 & 40.015 & 35.793 & 32.957 & 34.575 \\
5 & 1.0 & 1.0 & 100.0 & \COS & - & 0.669 & 2.302 & 0.619 & 3.552 & 42.777 & 38.202 & 34.473 & 36.991 \\
5 & 1.0 & 1.0 & 100.0 & \RBF & 10.0 & 0.680 & 2.356 & 0.628 & 3.635 & 43.820 & 39.084 & 34.737 & 37.409 \\
10 & 0.0 & 0.1 & 0.0 & \COS & - & 0.885 & 3.612 & 0.821 & 5.795 & 52.892 & 60.999 & 38.648 & 52.046 \\
10 & 0.0 & 0.1 & 0.0 & \RBF & 10.0 & 0.885 & 3.612 & 0.821 & 5.795 & 52.892 & 60.999 & 38.648 & 52.046 \\
10 & 0.0 & 0.1 & 1.0 & \COS & - & 0.885 & 3.612 & 0.821 & 5.795 & 52.887 & 60.999 & 38.648 & 52.051 \\
10 & 0.0 & 0.1 & 1.0 & \RBF & 10.0 & 0.885 & 3.612 & 0.821 & 5.795 & 52.887 & 60.999 & 38.648 & 52.046 \\
10 & 0.0 & 0.1 & 10.0 & \COS & - & 0.885 & 3.612 & 0.821 & 5.796 & 52.887 & 61.011 & 38.704 & 52.103 \\
10 & 0.0 & 0.1 & 10.0 & \RBF & 10.0 & 0.885 & 3.612 & 0.821 & 5.796 & 52.892 & 61.008 & 38.667 & 52.097 \\
10 & 0.0 & 0.1 & 100.0 & \COS & - & 0.882 & 3.591 & 0.819 & 5.777 & 52.609 & 60.740 & 40.469 & 53.495 \\
10 & 0.0 & 0.1 & 100.0 & \RBF & 10.0 & 0.883 & 3.596 & 0.819 & 5.785 & 52.667 & 60.836 & 39.903 & 53.061 \\
10 & 0.0 & 1.0 & 0.0 & \COS & - & 0.885 & 3.614 & 0.821 & 5.798 & 52.862 & 61.050 & 37.776 & 51.578 \\
10 & 0.0 & 1.0 & 0.0 & \RBF & 10.0 & 0.885 & 3.614 & 0.821 & 5.798 & 52.862 & 61.050 & 37.776 & 51.578 \\
10 & 0.0 & 1.0 & 1.0 & \COS & - & 0.885 & 3.614 & 0.821 & 5.798 & 52.862 & 61.050 & 37.813 & 51.578 \\
10 & 0.0 & 1.0 & 1.0 & \RBF & 10.0 & 0.885 & 3.614 & 0.821 & 5.798 & 52.862 & 61.050 & 37.813 & 51.578 \\
10 & 0.0 & 1.0 & 10.0 & \COS & - & 0.885 & 3.615 & 0.821 & 5.798 & 52.867 & 61.057 & 37.849 & 51.576 \\
10 & 0.0 & 1.0 & 10.0 & \RBF & 10.0 & 0.885 & 3.615 & 0.821 & 5.798 & 52.867 & 61.052 & 37.849 & 51.569 \\
10 & 0.0 & 1.0 & 100.0 & \COS & - & 0.886 & 3.613 & 0.821 & 5.796 & 52.867 & 61.026 & 38.033 & 51.753 \\
10 & 0.0 & 1.0 & 100.0 & \RBF & 10.0 & 0.885 & 3.613 & 0.821 & 5.795 & 52.862 & 61.021 & 37.991 & 51.713 \\
10 & 0.05 & 0.1 & 0.0 & \COS & - & 0.885 & 3.619 & 0.821 & 5.806 & 53.096 & 61.140 & 36.961 & 51.283 \\
10 & 0.05 & 0.1 & 0.0 & \RBF & 10.0 & 0.885 & 3.619 & 0.821 & 5.806 & 53.096 & 61.140 & 36.961 & 51.283 \\
10 & 0.05 & 0.1 & 1.0 & \COS & - & 0.885 & 3.619 & 0.821 & 5.806 & 53.101 & 61.143 & 36.961 & 51.292 \\
10 & 0.05 & 0.1 & 1.0 & \RBF & 10.0 & 0.885 & 3.619 & 0.821 & 5.806 & 53.101 & 61.143 & 36.961 & 51.292 \\
10 & 0.05 & 0.1 & 10.0 & \COS & - & 0.885 & 3.619 & 0.821 & 5.805 & 53.101 & 61.138 & 36.960 & 51.310 \\
10 & 0.05 & 0.1 & 10.0 & \RBF & 10.0 & 0.885 & 3.619 & 0.821 & 5.806 & 53.106 & 61.140 & 36.978 & 51.310 \\
10 & 0.05 & 0.1 & 100.0 & \COS & - & 0.885 & 3.616 & 0.821 & 5.801 & 53.048 & 61.101 & 37.251 & 51.345 \\
10 & 0.05 & 0.1 & 100.0 & \RBF & 10.0 & 0.885 & 3.618 & 0.821 & 5.803 & 53.077 & 61.111 & 37.227 & 51.332 \\
10 & 0.05 & 1.0 & 0.0 & \COS & - & 0.885 & 3.619 & 0.821 & 5.806 & 53.096 & 61.143 & 36.961 & 51.292 \\
10 & 0.05 & 1.0 & 0.0 & \RBF & 10.0 & 0.885 & 3.619 & 0.821 & 5.806 & 53.096 & 61.143 & 36.961 & 51.292 \\
10 & 0.05 & 1.0 & 1.0 & \COS & - & 0.885 & 3.619 & 0.821 & 5.806 & 53.101 & 61.143 & 36.961 & 51.292 \\
10 & 0.05 & 1.0 & 1.0 & \RBF & 10.0 & 0.885 & 3.619 & 0.821 & 5.806 & 53.101 & 61.143 & 36.961 & 51.292 \\
10 & 0.05 & 1.0 & 10.0 & \COS & - & 0.885 & 3.619 & 0.821 & 5.805 & 53.101 & 61.138 & 36.960 & 51.310 \\
10 & 0.05 & 1.0 & 10.0 & \RBF & 10.0 & 0.885 & 3.619 & 0.821 & 5.806 & 53.101 & 61.140 & 36.960 & 51.310 \\
10 & 0.05 & 1.0 & 100.0 & \COS & - & 0.885 & 3.616 & 0.821 & 5.801 & 53.048 & 61.101 & 37.251 & 51.345 \\
10 & 0.05 & 1.0 & 100.0 & \RBF & 10.0 & 0.885 & 3.617 & 0.821 & 5.803 & 53.077 & 61.111 & 37.227 & 51.332 \\
10 & 0.1 & 0.1 & 0.0 & \COS & - & 0.885 & 3.624 & 0.822 & 5.811 & 53.330 & 61.167 & 36.770 & 50.787 \\
10 & 0.1 & 0.1 & 0.0 & \RBF & 10.0 & 0.885 & 3.624 & 0.822 & 5.811 & 53.330 & 61.167 & 36.770 & 50.787 \\
10 & 0.1 & 0.1 & 1.0 & \COS & - & 0.885 & 3.624 & 0.822 & 5.811 & 53.325 & 61.167 & 36.770 & 50.787 \\
10 & 0.1 & 0.1 & 1.0 & \RBF & 10.0 & 0.885 & 3.624 & 0.822 & 5.811 & 53.325 & 61.167 & 36.770 & 50.787 \\
10 & 0.1 & 0.1 & 10.0 & \COS & - & 0.886 & 3.624 & 0.822 & 5.812 & 53.325 & 61.174 & 36.818 & 50.773 \\
10 & 0.1 & 0.1 & 10.0 & \RBF & 10.0 & 0.886 & 3.624 & 0.822 & 5.812 & 53.325 & 61.172 & 36.818 & 50.773 \\
10 & 0.1 & 0.1 & 100.0 & \COS & - & 0.885 & 3.621 & 0.821 & 5.813 & 53.281 & 61.211 & 37.008 & 51.126 \\
10 & 0.1 & 0.1 & 100.0 & \RBF & 10.0 & 0.885 & 3.621 & 0.821 & 5.812 & 53.281 & 61.199 & 37.025 & 51.077 \\
10 & 0.1 & 1.0 & 0.0 & \COS & - & 0.885 & 3.624 & 0.822 & 5.811 & 53.330 & 61.167 & 36.770 & 50.787 \\
10 & 0.1 & 1.0 & 0.0 & \RBF & 10.0 & 0.885 & 3.624 & 0.822 & 5.811 & 53.330 & 61.167 & 36.770 & 50.787 \\
10 & 0.1 & 1.0 & 1.0 & \COS & - & 0.885 & 3.624 & 0.822 & 5.811 & 53.325 & 61.164 & 36.770 & 50.787 \\
10 & 0.1 & 1.0 & 1.0 & \RBF & 10.0 & 0.885 & 3.624 & 0.822 & 5.811 & 53.325 & 61.167 & 36.770 & 50.787 \\
10 & 0.1 & 1.0 & 10.0 & \COS & - & 0.886 & 3.624 & 0.822 & 5.812 & 53.325 & 61.174 & 36.818 & 50.773 \\
10 & 0.1 & 1.0 & 10.0 & \RBF & 10.0 & 0.886 & 3.624 & 0.822 & 5.812 & 53.325 & 61.174 & 36.818 & 50.773 \\
10 & 0.1 & 1.0 & 100.0 & \COS & - & 0.885 & 3.621 & 0.821 & 5.813 & 53.281 & 61.211 & 37.008 & 51.126 \\
10 & 0.1 & 1.0 & 100.0 & \RBF & 10.0 & 0.885 & 3.621 & 0.821 & 5.812 & 53.281 & 61.199 & 37.025 & 51.077 \\
10 & 0.5 & 0.1 & 0.0 & \COS & - & 0.849 & 3.446 & 0.789 & 5.608 & 59.518 & 59.523 & 42.201 & 52.104 \\
10 & 0.5 & 0.1 & 0.0 & \RBF & 10.0 & 0.849 & 3.446 & 0.789 & 5.608 & 59.518 & 59.523 & 42.201 & 52.104 \\
10 & 0.5 & 0.1 & 1.0 & \COS & - & 0.849 & 3.445 & 0.789 & 5.609 & 59.513 & 59.527 & 42.182 & 52.127 \\
10 & 0.5 & 0.1 & 1.0 & \RBF & 10.0 & 0.849 & 3.445 & 0.789 & 5.608 & 59.513 & 59.525 & 42.182 & 52.127 \\
10 & 0.5 & 0.1 & 10.0 & \COS & - & 0.849 & 3.443 & 0.789 & 5.611 & 59.498 & 59.542 & 42.327 & 52.196 \\
10 & 0.5 & 0.1 & 10.0 & \RBF & 10.0 & 0.849 & 3.443 & 0.789 & 5.610 & 59.508 & 59.537 & 42.315 & 52.175 \\
10 & 0.5 & 0.1 & 100.0 & \COS & - & 0.850 & 3.441 & 0.790 & 5.590 & 59.508 & 59.369 & 43.655 & 53.130 \\
10 & 0.5 & 0.1 & 100.0 & \RBF & 10.0 & 0.850 & 3.439 & 0.790 & 5.592 & 59.445 & 59.401 & 43.290 & 53.031 \\
10 & 0.5 & 1.0 & 0.0 & \COS & - & 0.863 & 3.524 & 0.801 & 5.738 & 58.426 & 60.665 & 41.128 & 52.252 \\
10 & 0.5 & 1.0 & 0.0 & \RBF & 10.0 & 0.863 & 3.524 & 0.801 & 5.738 & 58.426 & 60.665 & 41.128 & 52.252 \\
10 & 0.5 & 1.0 & 1.0 & \COS & - & 0.863 & 3.526 & 0.801 & 5.738 & 58.426 & 60.663 & 41.110 & 52.183 \\
10 & 0.5 & 1.0 & 1.0 & \RBF & 10.0 & 0.863 & 3.526 & 0.801 & 5.737 & 58.426 & 60.663 & 41.110 & 52.169 \\
10 & 0.5 & 1.0 & 10.0 & \COS & - & 0.863 & 3.530 & 0.802 & 5.740 & 58.378 & 60.699 & 41.116 & 52.399 \\
10 & 0.5 & 1.0 & 10.0 & \RBF & 10.0 & 0.863 & 3.529 & 0.802 & 5.740 & 58.358 & 60.694 & 41.049 & 52.354 \\
10 & 0.5 & 1.0 & 100.0 & \COS & - & 0.863 & 3.521 & 0.802 & 5.726 & 58.232 & 60.575 & 41.573 & 53.013 \\
10 & 0.5 & 1.0 & 100.0 & \RBF & 10.0 & 0.864 & 3.527 & 0.803 & 5.731 & 58.231 & 60.609 & 41.366 & 52.694 \\
10 & 1.0 & 0.1 & 0.0 & \COS & - & 0.760 & 2.677 & 0.695 & 3.905 & 51.035 & 42.085 & 30.628 & 35.463 \\
10 & 1.0 & 0.1 & 0.0 & \RBF & 10.0 & 0.760 & 2.677 & 0.695 & 3.905 & 51.035 & 42.085 & 30.628 & 35.463 \\
10 & 1.0 & 0.1 & 1.0 & \COS & - & 0.759 & 2.682 & 0.695 & 3.907 & 51.089 & 42.122 & 30.969 & 35.668 \\
10 & 1.0 & 0.1 & 1.0 & \RBF & 10.0 & 0.760 & 2.681 & 0.695 & 3.908 & 51.074 & 42.127 & 30.933 & 35.637 \\
10 & 1.0 & 0.1 & 10.0 & \COS & - & 0.757 & 2.669 & 0.691 & 3.918 & 50.933 & 42.270 & 31.768 & 37.088 \\
10 & 1.0 & 0.1 & 10.0 & \RBF & 10.0 & 0.758 & 2.673 & 0.692 & 3.926 & 50.987 & 42.321 & 31.492 & 37.066 \\
10 & 1.0 & 0.1 & 100.0 & \COS & - & 0.759 & 2.653 & 0.689 & 3.978 & 50.572 & 42.916 & 33.244 & 39.584 \\
10 & 1.0 & 0.1 & 100.0 & \RBF & 10.0 & 0.760 & 2.670 & 0.691 & 3.986 & 50.899 & 43.030 & 33.210 & 39.339 \\
10 & 1.0 & 1.0 & 0.0 & \COS & - & 0.760 & 2.679 & 0.695 & 3.900 & 51.045 & 42.022 & 30.433 & 35.478 \\
10 & 1.0 & 1.0 & 0.0 & \RBF & 10.0 & 0.760 & 2.679 & 0.695 & 3.900 & 51.045 & 42.022 & 30.433 & 35.478 \\
10 & 1.0 & 1.0 & 1.0 & \COS & - & 0.762 & 2.687 & 0.696 & 3.919 & 51.206 & 42.239 & 30.793 & 35.838 \\
10 & 1.0 & 1.0 & 1.0 & \RBF & 10.0 & 0.761 & 2.686 & 0.696 & 3.918 & 51.186 & 42.222 & 30.781 & 35.788 \\
10 & 1.0 & 1.0 & 10.0 & \COS & - & 0.757 & 2.664 & 0.691 & 3.904 & 50.894 & 42.107 & 31.413 & 36.827 \\
10 & 1.0 & 1.0 & 10.0 & \RBF & 10.0 & 0.759 & 2.671 & 0.693 & 3.910 & 50.957 & 42.144 & 31.082 & 36.719 \\
10 & 1.0 & 1.0 & 100.0 & \COS & - & 0.761 & 2.670 & 0.692 & 3.983 & 50.865 & 42.967 & 33.207 & 39.703 \\
10 & 1.0 & 1.0 & 100.0 & \RBF & 10.0 & 0.760 & 2.666 & 0.691 & 3.971 & 50.797 & 42.845 & 33.421 & 39.305 \\
15 & 0.0 & 0.1 & 0.0 & \COS & - & 0.904 & 3.700 & 0.836 & 5.863 & 53.476 & 61.618 & 19.808 & 40.378 \\
15 & 0.0 & 0.1 & 0.0 & \RBF & 10.0 & 0.904 & 3.700 & 0.836 & 5.863 & 53.476 & 61.618 & 19.808 & 40.378 \\
15 & 0.0 & 0.1 & 1.0 & \COS & - & 0.904 & 3.700 & 0.836 & 5.864 & 53.476 & 61.622 & 19.808 & 40.387 \\
15 & 0.0 & 0.1 & 1.0 & \RBF & 10.0 & 0.904 & 3.700 & 0.836 & 5.864 & 53.476 & 61.622 & 19.808 & 40.387 \\
15 & 0.0 & 0.1 & 10.0 & \COS & - & 0.904 & 3.703 & 0.837 & 5.862 & 53.545 & 61.598 & 19.471 & 39.672 \\
15 & 0.0 & 0.1 & 10.0 & \RBF & 10.0 & 0.904 & 3.703 & 0.837 & 5.862 & 53.545 & 61.598 & 19.471 & 39.673 \\
15 & 0.0 & 0.1 & 100.0 & \COS & - & 0.898 & 3.676 & 0.832 & 5.868 & 53.335 & 61.642 & 25.486 & 45.951 \\
15 & 0.0 & 0.1 & 100.0 & \RBF & 10.0 & 0.899 & 3.687 & 0.833 & 5.872 & 53.442 & 61.693 & 23.872 & 44.381 \\
15 & 0.0 & 1.0 & 0.0 & \COS & - & 0.906 & 3.710 & 0.838 & 5.839 & 53.476 & 61.362 & 17.166 & 36.667 \\
15 & 0.0 & 1.0 & 0.0 & \RBF & 10.0 & 0.906 & 3.710 & 0.838 & 5.839 & 53.476 & 61.362 & 17.166 & 36.667 \\
15 & 0.0 & 1.0 & 1.0 & \COS & - & 0.906 & 3.710 & 0.838 & 5.839 & 53.476 & 61.359 & 17.166 & 36.660 \\
15 & 0.0 & 1.0 & 1.0 & \RBF & 10.0 & 0.906 & 3.710 & 0.838 & 5.839 & 53.476 & 61.359 & 17.166 & 36.660 \\
15 & 0.0 & 1.0 & 10.0 & \COS & - & 0.906 & 3.710 & 0.838 & 5.839 & 53.462 & 61.369 & 17.203 & 36.488 \\
15 & 0.0 & 1.0 & 10.0 & \RBF & 10.0 & 0.906 & 3.710 & 0.838 & 5.840 & 53.467 & 61.372 & 17.203 & 36.488 \\
15 & 0.0 & 1.0 & 100.0 & \COS & - & 0.905 & 3.701 & 0.837 & 5.850 & 53.408 & 61.479 & 18.273 & 38.211 \\
15 & 0.0 & 1.0 & 100.0 & \RBF & 10.0 & 0.906 & 3.704 & 0.838 & 5.844 & 53.389 & 61.403 & 17.135 & 36.886 \\
15 & 0.05 & 0.1 & 0.0 & \COS & - & 0.907 & 3.711 & 0.839 & 5.841 & 53.671 & 61.371 & 16.510 & 35.453 \\
15 & 0.05 & 0.1 & 0.0 & \RBF & 10.0 & 0.907 & 3.711 & 0.839 & 5.841 & 53.671 & 61.371 & 16.510 & 35.453 \\
15 & 0.05 & 0.1 & 1.0 & \COS & - & 0.907 & 3.712 & 0.839 & 5.841 & 53.671 & 61.369 & 16.528 & 35.453 \\
15 & 0.05 & 0.1 & 1.0 & \RBF & 10.0 & 0.907 & 3.711 & 0.839 & 5.841 & 53.666 & 61.369 & 16.510 & 35.453 \\
15 & 0.05 & 0.1 & 10.0 & \COS & - & 0.907 & 3.711 & 0.839 & 5.840 & 53.676 & 61.364 & 16.583 & 35.453 \\
15 & 0.05 & 0.1 & 10.0 & \RBF & 10.0 & 0.907 & 3.711 & 0.839 & 5.840 & 53.671 & 61.362 & 16.546 & 35.453 \\
15 & 0.05 & 0.1 & 100.0 & \COS & - & 0.906 & 3.710 & 0.838 & 5.839 & 53.632 & 61.347 & 16.715 & 35.742 \\
15 & 0.05 & 0.1 & 100.0 & \RBF & 10.0 & 0.906 & 3.709 & 0.839 & 5.838 & 53.627 & 61.354 & 16.697 & 35.646 \\
15 & 0.05 & 1.0 & 0.0 & \COS & - & 0.907 & 3.711 & 0.839 & 5.841 & 53.666 & 61.371 & 16.510 & 35.453 \\
15 & 0.05 & 1.0 & 0.0 & \RBF & 10.0 & 0.907 & 3.711 & 0.839 & 5.841 & 53.666 & 61.371 & 16.510 & 35.453 \\
15 & 0.05 & 1.0 & 1.0 & \COS & - & 0.907 & 3.711 & 0.839 & 5.841 & 53.676 & 61.369 & 16.546 & 35.453 \\
15 & 0.05 & 1.0 & 1.0 & \RBF & 10.0 & 0.907 & 3.711 & 0.839 & 5.841 & 53.671 & 61.369 & 16.528 & 35.453 \\
15 & 0.05 & 1.0 & 10.0 & \COS & - & 0.907 & 3.711 & 0.839 & 5.840 & 53.676 & 61.364 & 16.583 & 35.453 \\
15 & 0.05 & 1.0 & 10.0 & \RBF & 10.0 & 0.907 & 3.711 & 0.839 & 5.840 & 53.671 & 61.362 & 16.546 & 35.453 \\
15 & 0.05 & 1.0 & 100.0 & \COS & - & 0.906 & 3.709 & 0.838 & 5.837 & 53.617 & 61.340 & 16.715 & 35.639 \\
15 & 0.05 & 1.0 & 100.0 & \RBF & 10.0 & 0.906 & 3.709 & 0.839 & 5.838 & 53.627 & 61.354 & 16.697 & 35.646 \\
15 & 0.1 & 0.1 & 0.0 & \COS & - & 0.907 & 3.713 & 0.839 & 5.839 & 53.832 & 61.342 & 15.856 & 34.516 \\
15 & 0.1 & 0.1 & 0.0 & \RBF & 10.0 & 0.907 & 3.713 & 0.839 & 5.839 & 53.832 & 61.342 & 15.856 & 34.516 \\
15 & 0.1 & 0.1 & 1.0 & \COS & - & 0.907 & 3.713 & 0.839 & 5.839 & 53.827 & 61.342 & 15.856 & 34.516 \\
15 & 0.1 & 0.1 & 1.0 & \RBF & 10.0 & 0.907 & 3.713 & 0.839 & 5.839 & 53.827 & 61.342 & 15.856 & 34.516 \\
15 & 0.1 & 0.1 & 10.0 & \COS & - & 0.907 & 3.712 & 0.839 & 5.839 & 53.807 & 61.349 & 15.783 & 34.598 \\
15 & 0.1 & 0.1 & 10.0 & \RBF & 10.0 & 0.907 & 3.712 & 0.839 & 5.839 & 53.807 & 61.347 & 15.783 & 34.571 \\
15 & 0.1 & 0.1 & 100.0 & \COS & - & 0.907 & 3.710 & 0.839 & 5.839 & 53.803 & 61.335 & 16.245 & 34.822 \\
15 & 0.1 & 0.1 & 100.0 & \RBF & 10.0 & 0.907 & 3.712 & 0.839 & 5.840 & 53.827 & 61.347 & 16.208 & 34.906 \\
15 & 0.1 & 1.0 & 0.0 & \COS & - & 0.907 & 3.713 & 0.839 & 5.839 & 53.827 & 61.342 & 15.856 & 34.516 \\
15 & 0.1 & 1.0 & 0.0 & \RBF & 10.0 & 0.907 & 3.713 & 0.839 & 5.839 & 53.827 & 61.342 & 15.856 & 34.516 \\
15 & 0.1 & 1.0 & 1.0 & \COS & - & 0.907 & 3.713 & 0.839 & 5.839 & 53.822 & 61.342 & 15.820 & 34.516 \\
15 & 0.1 & 1.0 & 1.0 & \RBF & 10.0 & 0.907 & 3.713 & 0.839 & 5.839 & 53.822 & 61.342 & 15.820 & 34.516 \\
15 & 0.1 & 1.0 & 10.0 & \COS & - & 0.907 & 3.713 & 0.839 & 5.839 & 53.812 & 61.349 & 15.783 & 34.598 \\
15 & 0.1 & 1.0 & 10.0 & \RBF & 10.0 & 0.907 & 3.712 & 0.839 & 5.839 & 53.807 & 61.349 & 15.783 & 34.598 \\
15 & 0.1 & 1.0 & 100.0 & \COS & - & 0.907 & 3.710 & 0.839 & 5.839 & 53.798 & 61.337 & 16.245 & 34.831 \\
15 & 0.1 & 1.0 & 100.0 & \RBF & 10.0 & 0.907 & 3.712 & 0.839 & 5.840 & 53.827 & 61.347 & 16.208 & 34.906 \\
15 & 0.5 & 0.1 & 0.0 & \COS & - & 0.875 & 3.519 & 0.808 & 5.710 & 62.485 & 60.826 & 28.910 & 43.998 \\
15 & 0.5 & 0.1 & 0.0 & \RBF & 10.0 & 0.875 & 3.519 & 0.808 & 5.710 & 62.485 & 60.826 & 28.910 & 43.998 \\
15 & 0.5 & 0.1 & 1.0 & \COS & - & 0.875 & 3.518 & 0.808 & 5.711 & 62.485 & 60.835 & 28.855 & 44.043 \\
15 & 0.5 & 0.1 & 1.0 & \RBF & 10.0 & 0.875 & 3.518 & 0.808 & 5.711 & 62.475 & 60.835 & 28.855 & 44.043 \\
15 & 0.5 & 0.1 & 10.0 & \COS & - & 0.875 & 3.519 & 0.808 & 5.707 & 62.490 & 60.799 & 29.012 & 44.269 \\
15 & 0.5 & 0.1 & 10.0 & \RBF & 10.0 & 0.875 & 3.519 & 0.808 & 5.708 & 62.509 & 60.802 & 29.025 & 44.246 \\
15 & 0.5 & 0.1 & 100.0 & \COS & - & 0.871 & 3.506 & 0.805 & 5.684 & 62.363 & 60.497 & 31.477 & 45.924 \\
15 & 0.5 & 0.1 & 100.0 & \RBF & 10.0 & 0.872 & 3.508 & 0.805 & 5.693 & 62.407 & 60.606 & 31.106 & 45.633 \\
15 & 0.5 & 1.0 & 0.0 & \COS & - & 0.878 & 3.552 & 0.811 & 5.762 & 61.505 & 61.174 & 25.845 & 41.923 \\
15 & 0.5 & 1.0 & 0.0 & \RBF & 10.0 & 0.878 & 3.552 & 0.811 & 5.762 & 61.505 & 61.174 & 25.845 & 41.923 \\
15 & 0.5 & 1.0 & 1.0 & \COS & - & 0.878 & 3.552 & 0.812 & 5.765 & 61.452 & 61.189 & 25.652 & 41.852 \\
15 & 0.5 & 1.0 & 1.0 & \RBF & 10.0 & 0.879 & 3.552 & 0.812 & 5.764 & 61.452 & 61.189 & 25.652 & 41.838 \\
15 & 0.5 & 1.0 & 10.0 & \COS & - & 0.879 & 3.561 & 0.812 & 5.770 & 61.345 & 61.240 & 25.607 & 41.590 \\
15 & 0.5 & 1.0 & 10.0 & \RBF & 10.0 & 0.879 & 3.560 & 0.812 & 5.770 & 61.355 & 61.249 & 25.540 & 41.713 \\
15 & 0.5 & 1.0 & 100.0 & \COS & - & 0.877 & 3.548 & 0.809 & 5.762 & 61.160 & 61.162 & 27.027 & 43.266 \\
15 & 0.5 & 1.0 & 100.0 & \RBF & 10.0 & 0.877 & 3.552 & 0.809 & 5.767 & 61.155 & 61.216 & 26.811 & 43.041 \\
15 & 1.0 & 0.1 & 0.0 & \COS & - & 0.847 & 3.096 & 0.776 & 4.347 & 59.313 & 46.894 & 23.980 & 32.683 \\
15 & 1.0 & 0.1 & 0.0 & \RBF & 10.0 & 0.847 & 3.096 & 0.776 & 4.347 & 59.313 & 46.894 & 23.980 & 32.683 \\
15 & 1.0 & 0.1 & 1.0 & \COS & - & 0.848 & 3.096 & 0.776 & 4.348 & 59.318 & 46.911 & 24.503 & 32.995 \\
15 & 1.0 & 0.1 & 1.0 & \RBF & 10.0 & 0.847 & 3.096 & 0.776 & 4.347 & 59.323 & 46.899 & 24.394 & 32.948 \\
15 & 1.0 & 0.1 & 10.0 & \COS & - & 0.841 & 3.038 & 0.769 & 4.297 & 58.266 & 46.446 & 28.279 & 36.290 \\
15 & 1.0 & 0.1 & 10.0 & \RBF & 10.0 & 0.842 & 3.051 & 0.771 & 4.308 & 58.499 & 46.553 & 28.000 & 35.883 \\
15 & 1.0 & 0.1 & 100.0 & \COS & - & 0.821 & 2.858 & 0.742 & 4.165 & 54.943 & 44.972 & 32.395 & 40.372 \\
15 & 1.0 & 0.1 & 100.0 & \RBF & 10.0 & 0.817 & 2.845 & 0.740 & 4.147 & 54.753 & 44.741 & 32.496 & 40.427 \\
15 & 1.0 & 1.0 & 0.0 & \COS & - & 0.849 & 3.093 & 0.777 & 4.345 & 59.220 & 46.870 & 23.888 & 32.781 \\
15 & 1.0 & 1.0 & 0.0 & \RBF & 10.0 & 0.849 & 3.093 & 0.777 & 4.345 & 59.220 & 46.870 & 23.888 & 32.781 \\
15 & 1.0 & 1.0 & 1.0 & \COS & - & 0.849 & 3.097 & 0.777 & 4.353 & 59.313 & 46.965 & 24.470 & 33.114 \\
15 & 1.0 & 1.0 & 1.0 & \RBF & 10.0 & 0.849 & 3.096 & 0.777 & 4.353 & 59.308 & 46.962 & 24.432 & 33.109 \\
15 & 1.0 & 1.0 & 10.0 & \COS & - & 0.842 & 3.033 & 0.770 & 4.278 & 58.197 & 46.207 & 28.183 & 36.032 \\
15 & 1.0 & 1.0 & 10.0 & \RBF & 10.0 & 0.844 & 3.043 & 0.771 & 4.287 & 58.373 & 46.317 & 28.015 & 35.694 \\
15 & 1.0 & 1.0 & 100.0 & \COS & - & 0.817 & 2.839 & 0.739 & 4.145 & 54.631 & 44.716 & 33.076 & 40.777 \\
15 & 1.0 & 1.0 & 100.0 & \RBF & 10.0 & 0.825 & 2.894 & 0.748 & 4.192 & 55.679 & 45.272 & 32.245 & 40.015 \\
30 & 0.0 & 0.1 & 0.0 & \COS & - & 0.938 & 3.930 & 0.873 & 5.958 & 55.898 & 62.253 & 4.707 & 13.993 \\
30 & 0.0 & 0.1 & 0.0 & \RBF & 10.0 & 0.938 & 3.930 & 0.873 & 5.958 & 55.898 & 62.253 & 4.707 & 13.993 \\
30 & 0.0 & 0.1 & 1.0 & \COS & - & 0.938 & 3.931 & 0.873 & 5.957 & 55.898 & 62.249 & 4.594 & 13.668 \\
30 & 0.0 & 0.1 & 1.0 & \RBF & 10.0 & 0.938 & 3.931 & 0.873 & 5.956 & 55.898 & 62.246 & 4.594 & 13.668 \\
30 & 0.0 & 0.1 & 10.0 & \COS & - & 0.940 & 3.949 & 0.876 & 5.950 & 56.180 & 62.183 & 3.856 & 12.249 \\
30 & 0.0 & 0.1 & 10.0 & \RBF & 10.0 & 0.940 & 3.948 & 0.875 & 5.953 & 56.141 & 62.212 & 3.911 & 12.320 \\
30 & 0.0 & 0.1 & 100.0 & \COS & - & 0.905 & 3.747 & 0.839 & 5.930 & 54.173 & 62.046 & 24.055 & 37.370 \\
30 & 0.0 & 0.1 & 100.0 & \RBF & 10.0 & 0.915 & 3.800 & 0.849 & 5.969 & 54.650 & 62.434 & 16.795 & 30.313 \\
30 & 0.0 & 1.0 & 0.0 & \COS & - & 0.947 & 4.006 & 0.885 & 5.917 & 56.926 & 61.944 & 2.663 & 7.854 \\
30 & 0.0 & 1.0 & 0.0 & \RBF & 10.0 & 0.947 & 4.006 & 0.885 & 5.917 & 56.926 & 61.944 & 2.663 & 7.854 \\
30 & 0.0 & 1.0 & 1.0 & \COS & - & 0.947 & 4.011 & 0.886 & 5.917 & 56.994 & 61.939 & 2.602 & 7.742 \\
30 & 0.0 & 1.0 & 1.0 & \RBF & 10.0 & 0.947 & 4.011 & 0.886 & 5.917 & 56.994 & 61.939 & 2.602 & 7.742 \\
30 & 0.0 & 1.0 & 10.0 & \COS & - & 0.948 & 4.010 & 0.886 & 5.917 & 56.970 & 61.932 & 2.602 & 7.710 \\
30 & 0.0 & 1.0 & 10.0 & \RBF & 10.0 & 0.948 & 4.010 & 0.886 & 5.917 & 56.970 & 61.932 & 2.602 & 7.710 \\
30 & 0.0 & 1.0 & 100.0 & \COS & - & 0.930 & 3.890 & 0.865 & 5.961 & 55.503 & 62.300 & 6.932 & 18.147 \\
30 & 0.0 & 1.0 & 100.0 & \RBF & 10.0 & 0.938 & 3.933 & 0.874 & 5.947 & 55.956 & 62.163 & 4.210 & 12.839 \\
30 & 0.05 & 0.1 & 0.0 & \COS & - & 0.948 & 4.018 & 0.887 & 5.925 & 57.418 & 62.032 & 2.504 & 7.491 \\
30 & 0.05 & 0.1 & 0.0 & \RBF & 10.0 & 0.948 & 4.018 & 0.887 & 5.925 & 57.418 & 62.032 & 2.504 & 7.491 \\
30 & 0.05 & 0.1 & 1.0 & \COS & - & 0.948 & 4.018 & 0.887 & 5.926 & 57.418 & 62.029 & 2.504 & 7.463 \\
30 & 0.05 & 0.1 & 1.0 & \RBF & 10.0 & 0.948 & 4.018 & 0.887 & 5.926 & 57.418 & 62.029 & 2.504 & 7.463 \\
30 & 0.05 & 0.1 & 10.0 & \COS & - & 0.948 & 4.018 & 0.887 & 5.926 & 57.403 & 62.034 & 2.521 & 7.477 \\
30 & 0.05 & 0.1 & 10.0 & \RBF & 10.0 & 0.948 & 4.018 & 0.887 & 5.926 & 57.403 & 62.034 & 2.521 & 7.477 \\
30 & 0.05 & 0.1 & 100.0 & \COS & - & 0.933 & 3.906 & 0.868 & 5.963 & 56.185 & 62.326 & 6.110 & 16.455 \\
30 & 0.05 & 0.1 & 100.0 & \RBF & 10.0 & 0.940 & 3.956 & 0.877 & 5.951 & 56.765 & 62.192 & 3.618 & 11.409 \\
30 & 0.05 & 1.0 & 0.0 & \COS & - & 0.948 & 4.018 & 0.887 & 5.925 & 57.418 & 62.032 & 2.504 & 7.491 \\
30 & 0.05 & 1.0 & 0.0 & \RBF & 10.0 & 0.948 & 4.018 & 0.887 & 5.925 & 57.418 & 62.032 & 2.504 & 7.491 \\
30 & 0.05 & 1.0 & 1.0 & \COS & - & 0.948 & 4.018 & 0.887 & 5.926 & 57.418 & 62.029 & 2.504 & 7.463 \\
30 & 0.05 & 1.0 & 1.0 & \RBF & 10.0 & 0.948 & 4.018 & 0.887 & 5.926 & 57.418 & 62.029 & 2.504 & 7.463 \\
30 & 0.05 & 1.0 & 10.0 & \COS & - & 0.948 & 4.018 & 0.887 & 5.926 & 57.408 & 62.032 & 2.521 & 7.450 \\
30 & 0.05 & 1.0 & 10.0 & \RBF & 10.0 & 0.948 & 4.018 & 0.887 & 5.926 & 57.403 & 62.034 & 2.521 & 7.477 \\
30 & 0.05 & 1.0 & 100.0 & \COS & - & 0.943 & 3.979 & 0.880 & 5.942 & 56.955 & 62.107 & 3.038 & 9.726 \\
30 & 0.05 & 1.0 & 100.0 & \RBF & 10.0 & 0.947 & 4.010 & 0.886 & 5.923 & 57.262 & 62.002 & 2.559 & 7.750 \\
30 & 0.1 & 0.1 & 0.0 & \COS & - & 0.948 & 4.023 & 0.887 & 5.938 & 57.793 & 62.156 & 2.487 & 7.416 \\
30 & 0.1 & 0.1 & 0.0 & \RBF & 10.0 & 0.948 & 4.023 & 0.887 & 5.938 & 57.793 & 62.156 & 2.487 & 7.416 \\
30 & 0.1 & 0.1 & 1.0 & \COS & - & 0.948 & 4.023 & 0.887 & 5.938 & 57.793 & 62.153 & 2.487 & 7.416 \\
30 & 0.1 & 0.1 & 1.0 & \RBF & 10.0 & 0.948 & 4.023 & 0.887 & 5.938 & 57.793 & 62.153 & 2.487 & 7.416 \\
30 & 0.1 & 0.1 & 10.0 & \COS & - & 0.948 & 4.023 & 0.887 & 5.937 & 57.798 & 62.141 & 2.487 & 7.408 \\
30 & 0.1 & 0.1 & 10.0 & \RBF & 10.0 & 0.948 & 4.023 & 0.887 & 5.937 & 57.803 & 62.139 & 2.487 & 7.408 \\
30 & 0.1 & 0.1 & 100.0 & \COS & - & 0.938 & 3.954 & 0.875 & 5.967 & 57.282 & 62.363 & 4.427 & 12.491 \\
30 & 0.1 & 0.1 & 100.0 & \RBF & 10.0 & 0.945 & 4.003 & 0.884 & 5.942 & 57.564 & 62.180 & 2.782 & 8.541 \\
30 & 0.1 & 1.0 & 0.0 & \COS & - & 0.948 & 4.023 & 0.887 & 5.937 & 57.808 & 62.144 & 2.487 & 7.403 \\
30 & 0.1 & 1.0 & 0.0 & \RBF & 10.0 & 0.948 & 4.023 & 0.887 & 5.937 & 57.808 & 62.144 & 2.487 & 7.403 \\
30 & 0.1 & 1.0 & 1.0 & \COS & - & 0.948 & 4.023 & 0.887 & 5.937 & 57.808 & 62.144 & 2.487 & 7.403 \\
30 & 0.1 & 1.0 & 1.0 & \RBF & 10.0 & 0.948 & 4.023 & 0.887 & 5.937 & 57.808 & 62.144 & 2.487 & 7.403 \\
30 & 0.1 & 1.0 & 10.0 & \COS & - & 0.948 & 4.023 & 0.887 & 5.937 & 57.798 & 62.141 & 2.487 & 7.408 \\
30 & 0.1 & 1.0 & 10.0 & \RBF & 10.0 & 0.948 & 4.023 & 0.887 & 5.937 & 57.803 & 62.141 & 2.487 & 7.408 \\
30 & 0.1 & 1.0 & 100.0 & \COS & - & 0.945 & 4.003 & 0.883 & 5.942 & 57.535 & 62.185 & 2.782 & 8.591 \\
30 & 0.1 & 1.0 & 100.0 & \RBF & 10.0 & 0.948 & 4.018 & 0.886 & 5.935 & 57.725 & 62.134 & 2.486 & 7.571 \\
30 & 0.5 & 0.1 & 0.0 & \COS & - & 0.922 & 3.755 & 0.850 & 5.816 & 67.459 & 62.148 & 9.985 & 19.554 \\
30 & 0.5 & 0.1 & 0.0 & \RBF & 10.0 & 0.922 & 3.755 & 0.850 & 5.816 & 67.459 & 62.148 & 9.985 & 19.554 \\
30 & 0.5 & 0.1 & 1.0 & \COS & - & 0.922 & 3.755 & 0.850 & 5.814 & 67.469 & 62.139 & 9.985 & 19.593 \\
30 & 0.5 & 0.1 & 1.0 & \RBF & 10.0 & 0.922 & 3.755 & 0.850 & 5.814 & 67.469 & 62.134 & 9.985 & 19.573 \\
30 & 0.5 & 0.1 & 10.0 & \COS & - & 0.921 & 3.751 & 0.849 & 5.808 & 67.406 & 62.102 & 10.124 & 19.859 \\
30 & 0.5 & 0.1 & 10.0 & \RBF & 10.0 & 0.921 & 3.751 & 0.849 & 5.810 & 67.401 & 62.117 & 10.087 & 19.844 \\
30 & 0.5 & 0.1 & 100.0 & \COS & - & 0.913 & 3.707 & 0.841 & 5.767 & 66.738 & 61.691 & 12.476 & 23.133 \\
30 & 0.5 & 0.1 & 100.0 & \RBF & 10.0 & 0.914 & 3.713 & 0.842 & 5.775 & 66.816 & 61.766 & 12.146 & 22.590 \\
30 & 0.5 & 1.0 & 0.0 & \COS & - & 0.923 & 3.772 & 0.851 & 5.837 & 67.001 & 62.273 & 8.414 & 17.279 \\
30 & 0.5 & 1.0 & 0.0 & \RBF & 10.0 & 0.923 & 3.772 & 0.851 & 5.837 & 67.001 & 62.273 & 8.414 & 17.279 \\
30 & 0.5 & 1.0 & 1.0 & \COS & - & 0.923 & 3.772 & 0.851 & 5.837 & 66.957 & 62.275 & 8.386 & 17.187 \\
30 & 0.5 & 1.0 & 1.0 & \RBF & 10.0 & 0.923 & 3.773 & 0.851 & 5.838 & 66.962 & 62.278 & 8.368 & 17.187 \\
30 & 0.5 & 1.0 & 10.0 & \COS & - & 0.923 & 3.774 & 0.852 & 5.842 & 66.704 & 62.302 & 8.057 & 16.705 \\
30 & 0.5 & 1.0 & 10.0 & \RBF & 10.0 & 0.923 & 3.773 & 0.852 & 5.841 & 66.719 & 62.290 & 8.044 & 16.701 \\
30 & 0.5 & 1.0 & 100.0 & \COS & - & 0.917 & 3.736 & 0.845 & 5.799 & 66.300 & 61.868 & 9.872 & 19.434 \\
30 & 0.5 & 1.0 & 100.0 & \RBF & 10.0 & 0.919 & 3.746 & 0.848 & 5.810 & 66.222 & 61.942 & 9.179 & 18.183 \\
30 & 1.0 & 0.1 & 0.0 & \COS & - & 0.937 & 3.591 & 0.871 & 4.673 & 67.508 & 50.902 & 9.615 & 19.160 \\
30 & 1.0 & 0.1 & 0.0 & \RBF & 10.0 & 0.937 & 3.591 & 0.871 & 4.673 & 67.508 & 50.902 & 9.615 & 19.160 \\
30 & 1.0 & 0.1 & 1.0 & \COS & - & 0.936 & 3.582 & 0.869 & 4.681 & 67.406 & 51.006 & 10.368 & 19.829 \\
30 & 1.0 & 0.1 & 1.0 & \RBF & 10.0 & 0.936 & 3.584 & 0.869 & 4.680 & 67.415 & 50.991 & 10.301 & 19.770 \\
30 & 1.0 & 0.1 & 10.0 & \COS & - & 0.921 & 3.489 & 0.850 & 4.672 & 66.568 & 50.731 & 20.160 & 30.674 \\
30 & 1.0 & 0.1 & 10.0 & \RBF & 10.0 & 0.924 & 3.508 & 0.853 & 4.685 & 66.782 & 50.896 & 18.566 & 29.390 \\
30 & 1.0 & 0.1 & 100.0 & \COS & - & 0.892 & 3.108 & 0.802 & 4.435 & 60.029 & 47.766 & 30.481 & 42.831 \\
30 & 1.0 & 0.1 & 100.0 & \RBF & 10.0 & 0.891 & 3.141 & 0.803 & 4.459 & 60.658 & 48.085 & 30.903 & 42.882 \\
30 & 1.0 & 1.0 & 0.0 & \COS & - & 0.936 & 3.587 & 0.871 & 4.667 & 67.435 & 50.855 & 9.743 & 19.325 \\
30 & 1.0 & 1.0 & 0.0 & \RBF & 10.0 & 0.936 & 3.587 & 0.871 & 4.667 & 67.435 & 50.855 & 9.743 & 19.325 \\
30 & 1.0 & 1.0 & 1.0 & \COS & - & 0.936 & 3.581 & 0.869 & 4.681 & 67.381 & 51.033 & 10.252 & 19.627 \\
30 & 1.0 & 1.0 & 1.0 & \RBF & 10.0 & 0.936 & 3.582 & 0.869 & 4.683 & 67.401 & 51.040 & 10.187 & 19.609 \\
30 & 1.0 & 1.0 & 10.0 & \COS & - & 0.922 & 3.484 & 0.851 & 4.649 & 66.480 & 50.451 & 20.550 & 31.313 \\
30 & 1.0 & 1.0 & 10.0 & \RBF & 10.0 & 0.925 & 3.501 & 0.854 & 4.658 & 66.704 & 50.585 & 19.399 & 29.842 \\
30 & 1.0 & 1.0 & 100.0 & \COS & - & 0.889 & 3.125 & 0.802 & 4.434 & 60.322 & 47.766 & 31.508 & 42.788 \\
30 & 1.0 & 1.0 & 100.0 & \RBF & 10.0 & 0.892 & 3.153 & 0.805 & 4.468 & 60.853 & 48.132 & 31.375 & 42.962 \\
50 & 0.0 & 0.1 & 0.0 & \COS & - & 0.949 & 4.111 & 0.894 & 6.194 & 58.821 & 64.638 & 2.102 & 7.198 \\
50 & 0.0 & 0.1 & 0.0 & \RBF & 10.0 & 0.949 & 4.111 & 0.894 & 6.194 & 58.821 & 64.638 & 2.102 & 7.198 \\
50 & 0.0 & 0.1 & 1.0 & \COS & - & 0.953 & 4.133 & 0.898 & 6.189 & 59.143 & 64.628 & 1.537 & 5.928 \\
50 & 0.0 & 0.1 & 1.0 & \RBF & 10.0 & 0.953 & 4.133 & 0.898 & 6.189 & 59.143 & 64.628 & 1.537 & 5.928 \\
50 & 0.0 & 0.1 & 10.0 & \COS & - & 0.958 & 4.183 & 0.905 & 6.197 & 59.902 & 64.709 & 0.857 & 3.756 \\
50 & 0.0 & 0.1 & 10.0 & \RBF & 10.0 & 0.958 & 4.176 & 0.904 & 6.194 & 59.820 & 64.680 & 0.884 & 3.903 \\
50 & 0.0 & 0.1 & 100.0 & \COS & - & 0.904 & 3.760 & 0.838 & 6.001 & 54.348 & 62.731 & 27.350 & 39.077 \\
50 & 0.0 & 0.1 & 100.0 & \RBF & 10.0 & 0.911 & 3.832 & 0.848 & 6.078 & 55.420 & 63.518 & 21.996 & 31.845 \\
50 & 0.0 & 1.0 & 0.0 & \COS & - & 0.967 & 4.271 & 0.917 & 6.217 & 61.184 & 64.984 & 0.609 & 2.156 \\
50 & 0.0 & 1.0 & 0.0 & \RBF & 10.0 & 0.967 & 4.271 & 0.917 & 6.217 & 61.184 & 64.984 & 0.609 & 2.156 \\
50 & 0.0 & 1.0 & 1.0 & \COS & - & 0.967 & 4.271 & 0.917 & 6.216 & 61.179 & 64.982 & 0.609 & 2.156 \\
50 & 0.0 & 1.0 & 1.0 & \RBF & 10.0 & 0.967 & 4.271 & 0.917 & 6.216 & 61.179 & 64.982 & 0.609 & 2.156 \\
50 & 0.0 & 1.0 & 10.0 & \COS & - & 0.969 & 4.293 & 0.920 & 6.222 & 61.627 & 65.079 & 0.588 & 1.968 \\
50 & 0.0 & 1.0 & 10.0 & \RBF & 10.0 & 0.969 & 4.291 & 0.920 & 6.222 & 61.583 & 65.069 & 0.588 & 1.983 \\
50 & 0.0 & 1.0 & 100.0 & \COS & - & 0.926 & 3.933 & 0.865 & 6.168 & 56.658 & 64.358 & 10.464 & 19.709 \\
50 & 0.0 & 1.0 & 100.0 & \RBF & 10.0 & 0.940 & 4.031 & 0.882 & 6.180 & 57.871 & 64.429 & 4.482 & 11.708 \\
50 & 0.05 & 0.1 & 0.0 & \COS & - & 0.968 & 4.293 & 0.920 & 6.230 & 62.100 & 65.165 & 0.588 & 2.013 \\
50 & 0.05 & 0.1 & 0.0 & \RBF & 10.0 & 0.968 & 4.293 & 0.920 & 6.230 & 62.100 & 65.165 & 0.588 & 2.013 \\
50 & 0.05 & 0.1 & 1.0 & \COS & - & 0.968 & 4.293 & 0.919 & 6.230 & 62.095 & 65.165 & 0.588 & 2.013 \\
50 & 0.05 & 0.1 & 1.0 & \RBF & 10.0 & 0.968 & 4.293 & 0.919 & 6.230 & 62.095 & 65.165 & 0.588 & 2.013 \\
50 & 0.05 & 0.1 & 10.0 & \COS & - & 0.969 & 4.307 & 0.921 & 6.233 & 62.300 & 65.223 & 0.580 & 1.954 \\
50 & 0.05 & 0.1 & 10.0 & \RBF & 10.0 & 0.969 & 4.306 & 0.921 & 6.233 & 62.295 & 65.223 & 0.580 & 1.961 \\
50 & 0.05 & 0.1 & 100.0 & \COS & - & 0.918 & 3.898 & 0.857 & 6.123 & 58.100 & 63.990 & 18.299 & 28.140 \\
50 & 0.05 & 0.1 & 100.0 & \RBF & 10.0 & 0.934 & 4.006 & 0.876 & 6.181 & 58.791 & 64.546 & 7.393 & 16.115 \\
50 & 0.05 & 1.0 & 0.0 & \COS & - & 0.969 & 4.310 & 0.922 & 6.233 & 62.353 & 65.245 & 0.580 & 1.906 \\
50 & 0.05 & 1.0 & 0.0 & \RBF & 10.0 & 0.969 & 4.310 & 0.922 & 6.233 & 62.353 & 65.245 & 0.580 & 1.906 \\
50 & 0.05 & 1.0 & 1.0 & \COS & - & 0.969 & 4.310 & 0.922 & 6.233 & 62.348 & 65.242 & 0.580 & 1.906 \\
50 & 0.05 & 1.0 & 1.0 & \RBF & 10.0 & 0.969 & 4.310 & 0.922 & 6.233 & 62.348 & 65.242 & 0.580 & 1.906 \\
50 & 0.05 & 1.0 & 10.0 & \COS & - & 0.969 & 4.310 & 0.922 & 6.234 & 62.348 & 65.255 & 0.580 & 1.898 \\
50 & 0.05 & 1.0 & 10.0 & \RBF & 10.0 & 0.969 & 4.310 & 0.922 & 6.234 & 62.344 & 65.255 & 0.580 & 1.898 \\
50 & 0.05 & 1.0 & 100.0 & \COS & - & 0.942 & 4.055 & 0.885 & 6.184 & 59.118 & 64.546 & 4.104 & 11.075 \\
50 & 0.05 & 1.0 & 100.0 & \RBF & 10.0 & 0.956 & 4.166 & 0.902 & 6.191 & 60.404 & 64.670 & 1.091 & 4.507 \\
50 & 0.1 & 0.1 & 0.0 & \COS & - & 0.926 & 3.960 & 0.870 & 5.972 & 57.554 & 62.553 & 18.816 & 23.479 \\
50 & 0.1 & 0.1 & 0.0 & \RBF & 10.0 & 0.926 & 3.961 & 0.870 & 5.972 & 57.554 & 62.553 & 18.816 & 23.479 \\
50 & 0.1 & 0.1 & 1.0 & \COS & - & 0.969 & 4.298 & 0.920 & 6.241 & 62.675 & 65.313 & 0.598 & 2.041 \\
50 & 0.1 & 0.1 & 1.0 & \RBF & 10.0 & 0.969 & 4.298 & 0.920 & 6.241 & 62.675 & 65.313 & 0.598 & 2.041 \\
50 & 0.1 & 0.1 & 10.0 & \COS & - & 0.969 & 4.312 & 0.921 & 6.245 & 62.787 & 65.389 & 0.616 & 2.010 \\
50 & 0.1 & 0.1 & 10.0 & \RBF & 10.0 & 0.969 & 4.310 & 0.921 & 6.244 & 62.772 & 65.374 & 0.616 & 2.017 \\
50 & 0.1 & 0.1 & 100.0 & \COS & - & 0.924 & 3.939 & 0.863 & 6.182 & 61.880 & 64.675 & 16.814 & 25.781 \\
50 & 0.1 & 0.1 & 100.0 & \RBF & 10.0 & 0.931 & 3.994 & 0.872 & 6.183 & 61.120 & 64.643 & 10.606 & 19.454 \\
50 & 0.1 & 1.0 & 0.0 & \COS & - & 0.970 & 4.317 & 0.922 & 6.245 & 62.904 & 65.393 & 0.615 & 1.948 \\
50 & 0.1 & 1.0 & 0.0 & \RBF & 10.0 & 0.970 & 4.317 & 0.922 & 6.245 & 62.904 & 65.393 & 0.615 & 1.948 \\
50 & 0.1 & 1.0 & 1.0 & \COS & - & 0.970 & 4.317 & 0.922 & 6.245 & 62.904 & 65.396 & 0.615 & 1.948 \\
50 & 0.1 & 1.0 & 1.0 & \RBF & 10.0 & 0.970 & 4.317 & 0.922 & 6.245 & 62.904 & 65.396 & 0.615 & 1.948 \\
50 & 0.1 & 1.0 & 10.0 & \COS & - & 0.970 & 4.319 & 0.922 & 6.247 & 62.918 & 65.410 & 0.615 & 1.948 \\
50 & 0.1 & 1.0 & 10.0 & \RBF & 10.0 & 0.970 & 4.318 & 0.922 & 6.247 & 62.913 & 65.408 & 0.615 & 1.948 \\
50 & 0.1 & 1.0 & 100.0 & \COS & - & 0.943 & 4.075 & 0.887 & 6.193 & 60.726 & 64.704 & 4.003 & 10.863 \\
50 & 0.1 & 1.0 & 100.0 & \RBF & 10.0 & 0.956 & 4.186 & 0.904 & 6.207 & 61.535 & 64.891 & 0.977 & 4.121 \\
50 & 0.5 & 0.1 & 0.0 & \COS & - & 0.915 & 3.796 & 0.851 & 5.820 & 62.767 & 61.893 & 21.142 & 28.107 \\
50 & 0.5 & 0.1 & 0.0 & \RBF & 10.0 & 0.915 & 3.796 & 0.851 & 5.820 & 62.767 & 61.893 & 21.142 & 28.107 \\
50 & 0.5 & 0.1 & 1.0 & \COS & - & 0.915 & 3.795 & 0.851 & 5.820 & 62.762 & 61.888 & 21.142 & 28.107 \\
50 & 0.5 & 0.1 & 1.0 & \RBF & 10.0 & 0.915 & 3.795 & 0.850 & 5.820 & 62.762 & 61.893 & 21.142 & 28.107 \\
50 & 0.5 & 0.1 & 10.0 & \COS & - & 0.914 & 3.793 & 0.850 & 5.819 & 62.733 & 61.885 & 21.190 & 28.264 \\
50 & 0.5 & 0.1 & 10.0 & \RBF & 10.0 & 0.914 & 3.793 & 0.850 & 5.819 & 62.733 & 61.890 & 21.190 & 28.257 \\
50 & 0.5 & 0.1 & 100.0 & \COS & - & 0.910 & 3.742 & 0.843 & 5.789 & 62.134 & 61.518 & 22.382 & 30.222 \\
50 & 0.5 & 0.1 & 100.0 & \RBF & 10.0 & 0.910 & 3.751 & 0.844 & 5.792 & 62.246 & 61.557 & 22.119 & 29.947 \\
50 & 0.5 & 1.0 & 0.0 & \COS & - & 0.916 & 3.801 & 0.851 & 5.828 & 62.567 & 61.988 & 20.746 & 27.172 \\
50 & 0.5 & 1.0 & 0.0 & \RBF & 10.0 & 0.916 & 3.801 & 0.851 & 5.828 & 62.567 & 61.988 & 20.746 & 27.172 \\
50 & 0.5 & 1.0 & 1.0 & \COS & - & 0.916 & 3.802 & 0.852 & 5.830 & 62.543 & 61.988 & 20.698 & 27.020 \\
50 & 0.5 & 1.0 & 1.0 & \RBF & 10.0 & 0.916 & 3.800 & 0.851 & 5.828 & 62.538 & 61.978 & 20.710 & 27.118 \\
50 & 0.5 & 1.0 & 10.0 & \COS & - & 0.917 & 3.808 & 0.852 & 5.841 & 62.358 & 62.034 & 20.285 & 26.573 \\
50 & 0.5 & 1.0 & 10.0 & \RBF & 10.0 & 0.917 & 3.807 & 0.852 & 5.842 & 62.416 & 62.056 & 20.374 & 26.645 \\
50 & 0.5 & 1.0 & 100.0 & \COS & - & 0.911 & 3.756 & 0.844 & 5.795 & 62.075 & 61.583 & 21.533 & 29.392 \\
50 & 0.5 & 1.0 & 100.0 & \RBF & 10.0 & 0.913 & 3.772 & 0.847 & 5.807 & 62.037 & 61.693 & 20.867 & 28.119 \\
50 & 1.0 & 0.1 & 0.0 & \COS & - & 0.967 & 3.854 & 0.910 & 4.851 & 71.235 & 53.369 & 7.623 & 13.961 \\
50 & 1.0 & 0.1 & 0.0 & \RBF & 10.0 & 0.967 & 3.854 & 0.910 & 4.851 & 71.235 & 53.369 & 7.623 & 13.961 \\
50 & 1.0 & 0.1 & 1.0 & \COS & - & 0.965 & 3.839 & 0.907 & 4.864 & 71.109 & 53.513 & 8.285 & 14.805 \\
50 & 1.0 & 0.1 & 1.0 & \RBF & 10.0 & 0.965 & 3.841 & 0.907 & 4.863 & 71.103 & 53.498 & 8.172 & 14.693 \\
50 & 1.0 & 0.1 & 10.0 & \COS & - & 0.948 & 3.704 & 0.882 & 4.869 & 69.998 & 53.091 & 18.854 & 28.549 \\
50 & 1.0 & 0.1 & 10.0 & \RBF & 10.0 & 0.951 & 3.723 & 0.886 & 4.878 & 70.246 & 53.250 & 17.628 & 26.520 \\
50 & 1.0 & 0.1 & 100.0 & \COS & - & 0.909 & 3.216 & 0.819 & 4.599 & 62.149 & 49.603 & 30.909 & 44.194 \\
50 & 1.0 & 0.1 & 100.0 & \RBF & 10.0 & 0.915 & 3.275 & 0.827 & 4.644 & 63.264 & 50.166 & 29.751 & 42.998 \\
50 & 1.0 & 1.0 & 0.0 & \COS & - & 0.966 & 3.848 & 0.909 & 4.856 & 71.172 & 53.415 & 7.726 & 14.200 \\
50 & 1.0 & 1.0 & 0.0 & \RBF & 10.0 & 0.966 & 3.848 & 0.909 & 4.856 & 71.172 & 53.415 & 7.726 & 14.200 \\
50 & 1.0 & 1.0 & 1.0 & \COS & - & 0.964 & 3.838 & 0.906 & 4.865 & 71.089 & 53.520 & 8.249 & 14.718 \\
50 & 1.0 & 1.0 & 1.0 & \RBF & 10.0 & 0.964 & 3.840 & 0.907 & 4.866 & 71.099 & 53.525 & 8.149 & 14.661 \\
50 & 1.0 & 1.0 & 10.0 & \COS & - & 0.948 & 3.698 & 0.883 & 4.850 & 69.920 & 52.845 & 19.415 & 29.478 \\
50 & 1.0 & 1.0 & 10.0 & \RBF & 10.0 & 0.951 & 3.720 & 0.887 & 4.862 & 70.246 & 53.047 & 18.395 & 27.633 \\
50 & 1.0 & 1.0 & 100.0 & \COS & - & 0.912 & 3.243 & 0.822 & 4.623 & 62.723 & 49.890 & 30.505 & 43.681 \\
50 & 1.0 & 1.0 & 100.0 & \RBF & 10.0 & 0.914 & 3.263 & 0.825 & 4.633 & 63.099 & 50.051 & 30.070 & 43.690 \\


==> tables/known_5percent.tex <==
\begin{ThreePartTable}
    \begin{TableNotes}[flushleft]  %%% This should come before longtable and it is not tablenotes but TableNotes
  \small
  \item
    \begin{footnotesize}
        \bgroup
%        \def\arraystretch{0.5}%       
        \setstretch{1}
		The columns corresponding to ``$l$'', ``$\alpha$'',
                ``$\beta$'', ``$\gamma$'', ``usim'', and ``$\sigma$'' have the
                latent dimension, weighting factor,
                latent vector regularization parameter,
                cell line similarity regularization parameter,
                cell line similarity function, and parameter for rbf cell line similarity,
                respectively, for \MTCRP.
	      \par
              \egroup
   \end{footnotesize}
  \end{TableNotes}
  \begin{longtable}{
      @{\hspace{5pt}}>{\raggedleft}p{0.03\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.03\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.03\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.04\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.03\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.03\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft\arraybackslash}p{0.06\textwidth}@{\hspace{7pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
    }
    \caption{\mbox{\MTCRP Performance on New and Known Drugs ($\theta$ = 5)}}
    \label{supp:tbl:transductive:5percent}\\
  %
    \hline\hline
    $l$	& $\alpha$	& $\beta$	& $\gamma$	& usim	& $\sigma$	& AP@$5$	& AH@$5$	& AP@$10$	& AH@$10$	& AT@$5$\% 	& AT@$10$\% 	& NT@$5$\% 	& NT@$10$\% \\
    \hline
    \endfirsthead
  %
    \multicolumn{14}{c}{{\tablename\ \thetable{} -- continued from previous page}}\\
    \hline\hline
    $l$ & $\alpha$      & $\beta$       & $\gamma$      & usim  & $\sigma$      & AP@$5$        & AH@$5$        & AP@$10$       & AH@$10$       & AT@$5$\%      & AT@$10$\%     & NT@$5$\%      & NT@$10$\% \\
    \hline
    \endhead
  %
    \hline
    %  \midrule
    \multicolumn{14}{c}{{Continued on next page}} \\
    \hline
    %\midrule
    \endfoot
    %
    \hline\hline
    %\bottomrule
    \insertTableNotes         %% this added
    \endlastfoot
    %
    \input{tables/known_5percent_data.tex}
	
    \hline
  \end{longtable}
\end{ThreePartTable}


==> tables/known_5percent_KRL.tex <==
\begin{ThreePartTable}
    \begin{TableNotes}[flushleft]  %%% This should come before longtable and it is not tablenotes but TableNotes
  \small
  \item
    \begin{footnotesize}
        \bgroup
%        \def\arraystretch{0.5}%       
        \setstretch{1}
                The columns corresponding to ``$k$'', ``$\lambda$'',
                ``usim'', and ``$\sigma$'' have the
                two hyperparameters, cell line similarity function,
                and parameter for {$\RBF$} cell line similarity, respectively, 
                for {\KRL}.
	      \par
              \egroup
   \end{footnotesize}
  \end{TableNotes}
  \begin{longtable}{
      @{\hspace{5pt}}>{\raggedleft}p{0.03\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.07\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.03\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft\arraybackslash}p{0.06\textwidth}@{\hspace{7pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
    }
    \caption{\mbox{\KRL Performance on New and Known Drugs ($\theta$ = 5)}}
    \label{supp:tbl:transductive:5percent:KRL}\\
  %
    \hline\hline
    $k$	& $\lambda$	& usim	& $\sigma$	& AP@$5$	& AH@$5$	& AP@$10$	& AH@$10$	& AT@$5$\% 	& AT@$10$\% 	& NT@$5$\% 	& NT@$10$\% \\
    \hline
    \endfirsthead
  %
    \multicolumn{12}{c}{{\tablename\ \thetable{} -- continued from previous page}}\\
    \hline\hline
    $k$ & $\lambda$     & usim  & $\sigma$      & AP@$5$        & AH@$5$        & AP@$10$       & AH@$10$       & AT@$5$\%      & AT@$10$\%     & NT@$5$\%      & NT@$10$\% \\
    \hline
    \endhead
  %
    \hline
    %  \midrule
    \multicolumn{12}{c}{{Continued on next page}} \\
    \hline
    %\midrule
    \endfoot
    %
    \hline\hline
    %\bottomrule
    \insertTableNotes         %% this added
    \endlastfoot
    %
    \input{tables/known_5percent_KRL_data.tex}
	
    \hline
  \end{longtable}
\end{ThreePartTable}


==> tables/known_5percent_KRL_data.tex <==
10	&   0.000001	&       \LIN	&          -	& 0.780	& 3.012	& 0.714	& 5.435	& 48.010	& 47.781	& 36.423	& 41.896 \\
10	&   0.000001	&       \RBF	&     0.0001	& 0.929	& 4.208	& 0.890	& 7.155	& 45.998	& 52.660	& 45.952	& 53.290 \\
10	&   0.000001	&       \RBF	&      0.001	& 0.952	& 4.359	& 0.912	& 7.981	& 52.736	& 60.151	& 42.330	& 50.277 \\
10	&   0.000001	&       \RBF	&       0.01	& 1.000	& 4.970	& 1.000	& 9.833	& 75.971	& 75.065	&  2.641	&  4.135 \\
10	&    0.00001	&       \LIN	&          -	& 0.876	& 3.838	& 0.832	& 6.938	& 53.910	& 56.543	& 46.293	& 52.328 \\
10	&    0.00001	&       \RBF	&     0.0001	& 0.930	& 4.201	& 0.886	& 7.008	& 44.317	& 50.536	& 44.652	& 50.761 \\
10	&    0.00001	&       \RBF	&      0.001	& 0.952	& 4.359	& 0.912	& 7.981	& 52.736	& 60.151	& 42.330	& 50.277 \\
10	&    0.00001	&       \RBF	&       0.01	& 1.000	& 4.969	& 1.000	& 9.831	& 75.947	& 75.009	&  2.581	&  4.024 \\
10	&     0.0001	&       \LIN	&          -	& 0.894	& 3.935	& 0.849	& 7.211	& 48.254	& 54.543	& 46.424	& 54.512 \\
10	&     0.0001	&       \RBF	&     0.0001	& 0.930	& 4.201	& 0.886	& 7.008	& 44.317	& 50.536	& 44.652	& 50.761 \\
10	&     0.0001	&       \RBF	&      0.001	& 0.952	& 4.359	& 0.912	& 7.981	& 52.736	& 60.151	& 42.330	& 50.277 \\
10	&     0.0001	&       \RBF	&       0.01	& 1.000	& 4.969	& 1.000	& 9.831	& 75.947	& 74.984	&  2.581	&  3.997 \\
10	&      0.001	&       \LIN	&          -	& 0.909	& 3.926	& 0.851	& 7.077	& 45.325	& 52.533	& 45.740	& 52.935 \\
10	&      0.001	&       \RBF	&     0.0001	& 0.930	& 4.201	& 0.886	& 7.008	& 44.317	& 50.536	& 44.652	& 50.761 \\
10	&      0.001	&       \RBF	&      0.001	& 0.952	& 4.359	& 0.912	& 7.981	& 52.736	& 60.151	& 42.330	& 50.277 \\
10	&      0.001	&       \RBF	&       0.01	& 1.000	& 4.969	& 1.000	& 9.829	& 75.942	& 74.940	&  2.581	&  3.911 \\
10	&       0.01	&       \LIN	&          -	& 0.912	& 4.062	& 0.856	& 7.078	& 45.949	& 52.297	& 46.278	& 52.690 \\
10	&       0.01	&       \RBF	&     0.0001	& 0.930	& 4.201	& 0.886	& 7.008	& 44.317	& 50.536	& 44.652	& 50.761 \\
10	&       0.01	&       \RBF	&      0.001	& 0.952	& 4.359	& 0.912	& 7.981	& 52.736	& 60.151	& 42.330	& 50.277 \\
10	&       0.01	&       \RBF	&       0.01	& 1.000	& 4.968	& 1.000	& 9.827	& 75.927	& 74.904	&  2.544	&  3.768 \\
10	&        0.1	&       \LIN	&          -	& 0.929	& 4.201	& 0.886	& 7.111	& 45.657	& 52.224	& 45.475	& 52.227 \\
10	&        0.1	&       \RBF	&     0.0001	& 0.930	& 4.201	& 0.886	& 7.008	& 44.317	& 50.536	& 44.652	& 50.761 \\
10	&        0.1	&       \RBF	&      0.001	& 0.952	& 4.359	& 0.912	& 7.981	& 52.736	& 60.151	& 42.330	& 50.277 \\
10	&        0.1	&       \RBF	&       0.01	& 1.000	& 4.968	& 1.000	& 9.824	& 75.917	& 74.826	&  2.509	&  3.615 \\
10	&        0.2	&       \LIN	&          -	& 0.929	& 4.184	& 0.888	& 7.033	& 45.418	& 51.640	& 45.607	& 52.131 \\
10	&        0.2	&       \RBF	&     0.0001	& 0.930	& 4.201	& 0.886	& 7.008	& 44.317	& 50.536	& 44.652	& 50.761 \\
10	&        0.2	&       \RBF	&      0.001	& 0.952	& 4.359	& 0.912	& 7.981	& 52.736	& 60.151	& 42.330	& 50.277 \\
10	&        0.2	&       \RBF	&       0.01	& 1.000	& 4.968	& 1.000	& 9.824	& 75.917	& 74.814	&  2.509	&  3.572 \\
10	&        0.4	&       \LIN	&          -	& 0.929	& 4.197	& 0.885	& 6.957	& 44.258	& 50.219	& 44.613	& 50.574 \\
10	&        0.4	&       \RBF	&     0.0001	& 0.930	& 4.201	& 0.886	& 7.008	& 44.317	& 50.536	& 44.652	& 50.761 \\
10	&        0.4	&       \RBF	&      0.001	& 0.952	& 4.359	& 0.912	& 7.981	& 52.736	& 60.151	& 42.330	& 50.277 \\
10	&        0.4	&       \RBF	&       0.01	& 1.000	& 4.968	& 1.000	& 9.823	& 75.922	& 74.814	&  2.509	&  3.559 \\
10	&        0.6	&       \LIN	&          -	& 0.929	& 4.197	& 0.885	& 6.925	& 44.253	& 49.737	& 44.613	& 50.098 \\
10	&        0.6	&       \RBF	&     0.0001	& 0.930	& 4.201	& 0.886	& 7.008	& 44.317	& 50.536	& 44.652	& 50.761 \\
10	&        0.6	&       \RBF	&      0.001	& 0.952	& 4.359	& 0.912	& 7.981	& 52.736	& 60.151	& 42.330	& 50.277 \\
10	&        0.6	&       \RBF	&       0.01	& 1.000	& 4.967	& 1.000	& 9.823	& 75.912	& 74.787	&  2.397	&  3.495 \\
10	&        0.8	&       \LIN	&          -	& 0.929	& 4.197	& 0.885	& 6.925	& 44.253	& 49.737	& 44.613	& 50.098 \\
10	&        0.8	&       \RBF	&     0.0001	& 0.930	& 4.201	& 0.886	& 7.008	& 44.317	& 50.536	& 44.652	& 50.761 \\
10	&        0.8	&       \RBF	&      0.001	& 0.952	& 4.359	& 0.912	& 7.981	& 52.736	& 60.151	& 42.330	& 50.277 \\
10	&        0.8	&       \RBF	&       0.01	& 1.000	& 4.967	& 1.000	& 9.822	& 75.902	& 74.767	&  2.362	&  3.465 \\
10	&        1.0	&       \LIN	&          -	& 0.929	& 4.197	& 0.885	& 6.925	& 44.253	& 49.737	& 44.613	& 50.098 \\
10	&        1.0	&       \RBF	&     0.0001	& 0.930	& 4.201	& 0.886	& 7.008	& 44.317	& 50.536	& 44.652	& 50.761 \\
10	&        1.0	&       \RBF	&      0.001	& 0.952	& 4.359	& 0.912	& 7.981	& 52.736	& 60.151	& 42.330	& 50.277 \\
10	&        1.0	&       \RBF	&       0.01	& 1.000	& 4.967	& 1.000	& 9.823	& 75.907	& 74.746	&  2.362	&  3.451 \\
10	&         10	&       \LIN	&          -	& 0.929	& 4.197	& 0.885	& 6.925	& 44.253	& 49.737	& 44.613	& 50.098 \\
10	&         10	&       \RBF	&     0.0001	& 0.930	& 4.201	& 0.886	& 7.008	& 44.317	& 50.536	& 44.652	& 50.761 \\
10	&         10	&       \RBF	&      0.001	& 0.952	& 4.359	& 0.912	& 7.981	& 52.736	& 60.151	& 42.330	& 50.277 \\
10	&         10	&       \RBF	&       0.01	& 1.000	& 4.966	& 1.000	& 9.820	& 75.854	& 74.667	&  2.241	&  3.203 \\
10	&         50	&       \LIN	&          -	& 0.929	& 4.197	& 0.885	& 6.925	& 44.253	& 49.737	& 44.613	& 50.098 \\
10	&         50	&       \RBF	&     0.0001	& 0.930	& 4.201	& 0.886	& 7.008	& 44.317	& 50.536	& 44.652	& 50.761 \\
10	&         50	&       \RBF	&      0.001	& 0.952	& 4.359	& 0.912	& 7.981	& 52.736	& 60.154	& 42.330	& 50.277 \\
10	&         50	&       \RBF	&       0.01	& 1.000	& 4.965	& 1.000	& 9.819	& 75.830	& 74.668	&  2.101	&  3.122 \\
10	&        100	&       \LIN	&          -	& 0.929	& 4.197	& 0.885	& 6.925	& 44.253	& 49.737	& 44.613	& 50.098 \\
10	&        100	&       \RBF	&     0.0001	& 0.930	& 4.201	& 0.886	& 7.008	& 44.317	& 50.536	& 44.652	& 50.761 \\
10	&        100	&       \RBF	&      0.001	& 0.952	& 4.359	& 0.912	& 7.981	& 52.736	& 60.151	& 42.330	& 50.277 \\
10	&        100	&       \RBF	&       0.01	& 1.000	& 4.965	& 1.000	& 9.819	& 75.820	& 74.672	&  2.101	&  3.156 \\


==> tables/known_5percent_baseline.tex <==
\begin{ThreePartTable}
    \begin{TableNotes}[flushleft]  %%% This should come before longtable and it is not tablenotes but TableNotes
  \small
  \item
    \begin{footnotesize}
        \bgroup
%        \def\arraystretch{0.5}%       
        \setstretch{1}
                The columns corresponding to ``$\alpha_b$'', ``$\beta_b$'',
                ``usim'', and ``$\sigma$'' have the
                two hyperparameters, cell line similarity function,
                and parameter for \hl{$\RBF$} cell line similarity, respectively, for \BMTMKL.
	      \par
              \egroup
   \end{footnotesize}
  \end{TableNotes}
  \begin{longtable}{
      @{\hspace{5pt}}>{\raggedleft}p{0.05\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.05\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.05\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.05\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft}p{0.06\textwidth}@{\hspace{7pt}}
      @{\hspace{5pt}}>{\raggedleft\arraybackslash}p{0.06\textwidth}@{\hspace{7pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
%        @{\hspace{5pt}}c@{\hspace{5pt}}
    }
    \caption{\mbox{\BMTMKL Performance on New and Known Drugs ($\theta$ = 5)}}
    \label{supp:tbl:transductive:5percent:baseline}\\
  %
    \hline\hline
    $\alpha_b$	& $\beta_b$	& usim	& $\sigma$	& AP@$5$	& AH@$5$	& AP@$10$	& AH@$10$	& AT@$5$\% 	& AT@$10$\% 	& NT@$5$\% 	& NT@$10$\% \\
    \hline
    \endfirsthead
  %
    \multicolumn{12}{c}{{\tablename\ \thetable{} -- continued from previous page}}\\
    \hline\hline
    $\alpha_b$  & $\beta_b$     & usim  & $\sigma$      & AP@$5$        & AH@$5$        & AP@$10$       & AH@$10$       & AT@$5$\%      & AT@$10$\%     & NT@$5$\%      & NT@$10$\% \\
    \hline
    \endhead
  %
    \hline
    %  \midrule
    \multicolumn{12}{c}{{Continued on next page}} \\
    \hline
    %\midrule
    \endfoot
    %
    \hline\hline
    %\bottomrule
    \insertTableNotes         %% this added
    \endlastfoot
    %
    \input{tables/known_5percent_baseline_data.tex}
	
    \hline
  \end{longtable}
\end{ThreePartTable}


==> tables/known_5percent_baseline_data.tex <==
1e0     & 1e0   & \RBF   & 10.0  & 0.942 & 0.906 & 4.311 & 7.758 & 48.03 & 54.57 & 47.57 & 54.00 \\
1e-10   & 1e10  & \RBF   & 10.0  & 0.942 & 0.906 & 4.312 & 7.758 & 48.03 & 54.55 & 47.61 & 54.00 \\
1e-10   & 1e-10 & \RBF   & 10.0  & 0.942 & 0.906 & 4.308 & 7.756 & 47.99 & 54.49 & 47.62 & 54.01 \\
1e0     & 1e0   & \COS   & -     & 0.935 & 0.898 & 4.183 & 7.539 & 45.49 & 53.01 & 45.41 & 52.47 \\
1e-10   & 1e10  & \COS   & -     & 0.935 & 0.898 & 4.191 & 7.574 & 45.74 & 53.31 & 45.71 & 52.76 \\
1e-10   & 1e-10 & \COS   & -     & 0.936 & 0.900 & 4.200 & 7.551 & 45.54 & 53.17 & 45.65 & 52.69 \\


==> tables/known_5percent_data.tex <==
5 & 0.0 & 0.1 & 0.0 & \COS & - & 0.996 & 4.965 & 0.995 & 9.914 & 47.800 & 56.938 & 44.523 & 54.579 \\
5 & 0.0 & 0.1 & 0.0 & \RBF & 10.0 & 0.996 & 4.965 & 0.995 & 9.914 & 47.800 & 56.938 & 44.523 & 54.579 \\
5 & 0.0 & 0.1 & 1.0 & \COS & - & 0.996 & 4.965 & 0.995 & 9.914 & 47.800 & 56.938 & 44.542 & 54.579 \\
5 & 0.0 & 0.1 & 1.0 & \RBF & 10.0 & 0.996 & 4.965 & 0.995 & 9.914 & 47.800 & 56.938 & 44.542 & 54.579 \\
5 & 0.0 & 0.1 & 10.0 & \COS & - & 0.996 & 4.965 & 0.995 & 9.914 & 47.790 & 56.928 & 44.542 & 54.569 \\
5 & 0.0 & 0.1 & 10.0 & \RBF & 10.0 & 0.996 & 4.965 & 0.995 & 9.914 & 47.790 & 56.926 & 44.542 & 54.560 \\
5 & 0.0 & 0.1 & 100.0 & \COS & - & 0.996 & 4.965 & 0.995 & 9.913 & 47.747 & 56.865 & 44.429 & 54.453 \\
5 & 0.0 & 0.1 & 100.0 & \RBF & 10.0 & 0.996 & 4.965 & 0.995 & 9.913 & 47.737 & 56.867 & 44.429 & 54.464 \\
5 & 0.0 & 1.0 & 0.0 & \COS & - & 0.996 & 4.965 & 0.995 & 9.914 & 47.796 & 56.936 & 44.523 & 54.565 \\
5 & 0.0 & 1.0 & 0.0 & \RBF & 10.0 & 0.996 & 4.965 & 0.995 & 9.914 & 47.796 & 56.936 & 44.523 & 54.565 \\
5 & 0.0 & 1.0 & 1.0 & \COS & - & 0.996 & 4.965 & 0.995 & 9.914 & 47.800 & 56.938 & 44.542 & 54.579 \\
5 & 0.0 & 1.0 & 1.0 & \RBF & 10.0 & 0.996 & 4.965 & 0.995 & 9.914 & 47.800 & 56.936 & 44.542 & 54.565 \\
5 & 0.0 & 1.0 & 10.0 & \COS & - & 0.997 & 4.977 & 0.997 & 9.937 & 52.906 & 59.764 & 27.191 & 33.642 \\
5 & 0.0 & 1.0 & 10.0 & \RBF & 10.0 & 0.997 & 4.977 & 0.997 & 9.937 & 52.906 & 59.761 & 27.191 & 33.633 \\
5 & 0.0 & 1.0 & 100.0 & \COS & - & 0.996 & 4.965 & 0.995 & 9.913 & 47.747 & 56.865 & 44.429 & 54.453 \\
5 & 0.0 & 1.0 & 100.0 & \RBF & 10.0 & 0.996 & 4.965 & 0.995 & 9.913 & 47.737 & 56.867 & 44.429 & 54.464 \\
5 & 0.05 & 0.1 & 0.0 & \COS & - & 0.997 & 4.976 & 0.996 & 9.935 & 56.365 & 62.799 & 27.662 & 35.451 \\
5 & 0.05 & 0.1 & 0.0 & \RBF & 10.0 & 0.997 & 4.976 & 0.996 & 9.935 & 56.365 & 62.799 & 27.662 & 35.451 \\
5 & 0.05 & 0.1 & 1.0 & \COS & - & 0.997 & 4.976 & 0.996 & 9.935 & 56.268 & 62.721 & 27.624 & 35.344 \\
5 & 0.05 & 0.1 & 1.0 & \RBF & 10.0 & 0.997 & 4.976 & 0.996 & 9.935 & 56.302 & 62.748 & 27.662 & 35.426 \\
5 & 0.05 & 0.1 & 10.0 & \COS & - & 0.997 & 4.977 & 0.997 & 9.936 & 54.080 & 60.597 & 27.210 & 33.641 \\
5 & 0.05 & 0.1 & 10.0 & \RBF & 10.0 & 0.997 & 4.977 & 0.997 & 9.936 & 54.075 & 60.609 & 27.210 & 33.647 \\
5 & 0.05 & 0.1 & 100.0 & \COS & - & 0.997 & 4.976 & 0.996 & 9.933 & 58.733 & 65.109 & 28.793 & 39.563 \\
5 & 0.05 & 0.1 & 100.0 & \RBF & 10.0 & 0.997 & 4.976 & 0.996 & 9.934 & 58.577 & 64.894 & 28.725 & 38.953 \\
5 & 0.05 & 1.0 & 0.0 & \COS & - & 0.997 & 4.977 & 0.997 & 9.936 & 54.061 & 60.599 & 27.192 & 33.620 \\
5 & 0.05 & 1.0 & 0.0 & \RBF & 10.0 & 0.997 & 4.977 & 0.997 & 9.936 & 54.061 & 60.599 & 27.192 & 33.620 \\
5 & 0.05 & 1.0 & 1.0 & \COS & - & 0.997 & 4.977 & 0.997 & 9.936 & 54.056 & 60.599 & 27.192 & 33.620 \\
5 & 0.05 & 1.0 & 1.0 & \RBF & 10.0 & 0.997 & 4.977 & 0.997 & 9.936 & 54.056 & 60.599 & 27.192 & 33.620 \\
5 & 0.05 & 1.0 & 10.0 & \COS & - & 0.997 & 4.977 & 0.997 & 9.936 & 54.022 & 60.589 & 27.192 & 33.616 \\
5 & 0.05 & 1.0 & 10.0 & \RBF & 10.0 & 0.997 & 4.977 & 0.997 & 9.936 & 54.027 & 60.587 & 27.192 & 33.616 \\
5 & 0.05 & 1.0 & 100.0 & \COS & - & 0.997 & 4.976 & 0.996 & 9.932 & 57.876 & 64.200 & 28.564 & 38.644 \\
5 & 0.05 & 1.0 & 100.0 & \RBF & 10.0 & 0.997 & 4.976 & 0.996 & 9.932 & 57.442 & 63.868 & 28.400 & 38.049 \\
5 & 0.1 & 0.1 & 0.0 & \COS & - & 0.996 & 4.965 & 0.995 & 9.913 & 48.185 & 57.137 & 44.518 & 54.518 \\
5 & 0.1 & 0.1 & 0.0 & \RBF & 10.0 & 0.996 & 4.965 & 0.995 & 9.913 & 48.185 & 57.137 & 44.518 & 54.518 \\
5 & 0.1 & 0.1 & 1.0 & \COS & - & 0.996 & 4.965 & 0.995 & 9.913 & 48.180 & 57.137 & 44.500 & 54.518 \\
5 & 0.1 & 0.1 & 1.0 & \RBF & 10.0 & 0.996 & 4.965 & 0.995 & 9.913 & 48.180 & 57.137 & 44.500 & 54.518 \\
5 & 0.1 & 0.1 & 10.0 & \COS & - & 0.996 & 4.965 & 0.995 & 9.914 & 48.166 & 57.140 & 44.518 & 54.507 \\
5 & 0.1 & 0.1 & 10.0 & \RBF & 10.0 & 0.996 & 4.965 & 0.995 & 9.914 & 48.161 & 57.140 & 44.500 & 54.507 \\
5 & 0.1 & 0.1 & 100.0 & \COS & - & 0.996 & 4.965 & 0.995 & 9.913 & 48.161 & 57.091 & 44.692 & 54.537 \\
5 & 0.1 & 0.1 & 100.0 & \RBF & 10.0 & 0.996 & 4.965 & 0.995 & 9.913 & 48.166 & 57.096 & 44.692 & 54.542 \\
5 & 0.1 & 1.0 & 0.0 & \COS & - & 0.996 & 4.965 & 0.995 & 9.913 & 48.185 & 57.137 & 44.518 & 54.518 \\
5 & 0.1 & 1.0 & 0.0 & \RBF & 10.0 & 0.996 & 4.965 & 0.995 & 9.913 & 48.185 & 57.137 & 44.518 & 54.518 \\
5 & 0.1 & 1.0 & 1.0 & \COS & - & 0.996 & 4.965 & 0.995 & 9.913 & 48.180 & 57.137 & 44.500 & 54.518 \\
5 & 0.1 & 1.0 & 1.0 & \RBF & 10.0 & 0.996 & 4.965 & 0.995 & 9.913 & 48.180 & 57.137 & 44.500 & 54.518 \\
5 & 0.1 & 1.0 & 10.0 & \COS & - & 0.996 & 4.965 & 0.995 & 9.914 & 48.166 & 57.140 & 44.518 & 54.507 \\
5 & 0.1 & 1.0 & 10.0 & \RBF & 10.0 & 0.996 & 4.965 & 0.995 & 9.914 & 48.161 & 57.140 & 44.500 & 54.513 \\
5 & 0.1 & 1.0 & 100.0 & \COS & - & 0.996 & 4.965 & 0.995 & 9.913 & 48.161 & 57.089 & 44.692 & 54.537 \\
5 & 0.1 & 1.0 & 100.0 & \RBF & 10.0 & 0.996 & 4.965 & 0.995 & 9.913 & 48.166 & 57.096 & 44.692 & 54.542 \\
5 & 0.5 & 0.1 & 0.0 & \COS & - & 0.996 & 4.965 & 0.995 & 9.912 & 49.822 & 57.968 & 45.399 & 54.836 \\
5 & 0.5 & 0.1 & 0.0 & \RBF & 10.0 & 0.996 & 4.965 & 0.995 & 9.912 & 49.822 & 57.968 & 45.399 & 54.836 \\
5 & 0.5 & 0.1 & 1.0 & \COS & - & 0.996 & 4.965 & 0.995 & 9.912 & 49.822 & 57.961 & 45.399 & 54.836 \\
5 & 0.5 & 0.1 & 1.0 & \RBF & 10.0 & 0.996 & 4.965 & 0.995 & 9.912 & 49.822 & 57.961 & 45.399 & 54.836 \\
5 & 0.5 & 0.1 & 10.0 & \COS & - & 0.996 & 4.965 & 0.995 & 9.911 & 49.842 & 57.966 & 45.465 & 54.836 \\
5 & 0.5 & 0.1 & 10.0 & \RBF & 10.0 & 0.996 & 4.965 & 0.995 & 9.911 & 49.842 & 57.966 & 45.465 & 54.836 \\
5 & 0.5 & 0.1 & 100.0 & \COS & - & 0.996 & 4.965 & 0.995 & 9.910 & 49.817 & 57.920 & 45.443 & 54.707 \\
5 & 0.5 & 0.1 & 100.0 & \RBF & 10.0 & 0.996 & 4.965 & 0.995 & 9.910 & 49.817 & 57.929 & 45.407 & 54.748 \\
5 & 0.5 & 1.0 & 0.0 & \COS & - & 0.996 & 4.965 & 0.995 & 9.912 & 49.822 & 57.966 & 45.399 & 54.836 \\
5 & 0.5 & 1.0 & 0.0 & \RBF & 10.0 & 0.996 & 4.965 & 0.995 & 9.912 & 49.822 & 57.966 & 45.399 & 54.836 \\
5 & 0.5 & 1.0 & 1.0 & \COS & - & 0.996 & 4.965 & 0.995 & 9.912 & 49.822 & 57.961 & 45.399 & 54.836 \\
5 & 0.5 & 1.0 & 1.0 & \RBF & 10.0 & 0.996 & 4.965 & 0.995 & 9.912 & 49.822 & 57.961 & 45.399 & 54.836 \\
5 & 0.5 & 1.0 & 10.0 & \COS & - & 0.996 & 4.965 & 0.995 & 9.911 & 49.842 & 57.966 & 45.465 & 54.836 \\
5 & 0.5 & 1.0 & 10.0 & \RBF & 10.0 & 0.996 & 4.965 & 0.995 & 9.911 & 49.842 & 57.966 & 45.465 & 54.836 \\
5 & 0.5 & 1.0 & 100.0 & \COS & - & 0.996 & 4.965 & 0.995 & 9.910 & 49.817 & 57.920 & 45.443 & 54.707 \\
5 & 0.5 & 1.0 & 100.0 & \RBF & 10.0 & 0.996 & 4.965 & 0.995 & 9.910 & 49.817 & 57.929 & 45.407 & 54.748 \\
5 & 1.0 & 0.1 & 0.0 & \COS & - & 0.960 & 4.659 & 0.946 & 9.129 & 47.766 & 50.965 & 40.496 & 45.096 \\
5 & 1.0 & 0.1 & 0.0 & \RBF & 10.0 & 0.960 & 4.659 & 0.946 & 9.129 & 47.766 & 50.965 & 40.496 & 45.096 \\
5 & 1.0 & 0.1 & 1.0 & \COS & - & 0.962 & 4.670 & 0.948 & 9.152 & 48.073 & 51.274 & 40.583 & 45.399 \\
5 & 1.0 & 0.1 & 1.0 & \RBF & 10.0 & 0.961 & 4.669 & 0.948 & 9.149 & 48.049 & 51.213 & 40.583 & 45.333 \\
5 & 1.0 & 0.1 & 10.0 & \COS & - & 0.968 & 4.718 & 0.955 & 9.222 & 49.067 & 52.246 & 41.149 & 46.280 \\
5 & 1.0 & 0.1 & 10.0 & \RBF & 10.0 & 0.967 & 4.712 & 0.954 & 9.213 & 48.994 & 52.151 & 41.024 & 46.130 \\
5 & 1.0 & 0.1 & 100.0 & \COS & - & 0.980 & 4.833 & 0.973 & 9.501 & 52.521 & 55.756 & 44.319 & 48.895 \\
5 & 1.0 & 0.1 & 100.0 & \RBF & 10.0 & 0.980 & 4.831 & 0.972 & 9.473 & 52.307 & 55.340 & 44.207 & 48.730 \\
5 & 1.0 & 1.0 & 0.0 & \COS & - & 0.963 & 4.676 & 0.949 & 9.155 & 48.292 & 51.384 & 40.704 & 45.492 \\
5 & 1.0 & 1.0 & 0.0 & \RBF & 10.0 & 0.963 & 4.676 & 0.949 & 9.155 & 48.292 & 51.384 & 40.704 & 45.492 \\
5 & 1.0 & 1.0 & 1.0 & \COS & - & 0.964 & 4.683 & 0.950 & 9.166 & 48.395 & 51.525 & 40.861 & 45.618 \\
5 & 1.0 & 1.0 & 1.0 & \RBF & 10.0 & 0.963 & 4.683 & 0.950 & 9.166 & 48.400 & 51.515 & 40.861 & 45.602 \\
5 & 1.0 & 1.0 & 10.0 & \COS & - & 0.969 & 4.729 & 0.956 & 9.240 & 49.408 & 52.558 & 41.399 & 46.530 \\
5 & 1.0 & 1.0 & 10.0 & \RBF & 10.0 & 0.968 & 4.724 & 0.956 & 9.232 & 49.272 & 52.438 & 41.215 & 46.418 \\
5 & 1.0 & 1.0 & 100.0 & \COS & - & 0.981 & 4.835 & 0.973 & 9.503 & 52.667 & 55.822 & 44.323 & 49.057 \\
5 & 1.0 & 1.0 & 100.0 & \RBF & 10.0 & 0.980 & 4.830 & 0.973 & 9.474 & 52.321 & 55.420 & 44.134 & 48.756 \\
10 & 0.0 & 0.1 & 0.0 & \COS & - & 0.998 & 4.976 & 0.997 & 9.935 & 51.177 & 59.739 & 34.656 & 50.379 \\
10 & 0.0 & 0.1 & 0.0 & \RBF & 10.0 & 0.998 & 4.976 & 0.997 & 9.935 & 51.177 & 59.739 & 34.656 & 50.379 \\
10 & 0.0 & 0.1 & 1.0 & \COS & - & 0.998 & 4.976 & 0.997 & 9.934 & 51.186 & 59.732 & 34.730 & 50.379 \\
10 & 0.0 & 0.1 & 1.0 & \RBF & 10.0 & 0.998 & 4.976 & 0.997 & 9.934 & 51.186 & 59.734 & 34.730 & 50.379 \\
10 & 0.0 & 0.1 & 10.0 & \COS & - & 0.998 & 4.976 & 0.997 & 9.934 & 51.186 & 59.715 & 34.804 & 50.386 \\
10 & 0.0 & 0.1 & 10.0 & \RBF & 10.0 & 0.998 & 4.976 & 0.997 & 9.934 & 51.177 & 59.718 & 34.786 & 50.386 \\
10 & 0.0 & 0.1 & 100.0 & \COS & - & 0.998 & 4.977 & 0.997 & 9.934 & 51.172 & 59.705 & 34.988 & 50.570 \\
10 & 0.0 & 0.1 & 100.0 & \RBF & 10.0 & 0.998 & 4.977 & 0.997 & 9.934 & 51.176 & 59.708 & 34.988 & 50.505 \\
10 & 0.0 & 1.0 & 0.0 & \COS & - & 0.998 & 4.976 & 0.997 & 9.934 & 51.181 & 59.734 & 34.693 & 50.379 \\
10 & 0.0 & 1.0 & 0.0 & \RBF & 10.0 & 0.998 & 4.976 & 0.997 & 9.934 & 51.181 & 59.734 & 34.693 & 50.379 \\
10 & 0.0 & 1.0 & 1.0 & \COS & - & 0.998 & 4.976 & 0.997 & 9.934 & 51.186 & 59.732 & 34.730 & 50.379 \\
10 & 0.0 & 1.0 & 1.0 & \RBF & 10.0 & 0.998 & 4.976 & 0.997 & 9.934 & 51.186 & 59.732 & 34.730 & 50.379 \\
10 & 0.0 & 1.0 & 10.0 & \COS & - & 0.998 & 4.976 & 0.997 & 9.934 & 51.186 & 59.715 & 34.804 & 50.386 \\
10 & 0.0 & 1.0 & 10.0 & \RBF & 10.0 & 0.998 & 4.976 & 0.997 & 9.934 & 51.181 & 59.715 & 34.804 & 50.386 \\
10 & 0.0 & 1.0 & 100.0 & \COS & - & 0.998 & 4.977 & 0.997 & 9.934 & 51.172 & 59.705 & 34.988 & 50.570 \\
10 & 0.0 & 1.0 & 100.0 & \RBF & 10.0 & 0.998 & 4.977 & 0.997 & 9.934 & 51.176 & 59.708 & 34.988 & 50.505 \\
10 & 0.05 & 0.1 & 0.0 & \COS & - & 0.998 & 4.977 & 0.997 & 9.936 & 51.299 & 59.876 & 34.548 & 50.211 \\
10 & 0.05 & 0.1 & 0.0 & \RBF & 10.0 & 0.998 & 4.977 & 0.997 & 9.936 & 51.299 & 59.876 & 34.548 & 50.211 \\
10 & 0.05 & 0.1 & 1.0 & \COS & - & 0.998 & 4.977 & 0.997 & 9.936 & 51.303 & 59.876 & 34.585 & 50.211 \\
10 & 0.05 & 0.1 & 1.0 & \RBF & 10.0 & 0.998 & 4.977 & 0.997 & 9.936 & 51.303 & 59.876 & 34.585 & 50.211 \\
10 & 0.05 & 0.1 & 10.0 & \COS & - & 0.998 & 4.977 & 0.997 & 9.936 & 51.304 & 59.859 & 34.696 & 50.211 \\
10 & 0.05 & 0.1 & 10.0 & \RBF & 10.0 & 0.998 & 4.977 & 0.997 & 9.936 & 51.304 & 59.859 & 34.696 & 50.211 \\
10 & 0.05 & 0.1 & 100.0 & \COS & - & 0.998 & 4.977 & 0.997 & 9.934 & 51.318 & 59.825 & 34.833 & 50.363 \\
10 & 0.05 & 0.1 & 100.0 & \RBF & 10.0 & 0.998 & 4.977 & 0.997 & 9.934 & 51.323 & 59.839 & 34.850 & 50.338 \\
10 & 0.05 & 1.0 & 0.0 & \COS & - & 0.998 & 4.977 & 0.997 & 9.936 & 51.303 & 59.876 & 34.585 & 50.211 \\
10 & 0.05 & 1.0 & 0.0 & \RBF & 10.0 & 0.998 & 4.977 & 0.997 & 9.936 & 51.303 & 59.876 & 34.585 & 50.211 \\
10 & 0.05 & 1.0 & 1.0 & \COS & - & 0.998 & 4.977 & 0.997 & 9.936 & 51.303 & 59.876 & 34.585 & 50.211 \\
10 & 0.05 & 1.0 & 1.0 & \RBF & 10.0 & 0.998 & 4.977 & 0.997 & 9.936 & 51.303 & 59.876 & 34.585 & 50.211 \\
10 & 0.05 & 1.0 & 10.0 & \COS & - & 0.998 & 4.977 & 0.997 & 9.936 & 51.304 & 59.859 & 34.696 & 50.211 \\
10 & 0.05 & 1.0 & 10.0 & \RBF & 10.0 & 0.998 & 4.977 & 0.997 & 9.936 & 51.304 & 59.859 & 34.696 & 50.211 \\
10 & 0.05 & 1.0 & 100.0 & \COS & - & 0.998 & 4.977 & 0.997 & 9.934 & 51.318 & 59.825 & 34.833 & 50.377 \\
10 & 0.05 & 1.0 & 100.0 & \RBF & 10.0 & 0.998 & 4.977 & 0.997 & 9.934 & 51.323 & 59.839 & 34.850 & 50.338 \\
10 & 0.1 & 0.1 & 0.0 & \COS & - & 0.998 & 4.977 & 0.997 & 9.937 & 51.459 & 60.005 & 34.310 & 50.096 \\
10 & 0.1 & 0.1 & 0.0 & \RBF & 10.0 & 0.998 & 4.977 & 0.997 & 9.937 & 51.459 & 60.005 & 34.310 & 50.096 \\
10 & 0.1 & 0.1 & 1.0 & \COS & - & 0.998 & 4.977 & 0.997 & 9.937 & 51.464 & 60.002 & 34.345 & 50.109 \\
10 & 0.1 & 0.1 & 1.0 & \RBF & 10.0 & 0.998 & 4.977 & 0.997 & 9.937 & 51.464 & 60.002 & 34.345 & 50.096 \\
10 & 0.1 & 0.1 & 10.0 & \COS & - & 0.998 & 4.977 & 0.997 & 9.937 & 51.479 & 59.995 & 34.413 & 50.129 \\
10 & 0.1 & 0.1 & 10.0 & \RBF & 10.0 & 0.998 & 4.977 & 0.997 & 9.937 & 51.474 & 59.995 & 34.376 & 50.129 \\
10 & 0.1 & 0.1 & 100.0 & \COS & - & 0.998 & 4.977 & 0.997 & 9.936 & 51.450 & 59.963 & 34.744 & 50.187 \\
10 & 0.1 & 0.1 & 100.0 & \RBF & 10.0 & 0.998 & 4.977 & 0.997 & 9.936 & 51.440 & 59.973 & 34.678 & 50.165 \\
10 & 0.1 & 1.0 & 0.0 & \COS & - & 0.998 & 4.977 & 0.997 & 9.937 & 51.464 & 60.002 & 34.345 & 50.096 \\
10 & 0.1 & 1.0 & 0.0 & \RBF & 10.0 & 0.998 & 4.977 & 0.997 & 9.937 & 51.464 & 60.002 & 34.345 & 50.096 \\
10 & 0.1 & 1.0 & 1.0 & \COS & - & 0.998 & 4.977 & 0.997 & 9.937 & 51.464 & 60.002 & 34.345 & 50.109 \\
10 & 0.1 & 1.0 & 1.0 & \RBF & 10.0 & 0.998 & 4.977 & 0.997 & 9.937 & 51.464 & 60.002 & 34.345 & 50.096 \\
10 & 0.1 & 1.0 & 10.0 & \COS & - & 0.998 & 4.977 & 0.997 & 9.937 & 51.474 & 59.993 & 34.413 & 50.129 \\
10 & 0.1 & 1.0 & 10.0 & \RBF & 10.0 & 0.998 & 4.977 & 0.997 & 9.937 & 51.474 & 59.995 & 34.376 & 50.129 \\
10 & 0.1 & 1.0 & 100.0 & \COS & - & 0.998 & 4.977 & 0.997 & 9.936 & 51.450 & 59.961 & 34.744 & 50.187 \\
10 & 0.1 & 1.0 & 100.0 & \RBF & 10.0 & 0.998 & 4.977 & 0.997 & 9.936 & 51.440 & 59.973 & 34.678 & 50.165 \\
10 & 0.5 & 0.1 & 0.0 & \COS & - & 0.998 & 4.979 & 0.997 & 9.935 & 52.872 & 60.933 & 33.078 & 48.144 \\
10 & 0.5 & 0.1 & 0.0 & \RBF & 10.0 & 0.998 & 4.979 & 0.997 & 9.935 & 52.872 & 60.933 & 33.078 & 48.144 \\
10 & 0.5 & 0.1 & 1.0 & \COS & - & 0.998 & 4.979 & 0.997 & 9.935 & 52.872 & 60.936 & 33.078 & 48.144 \\
10 & 0.5 & 0.1 & 1.0 & \RBF & 10.0 & 0.998 & 4.979 & 0.997 & 9.935 & 52.872 & 60.936 & 33.078 & 48.144 \\
10 & 0.5 & 0.1 & 10.0 & \COS & - & 0.998 & 4.979 & 0.997 & 9.936 & 52.872 & 60.930 & 33.142 & 48.153 \\
10 & 0.5 & 0.1 & 10.0 & \RBF & 10.0 & 0.998 & 4.979 & 0.997 & 9.936 & 52.877 & 60.928 & 33.142 & 48.153 \\
10 & 0.5 & 0.1 & 100.0 & \COS & - & 0.998 & 4.979 & 0.997 & 9.936 & 52.833 & 60.906 & 33.391 & 48.236 \\
10 & 0.5 & 0.1 & 100.0 & \RBF & 10.0 & 0.998 & 4.979 & 0.997 & 9.935 & 52.833 & 60.914 & 33.355 & 48.223 \\
10 & 0.5 & 1.0 & 0.0 & \COS & - & 0.998 & 4.979 & 0.997 & 9.935 & 52.872 & 60.933 & 33.078 & 48.144 \\
10 & 0.5 & 1.0 & 0.0 & \RBF & 10.0 & 0.998 & 4.979 & 0.997 & 9.935 & 52.872 & 60.933 & 33.078 & 48.144 \\
10 & 0.5 & 1.0 & 1.0 & \COS & - & 0.998 & 4.979 & 0.997 & 9.935 & 52.872 & 60.936 & 33.078 & 48.144 \\
10 & 0.5 & 1.0 & 1.0 & \RBF & 10.0 & 0.998 & 4.979 & 0.997 & 9.935 & 52.872 & 60.936 & 33.078 & 48.144 \\
10 & 0.5 & 1.0 & 10.0 & \COS & - & 0.998 & 4.979 & 0.997 & 9.936 & 52.872 & 60.930 & 33.142 & 48.153 \\
10 & 0.5 & 1.0 & 10.0 & \RBF & 10.0 & 0.998 & 4.979 & 0.997 & 9.936 & 52.877 & 60.930 & 33.142 & 48.153 \\
10 & 0.5 & 1.0 & 100.0 & \COS & - & 0.998 & 4.979 & 0.997 & 9.936 & 52.838 & 60.906 & 33.391 & 48.243 \\
10 & 0.5 & 1.0 & 100.0 & \RBF & 10.0 & 0.998 & 4.979 & 0.997 & 9.935 & 52.833 & 60.914 & 33.355 & 48.223 \\
10 & 1.0 & 0.1 & 0.0 & \COS & - & 0.964 & 4.688 & 0.952 & 9.221 & 48.171 & 48.097 & 36.147 & 40.119 \\
10 & 1.0 & 0.1 & 0.0 & \RBF & 10.0 & 0.964 & 4.688 & 0.952 & 9.221 & 48.171 & 48.097 & 36.147 & 40.119 \\
10 & 1.0 & 0.1 & 1.0 & \COS & - & 0.967 & 4.700 & 0.954 & 9.247 & 48.828 & 48.833 & 36.451 & 40.566 \\
10 & 1.0 & 0.1 & 1.0 & \RBF & 10.0 & 0.966 & 4.699 & 0.954 & 9.244 & 48.823 & 48.828 & 36.461 & 40.550 \\
10 & 1.0 & 0.1 & 10.0 & \COS & - & 0.973 & 4.748 & 0.961 & 9.330 & 51.259 & 51.225 & 37.423 & 41.744 \\
10 & 1.0 & 0.1 & 10.0 & \RBF & 10.0 & 0.973 & 4.747 & 0.961 & 9.328 & 51.206 & 51.191 & 37.429 & 41.705 \\
10 & 1.0 & 0.1 & 100.0 & \COS & - & 0.983 & 4.842 & 0.975 & 9.546 & 57.233 & 57.591 & 39.206 & 45.555 \\
10 & 1.0 & 0.1 & 100.0 & \RBF & 10.0 & 0.983 & 4.841 & 0.975 & 9.537 & 57.004 & 57.330 & 39.157 & 45.410 \\
10 & 1.0 & 1.0 & 0.0 & \COS & - & 0.967 & 4.703 & 0.954 & 9.245 & 48.979 & 48.860 & 36.186 & 40.491 \\
10 & 1.0 & 1.0 & 0.0 & \RBF & 10.0 & 0.967 & 4.703 & 0.954 & 9.245 & 48.979 & 48.860 & 36.186 & 40.491 \\
10 & 1.0 & 1.0 & 1.0 & \COS & - & 0.968 & 4.715 & 0.956 & 9.265 & 49.676 & 49.530 & 36.763 & 40.747 \\
10 & 1.0 & 1.0 & 1.0 & \RBF & 10.0 & 0.968 & 4.713 & 0.956 & 9.264 & 49.632 & 49.476 & 36.700 & 40.797 \\
10 & 1.0 & 1.0 & 10.0 & \COS & - & 0.975 & 4.761 & 0.963 & 9.350 & 51.971 & 51.976 & 37.879 & 41.993 \\
10 & 1.0 & 1.0 & 10.0 & \RBF & 10.0 & 0.974 & 4.756 & 0.962 & 9.344 & 51.737 & 51.739 & 37.721 & 41.943 \\
10 & 1.0 & 1.0 & 100.0 & \COS & - & 0.984 & 4.854 & 0.977 & 9.564 & 57.598 & 57.988 & 39.404 & 45.730 \\
10 & 1.0 & 1.0 & 100.0 & \RBF & 10.0 & 0.983 & 4.844 & 0.975 & 9.537 & 57.033 & 57.386 & 39.109 & 45.325 \\
15 & 0.0 & 0.1 & 0.0 & \COS & - & 0.999 & 4.987 & 0.999 & 9.955 & 51.864 & 59.956 & 15.553 & 36.200 \\
15 & 0.0 & 0.1 & 0.0 & \RBF & 10.0 & 0.999 & 4.987 & 0.999 & 9.955 & 51.864 & 59.956 & 15.553 & 36.200 \\
15 & 0.0 & 0.1 & 1.0 & \COS & - & 0.999 & 4.987 & 0.999 & 9.955 & 51.864 & 59.959 & 15.553 & 36.200 \\
15 & 0.0 & 0.1 & 1.0 & \RBF & 10.0 & 0.999 & 4.987 & 0.999 & 9.955 & 51.864 & 59.959 & 15.553 & 36.200 \\
15 & 0.0 & 0.1 & 10.0 & \COS & - & 0.999 & 4.987 & 0.999 & 9.955 & 51.854 & 59.961 & 15.588 & 36.213 \\
15 & 0.0 & 0.1 & 10.0 & \RBF & 10.0 & 0.999 & 4.987 & 0.999 & 9.955 & 51.864 & 59.966 & 15.588 & 36.213 \\
15 & 0.0 & 0.1 & 100.0 & \COS & - & 0.999 & 4.988 & 0.999 & 9.954 & 51.795 & 59.912 & 15.802 & 36.447 \\
15 & 0.0 & 0.1 & 100.0 & \RBF & 10.0 & 0.999 & 4.988 & 0.999 & 9.954 & 51.834 & 59.920 & 15.755 & 36.299 \\
15 & 0.0 & 1.0 & 0.0 & \COS & - & 0.999 & 4.987 & 0.999 & 9.955 & 51.854 & 59.956 & 15.413 & 36.076 \\
15 & 0.0 & 1.0 & 0.0 & \RBF & 10.0 & 0.999 & 4.987 & 0.999 & 9.955 & 51.854 & 59.956 & 15.413 & 36.076 \\
15 & 0.0 & 1.0 & 1.0 & \COS & - & 0.999 & 4.987 & 0.999 & 9.955 & 51.854 & 59.961 & 15.413 & 36.076 \\
15 & 0.0 & 1.0 & 1.0 & \RBF & 10.0 & 0.999 & 4.987 & 0.999 & 9.955 & 51.854 & 59.961 & 15.413 & 36.076 \\
15 & 0.0 & 1.0 & 10.0 & \COS & - & 0.999 & 4.987 & 0.999 & 9.955 & 51.854 & 59.961 & 15.460 & 36.076 \\
15 & 0.0 & 1.0 & 10.0 & \RBF & 10.0 & 0.999 & 4.987 & 0.999 & 9.955 & 51.859 & 59.963 & 15.460 & 36.076 \\
15 & 0.0 & 1.0 & 100.0 & \COS & - & 0.999 & 4.988 & 0.999 & 9.954 & 51.849 & 59.912 & 15.774 & 36.317 \\
15 & 0.0 & 1.0 & 100.0 & \RBF & 10.0 & 0.999 & 4.988 & 0.999 & 9.954 & 51.834 & 59.917 & 15.755 & 36.299 \\
15 & 0.05 & 0.1 & 0.0 & \COS & - & 0.999 & 4.988 & 0.999 & 9.955 & 51.995 & 60.000 & 15.277 & 35.564 \\
15 & 0.05 & 0.1 & 0.0 & \RBF & 10.0 & 0.999 & 4.988 & 0.999 & 9.955 & 51.995 & 60.000 & 15.277 & 35.564 \\
15 & 0.05 & 0.1 & 1.0 & \COS & - & 0.999 & 4.988 & 0.999 & 9.955 & 52.000 & 59.997 & 15.277 & 35.554 \\
15 & 0.05 & 0.1 & 1.0 & \RBF & 10.0 & 0.999 & 4.988 & 0.999 & 9.955 & 52.000 & 59.997 & 15.277 & 35.554 \\
15 & 0.05 & 0.1 & 10.0 & \COS & - & 0.999 & 4.988 & 0.999 & 9.955 & 52.020 & 59.998 & 15.379 & 35.581 \\
15 & 0.05 & 0.1 & 10.0 & \RBF & 10.0 & 0.999 & 4.988 & 0.999 & 9.955 & 52.020 & 59.998 & 15.379 & 35.581 \\
15 & 0.05 & 0.1 & 100.0 & \COS & - & 0.999 & 4.988 & 0.999 & 9.954 & 51.980 & 59.983 & 15.628 & 35.861 \\
15 & 0.05 & 0.1 & 100.0 & \RBF & 10.0 & 0.999 & 4.988 & 0.999 & 9.954 & 51.985 & 59.978 & 15.606 & 35.787 \\
15 & 0.05 & 1.0 & 0.0 & \COS & - & 0.999 & 4.988 & 0.999 & 9.955 & 51.995 & 59.997 & 15.277 & 35.554 \\
15 & 0.05 & 1.0 & 0.0 & \RBF & 10.0 & 0.999 & 4.988 & 0.999 & 9.955 & 51.995 & 59.997 & 15.277 & 35.554 \\
15 & 0.05 & 1.0 & 1.0 & \COS & - & 0.999 & 4.988 & 0.999 & 9.955 & 52.000 & 59.997 & 15.277 & 35.554 \\
15 & 0.05 & 1.0 & 1.0 & \RBF & 10.0 & 0.999 & 4.988 & 0.999 & 9.955 & 52.000 & 59.997 & 15.277 & 35.554 \\
15 & 0.05 & 1.0 & 10.0 & \COS & - & 0.999 & 4.988 & 0.999 & 9.955 & 52.020 & 59.998 & 15.379 & 35.581 \\
15 & 0.05 & 1.0 & 10.0 & \RBF & 10.0 & 0.999 & 4.988 & 0.999 & 9.955 & 52.020 & 59.998 & 15.379 & 35.581 \\
15 & 0.05 & 1.0 & 100.0 & \COS & - & 0.999 & 4.988 & 0.999 & 9.954 & 51.980 & 59.983 & 15.628 & 35.875 \\
15 & 0.05 & 1.0 & 100.0 & \RBF & 10.0 & 0.999 & 4.988 & 0.999 & 9.954 & 51.985 & 59.978 & 15.606 & 35.787 \\
15 & 0.1 & 0.1 & 0.0 & \COS & - & 0.999 & 4.988 & 0.999 & 9.955 & 52.112 & 60.110 & 14.902 & 35.024 \\
15 & 0.1 & 0.1 & 0.0 & \RBF & 10.0 & 0.999 & 4.988 & 0.999 & 9.955 & 52.112 & 60.110 & 14.902 & 35.024 \\
15 & 0.1 & 0.1 & 1.0 & \COS & - & 0.999 & 4.988 & 0.999 & 9.955 & 52.112 & 60.105 & 14.902 & 34.988 \\
15 & 0.1 & 0.1 & 1.0 & \RBF & 10.0 & 0.999 & 4.988 & 0.999 & 9.955 & 52.112 & 60.105 & 14.902 & 34.988 \\
15 & 0.1 & 0.1 & 10.0 & \COS & - & 0.999 & 4.988 & 0.999 & 9.956 & 52.117 & 60.095 & 14.957 & 34.999 \\
15 & 0.1 & 0.1 & 10.0 & \RBF & 10.0 & 0.999 & 4.988 & 0.999 & 9.956 & 52.117 & 60.100 & 14.957 & 34.992 \\
15 & 0.1 & 0.1 & 100.0 & \COS & - & 0.999 & 4.988 & 0.999 & 9.955 & 52.097 & 60.058 & 15.405 & 35.248 \\
15 & 0.1 & 0.1 & 100.0 & \RBF & 10.0 & 0.999 & 4.988 & 0.999 & 9.955 & 52.107 & 60.049 & 15.286 & 35.211 \\
15 & 0.1 & 1.0 & 0.0 & \COS & - & 0.999 & 4.988 & 0.999 & 9.955 & 52.112 & 60.110 & 14.902 & 35.024 \\
15 & 0.1 & 1.0 & 0.0 & \RBF & 10.0 & 0.999 & 4.988 & 0.999 & 9.955 & 52.112 & 60.110 & 14.902 & 35.024 \\
15 & 0.1 & 1.0 & 1.0 & \COS & - & 0.999 & 4.988 & 0.999 & 9.955 & 52.107 & 60.105 & 14.902 & 34.988 \\
15 & 0.1 & 1.0 & 1.0 & \RBF & 10.0 & 0.999 & 4.988 & 0.999 & 9.955 & 52.107 & 60.105 & 14.902 & 34.988 \\
15 & 0.1 & 1.0 & 10.0 & \COS & - & 0.999 & 4.988 & 0.999 & 9.956 & 52.117 & 60.095 & 14.957 & 34.999 \\
15 & 0.1 & 1.0 & 10.0 & \RBF & 10.0 & 0.999 & 4.988 & 0.999 & 9.956 & 52.117 & 60.100 & 14.957 & 34.999 \\
15 & 0.1 & 1.0 & 100.0 & \COS & - & 0.999 & 4.988 & 0.999 & 9.955 & 52.097 & 60.056 & 15.405 & 35.248 \\
15 & 0.1 & 1.0 & 100.0 & \RBF & 10.0 & 0.999 & 4.988 & 0.999 & 9.955 & 52.112 & 60.049 & 15.298 & 35.211 \\
15 & 0.5 & 0.1 & 0.0 & \COS & - & 0.999 & 4.987 & 0.999 & 9.955 & 53.622 & 60.816 & 13.751 & 30.763 \\
15 & 0.5 & 0.1 & 0.0 & \RBF & 10.0 & 0.999 & 4.987 & 0.999 & 9.955 & 53.622 & 60.816 & 13.751 & 30.763 \\
15 & 0.5 & 0.1 & 1.0 & \COS & - & 0.999 & 4.987 & 0.999 & 9.955 & 53.622 & 60.821 & 13.751 & 30.799 \\
15 & 0.5 & 0.1 & 1.0 & \RBF & 10.0 & 0.999 & 4.987 & 0.999 & 9.955 & 53.622 & 60.821 & 13.751 & 30.799 \\
15 & 0.5 & 0.1 & 10.0 & \COS & - & 0.999 & 4.987 & 0.999 & 9.955 & 53.622 & 60.818 & 13.713 & 30.817 \\
15 & 0.5 & 0.1 & 10.0 & \RBF & 10.0 & 0.999 & 4.987 & 0.999 & 9.955 & 53.622 & 60.821 & 13.751 & 30.826 \\
15 & 0.5 & 0.1 & 100.0 & \COS & - & 0.999 & 4.987 & 0.999 & 9.956 & 53.647 & 60.821 & 13.871 & 30.864 \\
15 & 0.5 & 0.1 & 100.0 & \RBF & 10.0 & 0.999 & 4.987 & 0.999 & 9.956 & 53.647 & 60.816 & 13.871 & 30.845 \\
15 & 0.5 & 1.0 & 0.0 & \COS & - & 0.999 & 4.987 & 0.999 & 9.955 & 53.622 & 60.818 & 13.751 & 30.790 \\
15 & 0.5 & 1.0 & 0.0 & \RBF & 10.0 & 0.999 & 4.987 & 0.999 & 9.955 & 53.622 & 60.818 & 13.751 & 30.790 \\
15 & 0.5 & 1.0 & 1.0 & \COS & - & 0.999 & 4.987 & 0.999 & 9.955 & 53.627 & 60.819 & 13.751 & 30.799 \\
15 & 0.5 & 1.0 & 1.0 & \RBF & 10.0 & 0.999 & 4.987 & 0.999 & 9.955 & 53.622 & 60.819 & 13.751 & 30.799 \\
15 & 0.5 & 1.0 & 10.0 & \COS & - & 0.999 & 4.987 & 0.999 & 9.955 & 53.622 & 60.816 & 13.713 & 30.817 \\
15 & 0.5 & 1.0 & 10.0 & \RBF & 10.0 & 0.999 & 4.987 & 0.999 & 9.955 & 53.622 & 60.818 & 13.713 & 30.817 \\
15 & 0.5 & 1.0 & 100.0 & \COS & - & 0.999 & 4.987 & 0.999 & 9.956 & 53.647 & 60.818 & 13.871 & 30.864 \\
15 & 0.5 & 1.0 & 100.0 & \RBF & 10.0 & 0.999 & 4.987 & 0.999 & 9.956 & 53.647 & 60.816 & 13.871 & 30.845 \\
15 & 1.0 & 0.1 & 0.0 & \COS & - & 0.980 & 4.807 & 0.969 & 9.452 & 50.743 & 49.259 & 31.667 & 37.397 \\
15 & 1.0 & 0.1 & 0.0 & \RBF & 10.0 & 0.980 & 4.807 & 0.969 & 9.452 & 50.743 & 49.259 & 31.667 & 37.397 \\
15 & 1.0 & 0.1 & 1.0 & \COS & - & 0.981 & 4.815 & 0.971 & 9.475 & 52.322 & 50.526 & 32.346 & 37.624 \\
15 & 1.0 & 0.1 & 1.0 & \RBF & 10.0 & 0.981 & 4.814 & 0.971 & 9.471 & 52.131 & 50.412 & 32.232 & 37.572 \\
15 & 1.0 & 0.1 & 10.0 & \COS & - & 0.983 & 4.836 & 0.974 & 9.515 & 54.382 & 52.446 & 33.719 & 39.044 \\
15 & 1.0 & 0.1 & 10.0 & \RBF & 10.0 & 0.983 & 4.838 & 0.974 & 9.512 & 54.266 & 52.346 & 33.671 & 38.723 \\
15 & 1.0 & 0.1 & 100.0 & \COS & - & 0.987 & 4.873 & 0.980 & 9.612 & 61.671 & 59.681 & 37.358 & 43.800 \\
15 & 1.0 & 0.1 & 100.0 & \RBF & 10.0 & 0.986 & 4.871 & 0.980 & 9.607 & 61.315 & 59.160 & 37.678 & 43.743 \\
15 & 1.0 & 1.0 & 0.0 & \COS & - & 0.982 & 4.822 & 0.972 & 9.478 & 52.867 & 50.943 & 32.329 & 37.380 \\
15 & 1.0 & 1.0 & 0.0 & \RBF & 10.0 & 0.982 & 4.822 & 0.972 & 9.478 & 52.867 & 50.943 & 32.329 & 37.380 \\
15 & 1.0 & 1.0 & 1.0 & \COS & - & 0.982 & 4.829 & 0.973 & 9.495 & 53.822 & 51.871 & 32.445 & 37.933 \\
15 & 1.0 & 1.0 & 1.0 & \RBF & 10.0 & 0.982 & 4.828 & 0.973 & 9.493 & 53.710 & 51.803 & 32.462 & 37.939 \\
15 & 1.0 & 1.0 & 10.0 & \COS & - & 0.984 & 4.850 & 0.976 & 9.541 & 55.932 & 53.942 & 34.013 & 39.266 \\
15 & 1.0 & 1.0 & 10.0 & \RBF & 10.0 & 0.984 & 4.848 & 0.976 & 9.540 & 55.917 & 53.937 & 33.798 & 39.049 \\
15 & 1.0 & 1.0 & 100.0 & \COS & - & 0.987 & 4.874 & 0.980 & 9.614 & 61.720 & 59.800 & 37.300 & 43.938 \\
15 & 1.0 & 1.0 & 100.0 & \RBF & 10.0 & 0.985 & 4.866 & 0.979 & 9.595 & 60.692 & 58.572 & 37.110 & 43.416 \\
30 & 0.0 & 0.1 & 0.0 & \COS & - & 1.000 & 4.994 & 0.999 & 9.972 & 55.026 & 60.463 & 2.336 & 8.114 \\
30 & 0.0 & 0.1 & 0.0 & \RBF & 10.0 & 1.000 & 4.994 & 0.999 & 9.972 & 55.026 & 60.463 & 2.336 & 8.114 \\
30 & 0.0 & 0.1 & 1.0 & \COS & - & 1.000 & 4.994 & 0.999 & 9.972 & 55.021 & 60.460 & 2.336 & 8.107 \\
30 & 0.0 & 0.1 & 1.0 & \RBF & 10.0 & 1.000 & 4.994 & 0.999 & 9.972 & 55.026 & 60.460 & 2.336 & 8.107 \\
30 & 0.0 & 0.1 & 10.0 & \COS & - & 1.000 & 4.994 & 0.999 & 9.972 & 55.060 & 60.456 & 2.299 & 7.920 \\
30 & 0.0 & 0.1 & 10.0 & \RBF & 10.0 & 1.000 & 4.994 & 0.999 & 9.972 & 55.060 & 60.458 & 2.299 & 7.913 \\
30 & 0.0 & 0.1 & 100.0 & \COS & - & 1.000 & 4.993 & 0.999 & 9.970 & 53.160 & 60.085 & 3.970 & 14.969 \\
30 & 0.0 & 0.1 & 100.0 & \RBF & 10.0 & 1.000 & 4.994 & 0.999 & 9.971 & 54.265 & 60.192 & 2.971 & 10.651 \\
30 & 0.0 & 1.0 & 0.0 & \COS & - & 1.000 & 4.994 & 0.999 & 9.972 & 55.104 & 60.475 & 2.257 & 7.860 \\
30 & 0.0 & 1.0 & 0.0 & \RBF & 10.0 & 1.000 & 4.994 & 0.999 & 9.972 & 55.104 & 60.475 & 2.257 & 7.860 \\
30 & 0.0 & 1.0 & 1.0 & \COS & - & 1.000 & 4.994 & 0.999 & 9.972 & 55.104 & 60.470 & 2.257 & 7.854 \\
30 & 0.0 & 1.0 & 1.0 & \RBF & 10.0 & 1.000 & 4.994 & 0.999 & 9.972 & 55.104 & 60.470 & 2.257 & 7.854 \\
30 & 0.0 & 1.0 & 10.0 & \COS & - & 1.000 & 4.994 & 0.999 & 9.972 & 55.084 & 60.458 & 2.287 & 7.877 \\
30 & 0.0 & 1.0 & 10.0 & \RBF & 10.0 & 1.000 & 4.994 & 0.999 & 9.972 & 55.084 & 60.460 & 2.287 & 7.877 \\
30 & 0.0 & 1.0 & 100.0 & \COS & - & 1.000 & 4.994 & 0.999 & 9.972 & 54.816 & 60.363 & 2.302 & 8.422 \\
30 & 0.0 & 1.0 & 100.0 & \RBF & 10.0 & 1.000 & 4.994 & 0.999 & 9.972 & 54.967 & 60.424 & 2.263 & 7.960 \\
30 & 0.05 & 0.1 & 0.0 & \COS & - & 1.000 & 4.994 & 0.999 & 9.972 & 55.508 & 60.624 & 2.299 & 7.636 \\
30 & 0.05 & 0.1 & 0.0 & \RBF & 10.0 & 1.000 & 4.994 & 0.999 & 9.972 & 55.508 & 60.624 & 2.299 & 7.636 \\
30 & 0.05 & 0.1 & 1.0 & \COS & - & 1.000 & 4.994 & 0.999 & 9.972 & 55.508 & 60.624 & 2.299 & 7.636 \\
30 & 0.05 & 0.1 & 1.0 & \RBF & 10.0 & 1.000 & 4.994 & 0.999 & 9.972 & 55.508 & 60.624 & 2.299 & 7.636 \\
30 & 0.05 & 0.1 & 10.0 & \COS & - & 1.000 & 4.994 & 0.999 & 9.972 & 55.474 & 60.619 & 2.299 & 7.636 \\
30 & 0.05 & 0.1 & 10.0 & \RBF & 10.0 & 1.000 & 4.994 & 0.999 & 9.972 & 55.488 & 60.619 & 2.299 & 7.636 \\
30 & 0.05 & 0.1 & 100.0 & \COS & - & 1.000 & 4.994 & 0.999 & 9.972 & 55.367 & 60.553 & 2.305 & 7.727 \\
30 & 0.05 & 0.1 & 100.0 & \RBF & 10.0 & 1.000 & 4.994 & 0.999 & 9.972 & 55.372 & 60.551 & 2.322 & 7.707 \\
30 & 0.05 & 1.0 & 0.0 & \COS & - & 1.000 & 4.994 & 0.999 & 9.972 & 55.508 & 60.624 & 2.299 & 7.636 \\
30 & 0.05 & 1.0 & 0.0 & \RBF & 10.0 & 1.000 & 4.994 & 0.999 & 9.972 & 55.508 & 60.624 & 2.299 & 7.636 \\
30 & 0.05 & 1.0 & 1.0 & \COS & - & 1.000 & 4.994 & 0.999 & 9.972 & 55.508 & 60.624 & 2.299 & 7.636 \\
30 & 0.05 & 1.0 & 1.0 & \RBF & 10.0 & 1.000 & 4.994 & 0.999 & 9.972 & 55.508 & 60.624 & 2.299 & 7.636 \\
30 & 0.05 & 1.0 & 10.0 & \COS & - & 1.000 & 4.994 & 0.999 & 9.972 & 55.474 & 60.621 & 2.299 & 7.641 \\
30 & 0.05 & 1.0 & 10.0 & \RBF & 10.0 & 1.000 & 4.994 & 0.999 & 9.972 & 55.484 & 60.619 & 2.299 & 7.636 \\
30 & 0.05 & 1.0 & 100.0 & \COS & - & 1.000 & 4.994 & 0.999 & 9.972 & 55.367 & 60.551 & 2.305 & 7.727 \\
30 & 0.05 & 1.0 & 100.0 & \RBF & 10.0 & 1.000 & 4.994 & 0.999 & 9.972 & 55.372 & 60.548 & 2.322 & 7.698 \\
30 & 0.1 & 0.1 & 0.0 & \COS & - & 1.000 & 4.994 & 0.999 & 9.972 & 55.810 & 60.840 & 2.313 & 7.571 \\
30 & 0.1 & 0.1 & 0.0 & \RBF & 10.0 & 1.000 & 4.994 & 0.999 & 9.972 & 55.810 & 60.840 & 2.313 & 7.571 \\
30 & 0.1 & 0.1 & 1.0 & \COS & - & 1.000 & 4.994 & 0.999 & 9.972 & 55.810 & 60.833 & 2.313 & 7.571 \\
30 & 0.1 & 0.1 & 1.0 & \RBF & 10.0 & 1.000 & 4.994 & 0.999 & 9.972 & 55.810 & 60.836 & 2.313 & 7.571 \\
30 & 0.1 & 0.1 & 10.0 & \COS & - & 1.000 & 4.994 & 0.999 & 9.972 & 55.771 & 60.833 & 2.313 & 7.635 \\
30 & 0.1 & 0.1 & 10.0 & \RBF & 10.0 & 1.000 & 4.994 & 0.999 & 9.972 & 55.776 & 60.833 & 2.313 & 7.607 \\
30 & 0.1 & 0.1 & 100.0 & \COS & - & 1.000 & 4.994 & 0.999 & 9.972 & 55.683 & 60.762 & 2.311 & 7.605 \\
30 & 0.1 & 0.1 & 100.0 & \RBF & 10.0 & 1.000 & 4.994 & 0.999 & 9.972 & 55.698 & 60.762 & 2.311 & 7.606 \\
30 & 0.1 & 1.0 & 0.0 & \COS & - & 1.000 & 4.994 & 0.999 & 9.972 & 55.810 & 60.838 & 2.313 & 7.571 \\
30 & 0.1 & 1.0 & 0.0 & \RBF & 10.0 & 1.000 & 4.994 & 0.999 & 9.972 & 55.810 & 60.838 & 2.313 & 7.571 \\
30 & 0.1 & 1.0 & 1.0 & \COS & - & 1.000 & 4.994 & 0.999 & 9.972 & 55.810 & 60.833 & 2.313 & 7.571 \\
30 & 0.1 & 1.0 & 1.0 & \RBF & 10.0 & 1.000 & 4.994 & 0.999 & 9.972 & 55.810 & 60.833 & 2.313 & 7.571 \\
30 & 0.1 & 1.0 & 10.0 & \COS & - & 1.000 & 4.994 & 0.999 & 9.972 & 55.771 & 60.833 & 2.313 & 7.635 \\
30 & 0.1 & 1.0 & 10.0 & \RBF & 10.0 & 1.000 & 4.994 & 0.999 & 9.972 & 55.776 & 60.833 & 2.313 & 7.607 \\
30 & 0.1 & 1.0 & 100.0 & \COS & - & 1.000 & 4.994 & 0.999 & 9.972 & 55.683 & 60.760 & 2.311 & 7.605 \\
30 & 0.1 & 1.0 & 100.0 & \RBF & 10.0 & 1.000 & 4.994 & 0.999 & 9.972 & 55.698 & 60.762 & 2.311 & 7.606 \\
30 & 0.5 & 0.1 & 0.0 & \COS & - & 1.000 & 4.994 & 0.999 & 9.972 & 58.207 & 62.273 & 2.309 & 6.954 \\
30 & 0.5 & 0.1 & 0.0 & \RBF & 10.0 & 1.000 & 4.994 & 0.999 & 9.972 & 58.207 & 62.273 & 2.309 & 6.954 \\
30 & 0.5 & 0.1 & 1.0 & \COS & - & 1.000 & 4.994 & 0.999 & 9.972 & 58.207 & 62.273 & 2.309 & 6.954 \\
30 & 0.5 & 0.1 & 1.0 & \RBF & 10.0 & 1.000 & 4.994 & 0.999 & 9.972 & 58.207 & 62.273 & 2.309 & 6.954 \\
30 & 0.5 & 0.1 & 10.0 & \COS & - & 1.000 & 4.994 & 0.999 & 9.972 & 58.197 & 62.275 & 2.309 & 6.954 \\
30 & 0.5 & 0.1 & 10.0 & \RBF & 10.0 & 1.000 & 4.994 & 0.999 & 9.972 & 58.197 & 62.275 & 2.309 & 6.954 \\
30 & 0.5 & 0.1 & 100.0 & \COS & - & 1.000 & 4.994 & 0.999 & 9.972 & 58.149 & 62.229 & 2.328 & 6.999 \\
30 & 0.5 & 0.1 & 100.0 & \RBF & 10.0 & 1.000 & 4.994 & 0.999 & 9.972 & 58.173 & 62.236 & 2.328 & 6.990 \\
30 & 0.5 & 1.0 & 0.0 & \COS & - & 1.000 & 4.994 & 0.999 & 9.972 & 58.207 & 62.273 & 2.309 & 6.954 \\
30 & 0.5 & 1.0 & 0.0 & \RBF & 10.0 & 1.000 & 4.994 & 0.999 & 9.972 & 58.207 & 62.273 & 2.309 & 6.954 \\
30 & 0.5 & 1.0 & 1.0 & \COS & - & 1.000 & 4.994 & 0.999 & 9.972 & 58.207 & 62.273 & 2.309 & 6.954 \\
30 & 0.5 & 1.0 & 1.0 & \RBF & 10.0 & 1.000 & 4.994 & 0.999 & 9.972 & 58.207 & 62.273 & 2.309 & 6.954 \\
30 & 0.5 & 1.0 & 10.0 & \COS & - & 1.000 & 4.994 & 0.999 & 9.972 & 58.193 & 62.275 & 2.309 & 6.954 \\
30 & 0.5 & 1.0 & 10.0 & \RBF & 10.0 & 1.000 & 4.994 & 0.999 & 9.972 & 58.197 & 62.278 & 2.309 & 6.954 \\
30 & 0.5 & 1.0 & 100.0 & \COS & - & 1.000 & 4.994 & 0.999 & 9.972 & 58.149 & 62.229 & 2.328 & 6.999 \\
30 & 0.5 & 1.0 & 100.0 & \RBF & 10.0 & 1.000 & 4.994 & 0.999 & 9.972 & 58.173 & 62.236 & 2.328 & 6.990 \\
30 & 1.0 & 0.1 & 0.0 & \COS & - & 0.997 & 4.968 & 0.994 & 9.854 & 74.889 & 70.911 & 10.980 & 24.665 \\
30 & 1.0 & 0.1 & 0.0 & \RBF & 10.0 & 0.997 & 4.968 & 0.994 & 9.854 & 74.889 & 70.911 & 10.980 & 24.665 \\
30 & 1.0 & 0.1 & 1.0 & \COS & - & 0.997 & 4.969 & 0.995 & 9.856 & 74.982 & 71.104 & 11.421 & 25.163 \\
30 & 1.0 & 0.1 & 1.0 & \RBF & 10.0 & 0.997 & 4.968 & 0.995 & 9.856 & 74.943 & 71.094 & 11.227 & 25.056 \\
30 & 1.0 & 0.1 & 10.0 & \COS & - & 0.997 & 4.957 & 0.993 & 9.810 & 74.022 & 69.583 & 20.520 & 35.115 \\
30 & 1.0 & 0.1 & 10.0 & \RBF & 10.0 & 0.997 & 4.959 & 0.993 & 9.822 & 74.261 & 69.900 & 19.283 & 34.006 \\
30 & 1.0 & 0.1 & 100.0 & \COS & - & 0.994 & 4.921 & 0.987 & 9.706 & 71.547 & 66.358 & 32.438 & 44.142 \\
30 & 1.0 & 0.1 & 100.0 & \RBF & 10.0 & 0.993 & 4.920 & 0.987 & 9.712 & 71.664 & 66.390 & 32.060 & 43.777 \\
30 & 1.0 & 1.0 & 0.0 & \COS & - & 0.998 & 4.968 & 0.995 & 9.860 & 75.099 & 71.193 & 10.921 & 24.676 \\
30 & 1.0 & 1.0 & 0.0 & \RBF & 10.0 & 0.998 & 4.968 & 0.995 & 9.860 & 75.099 & 71.193 & 10.921 & 24.676 \\
30 & 1.0 & 1.0 & 1.0 & \COS & - & 0.997 & 4.968 & 0.995 & 9.861 & 75.167 & 71.337 & 11.360 & 24.808 \\
30 & 1.0 & 1.0 & 1.0 & \RBF & 10.0 & 0.997 & 4.968 & 0.995 & 9.860 & 75.162 & 71.333 & 11.326 & 24.803 \\
30 & 1.0 & 1.0 & 10.0 & \COS & - & 0.997 & 4.962 & 0.994 & 9.832 & 74.543 & 70.375 & 17.864 & 32.639 \\
30 & 1.0 & 1.0 & 10.0 & \RBF & 10.0 & 0.997 & 4.964 & 0.994 & 9.842 & 74.616 & 70.619 & 16.351 & 31.469 \\
30 & 1.0 & 1.0 & 100.0 & \COS & - & 0.993 & 4.921 & 0.988 & 9.716 & 71.834 & 66.721 & 32.605 & 44.346 \\
30 & 1.0 & 1.0 & 100.0 & \RBF & 10.0 & 0.994 & 4.922 & 0.988 & 9.718 & 71.961 & 66.679 & 32.066 & 43.754 \\
50 & 0.0 & 0.1 & 0.0 & \COS & - & 1.000 & 4.996 & 1.000 & 9.980 & 59.196 & 63.160 & 0.604 & 2.064 \\
50 & 0.0 & 0.1 & 0.0 & \RBF & 10.0 & 1.000 & 4.996 & 1.000 & 9.980 & 59.196 & 63.160 & 0.604 & 2.064 \\
50 & 0.0 & 0.1 & 1.0 & \COS & - & 1.000 & 4.996 & 1.000 & 9.980 & 59.298 & 63.216 & 0.587 & 2.037 \\
50 & 0.0 & 0.1 & 1.0 & \RBF & 10.0 & 1.000 & 4.996 & 1.000 & 9.980 & 59.250 & 63.184 & 0.587 & 2.051 \\
50 & 0.0 & 0.1 & 10.0 & \COS & - & 1.000 & 4.996 & 1.000 & 9.979 & 59.542 & 63.345 & 0.587 & 1.995 \\
50 & 0.0 & 0.1 & 10.0 & \RBF & 10.0 & 1.000 & 4.996 & 1.000 & 9.979 & 59.542 & 63.347 & 0.587 & 1.995 \\
50 & 0.0 & 0.1 & 100.0 & \COS & - & 1.000 & 4.994 & 0.999 & 9.970 & 52.521 & 61.111 & 9.252 & 22.422 \\
50 & 0.0 & 0.1 & 100.0 & \RBF & 10.0 & 1.000 & 4.995 & 1.000 & 9.976 & 54.548 & 61.501 & 2.741 & 10.398 \\
50 & 0.0 & 1.0 & 0.0 & \COS & - & 1.000 & 4.996 & 1.000 & 9.979 & 59.776 & 63.437 & 0.550 & 1.900 \\
50 & 0.0 & 1.0 & 0.0 & \RBF & 10.0 & 1.000 & 4.996 & 1.000 & 9.979 & 59.776 & 63.437 & 0.550 & 1.900 \\
50 & 0.0 & 1.0 & 1.0 & \COS & - & 1.000 & 4.996 & 1.000 & 9.979 & 59.771 & 63.437 & 0.550 & 1.900 \\
50 & 0.0 & 1.0 & 1.0 & \RBF & 10.0 & 1.000 & 4.996 & 1.000 & 9.979 & 59.771 & 63.437 & 0.550 & 1.900 \\
50 & 0.0 & 1.0 & 10.0 & \COS & - & 1.000 & 4.996 & 1.000 & 9.979 & 59.757 & 63.423 & 0.550 & 1.900 \\
50 & 0.0 & 1.0 & 10.0 & \RBF & 10.0 & 1.000 & 4.996 & 1.000 & 9.979 & 59.766 & 63.428 & 0.550 & 1.900 \\
50 & 0.0 & 1.0 & 100.0 & \COS & - & 1.000 & 4.996 & 1.000 & 9.977 & 56.034 & 61.849 & 1.140 & 5.142 \\
50 & 0.0 & 1.0 & 100.0 & \RBF & 10.0 & 1.000 & 4.996 & 1.000 & 9.979 & 57.895 & 62.519 & 0.835 & 2.680 \\
50 & 0.05 & 0.1 & 0.0 & \COS & - & 1.000 & 4.996 & 1.000 & 9.979 & 60.175 & 63.684 & 0.598 & 1.873 \\
50 & 0.05 & 0.1 & 0.0 & \RBF & 10.0 & 1.000 & 4.996 & 1.000 & 9.979 & 60.175 & 63.684 & 0.598 & 1.873 \\
50 & 0.05 & 0.1 & 1.0 & \COS & - & 1.000 & 4.996 & 1.000 & 9.979 & 60.170 & 63.676 & 0.598 & 1.873 \\
50 & 0.05 & 0.1 & 1.0 & \RBF & 10.0 & 1.000 & 4.996 & 1.000 & 9.979 & 60.170 & 63.679 & 0.598 & 1.873 \\
50 & 0.05 & 0.1 & 10.0 & \COS & - & 1.000 & 4.996 & 1.000 & 9.979 & 60.151 & 63.659 & 0.598 & 1.873 \\
50 & 0.05 & 0.1 & 10.0 & \RBF & 10.0 & 1.000 & 4.996 & 1.000 & 9.979 & 60.151 & 63.666 & 0.598 & 1.873 \\
50 & 0.05 & 0.1 & 100.0 & \COS & - & 1.000 & 4.996 & 1.000 & 9.978 & 57.408 & 62.414 & 0.926 & 3.766 \\
50 & 0.05 & 0.1 & 100.0 & \RBF & 10.0 & 1.000 & 4.996 & 1.000 & 9.979 & 59.362 & 63.262 & 0.604 & 2.162 \\
50 & 0.05 & 1.0 & 0.0 & \COS & - & 1.000 & 4.996 & 1.000 & 9.979 & 60.170 & 63.684 & 0.598 & 1.873 \\
50 & 0.05 & 1.0 & 0.0 & \RBF & 10.0 & 1.000 & 4.996 & 1.000 & 9.979 & 60.170 & 63.684 & 0.598 & 1.873 \\
50 & 0.05 & 1.0 & 1.0 & \COS & - & 1.000 & 4.996 & 1.000 & 9.979 & 60.166 & 63.676 & 0.598 & 1.873 \\
50 & 0.05 & 1.0 & 1.0 & \RBF & 10.0 & 1.000 & 4.996 & 1.000 & 9.979 & 60.166 & 63.676 & 0.598 & 1.873 \\
50 & 0.05 & 1.0 & 10.0 & \COS & - & 1.000 & 4.996 & 1.000 & 9.979 & 60.146 & 63.656 & 0.598 & 1.873 \\
50 & 0.05 & 1.0 & 10.0 & \RBF & 10.0 & 1.000 & 4.996 & 1.000 & 9.979 & 60.151 & 63.666 & 0.598 & 1.873 \\
50 & 0.05 & 1.0 & 100.0 & \COS & - & 1.000 & 4.996 & 1.000 & 9.980 & 59.255 & 63.172 & 0.623 & 2.186 \\
50 & 0.05 & 1.0 & 100.0 & \RBF & 10.0 & 1.000 & 4.996 & 1.000 & 9.979 & 59.947 & 63.581 & 0.568 & 1.887 \\
50 & 0.1 & 0.1 & 0.0 & \COS & - & 0.999 & 4.984 & 0.998 & 9.957 & 55.445 & 61.065 & 17.949 & 22.838 \\
50 & 0.1 & 0.1 & 0.0 & \RBF & 10.0 & 0.999 & 4.984 & 0.998 & 9.957 & 55.445 & 61.065 & 17.949 & 22.838 \\
50 & 0.1 & 0.1 & 1.0 & \COS & - & 1.000 & 4.996 & 1.000 & 9.979 & 60.560 & 63.900 & 0.598 & 1.910 \\
50 & 0.1 & 0.1 & 1.0 & \RBF & 10.0 & 1.000 & 4.996 & 1.000 & 9.979 & 60.560 & 63.900 & 0.598 & 1.910 \\
50 & 0.1 & 0.1 & 10.0 & \COS & - & 1.000 & 4.996 & 1.000 & 9.979 & 60.521 & 63.890 & 0.598 & 1.910 \\
50 & 0.1 & 0.1 & 10.0 & \RBF & 10.0 & 1.000 & 4.996 & 1.000 & 9.979 & 60.531 & 63.898 & 0.598 & 1.910 \\
50 & 0.1 & 0.1 & 100.0 & \COS & - & 1.000 & 4.996 & 1.000 & 9.979 & 59.927 & 63.596 & 0.616 & 2.003 \\
50 & 0.1 & 0.1 & 100.0 & \RBF & 10.0 & 1.000 & 4.996 & 1.000 & 9.979 & 60.399 & 63.820 & 0.598 & 1.896 \\
50 & 0.1 & 1.0 & 0.0 & \COS & - & 1.000 & 4.996 & 1.000 & 9.979 & 60.560 & 63.900 & 0.598 & 1.910 \\
50 & 0.1 & 1.0 & 0.0 & \RBF & 10.0 & 1.000 & 4.996 & 1.000 & 9.979 & 60.560 & 63.900 & 0.598 & 1.910 \\
50 & 0.1 & 1.0 & 1.0 & \COS & - & 1.000 & 4.996 & 1.000 & 9.979 & 60.560 & 63.903 & 0.598 & 1.910 \\
50 & 0.1 & 1.0 & 1.0 & \RBF & 10.0 & 1.000 & 4.996 & 1.000 & 9.979 & 60.560 & 63.903 & 0.598 & 1.910 \\
50 & 0.1 & 1.0 & 10.0 & \COS & - & 1.000 & 4.996 & 1.000 & 9.979 & 60.517 & 63.890 & 0.598 & 1.910 \\
50 & 0.1 & 1.0 & 10.0 & \RBF & 10.0 & 1.000 & 4.996 & 1.000 & 9.979 & 60.531 & 63.895 & 0.598 & 1.910 \\
50 & 0.1 & 1.0 & 100.0 & \COS & - & 1.000 & 4.996 & 1.000 & 9.979 & 60.395 & 63.798 & 0.598 & 1.889 \\
50 & 0.1 & 1.0 & 100.0 & \RBF & 10.0 & 1.000 & 4.996 & 1.000 & 9.979 & 60.399 & 63.820 & 0.598 & 1.896 \\
50 & 0.5 & 0.1 & 0.0 & \COS & - & 0.998 & 4.982 & 0.998 & 9.949 & 63.834 & 68.631 & 20.091 & 28.507 \\
50 & 0.5 & 0.1 & 0.0 & \RBF & 10.0 & 0.998 & 4.982 & 0.998 & 9.949 & 63.834 & 68.631 & 20.091 & 28.507 \\
50 & 0.5 & 0.1 & 1.0 & \COS & - & 0.998 & 4.982 & 0.998 & 9.949 & 63.698 & 68.494 & 20.062 & 28.385 \\
50 & 0.5 & 0.1 & 1.0 & \RBF & 10.0 & 0.998 & 4.982 & 0.998 & 9.949 & 63.712 & 68.516 & 20.062 & 28.405 \\
50 & 0.5 & 0.1 & 10.0 & \COS & - & 0.998 & 4.984 & 0.998 & 9.956 & 57.223 & 62.297 & 17.965 & 23.094 \\
50 & 0.5 & 0.1 & 10.0 & \RBF & 10.0 & 0.998 & 4.984 & 0.998 & 9.956 & 57.237 & 62.295 & 17.965 & 23.094 \\
50 & 0.5 & 0.1 & 100.0 & \COS & - & 0.998 & 4.982 & 0.998 & 9.948 & 64.136 & 69.228 & 21.314 & 32.323 \\
50 & 0.5 & 0.1 & 100.0 & \RBF & 10.0 & 0.998 & 4.982 & 0.998 & 9.949 & 63.786 & 68.914 & 20.947 & 31.269 \\
50 & 0.5 & 1.0 & 0.0 & \COS & - & 0.998 & 4.984 & 0.998 & 9.956 & 57.252 & 62.287 & 17.918 & 23.062 \\
50 & 0.5 & 1.0 & 0.0 & \RBF & 10.0 & 0.998 & 4.984 & 0.998 & 9.956 & 57.252 & 62.287 & 17.918 & 23.062 \\
50 & 0.5 & 1.0 & 1.0 & \COS & - & 0.998 & 4.984 & 0.998 & 9.956 & 57.291 & 62.248 & 17.918 & 23.057 \\
50 & 0.5 & 1.0 & 1.0 & \RBF & 10.0 & 0.998 & 4.984 & 0.998 & 9.956 & 57.276 & 62.268 & 17.918 & 23.057 \\
50 & 0.5 & 1.0 & 10.0 & \COS & - & 0.998 & 4.984 & 0.998 & 9.956 & 57.286 & 62.202 & 17.918 & 22.959 \\
50 & 0.5 & 1.0 & 10.0 & \RBF & 10.0 & 0.998 & 4.984 & 0.998 & 9.956 & 57.291 & 62.202 & 17.918 & 22.959 \\
50 & 0.5 & 1.0 & 100.0 & \COS & - & 0.998 & 4.982 & 0.998 & 9.949 & 62.665 & 67.963 & 20.868 & 30.726 \\
50 & 0.5 & 1.0 & 100.0 & \RBF & 10.0 & 0.998 & 4.983 & 0.998 & 9.951 & 62.080 & 67.355 & 20.395 & 29.911 \\
50 & 1.0 & 0.1 & 0.0 & \COS & - & 0.999 & 4.987 & 0.998 & 9.934 & 78.777 & 77.235 & 3.659 & 16.645 \\
50 & 1.0 & 0.1 & 0.0 & \RBF & 10.0 & 0.999 & 4.987 & 0.998 & 9.934 & 78.777 & 77.235 & 3.659 & 16.645 \\
50 & 1.0 & 0.1 & 1.0 & \COS & - & 0.999 & 4.987 & 0.998 & 9.938 & 78.728 & 77.230 & 3.735 & 16.302 \\
50 & 1.0 & 0.1 & 1.0 & \RBF & 10.0 & 0.999 & 4.987 & 0.998 & 9.938 & 78.719 & 77.233 & 3.716 & 16.335 \\
50 & 1.0 & 0.1 & 10.0 & \COS & - & 0.998 & 4.978 & 0.997 & 9.893 & 79.415 & 76.489 & 16.928 & 36.025 \\
50 & 1.0 & 0.1 & 10.0 & \RBF & 10.0 & 0.999 & 4.979 & 0.997 & 9.904 & 79.367 & 76.772 & 14.694 & 33.769 \\
50 & 1.0 & 0.1 & 100.0 & \COS & - & 0.996 & 4.946 & 0.991 & 9.770 & 77.096 & 71.152 & 32.855 & 46.931 \\
50 & 1.0 & 0.1 & 100.0 & \RBF & 10.0 & 0.996 & 4.946 & 0.991 & 9.769 & 77.228 & 71.274 & 32.806 & 46.652 \\
50 & 1.0 & 1.0 & 0.0 & \COS & - & 0.999 & 4.987 & 0.998 & 9.937 & 78.767 & 77.199 & 3.445 & 15.456 \\
50 & 1.0 & 1.0 & 0.0 & \RBF & 10.0 & 0.999 & 4.987 & 0.998 & 9.937 & 78.767 & 77.199 & 3.445 & 15.456 \\
50 & 1.0 & 1.0 & 1.0 & \COS & - & 0.999 & 4.987 & 0.998 & 9.937 & 78.762 & 77.160 & 3.569 & 15.290 \\
50 & 1.0 & 1.0 & 1.0 & \RBF & 10.0 & 0.999 & 4.987 & 0.998 & 9.937 & 78.762 & 77.162 & 3.557 & 15.161 \\
50 & 1.0 & 1.0 & 10.0 & \COS & - & 0.999 & 4.982 & 0.997 & 9.912 & 79.284 & 76.984 & 12.646 & 31.247 \\
50 & 1.0 & 1.0 & 10.0 & \RBF & 10.0 & 0.999 & 4.983 & 0.997 & 9.921 & 79.220 & 77.191 & 11.008 & 29.370 \\
50 & 1.0 & 1.0 & 100.0 & \COS & - & 0.996 & 4.948 & 0.991 & 9.778 & 77.198 & 71.425 & 32.661 & 46.862 \\
50 & 1.0 & 1.0 & 100.0 & \RBF & 10.0 & 0.996 & 4.950 & 0.992 & 9.777 & 77.413 & 71.766 & 31.886 & 46.296 \\


==> tables/overall_0.5percent.tex <==
\begin{table}[h!]
  \centering
  \caption{\mbox{Overall Result Comparision (0.5 percentile)}}
  \label{tbl:results:overall_1p}
  \vspace{-10pt}
  \begin{threeparttable}
      \begin{tabular}{
          @{\hspace{0pt}}c@{\hspace{1pt}}
          @{\hspace{1pt}}r@{\hspace{0pt}}
          @{\hspace{2pt}}r@{\hspace{2pt}}
          @{\hspace{2pt}}r@{\hspace{2pt}}
          @{\hspace{2pt}}r@{\hspace{2pt}}
          @{\hspace{2pt}}r@{\hspace{2pt}}
          @{\hspace{2pt}}r@{\hspace{2pt}}
          @{\hspace{2pt}}c@{\hspace{2pt}}
          @{\hspace{2pt}}c@{\hspace{2pt}}
          @{\hspace{2pt}}c@{\hspace{2pt}}
          @{\hspace{2pt}}c@{\hspace{0pt}}
        }        
        \toprule
        method   & \multicolumn{6}{c}{parameters} & \multicolumn{4}{c}{performance} \\
        \midrule
        \multirow{4}{*}{\BMTMKL}
        & \multicolumn{3}{c}{$\alpha_b$}  & \multicolumn{3}{c}{$\beta_b$} & \small{\rCI} & \small{\CI} & \small{AP@$5$} & \small{AP@$10$} \\
        \cline{2-11}
          & \multicolumn{3}{c}{1.0e0}   & \multicolumn{3}{c}{1.0e0}   & \textbf{0.904} & 0.803 & 0.882 & 0.873 \\
          & \multicolumn{3}{c}{1.0e-10} & \multicolumn{3}{c}{1.0e+10} & 0.901 & \underline{\textbf{0.805}} & 0.869 & 0.864 \\
        & \multicolumn{3}{c}{1.0e-10} & \multicolumn{3}{c}{1.0e-10} & 0.903 & 0.803 & \textbf{0.884} & \textbf{0.874} \\
        \midrule
        \multirow{5}{*}{\MTCRP}
        & d & $\alpha$ & $\beta$ & $\gamma$ & usim & $\sigma$ & \small{\rCI} & \small{\CI} & \small{AP@$5$} & \small{AP@$10$} \\
        \cline{2-11}
        & 15 & 0.0 & 0.0 & 1.0e4 & cos & - & \underline{\textbf{0.913}} & 0.505 & 0.916 & 0.864\\
          & 100 & 1.0 & 1.0e2 & 1.0e4 & rbf & 10.0 & 0.907 & \textbf{0.802} & 0.880 & 0.855 \\
        & 50 & 0.0 & 1.0e4 & 1.0e4 & cos & - & 0.907 & 0.486 & \underline{\textbf{0.940}} & 0.885  \\
        & 50 & 0.5 & 1.0e2 & 1.0e4 & cos & - & 0.894 & 0.488 & 0.921 & \underline{\textbf{0.901}} \\
        \bottomrule
      \end{tabular}
      \begin{tablenotes}
        \begin{footnotesize}
          \setlength\labelsep{0pt}
        \item The best performance of each method under each metric is in \textbf{bold}.
        The best performance of both the methods under each metric is \underline{underscored}. 
          \par
        \end{footnotesize}
      \end{tablenotes}
    \end{threeparttable}
%\vspace{-2em}
\end{table}


==> tables/overall_1percent.tex <==
\begin{table}[h!]
  \centering
  \caption{\mbox{Overall Result Comparision (2 percentile)}}
  \label{tbl:results:overall_2p}
  \vspace{-10pt}
  \begin{threeparttable}
      \begin{tabular}{
          @{\hspace{0pt}}c@{\hspace{1pt}}
          @{\hspace{1pt}}r@{\hspace{0pt}}
          @{\hspace{2pt}}r@{\hspace{2pt}}
          @{\hspace{2pt}}r@{\hspace{2pt}}
          @{\hspace{2pt}}r@{\hspace{2pt}}
          @{\hspace{2pt}}r@{\hspace{2pt}}
          @{\hspace{2pt}}r@{\hspace{2pt}}
          @{\hspace{2pt}}c@{\hspace{2pt}}
          @{\hspace{2pt}}c@{\hspace{2pt}}
          @{\hspace{2pt}}c@{\hspace{2pt}}
          @{\hspace{2pt}}c@{\hspace{0pt}}
        }        
        \toprule
        method   & \multicolumn{6}{c}{parameters} & \multicolumn{4}{c}{performance} \\
        \midrule
        \multirow{4}{*}{\BMTMKL}
        & \multicolumn{3}{c}{$\alpha_b$}  & \multicolumn{3}{c}{$\beta_b$} & \small{\rCI} & \small{\CI} & \small{AP@$5$} & \small{AP@$10$} \\
        \cline{2-11}
        & \multicolumn{3}{c}{1.0e0}   & \multicolumn{3}{c}{1.0e0}   & 0.673 & 0.803 & 0.815 & 0.804 \\
        & \multicolumn{3}{c}{1.0e-10} & \multicolumn{3}{c}{1.0e-10} & 0.673 & 0.803 & 0.816 & 0.805 \\
        & \multicolumn{3}{c}{1.0e-10} & \multicolumn{3}{c}{1.0e+10} & 0.667 & 0.805 & 0.805 & 0.796 \\
        \midrule
        \multirow{5}{*}{\MTCRP}
        & d & $\alpha$ & $\beta$ & $\gamma$ & usim & $\sigma$ & \small{\rCI} & \small{\CI} & \small{AP@$5$} & \small{AP@$10$} \\
        \cline{2-11}
        & 50 & 1.0 & 1.0 & 1.0e2 & rbf & 10.0 & 0.787 & 0.769 & 0.662 & 0.657\\
        & 30 & 0.2 & 1.0 & 20.0 & rbf & 10.0 & 0.657 & 0.806 & 0.463 & 0.461 \\
        & 10 & 0.0 & 0.1 & 1.0e2 & rbf & 10.0 & 0.759 & 0.778 & 0.775 & 0.771  \\
        & 10 & 0.0 & 0.1 & 1.0e2 & rbf & 10.0 & 0.759 & 0.778 & 0.775 & 0.771} \\
        \bottomrule
      \end{tabular}
      \begin{tablenotes}
        \begin{footnotesize}
          \setlength\labelsep{0pt}
        \item The best performance of each method under each metric is in \textbf{bold}.
          The best performance of both the methods under each metric is \underline{underscored}. 
          \par
        \end{footnotesize}
      \end{tablenotes}
    \end{threeparttable}
%\vspace{-2em}
\end{table}


==> tables/overall_2percent.tex <==
%\begin{table}[t!]
  \centering
  \tbl{\mbox{Performance on Ranking New Drugs ($\theta=2$)}}{
  \label{tbl:results:overall_2p}
%  \vspace{-10pt}
  \begin{threeparttable}
      \begin{tabular}{
        @{\hspace{10pt}}c@{\hspace{10pt}}
        @{\hspace{10pt}}c@{\hspace{0pt}}
        @{\hspace{10pt}}c@{\hspace{10pt}}
        @{\hspace{10pt}}c@{\hspace{10pt}}
        @{\hspace{10pt}}c@{\hspace{10pt}}
        @{\hspace{10pt}}c@{\hspace{10pt}}
        @{\hspace{10pt}}c@{\hspace{10pt}}
        @{\hspace{15pt}}c@{\hspace{10pt}}
        @{\hspace{10pt}}c@{\hspace{10pt}}
        @{\hspace{10pt}}c@{\hspace{10pt}}
        @{\hspace{10pt}}c@{\hspace{10pt}}          
        }        
        \toprule
        method   & \multicolumn{6}{c}{parameters} & \multicolumn{4}{c}{performance} \\
        \midrule
        \multirow{2}{*}{\BMTMKL}
        & \multicolumn{2}{c}{$\alpha_b$}  & \multicolumn{2}{c}{$\beta_b$} & usim & $\sigma$       & \small{AP@$5$} & \small{AP@$10$} & \small{\rCI}   & \small{\CI}               \\
        \cline{2-11}                                                                                                                                                             
        %                                                                                                                                                                        
%       & \multicolumn{2}{c}{1.0e0}   & \multicolumn{2}{c}{1.0e0}   	& rbf 	& 1.0e1 	  & 0.718          & 0.717 	     & \textbf{0.764} & \textbf{\underline{0.812}}\\
        & \multicolumn{2}{c}{1.0e-10} & \multicolumn{2}{c}{1.0e+10} 	& rbf 	& 1.0e1 	  & \textbf{0.719} & \textbf{0.718}  & \textbf{0.764} & \textbf{\underline{0.812}}\\
        \midrule
        \multirow{4}{*}{\MTCRP}
        & d	& $\alpha$	& $\beta$	& $\gamma$	& usim	& $\sigma$	   & \small{AP@$5$}& \small{AP@$10$} 				& \small{\rCI}			& \small{\CI}	\\
        \cline{2-11}                                                                                                                                                                                    
        & 50 & 1.0 & 1.0 & 1.0e2 & cos & - 						   & 0.661          & 0.656 					& \textbf{\underline{0.787}} 	& 0.770         \\
        & 30 & 0.1 & 1.0 & 1.0e2 & rbf & 1.0e1 						   & 0.488          & 0.484 					&         0.670  		& \textbf{0.805}\\
        & 10 & 0.0 & 0.1 & 1.0e2 & cos & - 						   & \textbf{\underline{0.777}} & \textbf{\underline{0.772}} 	&         0.759  		& 0.774         \\
%        & 10 & 0.0 & 0.1 & 1.0e2 & rbf & 10.0 &         0.759  & 0.777          & \textbf{0.775} & \textbf{0.771} \\        
        \bottomrule
      \end{tabular}
      \begin{tablenotes}
        \begin{scriptsize}
          \setlength\labelsep{0pt}
        \item 
%		The column block corresponding to ``method'' has the names of methods compared.
%		The column block corresponding to ``parameters'' has the parameters used in the experiments.
%		The column block corresponding to ``performance'' has the performance on each evaluation metric of the given methods.
		%
%		The row block corresponding to ``\BMTMKL'' has the results of the baseline method \BMTMKL.
%		The row block corresponding to ``\MTCRP'' has the results of the proposed method \MTCRP.
		%
		The columns corresponding to ``$\alpha_b$'', ``$\beta_b$'',
                ``usim'', and ``$\sigma$'' have the  
		two hyperparameters, cell line similarity function,
                and parameter for rbf cell line similarity, respectively, for \BMTMKL.
                %
		The columns corresponding to ``d'', ``$\alpha$'',
                ``$\beta$'', ``$\gamma$'', ``usim'', and ``$\sigma$'' have the
                latent dimension, weighting factor,
                latent vector regularization parameter,
                cell line similarity regularization parameter,
                cell line similarity function, and parameter for rbf cell line similarity,
                respectively, for \MTCRP. 
%		The columns corresponding to ``AP@$5$'', ``AP@$10$'', ``\rCI'', and ``$\CI$'' has the
%			\textcolor{blue}{AP@$5$, AP@$10$, \rCI, and $\CI$ evaluation values}, respectively.
		%
		The best performance of each method under each metric is in \textbf{bold}.
		The best performance of both the methods under each metric is \underline{underscored}. 
          \par
        \end{scriptsize}
      \end{tablenotes}
  \end{threeparttable}
  }
%\vspace{-2em}
%\end{table}


==> tables/overall_5percent.tex <==
%\begin{table}[t!]
  \centering
  \tbl{\mbox{Performance on Ranking New Drugs ($\theta=5$)}}{      
  \label{tbl:results:overall_5p}
%  \vspace{-10pt}
  \begin{threeparttable}
      \begin{tabular}{
        @{\hspace{10pt}}c@{\hspace{10pt}}
        @{\hspace{10pt}}c@{\hspace{0pt}}
        @{\hspace{10pt}}c@{\hspace{10pt}}
        @{\hspace{10pt}}c@{\hspace{10pt}}
        @{\hspace{10pt}}c@{\hspace{10pt}}
        @{\hspace{10pt}}c@{\hspace{10pt}}
        @{\hspace{10pt}}c@{\hspace{10pt}}
        @{\hspace{15pt}}c@{\hspace{10pt}}
        @{\hspace{10pt}}c@{\hspace{10pt}}
        @{\hspace{10pt}}c@{\hspace{10pt}}
        @{\hspace{10pt}}c@{\hspace{10pt}}          
        }        
        \toprule
        method   & \multicolumn{6}{c}{parameters} & \multicolumn{4}{c}{performance} \\
        \midrule
%        \multirow{4}{*}{\BMTMKL}
        & \multicolumn{2}{c}{$\alpha_b$}  & \multicolumn{2}{c}{$\beta_b$} & usim & $\sigma$ & \small{AP@$5$} & \small{AP@$10$} & \small{\rCI} & \small{\CI} \\
        \cline{2-11}        
        %
        \BMTMKL
        & \multicolumn{2}{c}{1e-10} &  \multicolumn{2}{c}{1e+10} & rbf & 1.0e1 &  \textbf{0.831} &  \textbf{0.820} & \textbf{0.678} &  \textbf{\underline{0.812}} \\   
        \midrule
        \multirow{5}{*}{\MTCRP}
        & d	& $\alpha$	& $\beta$	& $\gamma$	& usim	& $\sigma$	& \small{AP@$5$} & \small{AP@$10$} & \small{\rCI}	& \small{\CI} 	  \\
        \cline{2-11}
        & 50 & 1.0 & 1.0 & 1.0e2 & rbf & 1.0e1 & 0.775 & 0.764 						& \textbf{\underline{0.721}} 	&          0.726    \\
        & 30 & 0.1 & 1.0 & 1.0e2 & rbf & 1.0e1 & 0.744 & 0.731 						&          0.551 		& \textbf{0.810}    \\
        & 10 & 0.5 & 1.0 & 1.0e1 & rbf & 1.0e1 & \textbf{\underline{0.867}} & \textbf{\underline{0.856}}&          0.683 		&          0.804   	  \\
%        & 15 & 0.1 & 0.0 & 1.0e4 & cos & - & \underline{\textbf{0.677}} & 0.607 & 0.934 & 0.916 \\
%        & 75 & 1.0 & 100.0 & 1.0e4 & rbf & 10.0 & 0.669 & \textbf{0.802} & 0.915 & 0.892 \\
%        & 15 & 0.0 & 0.0 & 100.0 & rbf & 10.0 & 0.674 & 0.593 & \underline{\textbf{0.936}} & 0.913 \\
%        & 30 & 0.1 & 1.0e4 & 1.0e4 & rbf & 10.0 & 0.672 & 0.589 & 0.935 & \underline{\textbf{0.919}} \\
        \bottomrule
      \end{tabular}
      \begin{tablenotes}
        \begin{scriptsize}
          \setlength\labelsep{0pt}
        \item 
		%
		The columns corresponding to ``$\alpha_b$'', ``$\beta_b$'',
                ``usim'', and ``$\sigma$'' have the
                two hyperparameters, cell line similarity function,
                and parameter for rbf cell line similarity, respectively, for \BMTMKL.
                %
                The columns corresponding to ``d'', ``$\alpha$'',
                ``$\beta$'', ``$\gamma$'', ``usim'', and ``$\sigma$'' have the
                latent dimension, weighting factor,
                latent vector regularization parameter,
                cell line similarity regularization parameter,
                cell line similarity function, and parameter for rbf cell line similarity,
                respectively, for \MTCRP.
		%
		The best performance of each method under each metric is in \textbf{bold}.
		The best performance of both the methods under each metric is \underline{underscored}. 
          \par
        \end{scriptsize}
      \end{tablenotes}
  \end{threeparttable}
  }
%\vspace{-2em}
%\end{table}


==> tables/transductive_2percent.tex <==
%\begin{table}[t!]
  \centering
  \tbl{\mbox{Transductive Result Comparision (2 percentile)}}{
  \label{tbl:results:transductive_2p}        
%  \vspace{-10pt}                            
  \begin{threeparttable}
      \begin{tabular}{  
        @{\hspace{5pt}}c@{\hspace{5pt}}
        @{\hspace{5pt}}c@{\hspace{5pt}}         
        @{\hspace{5pt}}c@{\hspace{5pt}}
        @{\hspace{5pt}}c@{\hspace{5pt}}
        @{\hspace{5pt}}c@{\hspace{5pt}}
        @{\hspace{5pt}}c@{\hspace{5pt}}
        @{\hspace{5pt}}c@{\hspace{5pt}}
        @{\hspace{10pt}}c@{\hspace{5pt}}
        @{\hspace{5pt}}c@{\hspace{5pt}} 
        }
        \toprule
        method   & \multicolumn{6}{c}{parameters} & \multicolumn{2}{c}{performance}\\
        \midrule
        \multirow{5}{*}{\BMTMKL}
        & \multicolumn{2}{c}{$\alpha_b$}  & \multicolumn{2}{c}{$\beta_b$} & usim & $\sigma$ & top-5\% & top-10\%\\
        \cline{2-9}
        %
        & \multicolumn{2}{c}{1.0e-10} & \multicolumn{2}{c}{1.0e+10} & rbf & 1.0e1 & 15.10 & 9.60 \\
        & \multicolumn{2}{c}{1.0e0}   & \multicolumn{2}{c}{1.0e0}   & rbf & 1.0e1 & 15.10 & 9.60 \\
        & \multicolumn{2}{c}{1.0e-10} & \multicolumn{2}{c}{1.0e-10} & rbf & 1.0e1 & 15.10 & 9.60 \\        
        \midrule
        & d        & $\alpha$ & $\beta$ & $\gamma$ & usim & $\sigma$ &   top-5\% & top-10\% \\
        \cline{2-9}
        \multirow{4}{*}{\MTCRP} 
        & 50 & 1.0      & 0.1     & 0.0      & cos  & -        & 44.69 & 24.28 \\
%        & 50 & 1.0      & 0.1     & 0.0      & rbf  & 10.0     & 44.69 \\
        & 50 & 1.0      & 1.0     & 0.0      & cos  & -        & 44.61 & 24.18 \\
%        & 50 & 1.0      & 1.0     & 0.0      & rbf  & 10.0     & 44.61 \\
        & 50 & 1.0      & 1.0     & 1.0      & rbf  & 10.0     & 44.56 & 24.15 \\
        & 50 & 1.0      & 1.0     & 1.0      & cos  & -        & 44.53 & 24.15 \\
        \bottomrule
      \end{tabular}
      \begin{tablenotes}
        \begin{scriptsize}
          \setlength\labelsep{0pt}
        \item The best performance of each method under each metric is in \textbf{bold}.
          The best performance of both the methods under each metric is \underline{underscored}.
          \par
        \end{scriptsize}
      \end{tablenotes}
  \end{threeparttable}
    }
%\vspace{-2em}
%\end{table}


==> tables/transductive_5percent.tex <==
%\begin{table}[t!]
  \centering
  \tbl{\mbox{Transductive Result Comparision (5 percentile)}}{
  \label{tbl:results:transductive_5p}        
%  \vspace{-10pt}                            
  \begin{threeparttable}
      \begin{tabular}{  
        @{\hspace{5pt}}c@{\hspace{5pt}}
        @{\hspace{5pt}}c@{\hspace{5pt}}         
        @{\hspace{5pt}}c@{\hspace{5pt}}
        @{\hspace{5pt}}c@{\hspace{5pt}}
        @{\hspace{5pt}}c@{\hspace{5pt}}
        @{\hspace{5pt}}c@{\hspace{5pt}}
        @{\hspace{5pt}}c@{\hspace{5pt}}
        @{\hspace{10pt}}c@{\hspace{5pt}}
        @{\hspace{5pt}}c@{\hspace{5pt}} 
        }
        \toprule
        method   & \multicolumn{6}{c}{parameters} & \multicolumn{2}{c}{performance}\\
        \midrule
        \multirow{7}{*}{\BMTMKL}
        & $\alpha_\gamma$       & $\beta_\gamma$        & usim  & $\sigma$      & top-c5        & top-p5        & top-c10       & top-p1 \\
        \cline{2-9}
        & 1                     & 1                     & cos   & -             & 566           & 0.138         & 789           & 0.091         \\
        & 1e-10                 & 1e-10                 & cos   & -             & 565           & 0.138         & 752           & 0.092         \\
        & 1e-10                 & 1e10                  & cos   & -             & 566           & 0.138         & 747           & 0.091         \\
	& 1			& 1			& rbf	& 10.0	        & 621		& 0.151		& 790		& 0.096		\\
	& 1e-10			& 1e-10			& rbf	& 10.0	        & 620		& 0.151		& 790		& 0.096		\\
	& 1e-10			& 1e10			& rbf	& 10.0	        & 623		& 0.151		& 790		& 0.096		\\
        \midrule
        & $\alpha$ & $\beta$ & $\gamma$ & usim & $\sigma$ &  & top-5\% & top-10\% \\
        \cline{2-9}
        \multirow{4}{*}{\MTCRP} 
	& 50 & 1.0 & 1.0 & 1.0 & rbf & 10.0 &  51.93 & 34.25 \\
	& 50 & 1.0 & 1.0 & 0.0 & cos & -    &  51.92 & 34.20 \\
%	& 50 & 1.0 & 1.0 & 0.0 & rbf & 10.0 &  0.5192 \\
%	& 50 & 1.0 & 1.0 & 1.0 & cos & -    &  0.5192 \\
	& 50 & 1.0 & 0.1 & 0.0 & cos & -    &  51.90 & 34.15 \\
%	& 50 & 1.0 & 0.1 & 0.0 & rbf & 10.0 &  0.5190 \\
	& 50 & 1.0 & 0.1 & 1.0 & cos & -    &  51.84 & 34.12 \\
        \bottomrule
      \end{tabular}
      \begin{tablenotes}
        \begin{scriptsize}
          \setlength\labelsep{0pt}
        \item The best performance of each method under each metric is in \textbf{bold}.
          The best performance of both the methods under each metric is \underline{underscored}. 
          \par
        \end{scriptsize}
      \end{tablenotes}
  \end{threeparttable}
    }
%\vspace{-2em}
%\end{table}


==> tables/unknown_2percent.tex <==
\begin{ThreePartTable}
    \begin{TableNotes}[flushleft]  %%% This should come before longtable and it is not tablenotes but TableNotes
  \small
  \item
    \begin{footnotesize}
        \bgroup
%        \def\arraystretch{0.5}%       
        \setstretch{1}
		The columns corresponding to ``$l$'', ``$\alpha$'',
                ``$\beta$'', ``$\gamma$'', ``usim'', and ``$\sigma$'' have the
                latent dimension, weighting factor,
                latent vector regularization parameter,
                cell line similarity regularization parameter,
                cell line similarity function, and parameter for rbf cell line similarity,
                respectively, for \MTCRP.
	      \par
              \egroup
    \end{footnotesize}
  \end{TableNotes}
  \begin{longtable}{
      @{\hspace{0pt}}>{\raggedleft}p{0.05\textwidth}@{\hspace{5pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.05\textwidth}@{\hspace{5pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.05\textwidth}@{\hspace{5pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.07\textwidth}@{\hspace{5pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.05\textwidth}@{\hspace{5pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.05\textwidth}@{\hspace{5pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.08\textwidth}@{\hspace{0pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.08\textwidth}@{\hspace{0pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.08\textwidth}@{\hspace{0pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.08\textwidth}@{\hspace{0pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.08\textwidth}@{\hspace{0pt}}
      @{\hspace{0pt}}>{\raggedleft\arraybackslash}p{0.08\textwidth}@{\hspace{0pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
    }
    \caption{\mbox{\MTCRP Performance on New Drugs ($\theta$ = 2)}}
    \label{supp:tbl:overall:2percent}\\
  %
    \hline\hline
    $l$ & $\alpha$ & $\beta$ & $\gamma$ & usim & $\sigma$ & \small{AP@$5$} & \small{AH@$5$} & \small{AP@$10$} & \small{AH@$10$} & \small{\rCI} & \small{\CI} \\
    \hline
    \endfirsthead
  %
    \multicolumn{12}{c}{{\tablename\ \thetable{} -- continued from previous page}}\\
    \hline\hline
    $l$ & $\alpha$ & $\beta$ & $\gamma$ & usim & $\sigma$ & \small{AP@$5$} & \small{AH@$5$} & \small{AP@$10$} & \small{AH@$10$} & \small{\rCI} & \small{\CI} \\
    \hline
    \endhead
  %
    \hline
    %  \midrule
    \multicolumn{12}{c}{{Continued on next page}} \\
    \hline
    %\midrule
    \endfoot
    %
    \hline\hline
    %\bottomrule
    \insertTableNotes         %% this added
    \endlastfoot
    %
    \input{tables/unknown_2percent_data.tex}
	
    \hline
  \end{longtable}
\end{ThreePartTable}


==> tables/unknown_2percent_KRL.tex <==
\begin{ThreePartTable}
    \begin{TableNotes}[flushleft]  %%% This should come before longtable and it is not tablenotes but TableNotes
  \small
  \item
    \begin{footnotesize}
        \bgroup
%        \def\arraystretch{0.5}%       
        \setstretch{1}
                The columns corresponding to ``$k$'', ``$\lambda$'',
                ``usim'', and ``$\sigma$'' have the
                two hyperparameters, cell line similarity function,
                and parameter for {$\RBF$} cell line similarity, respectively, 
                for {\KRL}.
	      \par
              \egroup
    \end{footnotesize}
  \end{TableNotes}
  \begin{longtable}{
      @{\hspace{0pt}}>{\raggedleft}p{0.07\textwidth}@{\hspace{5pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.07\textwidth}@{\hspace{5pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.07\textwidth}@{\hspace{5pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.07\textwidth}@{\hspace{5pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{0pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{0pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{0pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{0pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{0pt}}
      @{\hspace{0pt}}>{\raggedleft\arraybackslash}p{0.08\textwidth}@{\hspace{0pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
    }
    \caption{\mbox{\KRL Performance on New Drugs ($\theta$ = 2)}}
    \label{supp:tbl:overall:2percent:KRL}\\
  %
    \hline\hline
    $k$ & $\lambda$ & usim & $\sigma$ & \small{AP@$5$} & \small{AH@$5$} & \small{AP@$10$} & \small{AH@$10$} & \small{\rCI} & \small{\CI} \\
    \hline
    \endfirsthead
  %
    \multicolumn{10}{c}{{\tablename\ \thetable{} -- continued from previous page}}\\
    \hline\hline
    $k$ & $\lambda$ & usim & $\sigma$ & \small{AP@$5$} & \small{AH@$5$} & \small{AP@$10$} & \small{AH@$10$} & \small{\rCI} & \small{\CI} \\
    \hline
    \endhead
  %
    \hline
    %  \midrule
    \multicolumn{10}{c}{{Continued on next page}} \\
    \hline
    %\midrule
    \endfoot
    %
    \hline\hline
    %\bottomrule
    \insertTableNotes         %% this added
    \endlastfoot
    %
    \input{tables/unknown_2percent_KRL_data.tex}
	
    \hline
  \end{longtable}
\end{ThreePartTable}


==> tables/unknown_2percent_KRL_data.tex <==
10	&   0.000001	&       \LIN	&          -	& 0.609	& 1.489	& 0.588	& 1.994	& 0.656	& 0.739 \\
10	&   0.000001	&       \RBF	&     0.0001	& 0.735	& 1.730	& 0.708	& 2.101	& 0.662	& 0.736 \\
10	&   0.000001	&       \RBF	&      0.001	& 0.753	& 1.784	& 0.725	& 2.137	& 0.673	& 0.702 \\
10	&   0.000001	&       \RBF	&       0.01	& 0.661	& 1.570	& 0.644	& 1.862	& 0.639	& 0.580 \\
10	&    0.00001	&       \LIN	&          -	& 0.668	& 1.620	& 0.642	& 2.065	& 0.683	& 0.745 \\
10	&    0.00001	&       \RBF	&     0.0001	& 0.735	& 1.730	& 0.708	& 2.101	& 0.662	& 0.736 \\
10	&    0.00001	&       \RBF	&      0.001	& 0.753	& 1.784	& 0.725	& 2.137	& 0.673	& 0.702 \\
10	&    0.00001	&       \RBF	&       0.01	& 0.635	& 1.477	& 0.620	& 1.728	& 0.631	& 0.574 \\
10	&     0.0001	&       \LIN	&          -	& 0.697	& 1.681	& 0.675	& 2.072	& 0.681	& 0.736 \\
10	&     0.0001	&       \RBF	&     0.0001	& 0.735	& 1.730	& 0.708	& 2.101	& 0.662	& 0.736 \\
10	&     0.0001	&       \RBF	&      0.001	& 0.753	& 1.784	& 0.725	& 2.137	& 0.673	& 0.702 \\
10	&     0.0001	&       \RBF	&       0.01	& 0.588	& 1.319	& 0.578	& 1.529	& 0.619	& 0.567 \\
10	&      0.001	&       \LIN	&          -	& 0.692	& 1.698	& 0.672	& 2.082	& 0.675	& 0.719 \\
10	&      0.001	&       \RBF	&     0.0001	& 0.735	& 1.730	& 0.708	& 2.101	& 0.662	& 0.736 \\
10	&      0.001	&       \RBF	&      0.001	& 0.753	& 1.784	& 0.725	& 2.137	& 0.673	& 0.702 \\
10	&      0.001	&       \RBF	&       0.01	& 0.513	& 1.113	& 0.509	& 1.284	& 0.607	& 0.557 \\
10	&       0.01	&       \LIN	&          -	& 0.701	& 1.718	& 0.680	& 2.089	& 0.672	& 0.697 \\
10	&       0.01	&       \RBF	&     0.0001	& 0.735	& 1.730	& 0.708	& 2.101	& 0.662	& 0.736 \\
10	&       0.01	&       \RBF	&      0.001	& 0.753	& 1.784	& 0.725	& 2.137	& 0.673	& 0.702 \\
10	&       0.01	&       \RBF	&       0.01	& 0.408	& 0.859	& 0.408	& 1.001	& 0.585	& 0.548 \\
10	&        0.1	&       \LIN	&          -	& 0.732	& 1.724	& 0.705	& 2.094	& 0.664	& 0.720 \\
10	&        0.1	&       \RBF	&     0.0001	& 0.735	& 1.730	& 0.708	& 2.101	& 0.662	& 0.736 \\
10	&        0.1	&       \RBF	&      0.001	& 0.753	& 1.784	& 0.725	& 2.137	& 0.673	& 0.702 \\
10	&        0.1	&       \RBF	&       0.01	& 0.310	& 0.629	& 0.314	& 0.753	& 0.560	& 0.541 \\
10	&        0.2	&       \LIN	&          -	& 0.731	& 1.722	& 0.705	& 2.092	& 0.663	& 0.720 \\
10	&        0.2	&       \RBF	&     0.0001	& 0.735	& 1.730	& 0.708	& 2.101	& 0.662	& 0.736 \\
10	&        0.2	&       \RBF	&      0.001	& 0.753	& 1.784	& 0.725	& 2.137	& 0.673	& 0.702 \\
10	&        0.2	&       \RBF	&       0.01	& 0.278	& 0.559	& 0.282	& 0.685	& 0.552	& 0.539 \\
10	&        0.4	&       \LIN	&          -	& 0.731	& 1.722	& 0.705	& 2.092	& 0.663	& 0.720 \\
10	&        0.4	&       \RBF	&     0.0001	& 0.735	& 1.730	& 0.708	& 2.101	& 0.662	& 0.736 \\
10	&        0.4	&       \RBF	&      0.001	& 0.753	& 1.784	& 0.725	& 2.137	& 0.673	& 0.702 \\
10	&        0.4	&       \RBF	&       0.01	& 0.244	& 0.493	& 0.250	& 0.617	& 0.542	& 0.537 \\
10	&        0.6	&       \LIN	&          -	& 0.731	& 1.722	& 0.705	& 2.092	& 0.663	& 0.720 \\
10	&        0.6	&       \RBF	&     0.0001	& 0.735	& 1.730	& 0.708	& 2.101	& 0.662	& 0.736 \\
10	&        0.6	&       \RBF	&      0.001	& 0.753	& 1.784	& 0.725	& 2.137	& 0.673	& 0.702 \\
10	&        0.6	&       \RBF	&       0.01	& 0.224	& 0.463	& 0.231	& 0.586	& 0.542	& 0.536 \\
10	&        0.8	&       \LIN	&          -	& 0.731	& 1.722	& 0.705	& 2.092	& 0.663	& 0.720 \\
10	&        0.8	&       \RBF	&     0.0001	& 0.735	& 1.730	& 0.708	& 2.101	& 0.662	& 0.736 \\
10	&        0.8	&       \RBF	&      0.001	& 0.753	& 1.784	& 0.725	& 2.137	& 0.673	& 0.702 \\
10	&        0.8	&       \RBF	&       0.01	& 0.214	& 0.441	& 0.221	& 0.567	& 0.540	& 0.536 \\
10	&        1.0	&       \LIN	&          -	& 0.731	& 1.722	& 0.705	& 2.092	& 0.663	& 0.720 \\
10	&        1.0	&       \RBF	&     0.0001	& 0.735	& 1.730	& 0.708	& 2.101	& 0.662	& 0.736 \\
10	&        1.0	&       \RBF	&      0.001	& 0.753	& 1.784	& 0.725	& 2.137	& 0.673	& 0.702 \\
10	&        1.0	&       \RBF	&       0.01	& 0.205	& 0.425	& 0.213	& 0.549	& 0.537	& 0.536 \\
10	&         10	&       \LIN	&          -	& 0.732	& 1.722	& 0.705	& 2.096	& 0.662	& 0.734 \\
10	&         10	&       \RBF	&     0.0001	& 0.735	& 1.730	& 0.708	& 2.101	& 0.662	& 0.736 \\
10	&         10	&       \RBF	&      0.001	& 0.753	& 1.784	& 0.725	& 2.137	& 0.673	& 0.702 \\
10	&         10	&       \RBF	&       0.01	& 0.146	& 0.318	& 0.156	& 0.452	& 0.521	& 0.533 \\
10	&         50	&       \LIN	&          -	& 0.733	& 1.723	& 0.705	& 2.095	& 0.662	& 0.737 \\
10	&         50	&       \RBF	&     0.0001	& 0.735	& 1.730	& 0.708	& 2.101	& 0.662	& 0.736 \\
10	&         50	&       \RBF	&      0.001	& 0.753	& 1.784	& 0.725	& 2.137	& 0.673	& 0.702 \\
10	&         50	&       \RBF	&       0.01	& 0.127	& 0.286	& 0.138	& 0.420	& 0.516	& 0.532 \\
10	&        100	&       \LIN	&          -	& 0.733	& 1.723	& 0.705	& 2.095	& 0.662	& 0.737 \\
10	&        100	&       \RBF	&     0.0001	& 0.735	& 1.730	& 0.708	& 2.101	& 0.662	& 0.736 \\
10	&        100	&       \RBF	&      0.001	& 0.753	& 1.783	& 0.725	& 2.137	& 0.673	& 0.702 \\
10	&        100	&       \RBF	&       0.01	& 0.121	& 0.277	& 0.132	& 0.411	& 0.514	& 0.532 \\


==> tables/unknown_2percent_baseline.tex <==
\begin{ThreePartTable}
    \begin{TableNotes}[flushleft]  %%% This should come before longtable and it is not tablenotes but TableNotes
  \small
  \item
    \begin{footnotesize}
        \bgroup
%        \def\arraystretch{0.5}%       
        \setstretch{1}
                The columns corresponding to ``$\alpha_b$'', ``$\beta_b$'',
                ``usim'', and ``$\sigma$'' have the
                two hyperparameters, cell line similarity function,
                and parameter for \hl{$\RBF$} cell line similarity, respectively, for \BMTMKL.

	      \par
              \egroup
    \end{footnotesize}
  \end{TableNotes}
  \begin{longtable}{
      @{\hspace{0pt}}>{\raggedleft}p{0.07\textwidth}@{\hspace{5pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.07\textwidth}@{\hspace{5pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.07\textwidth}@{\hspace{5pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.07\textwidth}@{\hspace{5pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{0pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{0pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{0pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{0pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{0pt}}
      @{\hspace{0pt}}>{\raggedleft\arraybackslash}p{0.08\textwidth}@{\hspace{0pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
    }
    \caption{\mbox{\BMTMKL Performance on New Drugs ($\theta$ = 2)}}
    \label{supp:tbl:overall:2percent:baseline}\\
  %
    \hline\hline
    $\alpha_b$ & $\beta_b$ & usim & $\sigma$ & \small{AP@$5$} & \small{AH@$5$} & \small{AP@$10$} & \small{AH@$10$} & \small{\rCI} & \small{\CI} \\
    \hline
    \endfirsthead
  %
    \multicolumn{10}{c}{{\tablename\ \thetable{} -- continued from previous page}}\\
    \hline\hline
    $\alpha_b$ & $\beta_b$ & usim & $\sigma$ & \small{AP@$5$} & \small{AH@$5$} & \small{AP@$10$} & \small{AH@$10$} & \small{\rCI} & \small{\CI} \\
    \hline
    \endhead
  %
    \hline
    %  \midrule
    \multicolumn{10}{c}{{Continued on next page}} \\
    \hline
    %\midrule
    \endfoot
    %
    \hline\hline
    %\bottomrule
    \insertTableNotes         %% this added
    \endlastfoot
    %
    \input{tables/unknown_2percent_baseline_data.tex}
	
    \hline
  \end{longtable}
\end{ThreePartTable}


==> tables/unknown_2percent_baseline_data.tex <==
1       &    1      &  \RBF  & 10.0 &   0.740 &  1.702 &  0.710 &  2.071 &  0.646 &  0.812 \\ 
1e-10   &    1e-10  &  \RBF  & 10.0 &   0.739 &  1.701 &  0.710 &  2.070 &  0.644 &  0.812 \\ 
1e-10   &    1e10   &  \RBF  & 10.0 &   0.740 &  1.702 &  0.711 &  2.072 &  0.646 &  0.812 \\ 
1       &    1      &  \COS  & -    &   0.728 &  1.659 &  0.700 &  2.034 &  0.641 &  0.808 \\ 
1e-10   &    1e-10  &  \COS  & -    &   0.727 &  1.657 &  0.696 &  2.030 &  0.636 &  0.807 \\ 
1e-10   &    1e10   &  \COS  & -    &   0.729 &  1.662 &  0.698 &  2.041 &  0.641 &  0.808 \\ 



==> tables/unknown_2percent_data.tex <==
      5 &    0.00 &     0.1 &     0.0 &     \COS &       - &   0.771 &   1.802 &   0.744 &   2.131 &   0.653 &   0.769 \\
      5 &    0.00 &     0.1 &     0.0 &     \RBF &    10.0 &   0.771 &   1.802 &   0.744 &   2.131 &   0.653 &   0.769 \\
      5 &    0.00 &     0.1 &     1.0 &     \COS &       - &   0.771 &   1.802 &   0.744 &   2.131 &   0.653 &   0.769 \\
      5 &    0.00 &     0.1 &     1.0 &     \RBF &    10.0 &   0.771 &   1.802 &   0.744 &   2.131 &   0.653 &   0.769 \\
      5 &    0.00 &     0.1 &    10.0 &     \COS &       - &   0.771 &   1.802 &   0.744 &   2.132 &   0.653 &   0.769 \\
      5 &    0.00 &     0.1 &    10.0 &     \RBF &    10.0 &   0.771 &   1.802 &   0.744 &   2.132 &   0.653 &   0.769 \\
      5 &    0.00 &     0.1 &   100.0 &     \COS &       - &   0.771 &   1.805 &   0.745 &   2.133 &   0.652 &   0.771 \\
      5 &    0.00 &     0.1 &   100.0 &     \RBF &    10.0 &   0.771 &   1.805 &   0.745 &   2.133 &   0.652 &   0.772 \\
      5 &    0.00 &     1.0 &     0.0 &     \COS &       - &   0.771 &   1.805 &   0.744 &   2.132 &   0.652 &   0.772 \\
      5 &    0.00 &     1.0 &     0.0 &     \RBF &    10.0 &   0.771 &   1.805 &   0.744 &   2.132 &   0.652 &   0.772 \\
      5 &    0.00 &     1.0 &     1.0 &     \COS &       - &   0.771 &   1.805 &   0.744 &   2.132 &   0.652 &   0.772 \\
      5 &    0.00 &     1.0 &     1.0 &     \RBF &    10.0 &   0.771 &   1.805 &   0.744 &   2.132 &   0.652 &   0.772 \\
      5 &    0.00 &     1.0 &    10.0 &     \COS &       - &   0.771 &   1.805 &   0.744 &   2.133 &   0.652 &   0.772 \\
      5 &    0.00 &     1.0 &    10.0 &     \RBF &    10.0 &   0.771 &   1.805 &   0.744 &   2.133 &   0.652 &   0.772 \\
      5 &    0.00 &     1.0 &   100.0 &     \COS &       - &   0.771 &   1.805 &   0.745 &   2.133 &   0.652 &   0.771 \\
      5 &    0.00 &     1.0 &   100.0 &     \RBF &    10.0 &   0.771 &   1.805 &   0.745 &   2.133 &   0.652 &   0.772 \\
      5 &    0.05 &     0.1 &     0.0 &     \COS &       - &   0.772 &   1.808 &   0.745 &   2.133 &   0.653 &   0.774 \\
      5 &    0.05 &     0.1 &     0.0 &     \RBF &    10.0 &   0.772 &   1.808 &   0.745 &   2.133 &   0.653 &   0.774 \\
      5 &    0.05 &     0.1 &     1.0 &     \COS &       - &   0.772 &   1.808 &   0.745 &   2.133 &   0.653 &   0.774 \\
      5 &    0.05 &     0.1 &     1.0 &     \RBF &    10.0 &   0.772 &   1.808 &   0.745 &   2.133 &   0.653 &   0.774 \\
      5 &    0.05 &     0.1 &    10.0 &     \COS &       - &   0.772 &   1.808 &   0.745 &   2.133 &   0.653 &   0.774 \\
      5 &    0.05 &     0.1 &    10.0 &     \RBF &    10.0 &   0.772 &   1.808 &   0.745 &   2.133 &   0.653 &   0.774 \\
      5 &    0.05 &     0.1 &   100.0 &     \COS &       - &   0.772 &   1.806 &   0.745 &   2.133 &   0.653 &   0.774 \\
      5 &    0.05 &     0.1 &   100.0 &     \RBF &    10.0 &   0.772 &   1.806 &   0.745 &   2.133 &   0.653 &   0.774 \\
      5 &    0.05 &     1.0 &     0.0 &     \COS &       - &   0.772 &   1.808 &   0.745 &   2.133 &   0.653 &   0.774 \\
      5 &    0.05 &     1.0 &     0.0 &     \RBF &    10.0 &   0.772 &   1.808 &   0.745 &   2.133 &   0.653 &   0.774 \\
      5 &    0.05 &     1.0 &     1.0 &     \COS &       - &   0.772 &   1.808 &   0.745 &   2.133 &   0.653 &   0.774 \\
      5 &    0.05 &     1.0 &     1.0 &     \RBF &    10.0 &   0.772 &   1.808 &   0.745 &   2.133 &   0.653 &   0.774 \\
      5 &    0.05 &     1.0 &    10.0 &     \COS &       - &   0.772 &   1.808 &   0.745 &   2.133 &   0.653 &   0.774 \\
      5 &    0.05 &     1.0 &    10.0 &     \RBF &    10.0 &   0.772 &   1.808 &   0.745 &   2.133 &   0.653 &   0.774 \\
      5 &    0.05 &     1.0 &   100.0 &     \COS &       - &   0.772 &   1.806 &   0.745 &   2.133 &   0.653 &   0.774 \\
      5 &    0.05 &     1.0 &   100.0 &     \RBF &    10.0 &   0.772 &   1.806 &   0.745 &   2.133 &   0.653 &   0.774 \\
      5 &    0.10 &     0.1 &     0.0 &     \COS &       - &   0.773 &   1.810 &   0.745 &   2.135 &   0.653 &   0.776 \\
      5 &    0.10 &     0.1 &     0.0 &     \RBF &    10.0 &   0.773 &   1.810 &   0.745 &   2.135 &   0.653 &   0.776 \\
      5 &    0.10 &     0.1 &     1.0 &     \COS &       - &   0.773 &   1.810 &   0.745 &   2.135 &   0.653 &   0.776 \\
      5 &    0.10 &     0.1 &     1.0 &     \RBF &    10.0 &   0.773 &   1.810 &   0.745 &   2.135 &   0.653 &   0.776 \\
      5 &    0.10 &     0.1 &    10.0 &     \COS &       - &   0.772 &   1.809 &   0.745 &   2.135 &   0.653 &   0.776 \\
      5 &    0.10 &     0.1 &    10.0 &     \RBF &    10.0 &   0.772 &   1.809 &   0.745 &   2.135 &   0.653 &   0.776 \\
      5 &    0.10 &     0.1 &   100.0 &     \COS &       - &   0.772 &   1.808 &   0.745 &   2.135 &   0.653 &   0.776 \\
      5 &    0.10 &     0.1 &   100.0 &     \RBF &    10.0 &   0.772 &   1.808 &   0.745 &   2.135 &   0.653 &   0.776 \\
      5 &    0.10 &     1.0 &     0.0 &     \COS &       - &   0.773 &   1.810 &   0.745 &   2.135 &   0.653 &   0.776 \\
      5 &    0.10 &     1.0 &     0.0 &     \RBF &    10.0 &   0.773 &   1.810 &   0.745 &   2.135 &   0.653 &   0.776 \\
      5 &    0.10 &     1.0 &     1.0 &     \COS &       - &   0.773 &   1.810 &   0.745 &   2.135 &   0.653 &   0.776 \\
      5 &    0.10 &     1.0 &     1.0 &     \RBF &    10.0 &   0.773 &   1.810 &   0.745 &   2.135 &   0.653 &   0.776 \\
      5 &    0.10 &     1.0 &    10.0 &     \COS &       - &   0.772 &   1.809 &   0.745 &   2.135 &   0.653 &   0.776 \\
      5 &    0.10 &     1.0 &    10.0 &     \RBF &    10.0 &   0.772 &   1.809 &   0.745 &   2.135 &   0.653 &   0.776 \\
      5 &    0.10 &     1.0 &   100.0 &     \COS &       - &   0.772 &   1.808 &   0.745 &   2.135 &   0.653 &   0.776 \\
      5 &    0.10 &     1.0 &   100.0 &     \RBF &    10.0 &   0.772 &   1.808 &   0.745 &   2.135 &   0.653 &   0.776 \\
      5 &    0.50 &     0.1 &     0.0 &     \COS &       - &   0.773 &   1.814 &   0.745 &   2.141 &   0.652 &   0.792 \\
      5 &    0.50 &     0.1 &     0.0 &     \RBF &    10.0 &   0.773 &   1.814 &   0.745 &   2.141 &   0.652 &   0.792 \\
      5 &    0.50 &     0.1 &     1.0 &     \COS &       - &   0.773 &   1.814 &   0.745 &   2.141 &   0.652 &   0.792 \\
      5 &    0.50 &     0.1 &     1.0 &     \RBF &    10.0 &   0.773 &   1.814 &   0.745 &   2.141 &   0.652 &   0.792 \\
      5 &    0.50 &     0.1 &    10.0 &     \COS &       - &   0.773 &   1.815 &   0.745 &   2.141 &   0.652 &   0.792 \\
      5 &    0.50 &     0.1 &    10.0 &     \RBF &    10.0 &   0.773 &   1.815 &   0.745 &   2.141 &   0.652 &   0.792 \\
      5 &    0.50 &     0.1 &   100.0 &     \COS &       - &   0.773 &   1.816 &   0.745 &   2.142 &   0.651 &   0.792 \\
      5 &    0.50 &     0.1 &   100.0 &     \RBF &    10.0 &   0.773 &   1.815 &   0.745 &   2.141 &   0.651 &   0.792 \\
      5 &    0.50 &     1.0 &     0.0 &     \COS &       - &   0.773 &   1.814 &   0.745 &   2.141 &   0.652 &   0.792 \\
      5 &    0.50 &     1.0 &     0.0 &     \RBF &    10.0 &   0.773 &   1.814 &   0.745 &   2.141 &   0.652 &   0.792 \\
      5 &    0.50 &     1.0 &     1.0 &     \COS &       - &   0.773 &   1.814 &   0.745 &   2.141 &   0.652 &   0.792 \\
      5 &    0.50 &     1.0 &     1.0 &     \RBF &    10.0 &   0.773 &   1.814 &   0.745 &   2.141 &   0.652 &   0.792 \\
      5 &    0.50 &     1.0 &    10.0 &     \COS &       - &   0.773 &   1.815 &   0.745 &   2.141 &   0.652 &   0.792 \\
      5 &    0.50 &     1.0 &    10.0 &     \RBF &    10.0 &   0.773 &   1.815 &   0.745 &   2.141 &   0.652 &   0.792 \\
      5 &    0.50 &     1.0 &   100.0 &     \COS &       - &   0.773 &   1.816 &   0.745 &   2.142 &   0.651 &   0.792 \\
      5 &    0.50 &     1.0 &   100.0 &     \RBF &    10.0 &   0.773 &   1.815 &   0.745 &   2.141 &   0.651 &   0.792 \\
      5 &    1.00 &     0.1 &     0.0 &     \COS &       - &   0.531 &   1.129 &   0.514 &   1.392 &   0.587 &   0.639 \\
      5 &    1.00 &     0.1 &     0.0 &     \RBF &    10.0 &   0.531 &   1.129 &   0.514 &   1.392 &   0.587 &   0.639 \\
      5 &    1.00 &     0.1 &     1.0 &     \COS &       - &   0.536 &   1.132 &   0.519 &   1.398 &   0.588 &   0.641 \\
      5 &    1.00 &     0.1 &     1.0 &     \RBF &    10.0 &   0.532 &   1.127 &   0.514 &   1.392 &   0.589 &   0.639 \\
      5 &    1.00 &     0.1 &    10.0 &     \COS &       - &   0.546 &   1.155 &   0.528 &   1.415 &   0.591 &   0.648 \\
      5 &    1.00 &     0.1 &    10.0 &     \RBF &    10.0 &   0.544 &   1.154 &   0.527 &   1.414 &   0.591 &   0.648 \\
      5 &    1.00 &     0.1 &   100.0 &     \COS &       - &   0.570 &   1.216 &   0.553 &   1.487 &   0.607 &   0.672 \\
      5 &    1.00 &     0.1 &   100.0 &     \RBF &    10.0 &   0.572 &   1.219 &   0.555 &   1.491 &   0.603 &   0.676 \\
      5 &    1.00 &     1.0 &     0.0 &     \COS &       - &   0.538 &   1.137 &   0.521 &   1.397 &   0.587 &   0.640 \\
      5 &    1.00 &     1.0 &     0.0 &     \RBF &    10.0 &   0.538 &   1.137 &   0.521 &   1.397 &   0.587 &   0.640 \\
      5 &    1.00 &     1.0 &     1.0 &     \COS &       - &   0.540 &   1.139 &   0.523 &   1.400 &   0.588 &   0.641 \\
      5 &    1.00 &     1.0 &     1.0 &     \RBF &    10.0 &   0.537 &   1.137 &   0.520 &   1.393 &   0.588 &   0.640 \\
      5 &    1.00 &     1.0 &    10.0 &     \COS &       - &   0.548 &   1.165 &   0.530 &   1.421 &   0.591 &   0.650 \\
      5 &    1.00 &     1.0 &    10.0 &     \RBF &    10.0 &   0.545 &   1.160 &   0.527 &   1.414 &   0.591 &   0.647 \\
      5 &    1.00 &     1.0 &   100.0 &     \COS &       - &   0.572 &   1.214 &   0.554 &   1.486 &   0.603 &   0.671 \\
      5 &    1.00 &     1.0 &   100.0 &     \RBF &    10.0 &   0.572 &   1.219 &   0.556 &   1.489 &   0.603 &   0.676 \\
     10 &    0.00 &     0.1 &     0.0 &     \COS &       - &   0.780 &   1.851 &   0.755 &   2.157 &   0.631 &   0.786 \\
     10 &    0.00 &     0.1 &     0.0 &     \RBF &    10.0 &   0.780 &   1.851 &   0.755 &   2.157 &   0.631 &   0.786 \\
     10 &    0.00 &     0.1 &     1.0 &     \COS &       - &   0.780 &   1.851 &   0.755 &   2.157 &   0.631 &   0.786 \\
     10 &    0.00 &     0.1 &     1.0 &     \RBF &    10.0 &   0.780 &   1.851 &   0.755 &   2.157 &   0.631 &   0.786 \\
     10 &    0.00 &     0.1 &    10.0 &     \COS &       - &   0.780 &   1.851 &   0.755 &   2.157 &   0.632 &   0.786 \\
     10 &    0.00 &     0.1 &    10.0 &     \RBF &    10.0 &   0.780 &   1.850 &   0.755 &   2.157 &   0.632 &   0.786 \\
     10 &    0.00 &     0.1 &   100.0 &     \COS &       - &   0.783 &   1.856 &   0.758 &   2.159 &   0.638 &   0.774 \\
     10 &    0.00 &     0.1 &   100.0 &     \RBF &    10.0 &   0.782 &   1.858 &   0.757 &   2.159 &   0.638 &   0.777 \\
     10 &    0.00 &     1.0 &     0.0 &     \COS &       - &   0.779 &   1.849 &   0.754 &   2.157 &   0.631 &   0.790 \\
     10 &    0.00 &     1.0 &     0.0 &     \RBF &    10.0 &   0.779 &   1.849 &   0.754 &   2.157 &   0.631 &   0.790 \\
     10 &    0.00 &     1.0 &     1.0 &     \COS &       - &   0.779 &   1.849 &   0.754 &   2.157 &   0.631 &   0.790 \\
     10 &    0.00 &     1.0 &     1.0 &     \RBF &    10.0 &   0.779 &   1.849 &   0.754 &   2.157 &   0.631 &   0.790 \\
     10 &    0.00 &     1.0 &    10.0 &     \COS &       - &   0.779 &   1.849 &   0.754 &   2.157 &   0.631 &   0.790 \\
     10 &    0.00 &     1.0 &    10.0 &     \RBF &    10.0 &   0.779 &   1.849 &   0.754 &   2.157 &   0.631 &   0.790 \\
     10 &    0.00 &     1.0 &   100.0 &     \COS &       - &   0.779 &   1.852 &   0.754 &   2.156 &   0.631 &   0.790 \\
     10 &    0.00 &     1.0 &   100.0 &     \RBF &    10.0 &   0.779 &   1.851 &   0.754 &   2.157 &   0.632 &   0.790 \\
     10 &    0.05 &     0.1 &     0.0 &     \COS &       - &   0.778 &   1.850 &   0.754 &   2.156 &   0.630 &   0.792 \\
     10 &    0.05 &     0.1 &     0.0 &     \RBF &    10.0 &   0.778 &   1.850 &   0.754 &   2.156 &   0.630 &   0.792 \\
     10 &    0.05 &     0.1 &     1.0 &     \COS &       - &   0.778 &   1.850 &   0.754 &   2.156 &   0.630 &   0.792 \\
     10 &    0.05 &     0.1 &     1.0 &     \RBF &    10.0 &   0.778 &   1.850 &   0.754 &   2.156 &   0.630 &   0.792 \\
     10 &    0.05 &     0.1 &    10.0 &     \COS &       - &   0.778 &   1.849 &   0.754 &   2.156 &   0.630 &   0.792 \\
     10 &    0.05 &     0.1 &    10.0 &     \RBF &    10.0 &   0.778 &   1.849 &   0.754 &   2.156 &   0.630 &   0.792 \\
     10 &    0.05 &     0.1 &   100.0 &     \COS &       - &   0.778 &   1.849 &   0.753 &   2.156 &   0.632 &   0.792 \\
     10 &    0.05 &     0.1 &   100.0 &     \RBF &    10.0 &   0.778 &   1.850 &   0.753 &   2.156 &   0.632 &   0.792 \\
     10 &    0.05 &     1.0 &     0.0 &     \COS &       - &   0.778 &   1.850 &   0.754 &   2.156 &   0.630 &   0.792 \\
     10 &    0.05 &     1.0 &     0.0 &     \RBF &    10.0 &   0.778 &   1.850 &   0.754 &   2.156 &   0.630 &   0.792 \\
     10 &    0.05 &     1.0 &     1.0 &     \COS &       - &   0.778 &   1.850 &   0.754 &   2.156 &   0.630 &   0.792 \\
     10 &    0.05 &     1.0 &     1.0 &     \RBF &    10.0 &   0.778 &   1.850 &   0.754 &   2.156 &   0.630 &   0.792 \\
     10 &    0.05 &     1.0 &    10.0 &     \COS &       - &   0.778 &   1.849 &   0.754 &   2.156 &   0.630 &   0.792 \\
     10 &    0.05 &     1.0 &    10.0 &     \RBF &    10.0 &   0.778 &   1.849 &   0.754 &   2.156 &   0.630 &   0.792 \\
     10 &    0.05 &     1.0 &   100.0 &     \COS &       - &   0.778 &   1.849 &   0.753 &   2.156 &   0.632 &   0.792 \\
     10 &    0.05 &     1.0 &   100.0 &     \RBF &    10.0 &   0.778 &   1.850 &   0.753 &   2.156 &   0.632 &   0.792 \\
     10 &    0.10 &     0.1 &     0.0 &     \COS &       - &   0.777 &   1.845 &   0.753 &   2.155 &   0.629 &   0.794 \\
     10 &    0.10 &     0.1 &     0.0 &     \RBF &    10.0 &   0.777 &   1.845 &   0.753 &   2.155 &   0.629 &   0.794 \\
     10 &    0.10 &     0.1 &     1.0 &     \COS &       - &   0.777 &   1.845 &   0.753 &   2.155 &   0.629 &   0.794 \\
     10 &    0.10 &     0.1 &     1.0 &     \RBF &    10.0 &   0.777 &   1.845 &   0.753 &   2.155 &   0.629 &   0.794 \\
     10 &    0.10 &     0.1 &    10.0 &     \COS &       - &   0.777 &   1.845 &   0.753 &   2.155 &   0.629 &   0.794 \\
     10 &    0.10 &     0.1 &    10.0 &     \RBF &    10.0 &   0.777 &   1.845 &   0.753 &   2.155 &   0.629 &   0.794 \\
     10 &    0.10 &     0.1 &   100.0 &     \COS &       - &   0.777 &   1.849 &   0.753 &   2.155 &   0.629 &   0.794 \\
     10 &    0.10 &     0.1 &   100.0 &     \RBF &    10.0 &   0.777 &   1.848 &   0.753 &   2.155 &   0.629 &   0.794 \\
     10 &    0.10 &     1.0 &     0.0 &     \COS &       - &   0.777 &   1.845 &   0.753 &   2.155 &   0.629 &   0.794 \\
     10 &    0.10 &     1.0 &     0.0 &     \RBF &    10.0 &   0.777 &   1.845 &   0.753 &   2.155 &   0.629 &   0.794 \\
     10 &    0.10 &     1.0 &     1.0 &     \COS &       - &   0.777 &   1.845 &   0.753 &   2.155 &   0.629 &   0.794 \\
     10 &    0.10 &     1.0 &     1.0 &     \RBF &    10.0 &   0.777 &   1.845 &   0.753 &   2.155 &   0.629 &   0.794 \\
     10 &    0.10 &     1.0 &    10.0 &     \COS &       - &   0.777 &   1.845 &   0.753 &   2.155 &   0.629 &   0.794 \\
     10 &    0.10 &     1.0 &    10.0 &     \RBF &    10.0 &   0.777 &   1.845 &   0.753 &   2.155 &   0.629 &   0.794 \\
     10 &    0.10 &     1.0 &   100.0 &     \COS &       - &   0.777 &   1.849 &   0.753 &   2.156 &   0.629 &   0.794 \\
     10 &    0.10 &     1.0 &   100.0 &     \RBF &    10.0 &   0.777 &   1.848 &   0.753 &   2.155 &   0.629 &   0.794 \\
     10 &    0.50 &     0.1 &     0.0 &     \COS &       - &   0.757 &   1.787 &   0.735 &   2.091 &   0.648 &   0.703 \\
     10 &    0.50 &     0.1 &     0.0 &     \RBF &    10.0 &   0.757 &   1.787 &   0.735 &   2.091 &   0.648 &   0.703 \\
     10 &    0.50 &     0.1 &     1.0 &     \COS &       - &   0.757 &   1.786 &   0.735 &   2.091 &   0.648 &   0.703 \\
     10 &    0.50 &     0.1 &     1.0 &     \RBF &    10.0 &   0.757 &   1.786 &   0.735 &   2.091 &   0.648 &   0.703 \\
     10 &    0.50 &     0.1 &    10.0 &     \COS &       - &   0.757 &   1.786 &   0.736 &   2.091 &   0.648 &   0.703 \\
     10 &    0.50 &     0.1 &    10.0 &     \RBF &    10.0 &   0.757 &   1.786 &   0.735 &   2.091 &   0.648 &   0.703 \\
     10 &    0.50 &     0.1 &   100.0 &     \COS &       - &   0.758 &   1.785 &   0.737 &   2.088 &   0.656 &   0.703 \\
     10 &    0.50 &     0.1 &   100.0 &     \RBF &    10.0 &   0.758 &   1.786 &   0.737 &   2.090 &   0.656 &   0.703 \\
     10 &    0.50 &     1.0 &     0.0 &     \COS &       - &   0.772 &   1.832 &   0.747 &   2.138 &   0.654 &   0.735 \\
     10 &    0.50 &     1.0 &     0.0 &     \RBF &    10.0 &   0.772 &   1.832 &   0.747 &   2.138 &   0.654 &   0.735 \\
     10 &    0.50 &     1.0 &     1.0 &     \COS &       - &   0.772 &   1.832 &   0.747 &   2.139 &   0.654 &   0.736 \\
     10 &    0.50 &     1.0 &     1.0 &     \RBF &    10.0 &   0.772 &   1.832 &   0.747 &   2.139 &   0.654 &   0.736 \\
     10 &    0.50 &     1.0 &    10.0 &     \COS &       - &   0.773 &   1.835 &   0.747 &   2.140 &   0.654 &   0.737 \\
     10 &    0.50 &     1.0 &    10.0 &     \RBF &    10.0 &   0.772 &   1.834 &   0.747 &   2.140 &   0.654 &   0.737 \\
     10 &    0.50 &     1.0 &   100.0 &     \COS &       - &   0.774 &   1.834 &   0.749 &   2.140 &   0.657 &   0.736 \\
     10 &    0.50 &     1.0 &   100.0 &     \RBF &    10.0 &   0.773 &   1.834 &   0.749 &   2.140 &   0.655 &   0.737 \\
     10 &    1.00 &     0.1 &     0.0 &     \COS &       - &   0.578 &   1.207 &   0.559 &   1.478 &   0.592 &   0.644 \\
     10 &    1.00 &     0.1 &     0.0 &     \RBF &    10.0 &   0.578 &   1.207 &   0.559 &   1.478 &   0.592 &   0.644 \\
     10 &    1.00 &     0.1 &     1.0 &     \COS &       - &   0.580 &   1.215 &   0.562 &   1.484 &   0.594 &   0.646 \\
     10 &    1.00 &     0.1 &     1.0 &     \RBF &    10.0 &   0.580 &   1.214 &   0.562 &   1.482 &   0.594 &   0.645 \\
     10 &    1.00 &     0.1 &    10.0 &     \COS &       - &   0.589 &   1.260 &   0.569 &   1.534 &   0.605 &   0.656 \\
     10 &    1.00 &     0.1 &    10.0 &     \RBF &    10.0 &   0.588 &   1.253 &   0.568 &   1.529 &   0.605 &   0.655 \\
     10 &    1.00 &     0.1 &   100.0 &     \COS &       - &   0.612 &   1.341 &   0.593 &   1.647 &   0.618 &   0.696 \\
     10 &    1.00 &     0.1 &   100.0 &     \RBF &    10.0 &   0.608 &   1.335 &   0.591 &   1.636 &   0.620 &   0.695 \\
     10 &    1.00 &     1.0 &     0.0 &     \COS &       - &   0.577 &   1.206 &   0.559 &   1.471 &   0.592 &   0.640 \\
     10 &    1.00 &     1.0 &     0.0 &     \RBF &    10.0 &   0.577 &   1.206 &   0.559 &   1.471 &   0.592 &   0.640 \\
     10 &    1.00 &     1.0 &     1.0 &     \COS &       - &   0.581 &   1.215 &   0.562 &   1.483 &   0.594 &   0.645 \\
     10 &    1.00 &     1.0 &     1.0 &     \RBF &    10.0 &   0.581 &   1.214 &   0.562 &   1.482 &   0.594 &   0.645 \\
     10 &    1.00 &     1.0 &    10.0 &     \COS &       - &   0.586 &   1.246 &   0.567 &   1.522 &   0.605 &   0.651 \\
     10 &    1.00 &     1.0 &    10.0 &     \RBF &    10.0 &   0.585 &   1.246 &   0.566 &   1.519 &   0.604 &   0.650 \\
     10 &    1.00 &     1.0 &   100.0 &     \COS &       - &   0.611 &   1.334 &   0.592 &   1.645 &   0.620 &   0.695 \\
     10 &    1.00 &     1.0 &   100.0 &     \RBF &    10.0 &   0.609 &   1.335 &   0.592 &   1.631 &   0.622 &   0.692 \\
     15 &    0.00 &     0.1 &     0.0 &     \COS &       - &   0.763 &   1.837 &   0.736 &   2.162 &   0.613 &   0.786 \\
     15 &    0.00 &     0.1 &     0.0 &     \RBF &    10.0 &   0.763 &   1.837 &   0.736 &   2.162 &   0.613 &   0.786 \\
     15 &    0.00 &     0.1 &     1.0 &     \COS &       - &   0.763 &   1.837 &   0.736 &   2.162 &   0.613 &   0.786 \\
     15 &    0.00 &     0.1 &     1.0 &     \RBF &    10.0 &   0.763 &   1.837 &   0.736 &   2.162 &   0.613 &   0.786 \\
     15 &    0.00 &     0.1 &    10.0 &     \COS &       - &   0.759 &   1.831 &   0.733 &   2.161 &   0.610 &   0.788 \\
     15 &    0.00 &     0.1 &    10.0 &     \RBF &    10.0 &   0.759 &   1.831 &   0.733 &   2.160 &   0.610 &   0.788 \\
     15 &    0.00 &     0.1 &   100.0 &     \COS &       - &   0.779 &   1.858 &   0.753 &   2.169 &   0.643 &   0.768 \\
     15 &    0.00 &     0.1 &   100.0 &     \RBF &    10.0 &   0.777 &   1.858 &   0.751 &   2.171 &   0.632 &   0.774 \\
     15 &    0.00 &     1.0 &     0.0 &     \COS &       - &   0.747 &   1.798 &   0.719 &   2.148 &   0.590 &   0.796 \\
     15 &    0.00 &     1.0 &     0.0 &     \RBF &    10.0 &   0.747 &   1.798 &   0.719 &   2.148 &   0.590 &   0.796 \\
     15 &    0.00 &     1.0 &     1.0 &     \COS &       - &   0.747 &   1.798 &   0.719 &   2.148 &   0.590 &   0.796 \\
     15 &    0.00 &     1.0 &     1.0 &     \RBF &    10.0 &   0.747 &   1.798 &   0.719 &   2.148 &   0.590 &   0.796 \\
     15 &    0.00 &     1.0 &    10.0 &     \COS &       - &   0.746 &   1.795 &   0.717 &   2.147 &   0.588 &   0.796 \\
     15 &    0.00 &     1.0 &    10.0 &     \RBF &    10.0 &   0.746 &   1.794 &   0.717 &   2.147 &   0.588 &   0.796 \\
     15 &    0.00 &     1.0 &   100.0 &     \COS &       - &   0.754 &   1.817 &   0.726 &   2.158 &   0.598 &   0.793 \\
     15 &    0.00 &     1.0 &   100.0 &     \RBF &    10.0 &   0.749 &   1.800 &   0.720 &   2.152 &   0.592 &   0.796 \\
     15 &    0.05 &     0.1 &     0.0 &     \COS &       - &   0.738 &   1.779 &   0.710 &   2.138 &   0.585 &   0.798 \\
     15 &    0.05 &     0.1 &     0.0 &     \RBF &    10.0 &   0.738 &   1.779 &   0.710 &   2.138 &   0.585 &   0.798 \\
     15 &    0.05 &     0.1 &     1.0 &     \COS &       - &   0.739 &   1.779 &   0.710 &   2.138 &   0.585 &   0.798 \\
     15 &    0.05 &     0.1 &     1.0 &     \RBF &    10.0 &   0.739 &   1.779 &   0.710 &   2.138 &   0.585 &   0.798 \\
     15 &    0.05 &     0.1 &    10.0 &     \COS &       - &   0.739 &   1.780 &   0.710 &   2.138 &   0.585 &   0.798 \\
     15 &    0.05 &     0.1 &    10.0 &     \RBF &    10.0 &   0.739 &   1.780 &   0.710 &   2.138 &   0.585 &   0.798 \\
     15 &    0.05 &     0.1 &   100.0 &     \COS &       - &   0.742 &   1.788 &   0.713 &   2.143 &   0.588 &   0.798 \\
     15 &    0.05 &     0.1 &   100.0 &     \RBF &    10.0 &   0.740 &   1.784 &   0.711 &   2.140 &   0.586 &   0.798 \\
     15 &    0.05 &     1.0 &     0.0 &     \COS &       - &   0.738 &   1.779 &   0.710 &   2.138 &   0.585 &   0.798 \\
     15 &    0.05 &     1.0 &     0.0 &     \RBF &    10.0 &   0.738 &   1.779 &   0.710 &   2.138 &   0.585 &   0.798 \\
     15 &    0.05 &     1.0 &     1.0 &     \COS &       - &   0.739 &   1.779 &   0.710 &   2.138 &   0.585 &   0.798 \\
     15 &    0.05 &     1.0 &     1.0 &     \RBF &    10.0 &   0.739 &   1.779 &   0.710 &   2.138 &   0.585 &   0.798 \\
     15 &    0.05 &     1.0 &    10.0 &     \COS &       - &   0.739 &   1.780 &   0.710 &   2.138 &   0.585 &   0.798 \\
     15 &    0.05 &     1.0 &    10.0 &     \RBF &    10.0 &   0.739 &   1.780 &   0.710 &   2.138 &   0.585 &   0.798 \\
     15 &    0.05 &     1.0 &   100.0 &     \COS &       - &   0.740 &   1.784 &   0.712 &   2.141 &   0.587 &   0.798 \\
     15 &    0.05 &     1.0 &   100.0 &     \RBF &    10.0 &   0.740 &   1.784 &   0.711 &   2.140 &   0.586 &   0.798 \\
     15 &    0.10 &     0.1 &     0.0 &     \COS &       - &   0.732 &   1.764 &   0.704 &   2.128 &   0.580 &   0.800 \\
     15 &    0.10 &     0.1 &     0.0 &     \RBF &    10.0 &   0.732 &   1.764 &   0.704 &   2.128 &   0.580 &   0.800 \\
     15 &    0.10 &     0.1 &     1.0 &     \COS &       - &   0.732 &   1.764 &   0.704 &   2.129 &   0.580 &   0.800 \\
     15 &    0.10 &     0.1 &     1.0 &     \RBF &    10.0 &   0.732 &   1.764 &   0.704 &   2.129 &   0.580 &   0.800 \\
     15 &    0.10 &     0.1 &    10.0 &     \COS &       - &   0.733 &   1.764 &   0.704 &   2.129 &   0.580 &   0.800 \\
     15 &    0.10 &     0.1 &    10.0 &     \RBF &    10.0 &   0.733 &   1.764 &   0.704 &   2.129 &   0.580 &   0.800 \\
     15 &    0.10 &     0.1 &   100.0 &     \COS &       - &   0.735 &   1.773 &   0.706 &   2.132 &   0.582 &   0.800 \\
     15 &    0.10 &     0.1 &   100.0 &     \RBF &    10.0 &   0.734 &   1.770 &   0.705 &   2.131 &   0.581 &   0.800 \\
     15 &    0.10 &     1.0 &     0.0 &     \COS &       - &   0.732 &   1.764 &   0.704 &   2.129 &   0.580 &   0.800 \\
     15 &    0.10 &     1.0 &     0.0 &     \RBF &    10.0 &   0.732 &   1.764 &   0.704 &   2.129 &   0.580 &   0.800 \\
     15 &    0.10 &     1.0 &     1.0 &     \COS &       - &   0.732 &   1.764 &   0.704 &   2.129 &   0.580 &   0.800 \\
     15 &    0.10 &     1.0 &     1.0 &     \RBF &    10.0 &   0.732 &   1.764 &   0.704 &   2.129 &   0.580 &   0.800 \\
     15 &    0.10 &     1.0 &    10.0 &     \COS &       - &   0.733 &   1.764 &   0.704 &   2.129 &   0.580 &   0.800 \\
     15 &    0.10 &     1.0 &    10.0 &     \RBF &    10.0 &   0.733 &   1.764 &   0.705 &   2.129 &   0.580 &   0.800 \\
     15 &    0.10 &     1.0 &   100.0 &     \COS &       - &   0.735 &   1.773 &   0.707 &   2.132 &   0.582 &   0.800 \\
     15 &    0.10 &     1.0 &   100.0 &     \RBF &    10.0 &   0.734 &   1.771 &   0.705 &   2.131 &   0.582 &   0.800 \\
     15 &    0.50 &     0.1 &     0.0 &     \COS &       - &   0.742 &   1.766 &   0.717 &   2.079 &   0.615 &   0.713 \\
     15 &    0.50 &     0.1 &     0.0 &     \RBF &    10.0 &   0.742 &   1.766 &   0.717 &   2.079 &   0.615 &   0.713 \\
     15 &    0.50 &     0.1 &     1.0 &     \COS &       - &   0.742 &   1.766 &   0.718 &   2.079 &   0.615 &   0.713 \\
     15 &    0.50 &     0.1 &     1.0 &     \RBF &    10.0 &   0.742 &   1.766 &   0.718 &   2.079 &   0.615 &   0.713 \\
     15 &    0.50 &     0.1 &    10.0 &     \COS &       - &   0.743 &   1.770 &   0.719 &   2.081 &   0.619 &   0.713 \\
     15 &    0.50 &     0.1 &    10.0 &     \RBF &    10.0 &   0.743 &   1.770 &   0.719 &   2.082 &   0.619 &   0.713 \\
     15 &    0.50 &     0.1 &   100.0 &     \COS &       - &   0.751 &   1.786 &   0.727 &   2.094 &   0.632 &   0.712 \\
     15 &    0.50 &     0.1 &   100.0 &     \RBF &    10.0 &   0.750 &   1.786 &   0.726 &   2.093 &   0.628 &   0.712 \\
     15 &    0.50 &     1.0 &     0.0 &     \COS &       - &   0.742 &   1.784 &   0.717 &   2.112 &   0.610 &   0.732 \\
     15 &    0.50 &     1.0 &     0.0 &     \RBF &    10.0 &   0.742 &   1.784 &   0.717 &   2.112 &   0.610 &   0.732 \\
     15 &    0.50 &     1.0 &     1.0 &     \COS &       - &   0.742 &   1.786 &   0.717 &   2.112 &   0.611 &   0.733 \\
     15 &    0.50 &     1.0 &     1.0 &     \RBF &    10.0 &   0.742 &   1.786 &   0.717 &   2.112 &   0.611 &   0.733 \\
     15 &    0.50 &     1.0 &    10.0 &     \COS &       - &   0.742 &   1.790 &   0.718 &   2.118 &   0.611 &   0.736 \\
     15 &    0.50 &     1.0 &    10.0 &     \RBF &    10.0 &   0.742 &   1.790 &   0.718 &   2.117 &   0.611 &   0.735 \\
     15 &    0.50 &     1.0 &   100.0 &     \COS &       - &   0.750 &   1.809 &   0.726 &   2.129 &   0.622 &   0.735 \\
     15 &    0.50 &     1.0 &   100.0 &     \RBF &    10.0 &   0.749 &   1.807 &   0.725 &   2.128 &   0.620 &   0.736 \\
     15 &    1.00 &     0.1 &     0.0 &     \COS &       - &   0.587 &   1.251 &   0.569 &   1.520 &   0.600 &   0.676 \\
     15 &    1.00 &     0.1 &     0.0 &     \RBF &    10.0 &   0.587 &   1.251 &   0.569 &   1.520 &   0.600 &   0.676 \\
     15 &    1.00 &     0.1 &     1.0 &     \COS &       - &   0.589 &   1.261 &   0.571 &   1.538 &   0.602 &   0.679 \\
     15 &    1.00 &     0.1 &     1.0 &     \RBF &    10.0 &   0.589 &   1.260 &   0.571 &   1.536 &   0.602 &   0.679 \\
     15 &    1.00 &     0.1 &    10.0 &     \COS &       - &   0.612 &   1.333 &   0.594 &   1.633 &   0.624 &   0.696 \\
     15 &    1.00 &     0.1 &    10.0 &     \RBF &    10.0 &   0.610 &   1.323 &   0.591 &   1.623 &   0.624 &   0.695 \\
     15 &    1.00 &     0.1 &   100.0 &     \COS &       - &   0.631 &   1.417 &   0.611 &   1.774 &   0.639 &   0.736 \\
     15 &    1.00 &     0.1 &   100.0 &     \RBF &    10.0 &   0.629 &   1.418 &   0.610 &   1.760 &   0.639 &   0.730 \\
     15 &    1.00 &     1.0 &     0.0 &     \COS &       - &   0.586 &   1.252 &   0.568 &   1.518 &   0.601 &   0.673 \\
     15 &    1.00 &     1.0 &     0.0 &     \RBF &    10.0 &   0.586 &   1.252 &   0.568 &   1.518 &   0.601 &   0.673 \\
     15 &    1.00 &     1.0 &     1.0 &     \COS &       - &   0.590 &   1.261 &   0.571 &   1.537 &   0.602 &   0.679 \\
     15 &    1.00 &     1.0 &     1.0 &     \RBF &    10.0 &   0.590 &   1.260 &   0.571 &   1.534 &   0.602 &   0.678 \\
     15 &    1.00 &     1.0 &    10.0 &     \COS &       - &   0.609 &   1.322 &   0.591 &   1.616 &   0.624 &   0.688 \\
     15 &    1.00 &     1.0 &    10.0 &     \RBF &    10.0 &   0.606 &   1.311 &   0.589 &   1.607 &   0.622 &   0.686 \\
     15 &    1.00 &     1.0 &   100.0 &     \COS &       - &   0.630 &   1.419 &   0.609 &   1.765 &   0.641 &   0.731 \\
     15 &    1.00 &     1.0 &   100.0 &     \RBF &    10.0 &   0.633 &   1.413 &   0.612 &   1.757 &   0.639 &   0.733 \\
     30 &    0.00 &     0.1 &     0.0 &     \COS &       - &   0.665 &   1.631 &   0.639 &   2.051 &   0.591 &   0.783 \\
     30 &    0.00 &     0.1 &     0.0 &     \RBF &    10.0 &   0.665 &   1.631 &   0.639 &   2.051 &   0.591 &   0.783 \\
     30 &    0.00 &     0.1 &     1.0 &     \COS &       - &   0.663 &   1.625 &   0.637 &   2.049 &   0.590 &   0.784 \\
     30 &    0.00 &     0.1 &     1.0 &     \RBF &    10.0 &   0.663 &   1.625 &   0.637 &   2.049 &   0.590 &   0.784 \\
     30 &    0.00 &     0.1 &    10.0 &     \COS &       - &   0.640 &   1.580 &   0.615 &   2.027 &   0.577 &   0.788 \\
     30 &    0.00 &     0.1 &    10.0 &     \RBF &    10.0 &   0.641 &   1.582 &   0.616 &   2.029 &   0.578 &   0.788 \\
     30 &    0.00 &     0.1 &   100.0 &     \COS &       - &   0.763 &   1.767 &   0.733 &   2.100 &   0.657 &   0.725 \\
     30 &    0.00 &     0.1 &   100.0 &     \RBF &    10.0 &   0.755 &   1.784 &   0.727 &   2.127 &   0.649 &   0.744 \\
     30 &    0.00 &     1.0 &     0.0 &     \COS &       - &   0.552 &   1.359 &   0.528 &   1.873 &   0.523 &   0.802 \\
     30 &    0.00 &     1.0 &     0.0 &     \RBF &    10.0 &   0.552 &   1.359 &   0.528 &   1.873 &   0.523 &   0.802 \\
     30 &    0.00 &     1.0 &     1.0 &     \COS &       - &   0.548 &   1.345 &   0.524 &   1.863 &   0.520 &   0.803 \\
     30 &    0.00 &     1.0 &     1.0 &     \RBF &    10.0 &   0.548 &   1.345 &   0.524 &   1.863 &   0.520 &   0.803 \\
     30 &    0.00 &     1.0 &    10.0 &     \COS &       - &   0.546 &   1.342 &   0.523 &   1.861 &   0.519 &   0.803 \\
     30 &    0.00 &     1.0 &    10.0 &     \RBF &    10.0 &   0.546 &   1.342 &   0.522 &   1.861 &   0.519 &   0.803 \\
     30 &    0.00 &     1.0 &   100.0 &     \COS &       - &   0.706 &   1.708 &   0.677 &   2.101 &   0.609 &   0.775 \\
     30 &    0.00 &     1.0 &   100.0 &     \RBF &    10.0 &   0.651 &   1.605 &   0.626 &   2.046 &   0.585 &   0.788 \\
     30 &    0.05 &     0.1 &     0.0 &     \COS &       - &   0.531 &   1.299 &   0.509 &   1.820 &   0.509 &   0.804 \\
     30 &    0.05 &     0.1 &     0.0 &     \RBF &    10.0 &   0.531 &   1.299 &   0.509 &   1.820 &   0.509 &   0.804 \\
     30 &    0.05 &     0.1 &     1.0 &     \COS &       - &   0.531 &   1.299 &   0.509 &   1.821 &   0.509 &   0.804 \\
     30 &    0.05 &     0.1 &     1.0 &     \RBF &    10.0 &   0.531 &   1.299 &   0.509 &   1.821 &   0.509 &   0.804 \\
     30 &    0.05 &     0.1 &    10.0 &     \COS &       - &   0.531 &   1.300 &   0.509 &   1.823 &   0.509 &   0.804 \\
     30 &    0.05 &     0.1 &    10.0 &     \RBF &    10.0 &   0.531 &   1.300 &   0.509 &   1.823 &   0.509 &   0.804 \\
     30 &    0.05 &     0.1 &   100.0 &     \COS &       - &   0.691 &   1.690 &   0.664 &   2.089 &   0.606 &   0.777 \\
     30 &    0.05 &     0.1 &   100.0 &     \RBF &    10.0 &   0.628 &   1.558 &   0.603 &   2.015 &   0.569 &   0.791 \\
     30 &    0.05 &     1.0 &     0.0 &     \COS &       - &   0.531 &   1.299 &   0.509 &   1.820 &   0.509 &   0.804 \\
     30 &    0.05 &     1.0 &     0.0 &     \RBF &    10.0 &   0.531 &   1.299 &   0.509 &   1.820 &   0.509 &   0.804 \\
     30 &    0.05 &     1.0 &     1.0 &     \COS &       - &   0.531 &   1.299 &   0.509 &   1.821 &   0.509 &   0.804 \\
     30 &    0.05 &     1.0 &     1.0 &     \RBF &    10.0 &   0.531 &   1.299 &   0.509 &   1.821 &   0.509 &   0.804 \\
     30 &    0.05 &     1.0 &    10.0 &     \COS &       - &   0.531 &   1.300 &   0.509 &   1.823 &   0.509 &   0.804 \\
     30 &    0.05 &     1.0 &    10.0 &     \RBF &    10.0 &   0.531 &   1.300 &   0.509 &   1.823 &   0.509 &   0.804 \\
     30 &    0.05 &     1.0 &   100.0 &     \COS &       - &   0.600 &   1.504 &   0.577 &   1.980 &   0.551 &   0.795 \\
     30 &    0.05 &     1.0 &   100.0 &     \RBF &    10.0 &   0.546 &   1.343 &   0.523 &   1.858 &   0.517 &   0.803 \\
     30 &    0.10 &     0.1 &     0.0 &     \COS &       - &   0.522 &   1.273 &   0.501 &   1.789 &   0.501 &   0.804 \\
     30 &    0.10 &     0.1 &     0.0 &     \RBF &    10.0 &   0.522 &   1.273 &   0.501 &   1.789 &   0.501 &   0.804 \\
     30 &    0.10 &     0.1 &     1.0 &     \COS &       - &   0.522 &   1.273 &   0.501 &   1.789 &   0.501 &   0.804 \\
     30 &    0.10 &     0.1 &     1.0 &     \RBF &    10.0 &   0.522 &   1.273 &   0.501 &   1.789 &   0.501 &   0.804 \\
     30 &    0.10 &     0.1 &    10.0 &     \COS &       - &   0.521 &   1.269 &   0.501 &   1.784 &   0.501 &   0.804 \\
     30 &    0.10 &     0.1 &    10.0 &     \RBF &    10.0 &   0.521 &   1.268 &   0.501 &   1.783 &   0.501 &   0.804 \\
     30 &    0.10 &     0.1 &   100.0 &     \COS &       - &   0.642 &   1.591 &   0.616 &   2.037 &   0.578 &   0.786 \\
     30 &    0.10 &     0.1 &   100.0 &     \RBF &    10.0 &   0.560 &   1.378 &   0.537 &   1.891 &   0.527 &   0.800 \\
     30 &    0.10 &     1.0 &     0.0 &     \COS &       - &   0.521 &   1.268 &   0.500 &   1.782 &   0.500 &   0.804 \\
     30 &    0.10 &     1.0 &     0.0 &     \RBF &    10.0 &   0.521 &   1.268 &   0.500 &   1.782 &   0.500 &   0.804 \\
     30 &    0.10 &     1.0 &     1.0 &     \COS &       - &   0.521 &   1.268 &   0.500 &   1.782 &   0.500 &   0.804 \\
     30 &    0.10 &     1.0 &     1.0 &     \RBF &    10.0 &   0.521 &   1.268 &   0.500 &   1.782 &   0.500 &   0.804 \\
     30 &    0.10 &     1.0 &    10.0 &     \COS &       - &   0.521 &   1.269 &   0.501 &   1.784 &   0.501 &   0.804 \\
     30 &    0.10 &     1.0 &    10.0 &     \RBF &    10.0 &   0.521 &   1.268 &   0.501 &   1.783 &   0.501 &   0.804 \\
     30 &    0.10 &     1.0 &   100.0 &     \COS &       - &   0.561 &   1.380 &   0.538 &   1.895 &   0.527 &   0.800 \\
     30 &    0.10 &     1.0 &   100.0 &     \RBF &    10.0 &   0.527 &   1.290 &   0.505 &   1.809 &   0.505 &   0.805 \\
     30 &    0.50 &     0.1 &     0.0 &     \COS &       - &   0.648 &   1.567 &   0.622 &   1.970 &   0.586 &   0.726 \\
     30 &    0.50 &     0.1 &     0.0 &     \RBF &    10.0 &   0.648 &   1.567 &   0.622 &   1.970 &   0.586 &   0.726 \\
     30 &    0.50 &     0.1 &     1.0 &     \COS &       - &   0.648 &   1.568 &   0.622 &   1.970 &   0.586 &   0.726 \\
     30 &    0.50 &     0.1 &     1.0 &     \RBF &    10.0 &   0.648 &   1.568 &   0.622 &   1.970 &   0.586 &   0.726 \\
     30 &    0.50 &     0.1 &    10.0 &     \COS &       - &   0.652 &   1.582 &   0.626 &   1.980 &   0.589 &   0.726 \\
     30 &    0.50 &     0.1 &    10.0 &     \RBF &    10.0 &   0.651 &   1.578 &   0.625 &   1.979 &   0.589 &   0.726 \\
     30 &    0.50 &     0.1 &   100.0 &     \COS &       - &   0.685 &   1.666 &   0.660 &   2.042 &   0.611 &   0.726 \\
     30 &    0.50 &     0.1 &   100.0 &     \RBF &    10.0 &   0.681 &   1.660 &   0.655 &   2.036 &   0.609 &   0.726 \\
     30 &    0.50 &     1.0 &     0.0 &     \COS &       - &   0.628 &   1.529 &   0.604 &   1.956 &   0.573 &   0.739 \\
     30 &    0.50 &     1.0 &     0.0 &     \RBF &    10.0 &   0.628 &   1.529 &   0.604 &   1.956 &   0.573 &   0.739 \\
     30 &    0.50 &     1.0 &     1.0 &     \COS &       - &   0.627 &   1.529 &   0.603 &   1.958 &   0.572 &   0.739 \\
     30 &    0.50 &     1.0 &     1.0 &     \RBF &    10.0 &   0.627 &   1.529 &   0.603 &   1.958 &   0.572 &   0.739 \\
     30 &    0.50 &     1.0 &    10.0 &     \COS &       - &   0.624 &   1.524 &   0.599 &   1.961 &   0.569 &   0.743 \\
     30 &    0.50 &     1.0 &    10.0 &     \RBF &    10.0 &   0.623 &   1.523 &   0.598 &   1.959 &   0.568 &   0.743 \\
     30 &    0.50 &     1.0 &   100.0 &     \COS &       - &   0.659 &   1.618 &   0.633 &   2.033 &   0.599 &   0.740 \\
     30 &    0.50 &     1.0 &   100.0 &     \RBF &    10.0 &   0.647 &   1.589 &   0.622 &   2.020 &   0.589 &   0.744 \\
     30 &    1.00 &     0.1 &     0.0 &     \COS &       - &   0.525 &   1.139 &   0.511 &   1.451 &   0.594 &   0.706 \\
     30 &    1.00 &     0.1 &     0.0 &     \RBF &    10.0 &   0.525 &   1.139 &   0.511 &   1.451 &   0.594 &   0.706 \\
     30 &    1.00 &     0.1 &     1.0 &     \COS &       - &   0.538 &   1.173 &   0.522 &   1.484 &   0.598 &   0.712 \\
     30 &    1.00 &     0.1 &     1.0 &     \RBF &    10.0 &   0.537 &   1.170 &   0.521 &   1.482 &   0.598 &   0.711 \\
     30 &    1.00 &     0.1 &    10.0 &     \COS &       - &   0.629 &   1.403 &   0.607 &   1.735 &   0.641 &   0.736 \\
     30 &    1.00 &     0.1 &    10.0 &     \RBF &    10.0 &   0.621 &   1.384 &   0.599 &   1.706 &   0.639 &   0.734 \\
     30 &    1.00 &     0.1 &   100.0 &     \COS &       - &   0.672 &   1.561 &   0.647 &   1.903 &   0.664 &   0.760 \\
     30 &    1.00 &     0.1 &   100.0 &     \RBF &    10.0 &   0.676 &   1.560 &   0.651 &   1.897 &   0.668 &   0.759 \\
     30 &    1.00 &     1.0 &     0.0 &     \COS &       - &   0.528 &   1.142 &   0.513 &   1.448 &   0.595 &   0.704 \\
     30 &    1.00 &     1.0 &     0.0 &     \RBF &    10.0 &   0.528 &   1.142 &   0.513 &   1.448 &   0.595 &   0.704 \\
     30 &    1.00 &     1.0 &     1.0 &     \COS &       - &   0.537 &   1.168 &   0.522 &   1.478 &   0.599 &   0.711 \\
     30 &    1.00 &     1.0 &     1.0 &     \RBF &    10.0 &   0.536 &   1.163 &   0.520 &   1.474 &   0.599 &   0.711 \\
     30 &    1.00 &     1.0 &    10.0 &     \COS &       - &   0.627 &   1.396 &   0.605 &   1.722 &   0.640 &   0.726 \\
     30 &    1.00 &     1.0 &    10.0 &     \RBF &    10.0 &   0.620 &   1.373 &   0.598 &   1.687 &   0.639 &   0.724 \\
     30 &    1.00 &     1.0 &   100.0 &     \COS &       - &   0.675 &   1.562 &   0.651 &   1.893 &   0.666 &   0.758 \\
     30 &    1.00 &     1.0 &   100.0 &     \RBF &    10.0 &   0.676 &   1.562 &   0.652 &   1.890 &   0.665 &   0.758 \\
     50 &    0.00 &     0.1 &     0.0 &     \COS &       - &   0.666 &   1.566 &   0.634 &   1.990 &   0.628 &   0.770 \\
     50 &    0.00 &     0.1 &     0.0 &     \RBF &    10.0 &   0.666 &   1.566 &   0.634 &   1.990 &   0.628 &   0.770 \\
     50 &    0.00 &     0.1 &     1.0 &     \COS &       - &   0.643 &   1.511 &   0.611 &   1.962 &   0.621 &   0.775 \\
     50 &    0.00 &     0.1 &     1.0 &     \RBF &    10.0 &   0.643 &   1.511 &   0.611 &   1.962 &   0.621 &   0.775 \\
     50 &    0.00 &     0.1 &    10.0 &     \COS &       - &   0.589 &   1.424 &   0.561 &   1.893 &   0.601 &   0.783 \\
     50 &    0.00 &     0.1 &    10.0 &     \RBF &    10.0 &   0.599 &   1.437 &   0.570 &   1.904 &   0.602 &   0.782 \\
     50 &    0.00 &     0.1 &   100.0 &     \COS &       - &   0.746 &   1.634 &   0.713 &   1.973 &   0.658 &   0.698 \\
     50 &    0.00 &     0.1 &   100.0 &     \RBF &    10.0 &   0.749 &   1.686 &   0.717 &   2.036 &   0.660 &   0.714 \\
     50 &    0.00 &     1.0 &     0.0 &     \COS &       - &   0.473 &   1.161 &   0.460 &   1.687 &   0.557 &   0.794 \\
     50 &    0.00 &     1.0 &     0.0 &     \RBF &    10.0 &   0.473 &   1.161 &   0.460 &   1.687 &   0.557 &   0.794 \\
     50 &    0.00 &     1.0 &     1.0 &     \COS &       - &   0.473 &   1.162 &   0.460 &   1.688 &   0.557 &   0.794 \\
     50 &    0.00 &     1.0 &     1.0 &     \RBF &    10.0 &   0.473 &   1.162 &   0.460 &   1.688 &   0.557 &   0.794 \\
     50 &    0.00 &     1.0 &    10.0 &     \COS &       - &   0.435 &   1.052 &   0.426 &   1.596 &   0.535 &   0.797 \\
     50 &    0.00 &     1.0 &    10.0 &     \RBF &    10.0 &   0.438 &   1.057 &   0.428 &   1.604 &   0.535 &   0.796 \\
     50 &    0.00 &     1.0 &   100.0 &     \COS &       - &   0.740 &   1.717 &   0.709 &   2.088 &   0.654 &   0.745 \\
     50 &    0.00 &     1.0 &   100.0 &     \RBF &    10.0 &   0.710 &   1.651 &   0.676 &   2.053 &   0.644 &   0.763 \\
     50 &    0.05 &     0.1 &     0.0 &     \COS &       - &   0.433 &   1.052 &   0.426 &   1.595 &   0.539 &   0.796 \\
     50 &    0.05 &     0.1 &     0.0 &     \RBF &    10.0 &   0.433 &   1.052 &   0.426 &   1.595 &   0.539 &   0.796 \\
     50 &    0.05 &     0.1 &     1.0 &     \COS &       - &   0.434 &   1.053 &   0.426 &   1.596 &   0.539 &   0.796 \\
     50 &    0.05 &     0.1 &     1.0 &     \RBF &    10.0 &   0.434 &   1.053 &   0.426 &   1.595 &   0.539 &   0.796 \\
     50 &    0.05 &     0.1 &    10.0 &     \COS &       - &   0.415 &   0.993 &   0.409 &   1.524 &   0.524 &   0.797 \\
     50 &    0.05 &     0.1 &    10.0 &     \RBF &    10.0 &   0.417 &   1.001 &   0.410 &   1.534 &   0.525 &   0.797 \\
     50 &    0.05 &     0.1 &   100.0 &     \COS &       - &   0.753 &   1.713 &   0.722 &   2.061 &   0.666 &   0.715 \\
     50 &    0.05 &     0.1 &   100.0 &     \RBF &    10.0 &   0.729 &   1.711 &   0.698 &   2.088 &   0.658 &   0.747 \\
     50 &    0.05 &     1.0 &     0.0 &     \COS &       - &   0.406 &   0.965 &   0.400 &   1.491 &   0.522 &   0.798 \\
     50 &    0.05 &     1.0 &     0.0 &     \RBF &    10.0 &   0.406 &   0.965 &   0.400 &   1.491 &   0.522 &   0.798 \\
     50 &    0.05 &     1.0 &     1.0 &     \COS &       - &   0.406 &   0.965 &   0.400 &   1.491 &   0.522 &   0.798 \\
     50 &    0.05 &     1.0 &     1.0 &     \RBF &    10.0 &   0.406 &   0.965 &   0.400 &   1.491 &   0.522 &   0.798 \\
     50 &    0.05 &     1.0 &    10.0 &     \COS &       - &   0.404 &   0.960 &   0.398 &   1.489 &   0.521 &   0.798 \\
     50 &    0.05 &     1.0 &    10.0 &     \RBF &    10.0 &   0.404 &   0.960 &   0.398 &   1.488 &   0.521 &   0.798 \\
     50 &    0.05 &     1.0 &   100.0 &     \COS &       - &   0.706 &   1.655 &   0.673 &   2.065 &   0.645 &   0.760 \\
     50 &    0.05 &     1.0 &   100.0 &     \RBF &    10.0 &   0.617 &   1.476 &   0.588 &   1.938 &   0.615 &   0.781 \\
     50 &    0.10 &     0.1 &     0.0 &     \COS &       - &   0.424 &   1.023 &   0.416 &   1.554 &   0.531 &   0.796 \\
     50 &    0.10 &     0.1 &     0.0 &     \RBF &    10.0 &   0.424 &   1.023 &   0.416 &   1.554 &   0.531 &   0.796 \\
     50 &    0.10 &     0.1 &     1.0 &     \COS &       - &   0.423 &   1.018 &   0.415 &   1.548 &   0.531 &   0.796 \\
     50 &    0.10 &     0.1 &     1.0 &     \RBF &    10.0 &   0.423 &   1.018 &   0.415 &   1.548 &   0.531 &   0.796 \\
     50 &    0.10 &     0.1 &    10.0 &     \COS &       - &   0.404 &   0.959 &   0.399 &   1.484 &   0.523 &   0.797 \\
     50 &    0.10 &     0.1 &    10.0 &     \RBF &    10.0 &   0.406 &   0.963 &   0.400 &   1.490 &   0.524 &   0.797 \\
     50 &    0.10 &     0.1 &   100.0 &     \COS &       - &   0.757 &   1.720 &   0.727 &   2.059 &   0.673 &   0.707 \\
     50 &    0.10 &     0.1 &   100.0 &     \RBF &    10.0 &   0.746 &   1.724 &   0.716 &   2.080 &   0.668 &   0.727 \\
     50 &    0.10 &     1.0 &     0.0 &     \COS &       - &   0.397 &   0.933 &   0.392 &   1.451 &   0.521 &   0.798 \\
     50 &    0.10 &     1.0 &     0.0 &     \RBF &    10.0 &   0.397 &   0.933 &   0.392 &   1.451 &   0.521 &   0.798 \\
     50 &    0.10 &     1.0 &     1.0 &     \COS &       - &   0.397 &   0.933 &   0.392 &   1.451 &   0.521 &   0.798 \\
     50 &    0.10 &     1.0 &     1.0 &     \RBF &    10.0 &   0.397 &   0.933 &   0.392 &   1.451 &   0.521 &   0.798 \\
     50 &    0.10 &     1.0 &    10.0 &     \COS &       - &   0.396 &   0.931 &   0.391 &   1.448 &   0.520 &   0.798 \\
     50 &    0.10 &     1.0 &    10.0 &     \RBF &    10.0 &   0.396 &   0.930 &   0.391 &   1.447 &   0.520 &   0.798 \\
     50 &    0.10 &     1.0 &   100.0 &     \COS &       - &   0.700 &   1.664 &   0.670 &   2.069 &   0.649 &   0.757 \\
     50 &    0.10 &     1.0 &   100.0 &     \RBF &    10.0 &   0.601 &   1.458 &   0.573 &   1.931 &   0.608 &   0.781 \\
     50 &    0.50 &     0.1 &     0.0 &     \COS &       - &   0.604 &   1.466 &   0.583 &   1.893 &   0.622 &   0.731 \\
     50 &    0.50 &     0.1 &     0.0 &     \RBF &    10.0 &   0.604 &   1.466 &   0.583 &   1.893 &   0.622 &   0.731 \\
     50 &    0.50 &     0.1 &     1.0 &     \COS &       - &   0.605 &   1.468 &   0.583 &   1.894 &   0.622 &   0.731 \\
     50 &    0.50 &     0.1 &     1.0 &     \RBF &    10.0 &   0.604 &   1.467 &   0.583 &   1.894 &   0.622 &   0.731 \\
     50 &    0.50 &     0.1 &    10.0 &     \COS &       - &   0.611 &   1.484 &   0.588 &   1.912 &   0.625 &   0.731 \\
     50 &    0.50 &     0.1 &    10.0 &     \RBF &    10.0 &   0.610 &   1.482 &   0.588 &   1.909 &   0.625 &   0.731 \\
     50 &    0.50 &     0.1 &   100.0 &     \COS &       - &   0.665 &   1.611 &   0.642 &   2.014 &   0.646 &   0.734 \\
     50 &    0.50 &     0.1 &   100.0 &     \RBF &    10.0 &   0.658 &   1.596 &   0.634 &   2.005 &   0.643 &   0.734 \\
     50 &    0.50 &     1.0 &     0.0 &     \COS &       - &   0.579 &   1.417 &   0.558 &   1.868 &   0.615 &   0.740 \\
     50 &    0.50 &     1.0 &     0.0 &     \RBF &    10.0 &   0.579 &   1.417 &   0.558 &   1.868 &   0.615 &   0.740 \\
     50 &    0.50 &     1.0 &     1.0 &     \COS &       - &   0.577 &   1.411 &   0.556 &   1.865 &   0.615 &   0.741 \\
     50 &    0.50 &     1.0 &     1.0 &     \RBF &    10.0 &   0.578 &   1.414 &   0.558 &   1.868 &   0.615 &   0.740 \\
     50 &    0.50 &     1.0 &    10.0 &     \COS &       - &   0.565 &   1.375 &   0.542 &   1.855 &   0.609 &   0.748 \\
     50 &    0.50 &     1.0 &    10.0 &     \RBF &    10.0 &   0.567 &   1.384 &   0.545 &   1.856 &   0.611 &   0.747 \\
     50 &    0.50 &     1.0 &   100.0 &     \COS &       - &   0.649 &   1.589 &   0.625 &   2.000 &   0.642 &   0.740 \\
     50 &    0.50 &     1.0 &   100.0 &     \RBF &    10.0 &   0.622 &   1.524 &   0.597 &   1.968 &   0.630 &   0.746 \\
     50 &    1.00 &     0.1 &     0.0 &     \COS &       - &   0.512 &   1.034 &   0.501 &   1.287 &   0.628 &   0.706 \\
     50 &    1.00 &     0.1 &     0.0 &     \RBF &    10.0 &   0.512 &   1.034 &   0.501 &   1.287 &   0.628 &   0.706 \\
     50 &    1.00 &     0.1 &     1.0 &     \COS &       - &   0.530 &   1.071 &   0.516 &   1.331 &   0.631 &   0.715 \\
     50 &    1.00 &     0.1 &     1.0 &     \RBF &    10.0 &   0.528 &   1.066 &   0.514 &   1.326 &   0.631 &   0.714 \\
     50 &    1.00 &     0.1 &    10.0 &     \COS &       - &   0.650 &   1.420 &   0.626 &   1.724 &   0.665 &   0.750 \\
     50 &    1.00 &     0.1 &    10.0 &     \RBF &    10.0 &   0.641 &   1.384 &   0.617 &   1.686 &   0.664 &   0.748 \\
     50 &    1.00 &     0.1 &   100.0 &     \COS &       - &   0.687 &   1.612 &   0.664 &   1.941 &   0.679 &   0.770 \\
     50 &    1.00 &     0.1 &   100.0 &     \RBF &    10.0 &   0.689 &   1.609 &   0.664 &   1.940 &   0.679 &   0.772 \\
     50 &    1.00 &     1.0 &     0.0 &     \COS &       - &   0.515 &   1.034 &   0.503 &   1.284 &   0.627 &   0.706 \\
     50 &    1.00 &     1.0 &     0.0 &     \RBF &    10.0 &   0.515 &   1.034 &   0.503 &   1.284 &   0.627 &   0.706 \\
     50 &    1.00 &     1.0 &     1.0 &     \COS &       - &   0.527 &   1.063 &   0.514 &   1.322 &   0.632 &   0.713 \\
     50 &    1.00 &     1.0 &     1.0 &     \RBF &    10.0 &   0.525 &   1.059 &   0.512 &   1.319 &   0.631 &   0.713 \\
     50 &    1.00 &     1.0 &    10.0 &     \COS &       - &   0.649 &   1.403 &   0.625 &   1.703 &   0.664 &   0.741 \\
     50 &    1.00 &     1.0 &    10.0 &     \RBF &    10.0 &   0.639 &   1.377 &   0.615 &   1.667 &   0.662 &   0.738 \\
     50 &    1.00 &     1.0 &   100.0 &     \COS &       - &   0.686 &   1.606 &   0.663 &   1.938 &   0.680 &   0.770 \\
     50 &    1.00 &     1.0 &   100.0 &     \RBF &    10.0 &   0.688 &   1.603 &   0.663 &   1.932 &   0.680 &   0.769 \\


==> tables/unknown_5percent.tex <==
\begin{ThreePartTable}
    \begin{TableNotes}[flushleft]  %%% This should come before longtable and it is not tablenotes but TableNotes
  \small
  \item
    \begin{footnotesize}
        \bgroup
%        \def\arraystretch{0.5}%       
        \setstretch{1}
		The columns corresponding to ``$l$'', ``$\alpha$'',
                ``$\beta$'', ``$\gamma$'', ``usim'', and ``$\sigma$'' have the
                latent dimension, weighting factor,
                latent vector regularization parameter,
                cell line similarity regularization parameter,
                cell line similarity function, and parameter for rbf cell line similarity,
                respectively, for \MTCRP.
	      \par
              \egroup
    \end{footnotesize}
  \end{TableNotes}
  \begin{longtable}{
      @{\hspace{0pt}}>{\raggedleft}p{0.05\textwidth}@{\hspace{5pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.05\textwidth}@{\hspace{5pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.05\textwidth}@{\hspace{5pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.07\textwidth}@{\hspace{5pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.05\textwidth}@{\hspace{5pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.05\textwidth}@{\hspace{5pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.08\textwidth}@{\hspace{0pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.08\textwidth}@{\hspace{0pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.08\textwidth}@{\hspace{0pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.08\textwidth}@{\hspace{0pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.08\textwidth}@{\hspace{0pt}}
      @{\hspace{0pt}}>{\raggedleft\arraybackslash}p{0.08\textwidth}@{\hspace{0pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
    }
    \caption{\mbox{\MTCRP Performance on New Drugs ($\theta$ = 5)}}
    \label{supp:tbl:overall:5percent}\\
  %
    \hline\hline
    $l$ & $\alpha$ & $\beta$ & $\gamma$ & usim & $\sigma$ & \small{AP@$5$} & \small{AH@$5$} & \small{AP@$10$} & \small{AH@$10$} & \small{\rCI} & \small{\CI} \\
    \hline
    \endfirsthead
  %
    \multicolumn{12}{c}{{\tablename\ \thetable{} -- continued from previous page}}\\
    \hline\hline
    $l$ & $\alpha$ & $\beta$ & $\gamma$ & usim & $\sigma$ & \small{AP@$5$} & \small{AH@$5$} & \small{AP@$10$} & \small{AH@$10$} & \small{\rCI} & \small{\CI} \\
    \hline
    \endhead
  %
    \hline
    %  \midrule
    \multicolumn{12}{c}{{Continued on next page}} \\
    \hline
    %\midrule
    \endfoot
    %
    \hline\hline
    %\bottomrule
    \insertTableNotes         %% this added
    \endlastfoot
    %
    \input{tables/unknown_5percent_data.tex}
	
    \hline
  \end{longtable}
\end{ThreePartTable}


==> tables/unknown_5percent_KRL.tex <==
\begin{ThreePartTable}
    \begin{TableNotes}[flushleft]  %%% This should come before longtable and it is not tablenotes but TableNotes
  \small
  \item
    \begin{footnotesize}
        \bgroup
%        \def\arraystretch{0.5}%       
        \setstretch{1}
                The columns corresponding to ``$k$'', ``$\lambda$'',
                ``usim'', and ``$\sigma$'' have the
                two hyperparameters, cell line similarity function,
                and parameter for {$\RBF$} cell line similarity, respectively, 
                for {\KRL}.
	      \par
              \egroup
    \end{footnotesize}
  \end{TableNotes}
  \begin{longtable}{
      @{\hspace{0pt}}>{\raggedleft}p{0.07\textwidth}@{\hspace{5pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.07\textwidth}@{\hspace{5pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.07\textwidth}@{\hspace{5pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.07\textwidth}@{\hspace{5pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{0pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{0pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{0pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{0pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{0pt}}
      @{\hspace{0pt}}>{\raggedleft\arraybackslash}p{0.08\textwidth}@{\hspace{0pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
    }
    \caption{\mbox{\KRL Performance on New Drugs ($\theta$ = 5)}}
    \label{supp:tbl:overall:5percent:KRL}\\
  %
    \hline\hline
    $k$ & $\lambda$ & usim & $\sigma$ & \small{AP@$5$} & \small{AH@$5$} & \small{AP@$10$} & \small{AH@$10$} & \small{\rCI} & \small{\CI} \\
    \hline
    \endfirsthead
  %
    \multicolumn{10}{c}{{\tablename\ \thetable{} -- continued from previous page}}\\
    \hline\hline
    $k$ & $\lambda$ & usim & $\sigma$ & \small{AP@$5$} & \small{AH@$5$} & \small{AP@$10$} & \small{AH@$10$} & \small{\rCI} & \small{\CI} \\
    \hline
    \endhead
  %
    \hline
    %  \midrule
    \multicolumn{10}{c}{{Continued on next page}} \\
    \hline
    %\midrule
    \endfoot
    %
    \hline\hline
    %\bottomrule
    \insertTableNotes         %% this added
    \endlastfoot
    %
    \input{tables/unknown_5percent_KRL_data.tex}
	
    \hline
  \end{longtable}
\end{ThreePartTable}


==> tables/unknown_5percent_KRL_data.tex <==
10	&   0.000001	&       \LIN	&          -	& 0.665	& 2.088	& 0.615	& 3.214	& 0.657	& 0.722 \\
10	&   0.000001	&       \RBF	&     0.0001	& 0.805	& 2.627	& 0.746	& 3.733	& 0.675	& 0.760 \\
10	&   0.000001	&       \RBF	&      0.001	& 0.817	& 2.715	& 0.761	& 3.798	& 0.676	& 0.762 \\
10	&   0.000001	&       \RBF	&       0.01	& 0.735	& 2.321	& 0.684	& 3.256	& 0.635	& 0.637 \\
10	&    0.00001	&       \LIN	&          -	& 0.769	& 2.440	& 0.708	& 3.528	& 0.683	& 0.739 \\
10	&    0.00001	&       \RBF	&     0.0001	& 0.796	& 2.547	& 0.736	& 3.560	& 0.660	& 0.768 \\
10	&    0.00001	&       \RBF	&      0.001	& 0.817	& 2.715	& 0.761	& 3.798	& 0.676	& 0.762 \\
10	&    0.00001	&       \RBF	&       0.01	& 0.713	& 2.224	& 0.666	& 3.078	& 0.625	& 0.624 \\
10	&     0.0001	&       \LIN	&          -	& 0.789	& 2.580	& 0.730	& 3.690	& 0.689	& 0.756 \\
10	&     0.0001	&       \RBF	&     0.0001	& 0.796	& 2.547	& 0.736	& 3.560	& 0.660	& 0.768 \\
10	&     0.0001	&       \RBF	&      0.001	& 0.817	& 2.715	& 0.761	& 3.798	& 0.676	& 0.762 \\
10	&     0.0001	&       \RBF	&       0.01	& 0.674	& 2.046	& 0.633	& 2.804	& 0.608	& 0.606 \\
10	&      0.001	&       \LIN	&          -	& 0.785	& 2.521	& 0.722	& 3.618	& 0.676	& 0.714 \\
10	&      0.001	&       \RBF	&     0.0001	& 0.796	& 2.547	& 0.736	& 3.560	& 0.660	& 0.768 \\
10	&      0.001	&       \RBF	&      0.001	& 0.817	& 2.715	& 0.761	& 3.798	& 0.676	& 0.762 \\
10	&      0.001	&       \RBF	&       0.01	& 0.608	& 1.781	& 0.577	& 2.382	& 0.589	& 0.585 \\
10	&       0.01	&       \LIN	&          -	& 0.792	& 2.570	& 0.731	& 3.668	& 0.679	& 0.716 \\
10	&       0.01	&       \RBF	&     0.0001	& 0.796	& 2.547	& 0.736	& 3.560	& 0.660	& 0.768 \\
10	&       0.01	&       \RBF	&      0.001	& 0.817	& 2.715	& 0.761	& 3.798	& 0.676	& 0.762 \\
10	&       0.01	&       \RBF	&       0.01	& 0.512	& 1.436	& 0.494	& 1.905	& 0.566	& 0.565 \\
10	&        0.1	&       \LIN	&          -	& 0.799	& 2.556	& 0.736	& 3.663	& 0.676	& 0.662 \\
10	&        0.1	&       \RBF	&     0.0001	& 0.796	& 2.547	& 0.736	& 3.560	& 0.660	& 0.768 \\
10	&        0.1	&       \RBF	&      0.001	& 0.817	& 2.715	& 0.761	& 3.798	& 0.676	& 0.762 \\
10	&        0.1	&       \RBF	&       0.01	& 0.418	& 1.093	& 0.410	& 1.444	& 0.538	& 0.549 \\
10	&        0.2	&       \LIN	&          -	& 0.800	& 2.593	& 0.739	& 3.701	& 0.673	& 0.738 \\
10	&        0.2	&       \RBF	&     0.0001	& 0.796	& 2.547	& 0.736	& 3.560	& 0.660	& 0.768 \\
10	&        0.2	&       \RBF	&      0.001	& 0.817	& 2.715	& 0.761	& 3.798	& 0.676	& 0.762 \\
10	&        0.2	&       \RBF	&       0.01	& 0.386	& 0.987	& 0.380	& 1.317	& 0.531	& 0.545 \\
10	&        0.4	&       \LIN	&          -	& 0.797	& 2.556	& 0.735	& 3.619	& 0.663	& 0.743 \\
10	&        0.4	&       \RBF	&     0.0001	& 0.796	& 2.547	& 0.736	& 3.560	& 0.660	& 0.768 \\
10	&        0.4	&       \RBF	&      0.001	& 0.817	& 2.715	& 0.761	& 3.798	& 0.676	& 0.762 \\
10	&        0.4	&       \RBF	&       0.01	& 0.351	& 0.888	& 0.349	& 1.180	& 0.524	& 0.541 \\
10	&        0.6	&       \LIN	&          -	& 0.794	& 2.535	& 0.735	& 3.529	& 0.658	& 0.738 \\
10	&        0.6	&       \RBF	&     0.0001	& 0.796	& 2.547	& 0.736	& 3.560	& 0.660	& 0.768 \\
10	&        0.6	&       \RBF	&      0.001	& 0.817	& 2.715	& 0.761	& 3.798	& 0.676	& 0.762 \\
10	&        0.6	&       \RBF	&       0.01	& 0.332	& 0.834	& 0.332	& 1.120	& 0.520	& 0.539 \\
10	&        0.8	&       \LIN	&          -	& 0.794	& 2.535	& 0.735	& 3.529	& 0.658	& 0.738 \\
10	&        0.8	&       \RBF	&     0.0001	& 0.796	& 2.547	& 0.736	& 3.560	& 0.660	& 0.768 \\
10	&        0.8	&       \RBF	&      0.001	& 0.817	& 2.715	& 0.761	& 3.798	& 0.676	& 0.762 \\
10	&        0.8	&       \RBF	&       0.01	& 0.320	& 0.802	& 0.321	& 1.078	& 0.518	& 0.538 \\
10	&        1.0	&       \LIN	&          -	& 0.794	& 2.535	& 0.735	& 3.529	& 0.658	& 0.738 \\
10	&        1.0	&       \RBF	&     0.0001	& 0.796	& 2.547	& 0.736	& 3.560	& 0.660	& 0.768 \\
10	&        1.0	&       \RBF	&      0.001	& 0.817	& 2.715	& 0.761	& 3.798	& 0.676	& 0.762 \\
10	&        1.0	&       \RBF	&       0.01	& 0.310	& 0.773	& 0.311	& 1.052	& 0.517	& 0.537 \\
10	&         10	&       \LIN	&          -	& 0.794	& 2.535	& 0.735	& 3.529	& 0.658	& 0.738 \\
10	&         10	&       \RBF	&     0.0001	& 0.796	& 2.547	& 0.736	& 3.560	& 0.660	& 0.768 \\
10	&         10	&       \RBF	&      0.001	& 0.817	& 2.715	& 0.761	& 3.798	& 0.676	& 0.762 \\
10	&         10	&       \RBF	&       0.01	& 0.246	& 0.595	& 0.250	& 0.853	& 0.503	& 0.532 \\
10	&         50	&       \LIN	&          -	& 0.794	& 2.535	& 0.735	& 3.529	& 0.658	& 0.738 \\
10	&         50	&       \RBF	&     0.0001	& 0.796	& 2.547	& 0.736	& 3.560	& 0.660	& 0.768 \\
10	&         50	&       \RBF	&      0.001	& 0.817	& 2.715	& 0.761	& 3.798	& 0.676	& 0.762 \\
10	&         50	&       \RBF	&       0.01	& 0.223	& 0.538	& 0.231	& 0.788	& 0.497	& 0.530 \\
10	&        100	&       \LIN	&          -	& 0.794	& 2.535	& 0.735	& 3.529	& 0.658	& 0.738 \\
10	&        100	&       \RBF	&     0.0001	& 0.796	& 2.547	& 0.736	& 3.560	& 0.660	& 0.768 \\
10	&        100	&       \RBF	&      0.001	& 0.817	& 2.715	& 0.761	& 3.798	& 0.676	& 0.762 \\
10	&        100	&       \RBF	&       0.01	& 0.216	& 0.522	& 0.224	& 0.773	& 0.497	& 0.529 \\


==> tables/unknown_5percent_baseline.tex <==
\begin{ThreePartTable}
    \begin{TableNotes}[flushleft]  %%% This should come before longtable and it is not tablenotes but TableNotes
  \small
  \item
    \begin{footnotesize}
        \bgroup
%        \def\arraystretch{0.5}%       
        \setstretch{1}
                The columns corresponding to ``$\alpha_b$'', ``$\beta_b$'',
                ``usim'', and ``$\sigma$'' have the
                two hyperparameters, cell line similarity function,
                and parameter for \hl{$\RBF$} cell line similarity, respectively, for \BMTMKL.
	      \par
              \egroup
    \end{footnotesize}
  \end{TableNotes}
  \begin{longtable}{
      @{\hspace{0pt}}>{\raggedleft}p{0.07\textwidth}@{\hspace{5pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.07\textwidth}@{\hspace{5pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.07\textwidth}@{\hspace{5pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.07\textwidth}@{\hspace{5pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{0pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{0pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{0pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{0pt}}
      @{\hspace{0pt}}>{\raggedleft}p{0.10\textwidth}@{\hspace{0pt}}
      @{\hspace{0pt}}>{\raggedleft\arraybackslash}p{0.08\textwidth}@{\hspace{0pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
%      @{\hspace{0pt}}c@{\hspace{5pt}}
    }
    \caption{\mbox{\BMTMKL Performance on New Drugs ($\theta$ = 5)}}
    \label{supp:tbl:overall:5percent:baseline}\\
  %
    \hline\hline
    $\alpha_b$ & $\beta_b$ & usim & $\sigma$ & \small{AP@$5$} & \small{AH@$5$} & \small{AP@$10$} & \small{AH@$10$} & \small{\rCI} & \small{\CI} \\
    \hline
    \endfirsthead
  %
    \multicolumn{10}{c}{{\tablename\ \thetable{} -- continued from previous page}}\\
    \hline\hline
    $\alpha_b$ & $\beta_b$ & usim & $\sigma$ & \small{AP@$5$} & \small{AH@$5$} & \small{AP@$10$} & \small{AH@$10$} & \small{\rCI} & \small{\CI} \\
    \hline
    \endhead
  %
    \hline
    %  \midrule
    \multicolumn{10}{c}{{Continued on next page}} \\
    \hline
    %\midrule
    \endfoot
    %
    \hline\hline
    %\bottomrule
    \insertTableNotes         %% this added
    \endlastfoot
    %
    \input{tables/unknown_5percent_baseline_data.tex}
	
    \hline
  \end{longtable}
\end{ThreePartTable}


==> tables/unknown_5percent_baseline_data.tex <==
1     &  1      & \RBF  & 10.0 &  0.827 &  2.735 &  0.772 &  3.760 &  0.653 &  0.812  \\ 
1e-10 &  1e-10  & \RBF  & 10.0 &  0.826 &  2.734 &  0.771 &  3.757 &  0.652 &  0.811  \\ 
1e-10 &  1e10   & \RBF  & 10.0 &  0.828 &  2.736 &  0.772 &  3.761 &  0.652 &  0.812  \\ 
1     &  1      & \COS  & -    &  0.815 &  2.650 &  0.757 &  3.690 &  0.648 &  0.808  \\ 
1e-10 &  1e-10  & \COS  & -    &  0.817 &  2.647 &  0.759 &  3.670 &  0.646 &  0.807  \\ 
1e-10 &  1e10   & \COS  & -    &  0.815 &  2.661 &  0.758 &  3.693 &  0.649 &  0.808  \\ 


==> tables/unknown_5percent_data.tex <==
      5 &    0.00 &     0.1 &     0.0 &     \COS &       - &   0.842 &   2.858 &   0.789 &   3.897 &   0.665 &   0.769 \\
      5 &    0.00 &     0.1 &     0.0 &     \RBF &    10.0 &   0.842 &   2.858 &   0.789 &   3.897 &   0.665 &   0.769 \\
      5 &    0.00 &     0.1 &     1.0 &     \COS &       - &   0.842 &   2.858 &   0.789 &   3.897 &   0.665 &   0.769 \\
      5 &    0.00 &     0.1 &     1.0 &     \RBF &    10.0 &   0.842 &   2.858 &   0.789 &   3.897 &   0.665 &   0.769 \\
      5 &    0.00 &     0.1 &    10.0 &     \COS &       - &   0.842 &   2.858 &   0.789 &   3.897 &   0.665 &   0.769 \\
      5 &    0.00 &     0.1 &    10.0 &     \RBF &    10.0 &   0.842 &   2.858 &   0.789 &   3.897 &   0.665 &   0.769 \\
      5 &    0.00 &     0.1 &   100.0 &     \COS &       - &   0.841 &   2.857 &   0.789 &   3.896 &   0.665 &   0.768 \\
      5 &    0.00 &     0.1 &   100.0 &     \RBF &    10.0 &   0.842 &   2.857 &   0.789 &   3.896 &   0.665 &   0.769 \\
      5 &    0.00 &     1.0 &     0.0 &     \COS &       - &   0.842 &   2.858 &   0.789 &   3.897 &   0.665 &   0.769 \\
      5 &    0.00 &     1.0 &     0.0 &     \RBF &    10.0 &   0.842 &   2.858 &   0.789 &   3.897 &   0.665 &   0.769 \\
      5 &    0.00 &     1.0 &     1.0 &     \COS &       - &   0.842 &   2.858 &   0.789 &   3.897 &   0.665 &   0.769 \\
      5 &    0.00 &     1.0 &     1.0 &     \RBF &    10.0 &   0.842 &   2.858 &   0.789 &   3.897 &   0.665 &   0.769 \\
      5 &    0.00 &     1.0 &    10.0 &     \COS &       - &   0.842 &   2.858 &   0.789 &   3.897 &   0.665 &   0.769 \\
      5 &    0.00 &     1.0 &    10.0 &     \RBF &    10.0 &   0.842 &   2.858 &   0.789 &   3.897 &   0.665 &   0.769 \\
      5 &    0.00 &     1.0 &   100.0 &     \COS &       - &   0.841 &   2.857 &   0.789 &   3.896 &   0.665 &   0.768 \\
      5 &    0.00 &     1.0 &   100.0 &     \RBF &    10.0 &   0.842 &   2.857 &   0.789 &   3.896 &   0.665 &   0.769 \\
      5 &    0.05 &     0.1 &     0.0 &     \COS &       - &   0.843 &   2.863 &   0.789 &   3.900 &   0.665 &   0.771 \\
      5 &    0.05 &     0.1 &     0.0 &     \RBF &    10.0 &   0.843 &   2.863 &   0.789 &   3.900 &   0.665 &   0.771 \\
      5 &    0.05 &     0.1 &     1.0 &     \COS &       - &   0.843 &   2.863 &   0.789 &   3.900 &   0.665 &   0.771 \\
      5 &    0.05 &     0.1 &     1.0 &     \RBF &    10.0 &   0.843 &   2.863 &   0.789 &   3.900 &   0.665 &   0.771 \\
      5 &    0.05 &     0.1 &    10.0 &     \COS &       - &   0.843 &   2.861 &   0.789 &   3.900 &   0.665 &   0.771 \\
      5 &    0.05 &     0.1 &    10.0 &     \RBF &    10.0 &   0.843 &   2.862 &   0.789 &   3.900 &   0.665 &   0.771 \\
      5 &    0.05 &     0.1 &   100.0 &     \COS &       - &   0.842 &   2.860 &   0.789 &   3.900 &   0.665 &   0.770 \\
      5 &    0.05 &     0.1 &   100.0 &     \RBF &    10.0 &   0.843 &   2.860 &   0.789 &   3.899 &   0.665 &   0.770 \\
      5 &    0.05 &     1.0 &     0.0 &     \COS &       - &   0.843 &   2.863 &   0.789 &   3.900 &   0.665 &   0.771 \\
      5 &    0.05 &     1.0 &     0.0 &     \RBF &    10.0 &   0.843 &   2.863 &   0.789 &   3.900 &   0.665 &   0.771 \\
      5 &    0.05 &     1.0 &     1.0 &     \COS &       - &   0.843 &   2.862 &   0.789 &   3.900 &   0.665 &   0.771 \\
      5 &    0.05 &     1.0 &     1.0 &     \RBF &    10.0 &   0.843 &   2.862 &   0.789 &   3.900 &   0.665 &   0.771 \\
      5 &    0.05 &     1.0 &    10.0 &     \COS &       - &   0.843 &   2.861 &   0.789 &   3.900 &   0.665 &   0.771 \\
      5 &    0.05 &     1.0 &    10.0 &     \RBF &    10.0 &   0.843 &   2.861 &   0.789 &   3.900 &   0.665 &   0.771 \\
      5 &    0.05 &     1.0 &   100.0 &     \COS &       - &   0.842 &   2.860 &   0.789 &   3.900 &   0.665 &   0.770 \\
      5 &    0.05 &     1.0 &   100.0 &     \RBF &    10.0 &   0.843 &   2.860 &   0.789 &   3.899 &   0.665 &   0.770 \\
      5 &    0.10 &     0.1 &     0.0 &     \COS &       - &   0.843 &   2.867 &   0.790 &   3.901 &   0.665 &   0.773 \\
      5 &    0.10 &     0.1 &     0.0 &     \RBF &    10.0 &   0.843 &   2.867 &   0.790 &   3.901 &   0.665 &   0.773 \\
      5 &    0.10 &     0.1 &     1.0 &     \COS &       - &   0.843 &   2.867 &   0.790 &   3.901 &   0.665 &   0.773 \\
      5 &    0.10 &     0.1 &     1.0 &     \RBF &    10.0 &   0.843 &   2.867 &   0.790 &   3.901 &   0.665 &   0.773 \\
      5 &    0.10 &     0.1 &    10.0 &     \COS &       - &   0.843 &   2.867 &   0.790 &   3.901 &   0.665 &   0.773 \\
      5 &    0.10 &     0.1 &    10.0 &     \RBF &    10.0 &   0.843 &   2.867 &   0.790 &   3.901 &   0.665 &   0.773 \\
      5 &    0.10 &     0.1 &   100.0 &     \COS &       - &   0.842 &   2.864 &   0.789 &   3.902 &   0.665 &   0.772 \\
      5 &    0.10 &     0.1 &   100.0 &     \RBF &    10.0 &   0.843 &   2.865 &   0.789 &   3.902 &   0.665 &   0.772 \\
      5 &    0.10 &     1.0 &     0.0 &     \COS &       - &   0.843 &   2.867 &   0.790 &   3.901 &   0.665 &   0.773 \\
      5 &    0.10 &     1.0 &     0.0 &     \RBF &    10.0 &   0.843 &   2.867 &   0.790 &   3.901 &   0.665 &   0.773 \\
      5 &    0.10 &     1.0 &     1.0 &     \COS &       - &   0.843 &   2.867 &   0.790 &   3.901 &   0.665 &   0.773 \\
      5 &    0.10 &     1.0 &     1.0 &     \RBF &    10.0 &   0.843 &   2.867 &   0.790 &   3.901 &   0.665 &   0.773 \\
      5 &    0.10 &     1.0 &    10.0 &     \COS &       - &   0.843 &   2.867 &   0.790 &   3.901 &   0.665 &   0.773 \\
      5 &    0.10 &     1.0 &    10.0 &     \RBF &    10.0 &   0.843 &   2.867 &   0.790 &   3.901 &   0.665 &   0.773 \\
      5 &    0.10 &     1.0 &   100.0 &     \COS &       - &   0.843 &   2.864 &   0.789 &   3.902 &   0.665 &   0.772 \\
      5 &    0.10 &     1.0 &   100.0 &     \RBF &    10.0 &   0.843 &   2.865 &   0.789 &   3.902 &   0.665 &   0.772 \\
      5 &    0.50 &     0.1 &     0.0 &     \COS &       - &   0.845 &   2.880 &   0.792 &   3.923 &   0.668 &   0.789 \\
      5 &    0.50 &     0.1 &     0.0 &     \RBF &    10.0 &   0.845 &   2.880 &   0.792 &   3.923 &   0.668 &   0.789 \\
      5 &    0.50 &     0.1 &     1.0 &     \COS &       - &   0.845 &   2.880 &   0.792 &   3.923 &   0.668 &   0.789 \\
      5 &    0.50 &     0.1 &     1.0 &     \RBF &    10.0 &   0.845 &   2.880 &   0.792 &   3.923 &   0.668 &   0.789 \\
      5 &    0.50 &     0.1 &    10.0 &     \COS &       - &   0.845 &   2.880 &   0.792 &   3.923 &   0.668 &   0.789 \\
      5 &    0.50 &     0.1 &    10.0 &     \RBF &    10.0 &   0.845 &   2.880 &   0.792 &   3.923 &   0.668 &   0.789 \\
      5 &    0.50 &     0.1 &   100.0 &     \COS &       - &   0.845 &   2.879 &   0.792 &   3.920 &   0.669 &   0.789 \\
      5 &    0.50 &     0.1 &   100.0 &     \RBF &    10.0 &   0.845 &   2.879 &   0.792 &   3.921 &   0.668 &   0.789 \\
      5 &    0.50 &     1.0 &     0.0 &     \COS &       - &   0.845 &   2.880 &   0.792 &   3.923 &   0.668 &   0.789 \\
      5 &    0.50 &     1.0 &     0.0 &     \RBF &    10.0 &   0.845 &   2.880 &   0.792 &   3.923 &   0.668 &   0.789 \\
      5 &    0.50 &     1.0 &     1.0 &     \COS &       - &   0.845 &   2.880 &   0.792 &   3.923 &   0.668 &   0.789 \\
      5 &    0.50 &     1.0 &     1.0 &     \RBF &    10.0 &   0.845 &   2.880 &   0.792 &   3.923 &   0.668 &   0.789 \\
      5 &    0.50 &     1.0 &    10.0 &     \COS &       - &   0.845 &   2.880 &   0.792 &   3.923 &   0.669 &   0.789 \\
      5 &    0.50 &     1.0 &    10.0 &     \RBF &    10.0 &   0.845 &   2.880 &   0.792 &   3.923 &   0.668 &   0.789 \\
      5 &    0.50 &     1.0 &   100.0 &     \COS &       - &   0.845 &   2.879 &   0.792 &   3.920 &   0.668 &   0.789 \\
      5 &    0.50 &     1.0 &   100.0 &     \RBF &    10.0 &   0.845 &   2.879 &   0.792 &   3.920 &   0.668 &   0.789 \\
      5 &    1.00 &     0.1 &     0.0 &     \COS &       - &   0.689 &   2.080 &   0.638 &   2.981 &   0.668 &   0.696 \\
      5 &    1.00 &     0.1 &     0.0 &     \RBF &    10.0 &   0.689 &   2.080 &   0.638 &   2.981 &   0.668 &   0.696 \\
      5 &    1.00 &     0.1 &     1.0 &     \COS &       - &   0.692 &   2.091 &   0.641 &   2.994 &   0.668 &   0.698 \\
      5 &    1.00 &     0.1 &     1.0 &     \RBF &    10.0 &   0.692 &   2.089 &   0.641 &   2.993 &   0.669 &   0.697 \\
      5 &    1.00 &     0.1 &    10.0 &     \COS &       - &   0.703 &   2.129 &   0.651 &   3.029 &   0.669 &   0.704 \\
      5 &    1.00 &     0.1 &    10.0 &     \RBF &    10.0 &   0.702 &   2.127 &   0.651 &   3.025 &   0.669 &   0.703 \\
      5 &    1.00 &     0.1 &   100.0 &     \COS &       - &   0.737 &   2.227 &   0.681 &   3.125 &   0.675 &   0.727 \\
      5 &    1.00 &     0.1 &   100.0 &     \RBF &    10.0 &   0.733 &   2.213 &   0.676 &   3.107 &   0.675 &   0.722 \\
      5 &    1.00 &     1.0 &     0.0 &     \COS &       - &   0.693 &   2.091 &   0.642 &   2.985 &   0.668 &   0.695 \\
      5 &    1.00 &     1.0 &     0.0 &     \RBF &    10.0 &   0.693 &   2.091 &   0.642 &   2.985 &   0.668 &   0.695 \\
      5 &    1.00 &     1.0 &     1.0 &     \COS &       - &   0.695 &   2.101 &   0.644 &   2.991 &   0.669 &   0.696 \\
      5 &    1.00 &     1.0 &     1.0 &     \RBF &    10.0 &   0.694 &   2.101 &   0.644 &   2.992 &   0.669 &   0.696 \\
      5 &    1.00 &     1.0 &    10.0 &     \COS &       - &   0.705 &   2.134 &   0.654 &   3.026 &   0.669 &   0.702 \\
      5 &    1.00 &     1.0 &    10.0 &     \RBF &    10.0 &   0.704 &   2.133 &   0.652 &   3.026 &   0.669 &   0.702 \\
      5 &    1.00 &     1.0 &   100.0 &     \COS &       - &   0.737 &   2.231 &   0.682 &   3.120 &   0.675 &   0.725 \\
      5 &    1.00 &     1.0 &   100.0 &     \RBF &    10.0 &   0.733 &   2.212 &   0.677 &   3.101 &   0.675 &   0.720 \\
     10 &    0.00 &     0.1 &     0.0 &     \COS &       - &   0.854 &   2.954 &   0.804 &   3.978 &   0.659 &   0.786 \\
     10 &    0.00 &     0.1 &     0.0 &     \RBF &    10.0 &   0.854 &   2.954 &   0.804 &   3.978 &   0.659 &   0.786 \\
     10 &    0.00 &     0.1 &     1.0 &     \COS &       - &   0.854 &   2.954 &   0.804 &   3.978 &   0.659 &   0.786 \\
     10 &    0.00 &     0.1 &     1.0 &     \RBF &    10.0 &   0.854 &   2.954 &   0.804 &   3.978 &   0.659 &   0.786 \\
     10 &    0.00 &     0.1 &    10.0 &     \COS &       - &   0.854 &   2.954 &   0.804 &   3.977 &   0.659 &   0.786 \\
     10 &    0.00 &     0.1 &    10.0 &     \RBF &    10.0 &   0.854 &   2.954 &   0.804 &   3.977 &   0.659 &   0.786 \\
     10 &    0.00 &     0.1 &   100.0 &     \COS &       - &   0.854 &   2.953 &   0.804 &   3.977 &   0.659 &   0.785 \\
     10 &    0.00 &     0.1 &   100.0 &     \RBF &    10.0 &   0.854 &   2.953 &   0.804 &   3.977 &   0.659 &   0.785 \\
     10 &    0.00 &     1.0 &     0.0 &     \COS &       - &   0.854 &   2.954 &   0.804 &   3.978 &   0.659 &   0.786 \\
     10 &    0.00 &     1.0 &     0.0 &     \RBF &    10.0 &   0.854 &   2.954 &   0.804 &   3.978 &   0.659 &   0.786 \\
     10 &    0.00 &     1.0 &     1.0 &     \COS &       - &   0.854 &   2.954 &   0.804 &   3.978 &   0.659 &   0.786 \\
     10 &    0.00 &     1.0 &     1.0 &     \RBF &    10.0 &   0.854 &   2.954 &   0.804 &   3.978 &   0.659 &   0.786 \\
     10 &    0.00 &     1.0 &    10.0 &     \COS &       - &   0.854 &   2.954 &   0.805 &   3.977 &   0.659 &   0.786 \\
     10 &    0.00 &     1.0 &    10.0 &     \RBF &    10.0 &   0.854 &   2.954 &   0.804 &   3.977 &   0.659 &   0.786 \\
     10 &    0.00 &     1.0 &   100.0 &     \COS &       - &   0.854 &   2.953 &   0.804 &   3.977 &   0.659 &   0.785 \\
     10 &    0.00 &     1.0 &   100.0 &     \RBF &    10.0 &   0.854 &   2.953 &   0.804 &   3.977 &   0.659 &   0.785 \\
     10 &    0.05 &     0.1 &     0.0 &     \COS &       - &   0.853 &   2.958 &   0.804 &   3.983 &   0.660 &   0.787 \\
     10 &    0.05 &     0.1 &     0.0 &     \RBF &    10.0 &   0.853 &   2.958 &   0.804 &   3.983 &   0.660 &   0.787 \\
     10 &    0.05 &     0.1 &     1.0 &     \COS &       - &   0.853 &   2.958 &   0.804 &   3.983 &   0.659 &   0.787 \\
     10 &    0.05 &     0.1 &     1.0 &     \RBF &    10.0 &   0.853 &   2.958 &   0.804 &   3.983 &   0.659 &   0.787 \\
     10 &    0.05 &     0.1 &    10.0 &     \COS &       - &   0.853 &   2.958 &   0.804 &   3.982 &   0.660 &   0.787 \\
     10 &    0.05 &     0.1 &    10.0 &     \RBF &    10.0 &   0.853 &   2.958 &   0.804 &   3.983 &   0.660 &   0.787 \\
     10 &    0.05 &     0.1 &   100.0 &     \COS &       - &   0.853 &   2.955 &   0.804 &   3.980 &   0.660 &   0.787 \\
     10 &    0.05 &     0.1 &   100.0 &     \RBF &    10.0 &   0.853 &   2.955 &   0.804 &   3.980 &   0.660 &   0.787 \\
     10 &    0.05 &     1.0 &     0.0 &     \COS &       - &   0.853 &   2.958 &   0.804 &   3.983 &   0.659 &   0.787 \\
     10 &    0.05 &     1.0 &     0.0 &     \RBF &    10.0 &   0.853 &   2.958 &   0.804 &   3.983 &   0.659 &   0.787 \\
     10 &    0.05 &     1.0 &     1.0 &     \COS &       - &   0.853 &   2.958 &   0.804 &   3.983 &   0.659 &   0.787 \\
     10 &    0.05 &     1.0 &     1.0 &     \RBF &    10.0 &   0.853 &   2.958 &   0.804 &   3.983 &   0.659 &   0.787 \\
     10 &    0.05 &     1.0 &    10.0 &     \COS &       - &   0.853 &   2.958 &   0.804 &   3.982 &   0.660 &   0.787 \\
     10 &    0.05 &     1.0 &    10.0 &     \RBF &    10.0 &   0.853 &   2.958 &   0.804 &   3.983 &   0.660 &   0.787 \\
     10 &    0.05 &     1.0 &   100.0 &     \COS &       - &   0.853 &   2.955 &   0.804 &   3.980 &   0.660 &   0.787 \\
     10 &    0.05 &     1.0 &   100.0 &     \RBF &    10.0 &   0.853 &   2.955 &   0.804 &   3.980 &   0.660 &   0.787 \\
     10 &    0.10 &     0.1 &     0.0 &     \COS &       - &   0.854 &   2.960 &   0.805 &   3.981 &   0.661 &   0.789 \\
     10 &    0.10 &     0.1 &     0.0 &     \RBF &    10.0 &   0.854 &   2.960 &   0.805 &   3.981 &   0.661 &   0.789 \\
     10 &    0.10 &     0.1 &     1.0 &     \COS &       - &   0.854 &   2.960 &   0.805 &   3.980 &   0.661 &   0.789 \\
     10 &    0.10 &     0.1 &     1.0 &     \RBF &    10.0 &   0.854 &   2.960 &   0.805 &   3.980 &   0.661 &   0.789 \\
     10 &    0.10 &     0.1 &    10.0 &     \COS &       - &   0.854 &   2.960 &   0.805 &   3.981 &   0.661 &   0.789 \\
     10 &    0.10 &     0.1 &    10.0 &     \RBF &    10.0 &   0.854 &   2.960 &   0.805 &   3.981 &   0.661 &   0.789 \\
     10 &    0.10 &     0.1 &   100.0 &     \COS &       - &   0.853 &   2.958 &   0.804 &   3.982 &   0.661 &   0.789 \\
     10 &    0.10 &     0.1 &   100.0 &     \RBF &    10.0 &   0.853 &   2.958 &   0.804 &   3.982 &   0.661 &   0.789 \\
     10 &    0.10 &     1.0 &     0.0 &     \COS &       - &   0.854 &   2.960 &   0.805 &   3.980 &   0.661 &   0.789 \\
     10 &    0.10 &     1.0 &     0.0 &     \RBF &    10.0 &   0.854 &   2.960 &   0.805 &   3.980 &   0.661 &   0.789 \\
     10 &    0.10 &     1.0 &     1.0 &     \COS &       - &   0.854 &   2.960 &   0.805 &   3.980 &   0.661 &   0.789 \\
     10 &    0.10 &     1.0 &     1.0 &     \RBF &    10.0 &   0.854 &   2.960 &   0.805 &   3.980 &   0.661 &   0.789 \\
     10 &    0.10 &     1.0 &    10.0 &     \COS &       - &   0.854 &   2.960 &   0.805 &   3.981 &   0.661 &   0.789 \\
     10 &    0.10 &     1.0 &    10.0 &     \RBF &    10.0 &   0.854 &   2.960 &   0.805 &   3.981 &   0.661 &   0.789 \\
     10 &    0.10 &     1.0 &   100.0 &     \COS &       - &   0.853 &   2.958 &   0.804 &   3.981 &   0.661 &   0.789 \\
     10 &    0.10 &     1.0 &   100.0 &     \RBF &    10.0 &   0.853 &   2.958 &   0.804 &   3.982 &   0.661 &   0.789 \\
     10 &    0.50 &     0.1 &     0.0 &     \COS &       - &   0.855 &   2.965 &   0.806 &   3.985 &   0.658 &   0.804 \\
     10 &    0.50 &     0.1 &     0.0 &     \RBF &    10.0 &   0.855 &   2.965 &   0.806 &   3.985 &   0.658 &   0.804 \\
     10 &    0.50 &     0.1 &     1.0 &     \COS &       - &   0.855 &   2.965 &   0.806 &   3.985 &   0.658 &   0.804 \\
     10 &    0.50 &     0.1 &     1.0 &     \RBF &    10.0 &   0.855 &   2.965 &   0.806 &   3.985 &   0.658 &   0.804 \\
     10 &    0.50 &     0.1 &    10.0 &     \COS &       - &   0.855 &   2.965 &   0.806 &   3.985 &   0.658 &   0.804 \\
     10 &    0.50 &     0.1 &    10.0 &     \RBF &    10.0 &   0.855 &   2.965 &   0.806 &   3.985 &   0.658 &   0.804 \\
     10 &    0.50 &     0.1 &   100.0 &     \COS &       - &   0.855 &   2.965 &   0.806 &   3.986 &   0.658 &   0.804 \\
     10 &    0.50 &     0.1 &   100.0 &     \RBF &    10.0 &   0.855 &   2.965 &   0.806 &   3.985 &   0.658 &   0.804 \\
     10 &    0.50 &     1.0 &     0.0 &     \COS &       - &   0.855 &   2.965 &   0.806 &   3.985 &   0.658 &   0.804 \\
     10 &    0.50 &     1.0 &     0.0 &     \RBF &    10.0 &   0.855 &   2.965 &   0.806 &   3.985 &   0.658 &   0.804 \\
     10 &    0.50 &     1.0 &     1.0 &     \COS &       - &   0.855 &   2.965 &   0.806 &   3.985 &   0.658 &   0.804 \\
     10 &    0.50 &     1.0 &     1.0 &     \RBF &    10.0 &   0.855 &   2.965 &   0.806 &   3.985 &   0.658 &   0.804 \\
     10 &    0.50 &     1.0 &    10.0 &     \COS &       - &   0.855 &   2.965 &   0.806 &   3.985 &   0.658 &   0.804 \\
     10 &    0.50 &     1.0 &    10.0 &     \RBF &    10.0 &   0.855 &   2.965 &   0.806 &   3.985 &   0.658 &   0.804 \\
     10 &    0.50 &     1.0 &   100.0 &     \COS &       - &   0.855 &   2.965 &   0.806 &   3.986 &   0.658 &   0.804 \\
     10 &    0.50 &     1.0 &   100.0 &     \RBF &    10.0 &   0.855 &   2.965 &   0.806 &   3.986 &   0.658 &   0.804 \\
     10 &    1.00 &     0.1 &     0.0 &     \COS &       - &   0.665 &   1.918 &   0.620 &   2.663 &   0.637 &   0.640 \\
     10 &    1.00 &     0.1 &     0.0 &     \RBF &    10.0 &   0.665 &   1.918 &   0.620 &   2.663 &   0.637 &   0.640 \\
     10 &    1.00 &     0.1 &     1.0 &     \COS &       - &   0.668 &   1.938 &   0.623 &   2.686 &   0.637 &   0.644 \\
     10 &    1.00 &     0.1 &     1.0 &     \RBF &    10.0 &   0.668 &   1.939 &   0.623 &   2.685 &   0.637 &   0.644 \\
     10 &    1.00 &     0.1 &    10.0 &     \COS &       - &   0.685 &   1.994 &   0.637 &   2.752 &   0.640 &   0.657 \\
     10 &    1.00 &     0.1 &    10.0 &     \RBF &    10.0 &   0.684 &   2.001 &   0.637 &   2.754 &   0.640 &   0.657 \\
     10 &    1.00 &     0.1 &   100.0 &     \COS &       - &   0.726 &   2.188 &   0.675 &   2.991 &   0.655 &   0.708 \\
     10 &    1.00 &     0.1 &   100.0 &     \RBF &    10.0 &   0.726 &   2.178 &   0.674 &   2.979 &   0.654 &   0.705 \\
     10 &    1.00 &     1.0 &     0.0 &     \COS &       - &   0.668 &   1.929 &   0.624 &   2.669 &   0.637 &   0.638 \\
     10 &    1.00 &     1.0 &     0.0 &     \RBF &    10.0 &   0.668 &   1.929 &   0.624 &   2.669 &   0.637 &   0.638 \\
     10 &    1.00 &     1.0 &     1.0 &     \COS &       - &   0.672 &   1.953 &   0.627 &   2.688 &   0.636 &   0.642 \\
     10 &    1.00 &     1.0 &     1.0 &     \RBF &    10.0 &   0.672 &   1.952 &   0.627 &   2.687 &   0.636 &   0.641 \\
     10 &    1.00 &     1.0 &    10.0 &     \COS &       - &   0.690 &   2.014 &   0.642 &   2.768 &   0.640 &   0.656 \\
     10 &    1.00 &     1.0 &    10.0 &     \RBF &    10.0 &   0.688 &   2.006 &   0.640 &   2.756 &   0.640 &   0.655 \\
     10 &    1.00 &     1.0 &   100.0 &     \COS &       - &   0.731 &   2.194 &   0.678 &   3.001 &   0.656 &   0.710 \\
     10 &    1.00 &     1.0 &   100.0 &     \RBF &    10.0 &   0.726 &   2.174 &   0.675 &   2.966 &   0.654 &   0.702 \\
     15 &    0.00 &     0.1 &     0.0 &     \COS &       - &   0.850 &   2.961 &   0.802 &   4.004 &   0.638 &   0.791 \\
     15 &    0.00 &     0.1 &     0.0 &     \RBF &    10.0 &   0.850 &   2.961 &   0.802 &   4.004 &   0.638 &   0.791 \\
     15 &    0.00 &     0.1 &     1.0 &     \COS &       - &   0.850 &   2.961 &   0.802 &   4.004 &   0.638 &   0.791 \\
     15 &    0.00 &     0.1 &     1.0 &     \RBF &    10.0 &   0.850 &   2.961 &   0.802 &   4.004 &   0.638 &   0.791 \\
     15 &    0.00 &     0.1 &    10.0 &     \COS &       - &   0.849 &   2.961 &   0.802 &   4.005 &   0.638 &   0.791 \\
     15 &    0.00 &     0.1 &    10.0 &     \RBF &    10.0 &   0.849 &   2.962 &   0.802 &   4.004 &   0.638 &   0.791 \\
     15 &    0.00 &     0.1 &   100.0 &     \COS &       - &   0.850 &   2.962 &   0.802 &   4.007 &   0.638 &   0.791 \\
     15 &    0.00 &     0.1 &   100.0 &     \RBF &    10.0 &   0.850 &   2.960 &   0.802 &   4.007 &   0.638 &   0.792 \\
     15 &    0.00 &     1.0 &     0.0 &     \COS &       - &   0.850 &   2.960 &   0.802 &   4.005 &   0.637 &   0.792 \\
     15 &    0.00 &     1.0 &     0.0 &     \RBF &    10.0 &   0.850 &   2.960 &   0.802 &   4.005 &   0.637 &   0.792 \\
     15 &    0.00 &     1.0 &     1.0 &     \COS &       - &   0.850 &   2.960 &   0.802 &   4.005 &   0.637 &   0.792 \\
     15 &    0.00 &     1.0 &     1.0 &     \RBF &    10.0 &   0.850 &   2.960 &   0.802 &   4.005 &   0.637 &   0.792 \\
     15 &    0.00 &     1.0 &    10.0 &     \COS &       - &   0.849 &   2.961 &   0.802 &   4.005 &   0.637 &   0.792 \\
     15 &    0.00 &     1.0 &    10.0 &     \RBF &    10.0 &   0.849 &   2.961 &   0.802 &   4.005 &   0.637 &   0.792 \\
     15 &    0.00 &     1.0 &   100.0 &     \COS &       - &   0.850 &   2.960 &   0.802 &   4.007 &   0.638 &   0.791 \\
     15 &    0.00 &     1.0 &   100.0 &     \RBF &    10.0 &   0.850 &   2.960 &   0.802 &   4.007 &   0.638 &   0.792 \\
     15 &    0.05 &     0.1 &     0.0 &     \COS &       - &   0.849 &   2.956 &   0.801 &   4.006 &   0.636 &   0.793 \\
     15 &    0.05 &     0.1 &     0.0 &     \RBF &    10.0 &   0.849 &   2.956 &   0.801 &   4.006 &   0.636 &   0.793 \\
     15 &    0.05 &     0.1 &     1.0 &     \COS &       - &   0.849 &   2.956 &   0.801 &   4.006 &   0.636 &   0.793 \\
     15 &    0.05 &     0.1 &     1.0 &     \RBF &    10.0 &   0.849 &   2.956 &   0.801 &   4.006 &   0.636 &   0.793 \\
     15 &    0.05 &     0.1 &    10.0 &     \COS &       - &   0.849 &   2.956 &   0.801 &   4.006 &   0.636 &   0.793 \\
     15 &    0.05 &     0.1 &    10.0 &     \RBF &    10.0 &   0.849 &   2.956 &   0.801 &   4.006 &   0.636 &   0.793 \\
     15 &    0.05 &     0.1 &   100.0 &     \COS &       - &   0.849 &   2.960 &   0.801 &   4.005 &   0.637 &   0.793 \\
     15 &    0.05 &     0.1 &   100.0 &     \RBF &    10.0 &   0.849 &   2.960 &   0.801 &   4.006 &   0.636 &   0.793 \\
     15 &    0.05 &     1.0 &     0.0 &     \COS &       - &   0.849 &   2.956 &   0.801 &   4.006 &   0.636 &   0.793 \\
     15 &    0.05 &     1.0 &     0.0 &     \RBF &    10.0 &   0.849 &   2.956 &   0.801 &   4.006 &   0.636 &   0.793 \\
     15 &    0.05 &     1.0 &     1.0 &     \COS &       - &   0.849 &   2.956 &   0.801 &   4.006 &   0.636 &   0.793 \\
     15 &    0.05 &     1.0 &     1.0 &     \RBF &    10.0 &   0.849 &   2.956 &   0.801 &   4.006 &   0.636 &   0.793 \\
     15 &    0.05 &     1.0 &    10.0 &     \COS &       - &   0.849 &   2.956 &   0.801 &   4.006 &   0.636 &   0.793 \\
     15 &    0.05 &     1.0 &    10.0 &     \RBF &    10.0 &   0.849 &   2.956 &   0.801 &   4.006 &   0.636 &   0.793 \\
     15 &    0.05 &     1.0 &   100.0 &     \COS &       - &   0.849 &   2.960 &   0.801 &   4.005 &   0.637 &   0.793 \\
     15 &    0.05 &     1.0 &   100.0 &     \RBF &    10.0 &   0.849 &   2.960 &   0.801 &   4.006 &   0.636 &   0.793 \\
     15 &    0.10 &     0.1 &     0.0 &     \COS &       - &   0.848 &   2.951 &   0.800 &   4.007 &   0.635 &   0.795 \\
     15 &    0.10 &     0.1 &     0.0 &     \RBF &    10.0 &   0.848 &   2.951 &   0.800 &   4.007 &   0.635 &   0.795 \\
     15 &    0.10 &     0.1 &     1.0 &     \COS &       - &   0.848 &   2.951 &   0.800 &   4.007 &   0.635 &   0.795 \\
     15 &    0.10 &     0.1 &     1.0 &     \RBF &    10.0 &   0.848 &   2.951 &   0.800 &   4.007 &   0.635 &   0.795 \\
     15 &    0.10 &     0.1 &    10.0 &     \COS &       - &   0.848 &   2.952 &   0.800 &   4.007 &   0.635 &   0.795 \\
     15 &    0.10 &     0.1 &    10.0 &     \RBF &    10.0 &   0.848 &   2.952 &   0.800 &   4.007 &   0.635 &   0.795 \\
     15 &    0.10 &     0.1 &   100.0 &     \COS &       - &   0.848 &   2.956 &   0.800 &   4.007 &   0.636 &   0.795 \\
     15 &    0.10 &     0.1 &   100.0 &     \RBF &    10.0 &   0.848 &   2.955 &   0.800 &   4.008 &   0.636 &   0.795 \\
     15 &    0.10 &     1.0 &     0.0 &     \COS &       - &   0.848 &   2.951 &   0.800 &   4.007 &   0.635 &   0.795 \\
     15 &    0.10 &     1.0 &     0.0 &     \RBF &    10.0 &   0.848 &   2.951 &   0.800 &   4.007 &   0.635 &   0.795 \\
     15 &    0.10 &     1.0 &     1.0 &     \COS &       - &   0.848 &   2.951 &   0.800 &   4.007 &   0.635 &   0.795 \\
     15 &    0.10 &     1.0 &     1.0 &     \RBF &    10.0 &   0.848 &   2.951 &   0.800 &   4.007 &   0.635 &   0.795 \\
     15 &    0.10 &     1.0 &    10.0 &     \COS &       - &   0.848 &   2.952 &   0.800 &   4.007 &   0.635 &   0.795 \\
     15 &    0.10 &     1.0 &    10.0 &     \RBF &    10.0 &   0.848 &   2.952 &   0.800 &   4.007 &   0.635 &   0.795 \\
     15 &    0.10 &     1.0 &   100.0 &     \COS &       - &   0.848 &   2.956 &   0.800 &   4.007 &   0.636 &   0.795 \\
     15 &    0.10 &     1.0 &   100.0 &     \RBF &    10.0 &   0.848 &   2.955 &   0.800 &   4.008 &   0.636 &   0.795 \\
     15 &    0.50 &     0.1 &     0.0 &     \COS &       - &   0.838 &   2.893 &   0.789 &   3.952 &   0.613 &   0.808 \\
     15 &    0.50 &     0.1 &     0.0 &     \RBF &    10.0 &   0.838 &   2.893 &   0.789 &   3.952 &   0.613 &   0.808 \\
     15 &    0.50 &     0.1 &     1.0 &     \COS &       - &   0.838 &   2.893 &   0.789 &   3.952 &   0.613 &   0.808 \\
     15 &    0.50 &     0.1 &     1.0 &     \RBF &    10.0 &   0.838 &   2.893 &   0.789 &   3.952 &   0.613 &   0.808 \\
     15 &    0.50 &     0.1 &    10.0 &     \COS &       - &   0.838 &   2.893 &   0.789 &   3.953 &   0.613 &   0.808 \\
     15 &    0.50 &     0.1 &    10.0 &     \RBF &    10.0 &   0.838 &   2.893 &   0.789 &   3.954 &   0.613 &   0.808 \\
     15 &    0.50 &     0.1 &   100.0 &     \COS &       - &   0.838 &   2.897 &   0.789 &   3.958 &   0.615 &   0.808 \\
     15 &    0.50 &     0.1 &   100.0 &     \RBF &    10.0 &   0.838 &   2.897 &   0.789 &   3.956 &   0.614 &   0.808 \\
     15 &    0.50 &     1.0 &     0.0 &     \COS &       - &   0.838 &   2.893 &   0.789 &   3.952 &   0.613 &   0.808 \\
     15 &    0.50 &     1.0 &     0.0 &     \RBF &    10.0 &   0.838 &   2.893 &   0.789 &   3.952 &   0.613 &   0.808 \\
     15 &    0.50 &     1.0 &     1.0 &     \COS &       - &   0.838 &   2.892 &   0.789 &   3.952 &   0.613 &   0.808 \\
     15 &    0.50 &     1.0 &     1.0 &     \RBF &    10.0 &   0.838 &   2.892 &   0.789 &   3.952 &   0.613 &   0.808 \\
     15 &    0.50 &     1.0 &    10.0 &     \COS &       - &   0.838 &   2.893 &   0.789 &   3.953 &   0.613 &   0.808 \\
     15 &    0.50 &     1.0 &    10.0 &     \RBF &    10.0 &   0.838 &   2.893 &   0.789 &   3.954 &   0.613 &   0.808 \\
     15 &    0.50 &     1.0 &   100.0 &     \COS &       - &   0.838 &   2.897 &   0.789 &   3.958 &   0.615 &   0.808 \\
     15 &    0.50 &     1.0 &   100.0 &     \RBF &    10.0 &   0.838 &   2.897 &   0.789 &   3.957 &   0.614 &   0.808 \\
     15 &    1.00 &     0.1 &     0.0 &     \COS &       - &   0.670 &   1.869 &   0.626 &   2.544 &   0.597 &   0.603 \\
     15 &    1.00 &     0.1 &     0.0 &     \RBF &    10.0 &   0.670 &   1.869 &   0.626 &   2.544 &   0.597 &   0.603 \\
     15 &    1.00 &     0.1 &     1.0 &     \COS &       - &   0.676 &   1.896 &   0.630 &   2.585 &   0.601 &   0.613 \\
     15 &    1.00 &     0.1 &     1.0 &     \RBF &    10.0 &   0.675 &   1.893 &   0.629 &   2.578 &   0.601 &   0.612 \\
     15 &    1.00 &     0.1 &    10.0 &     \COS &       - &   0.685 &   1.961 &   0.639 &   2.671 &   0.608 &   0.631 \\
     15 &    1.00 &     0.1 &    10.0 &     \RBF &    10.0 &   0.685 &   1.955 &   0.638 &   2.668 &   0.608 &   0.630 \\
     15 &    1.00 &     0.1 &   100.0 &     \COS &       - &   0.726 &   2.159 &   0.674 &   2.965 &   0.644 &   0.700 \\
     15 &    1.00 &     0.1 &   100.0 &     \RBF &    10.0 &   0.724 &   2.155 &   0.673 &   2.939 &   0.644 &   0.693 \\
     15 &    1.00 &     1.0 &     0.0 &     \COS &       - &   0.674 &   1.889 &   0.629 &   2.573 &   0.602 &   0.605 \\
     15 &    1.00 &     1.0 &     0.0 &     \RBF &    10.0 &   0.674 &   1.889 &   0.629 &   2.573 &   0.602 &   0.605 \\
     15 &    1.00 &     1.0 &     1.0 &     \COS &       - &   0.677 &   1.910 &   0.631 &   2.606 &   0.603 &   0.613 \\
     15 &    1.00 &     1.0 &     1.0 &     \RBF &    10.0 &   0.677 &   1.909 &   0.631 &   2.600 &   0.603 &   0.612 \\
     15 &    1.00 &     1.0 &    10.0 &     \COS &       - &   0.690 &   1.982 &   0.643 &   2.693 &   0.610 &   0.632 \\
     15 &    1.00 &     1.0 &    10.0 &     \RBF &    10.0 &   0.688 &   1.971 &   0.642 &   2.688 &   0.609 &   0.632 \\
     15 &    1.00 &     1.0 &   100.0 &     \COS &       - &   0.727 &   2.161 &   0.676 &   2.959 &   0.647 &   0.695 \\
     15 &    1.00 &     1.0 &   100.0 &     \RBF &    10.0 &   0.720 &   2.124 &   0.670 &   2.892 &   0.642 &   0.680 \\
     30 &    0.00 &     0.1 &     0.0 &     \COS &       - &   0.795 &   2.798 &   0.747 &   3.917 &   0.578 &   0.799 \\
     30 &    0.00 &     0.1 &     0.0 &     \RBF &    10.0 &   0.795 &   2.798 &   0.747 &   3.917 &   0.578 &   0.799 \\
     30 &    0.00 &     0.1 &     1.0 &     \COS &       - &   0.795 &   2.798 &   0.747 &   3.917 &   0.578 &   0.799 \\
     30 &    0.00 &     0.1 &     1.0 &     \RBF &    10.0 &   0.795 &   2.798 &   0.747 &   3.917 &   0.578 &   0.799 \\
     30 &    0.00 &     0.1 &    10.0 &     \COS &       - &   0.792 &   2.791 &   0.745 &   3.913 &   0.576 &   0.800 \\
     30 &    0.00 &     0.1 &    10.0 &     \RBF &    10.0 &   0.792 &   2.791 &   0.745 &   3.913 &   0.576 &   0.800 \\
     30 &    0.00 &     0.1 &   100.0 &     \COS &       - &   0.834 &   2.951 &   0.788 &   4.006 &   0.633 &   0.780 \\
     30 &    0.00 &     0.1 &   100.0 &     \RBF &    10.0 &   0.817 &   2.900 &   0.771 &   3.981 &   0.608 &   0.791 \\
     30 &    0.00 &     1.0 &     0.0 &     \COS &       - &   0.791 &   2.785 &   0.743 &   3.911 &   0.574 &   0.800 \\
     30 &    0.00 &     1.0 &     0.0 &     \RBF &    10.0 &   0.791 &   2.785 &   0.743 &   3.911 &   0.574 &   0.800 \\
     30 &    0.00 &     1.0 &     1.0 &     \COS &       - &   0.791 &   2.785 &   0.743 &   3.911 &   0.574 &   0.800 \\
     30 &    0.00 &     1.0 &     1.0 &     \RBF &    10.0 &   0.791 &   2.785 &   0.743 &   3.911 &   0.574 &   0.800 \\
     30 &    0.00 &     1.0 &    10.0 &     \COS &       - &   0.791 &   2.785 &   0.743 &   3.912 &   0.575 &   0.800 \\
     30 &    0.00 &     1.0 &    10.0 &     \RBF &    10.0 &   0.791 &   2.786 &   0.743 &   3.912 &   0.575 &   0.800 \\
     30 &    0.00 &     1.0 &   100.0 &     \COS &       - &   0.799 &   2.823 &   0.752 &   3.940 &   0.584 &   0.799 \\
     30 &    0.00 &     1.0 &   100.0 &     \RBF &    10.0 &   0.793 &   2.797 &   0.746 &   3.917 &   0.576 &   0.801 \\
     30 &    0.05 &     0.1 &     0.0 &     \COS &       - &   0.787 &   2.755 &   0.738 &   3.892 &   0.569 &   0.802 \\
     30 &    0.05 &     0.1 &     0.0 &     \RBF &    10.0 &   0.787 &   2.755 &   0.738 &   3.892 &   0.569 &   0.802 \\
     30 &    0.05 &     0.1 &     1.0 &     \COS &       - &   0.787 &   2.755 &   0.738 &   3.892 &   0.569 &   0.802 \\
     30 &    0.05 &     0.1 &     1.0 &     \RBF &    10.0 &   0.787 &   2.755 &   0.738 &   3.892 &   0.569 &   0.802 \\
     30 &    0.05 &     0.1 &    10.0 &     \COS &       - &   0.787 &   2.757 &   0.738 &   3.893 &   0.569 &   0.802 \\
     30 &    0.05 &     0.1 &    10.0 &     \RBF &    10.0 &   0.787 &   2.757 &   0.738 &   3.893 &   0.569 &   0.802 \\
     30 &    0.05 &     0.1 &   100.0 &     \COS &       - &   0.789 &   2.770 &   0.740 &   3.905 &   0.573 &   0.802 \\
     30 &    0.05 &     0.1 &   100.0 &     \RBF &    10.0 &   0.789 &   2.767 &   0.740 &   3.903 &   0.572 &   0.802 \\
     30 &    0.05 &     1.0 &     0.0 &     \COS &       - &   0.787 &   2.755 &   0.738 &   3.892 &   0.569 &   0.802 \\
     30 &    0.05 &     1.0 &     0.0 &     \RBF &    10.0 &   0.787 &   2.755 &   0.738 &   3.892 &   0.569 &   0.802 \\
     30 &    0.05 &     1.0 &     1.0 &     \COS &       - &   0.787 &   2.755 &   0.738 &   3.892 &   0.569 &   0.802 \\
     30 &    0.05 &     1.0 &     1.0 &     \RBF &    10.0 &   0.787 &   2.755 &   0.738 &   3.892 &   0.569 &   0.802 \\
     30 &    0.05 &     1.0 &    10.0 &     \COS &       - &   0.787 &   2.757 &   0.738 &   3.893 &   0.569 &   0.802 \\
     30 &    0.05 &     1.0 &    10.0 &     \RBF &    10.0 &   0.787 &   2.757 &   0.738 &   3.893 &   0.569 &   0.802 \\
     30 &    0.05 &     1.0 &   100.0 &     \COS &       - &   0.789 &   2.770 &   0.740 &   3.905 &   0.573 &   0.802 \\
     30 &    0.05 &     1.0 &   100.0 &     \RBF &    10.0 &   0.789 &   2.767 &   0.740 &   3.903 &   0.572 &   0.802 \\
     30 &    0.10 &     0.1 &     0.0 &     \COS &       - &   0.781 &   2.724 &   0.732 &   3.866 &   0.561 &   0.803 \\
     30 &    0.10 &     0.1 &     0.0 &     \RBF &    10.0 &   0.781 &   2.724 &   0.732 &   3.866 &   0.561 &   0.803 \\
     30 &    0.10 &     0.1 &     1.0 &     \COS &       - &   0.781 &   2.724 &   0.732 &   3.866 &   0.561 &   0.803 \\
     30 &    0.10 &     0.1 &     1.0 &     \RBF &    10.0 &   0.781 &   2.724 &   0.732 &   3.866 &   0.561 &   0.803 \\
     30 &    0.10 &     0.1 &    10.0 &     \COS &       - &   0.781 &   2.727 &   0.732 &   3.868 &   0.561 &   0.803 \\
     30 &    0.10 &     0.1 &    10.0 &     \RBF &    10.0 &   0.781 &   2.727 &   0.732 &   3.868 &   0.561 &   0.803 \\
     30 &    0.10 &     0.1 &   100.0 &     \COS &       - &   0.783 &   2.744 &   0.735 &   3.881 &   0.565 &   0.803 \\
     30 &    0.10 &     0.1 &   100.0 &     \RBF &    10.0 &   0.783 &   2.741 &   0.735 &   3.878 &   0.564 &   0.803 \\
     30 &    0.10 &     1.0 &     0.0 &     \COS &       - &   0.781 &   2.724 &   0.732 &   3.866 &   0.561 &   0.803 \\
     30 &    0.10 &     1.0 &     0.0 &     \RBF &    10.0 &   0.781 &   2.724 &   0.732 &   3.866 &   0.561 &   0.803 \\
     30 &    0.10 &     1.0 &     1.0 &     \COS &       - &   0.781 &   2.724 &   0.732 &   3.867 &   0.561 &   0.803 \\
     30 &    0.10 &     1.0 &     1.0 &     \RBF &    10.0 &   0.781 &   2.724 &   0.732 &   3.866 &   0.561 &   0.803 \\
     30 &    0.10 &     1.0 &    10.0 &     \COS &       - &   0.781 &   2.727 &   0.732 &   3.868 &   0.561 &   0.803 \\
     30 &    0.10 &     1.0 &    10.0 &     \RBF &    10.0 &   0.781 &   2.727 &   0.732 &   3.868 &   0.561 &   0.803 \\
     30 &    0.10 &     1.0 &   100.0 &     \COS &       - &   0.783 &   2.744 &   0.735 &   3.881 &   0.565 &   0.803 \\
     30 &    0.10 &     1.0 &   100.0 &     \RBF &    10.0 &   0.783 &   2.741 &   0.735 &   3.879 &   0.564 &   0.803 \\
     30 &    0.50 &     0.1 &     0.0 &     \COS &       - &   0.742 &   2.444 &   0.685 &   3.556 &   0.512 &   0.810 \\
     30 &    0.50 &     0.1 &     0.0 &     \RBF &    10.0 &   0.742 &   2.444 &   0.685 &   3.556 &   0.512 &   0.810 \\
     30 &    0.50 &     0.1 &     1.0 &     \COS &       - &   0.742 &   2.444 &   0.685 &   3.557 &   0.512 &   0.810 \\
     30 &    0.50 &     0.1 &     1.0 &     \RBF &    10.0 &   0.742 &   2.444 &   0.685 &   3.556 &   0.512 &   0.810 \\
     30 &    0.50 &     0.1 &    10.0 &     \COS &       - &   0.742 &   2.446 &   0.685 &   3.559 &   0.513 &   0.810 \\
     30 &    0.50 &     0.1 &    10.0 &     \RBF &    10.0 &   0.742 &   2.446 &   0.685 &   3.559 &   0.513 &   0.810 \\
     30 &    0.50 &     0.1 &   100.0 &     \COS &       - &   0.744 &   2.461 &   0.687 &   3.581 &   0.516 &   0.810 \\
     30 &    0.50 &     0.1 &   100.0 &     \RBF &    10.0 &   0.744 &   2.458 &   0.686 &   3.578 &   0.515 &   0.810 \\
     30 &    0.50 &     1.0 &     0.0 &     \COS &       - &   0.742 &   2.444 &   0.685 &   3.557 &   0.512 &   0.810 \\
     30 &    0.50 &     1.0 &     0.0 &     \RBF &    10.0 &   0.742 &   2.444 &   0.685 &   3.557 &   0.512 &   0.810 \\
     30 &    0.50 &     1.0 &     1.0 &     \COS &       - &   0.742 &   2.444 &   0.685 &   3.557 &   0.512 &   0.810 \\
     30 &    0.50 &     1.0 &     1.0 &     \RBF &    10.0 &   0.742 &   2.444 &   0.685 &   3.557 &   0.512 &   0.810 \\
     30 &    0.50 &     1.0 &    10.0 &     \COS &       - &   0.742 &   2.446 &   0.685 &   3.559 &   0.513 &   0.810 \\
     30 &    0.50 &     1.0 &    10.0 &     \RBF &    10.0 &   0.742 &   2.446 &   0.685 &   3.559 &   0.513 &   0.810 \\
     30 &    0.50 &     1.0 &   100.0 &     \COS &       - &   0.744 &   2.461 &   0.687 &   3.581 &   0.516 &   0.810 \\
     30 &    0.50 &     1.0 &   100.0 &     \RBF &    10.0 &   0.744 &   2.458 &   0.687 &   3.578 &   0.515 &   0.810 \\
     30 &    1.00 &     0.1 &     0.0 &     \COS &       - &   0.689 &   1.996 &   0.644 &   2.697 &   0.598 &   0.633 \\
     30 &    1.00 &     0.1 &     0.0 &     \RBF &    10.0 &   0.689 &   1.996 &   0.644 &   2.697 &   0.598 &   0.633 \\
     30 &    1.00 &     0.1 &     1.0 &     \COS &       - &   0.696 &   2.030 &   0.650 &   2.750 &   0.598 &   0.651 \\
     30 &    1.00 &     0.1 &     1.0 &     \RBF &    10.0 &   0.695 &   2.027 &   0.650 &   2.746 &   0.597 &   0.650 \\
     30 &    1.00 &     0.1 &    10.0 &     \COS &       - &   0.730 &   2.198 &   0.680 &   2.973 &   0.642 &   0.668 \\
     30 &    1.00 &     0.1 &    10.0 &     \RBF &    10.0 &   0.728 &   2.177 &   0.678 &   2.954 &   0.637 &   0.667 \\
     30 &    1.00 &     0.1 &   100.0 &     \COS &       - &   0.750 &   2.294 &   0.697 &   3.122 &   0.671 &   0.709 \\
     30 &    1.00 &     0.1 &   100.0 &     \RBF &    10.0 &   0.748 &   2.284 &   0.695 &   3.110 &   0.669 &   0.705 \\
     30 &    1.00 &     1.0 &     0.0 &     \COS &       - &   0.691 &   2.007 &   0.646 &   2.715 &   0.595 &   0.643 \\
     30 &    1.00 &     1.0 &     0.0 &     \RBF &    10.0 &   0.691 &   2.007 &   0.646 &   2.715 &   0.595 &   0.643 \\
     30 &    1.00 &     1.0 &     1.0 &     \COS &       - &   0.696 &   2.033 &   0.649 &   2.752 &   0.595 &   0.654 \\
     30 &    1.00 &     1.0 &     1.0 &     \RBF &    10.0 &   0.695 &   2.031 &   0.649 &   2.747 &   0.595 &   0.653 \\
     30 &    1.00 &     1.0 &    10.0 &     \COS &       - &   0.726 &   2.170 &   0.677 &   2.941 &   0.634 &   0.667 \\
     30 &    1.00 &     1.0 &    10.0 &     \RBF &    10.0 &   0.721 &   2.161 &   0.674 &   2.926 &   0.630 &   0.667 \\
     30 &    1.00 &     1.0 &   100.0 &     \COS &       - &   0.753 &   2.301 &   0.700 &   3.126 &   0.673 &   0.707 \\
     30 &    1.00 &     1.0 &   100.0 &     \RBF &    10.0 &   0.751 &   2.289 &   0.698 &   3.107 &   0.670 &   0.700 \\
     50 &    0.00 &     0.1 &     0.0 &     \COS &       - &   0.753 &   2.566 &   0.700 &   3.725 &   0.580 &   0.799 \\
     50 &    0.00 &     0.1 &     0.0 &     \RBF &    10.0 &   0.753 &   2.566 &   0.700 &   3.725 &   0.580 &   0.799 \\
     50 &    0.00 &     0.1 &     1.0 &     \COS &       - &   0.749 &   2.546 &   0.696 &   3.707 &   0.577 &   0.799 \\
     50 &    0.00 &     0.1 &     1.0 &     \RBF &    10.0 &   0.751 &   2.557 &   0.699 &   3.716 &   0.579 &   0.799 \\
     50 &    0.00 &     0.1 &    10.0 &     \COS &       - &   0.739 &   2.500 &   0.686 &   3.667 &   0.571 &   0.800 \\
     50 &    0.00 &     0.1 &    10.0 &     \RBF &    10.0 &   0.739 &   2.500 &   0.686 &   3.667 &   0.571 &   0.800 \\
     50 &    0.00 &     0.1 &   100.0 &     \COS &       - &   0.857 &   2.919 &   0.805 &   3.934 &   0.663 &   0.742 \\
     50 &    0.00 &     0.1 &   100.0 &     \RBF &    10.0 &   0.847 &   2.919 &   0.796 &   3.978 &   0.658 &   0.768 \\
     50 &    0.00 &     1.0 &     0.0 &     \COS &       - &   0.733 &   2.469 &   0.679 &   3.646 &   0.566 &   0.801 \\
     50 &    0.00 &     1.0 &     0.0 &     \RBF &    10.0 &   0.733 &   2.469 &   0.679 &   3.646 &   0.566 &   0.801 \\
     50 &    0.00 &     1.0 &     1.0 &     \COS &       - &   0.733 &   2.469 &   0.679 &   3.646 &   0.566 &   0.801 \\
     50 &    0.00 &     1.0 &     1.0 &     \RBF &    10.0 &   0.733 &   2.469 &   0.679 &   3.646 &   0.566 &   0.801 \\
     50 &    0.00 &     1.0 &    10.0 &     \COS &       - &   0.733 &   2.472 &   0.679 &   3.648 &   0.567 &   0.801 \\
     50 &    0.00 &     1.0 &    10.0 &     \RBF &    10.0 &   0.733 &   2.472 &   0.679 &   3.648 &   0.567 &   0.801 \\
     50 &    0.00 &     1.0 &   100.0 &     \COS &       - &   0.833 &   2.878 &   0.781 &   3.946 &   0.642 &   0.781 \\
     50 &    0.00 &     1.0 &   100.0 &     \RBF &    10.0 &   0.793 &   2.744 &   0.742 &   3.864 &   0.611 &   0.793 \\
     50 &    0.05 &     0.1 &     0.0 &     \COS &       - &   0.723 &   2.425 &   0.669 &   3.603 &   0.562 &   0.802 \\
     50 &    0.05 &     0.1 &     0.0 &     \RBF &    10.0 &   0.723 &   2.425 &   0.669 &   3.603 &   0.562 &   0.802 \\
     50 &    0.05 &     0.1 &     1.0 &     \COS &       - &   0.723 &   2.425 &   0.669 &   3.603 &   0.562 &   0.802 \\
     50 &    0.05 &     0.1 &     1.0 &     \RBF &    10.0 &   0.723 &   2.425 &   0.669 &   3.603 &   0.562 &   0.802 \\
     50 &    0.05 &     0.1 &    10.0 &     \COS &       - &   0.724 &   2.428 &   0.670 &   3.606 &   0.563 &   0.802 \\
     50 &    0.05 &     0.1 &    10.0 &     \RBF &    10.0 &   0.724 &   2.428 &   0.670 &   3.605 &   0.563 &   0.802 \\
     50 &    0.05 &     0.1 &   100.0 &     \COS &       - &   0.816 &   2.825 &   0.764 &   3.912 &   0.628 &   0.787 \\
     50 &    0.05 &     0.1 &   100.0 &     \RBF &    10.0 &   0.752 &   2.565 &   0.700 &   3.727 &   0.581 &   0.800 \\
     50 &    0.05 &     1.0 &     0.0 &     \COS &       - &   0.723 &   2.425 &   0.669 &   3.603 &   0.562 &   0.802 \\
     50 &    0.05 &     1.0 &     0.0 &     \RBF &    10.0 &   0.723 &   2.425 &   0.669 &   3.603 &   0.562 &   0.802 \\
     50 &    0.05 &     1.0 &     1.0 &     \COS &       - &   0.723 &   2.425 &   0.669 &   3.603 &   0.562 &   0.802 \\
     50 &    0.05 &     1.0 &     1.0 &     \RBF &    10.0 &   0.723 &   2.425 &   0.669 &   3.603 &   0.562 &   0.802 \\
     50 &    0.05 &     1.0 &    10.0 &     \COS &       - &   0.724 &   2.428 &   0.670 &   3.606 &   0.563 &   0.802 \\
     50 &    0.05 &     1.0 &    10.0 &     \RBF &    10.0 &   0.724 &   2.428 &   0.670 &   3.606 &   0.563 &   0.802 \\
     50 &    0.05 &     1.0 &   100.0 &     \COS &       - &   0.757 &   2.582 &   0.704 &   3.747 &   0.585 &   0.799 \\
     50 &    0.05 &     1.0 &   100.0 &     \RBF &    10.0 &   0.729 &   2.451 &   0.675 &   3.630 &   0.566 &   0.802 \\
     50 &    0.10 &     0.1 &     0.0 &     \COS &       - &   0.715 &   2.382 &   0.661 &   3.555 &   0.556 &   0.802 \\
     50 &    0.10 &     0.1 &     0.0 &     \RBF &    10.0 &   0.715 &   2.382 &   0.661 &   3.555 &   0.556 &   0.802 \\
     50 &    0.10 &     0.1 &     1.0 &     \COS &       - &   0.715 &   2.382 &   0.661 &   3.555 &   0.556 &   0.802 \\
     50 &    0.10 &     0.1 &     1.0 &     \RBF &    10.0 &   0.715 &   2.382 &   0.661 &   3.555 &   0.556 &   0.802 \\
     50 &    0.10 &     0.1 &    10.0 &     \COS &       - &   0.715 &   2.385 &   0.662 &   3.558 &   0.556 &   0.802 \\
     50 &    0.10 &     0.1 &    10.0 &     \RBF &    10.0 &   0.715 &   2.384 &   0.662 &   3.558 &   0.556 &   0.802 \\
     50 &    0.10 &     0.1 &   100.0 &     \COS &       - &   0.739 &   2.504 &   0.685 &   3.671 &   0.572 &   0.801 \\
     50 &    0.10 &     0.1 &   100.0 &     \RBF &    10.0 &   0.719 &   2.409 &   0.665 &   3.587 &   0.561 &   0.803 \\
     50 &    0.10 &     1.0 &     0.0 &     \COS &       - &   0.715 &   2.382 &   0.661 &   3.555 &   0.556 &   0.802 \\
     50 &    0.10 &     1.0 &     0.0 &     \RBF &    10.0 &   0.715 &   2.382 &   0.661 &   3.555 &   0.556 &   0.802 \\
     50 &    0.10 &     1.0 &     1.0 &     \COS &       - &   0.715 &   2.382 &   0.661 &   3.556 &   0.556 &   0.802 \\
     50 &    0.10 &     1.0 &     1.0 &     \RBF &    10.0 &   0.715 &   2.382 &   0.661 &   3.555 &   0.556 &   0.802 \\
     50 &    0.10 &     1.0 &    10.0 &     \COS &       - &   0.715 &   2.385 &   0.662 &   3.558 &   0.556 &   0.802 \\
     50 &    0.10 &     1.0 &    10.0 &     \RBF &    10.0 &   0.715 &   2.384 &   0.662 &   3.558 &   0.556 &   0.802 \\
     50 &    0.10 &     1.0 &   100.0 &     \COS &       - &   0.720 &   2.413 &   0.666 &   3.592 &   0.561 &   0.803 \\
     50 &    0.10 &     1.0 &   100.0 &     \RBF &    10.0 &   0.719 &   2.409 &   0.665 &   3.587 &   0.561 &   0.803 \\
     50 &    0.50 &     0.1 &     0.0 &     \COS &       - &   0.769 &   2.574 &   0.720 &   3.573 &   0.596 &   0.711 \\
     50 &    0.50 &     0.1 &     0.0 &     \RBF &    10.0 &   0.769 &   2.574 &   0.720 &   3.573 &   0.596 &   0.711 \\
     50 &    0.50 &     0.1 &     1.0 &     \COS &       - &   0.769 &   2.578 &   0.720 &   3.588 &   0.598 &   0.714 \\
     50 &    0.50 &     0.1 &     1.0 &     \RBF &    10.0 &   0.769 &   2.576 &   0.720 &   3.583 &   0.598 &   0.713 \\
     50 &    0.50 &     0.1 &    10.0 &     \COS &       - &   0.673 &   2.161 &   0.620 &   3.274 &   0.527 &   0.801 \\
     50 &    0.50 &     0.1 &    10.0 &     \RBF &    10.0 &   0.675 &   2.171 &   0.622 &   3.286 &   0.529 &   0.801 \\
     50 &    0.50 &     0.1 &   100.0 &     \COS &       - &   0.824 &   2.818 &   0.778 &   3.780 &   0.651 &   0.692 \\
     50 &    0.50 &     0.1 &   100.0 &     \RBF &    10.0 &   0.819 &   2.797 &   0.773 &   3.770 &   0.647 &   0.697 \\
     50 &    0.50 &     1.0 &     0.0 &     \COS &       - &   0.664 &   2.108 &   0.611 &   3.205 &   0.519 &   0.802 \\
     50 &    0.50 &     1.0 &     0.0 &     \RBF &    10.0 &   0.664 &   2.108 &   0.611 &   3.205 &   0.519 &   0.802 \\
     50 &    0.50 &     1.0 &     1.0 &     \COS &       - &   0.659 &   2.090 &   0.607 &   3.184 &   0.517 &   0.802 \\
     50 &    0.50 &     1.0 &     1.0 &     \RBF &    10.0 &   0.661 &   2.098 &   0.609 &   3.193 &   0.518 &   0.802 \\
     50 &    0.50 &     1.0 &    10.0 &     \COS &       - &   0.654 &   2.052 &   0.601 &   3.134 &   0.511 &   0.803 \\
     50 &    0.50 &     1.0 &    10.0 &     \RBF &    10.0 &   0.654 &   2.053 &   0.601 &   3.133 &   0.511 &   0.803 \\
     50 &    0.50 &     1.0 &   100.0 &     \COS &       - &   0.824 &   2.833 &   0.776 &   3.825 &   0.651 &   0.713 \\
     50 &    0.50 &     1.0 &   100.0 &     \RBF &    10.0 &   0.821 &   2.830 &   0.773 &   3.836 &   0.649 &   0.721 \\
     50 &    1.00 &     0.1 &     0.0 &     \COS &       - &   0.703 &   1.983 &   0.658 &   2.601 &   0.644 &   0.644 \\
     50 &    1.00 &     0.1 &     0.0 &     \RBF &    10.0 &   0.703 &   1.983 &   0.658 &   2.601 &   0.644 &   0.644 \\
     50 &    1.00 &     0.1 &     1.0 &     \COS &       - &   0.710 &   2.020 &   0.663 &   2.653 &   0.645 &   0.665 \\
     50 &    1.00 &     0.1 &     1.0 &     \RBF &    10.0 &   0.709 &   2.016 &   0.663 &   2.648 &   0.645 &   0.663 \\
     50 &    1.00 &     0.1 &    10.0 &     \COS &       - &   0.770 &   2.307 &   0.718 &   3.058 &   0.681 &   0.690 \\
     50 &    1.00 &     0.1 &    10.0 &     \RBF &    10.0 &   0.765 &   2.292 &   0.714 &   3.038 &   0.679 &   0.688 \\
     50 &    1.00 &     0.1 &   100.0 &     \COS &       - &   0.779 &   2.382 &   0.720 &   3.246 &   0.698 &   0.735 \\
     50 &    1.00 &     0.1 &   100.0 &     \RBF &    10.0 &   0.779 &   2.374 &   0.720 &   3.234 &   0.698 &   0.730 \\
     50 &    1.00 &     1.0 &     0.0 &     \COS &       - &   0.701 &   1.971 &   0.656 &   2.588 &   0.640 &   0.655 \\
     50 &    1.00 &     1.0 &     0.0 &     \RBF &    10.0 &   0.701 &   1.971 &   0.656 &   2.588 &   0.640 &   0.655 \\
     50 &    1.00 &     1.0 &     1.0 &     \COS &       - &   0.706 &   1.998 &   0.660 &   2.626 &   0.641 &   0.668 \\
     50 &    1.00 &     1.0 &     1.0 &     \RBF &    10.0 &   0.704 &   1.994 &   0.658 &   2.620 &   0.641 &   0.667 \\
     50 &    1.00 &     1.0 &    10.0 &     \COS &       - &   0.761 &   2.272 &   0.710 &   2.996 &   0.676 &   0.686 \\
     50 &    1.00 &     1.0 &    10.0 &     \RBF &    10.0 &   0.756 &   2.250 &   0.706 &   2.971 &   0.674 &   0.684 \\
     50 &    1.00 &     1.0 &   100.0 &     \COS &       - &   0.780 &   2.385 &   0.723 &   3.233 &   0.698 &   0.733 \\
     50 &    1.00 &     1.0 &   100.0 &     \RBF &    10.0 &   0.779 &   2.376 &   0.721 &   3.228 &   0.699 &   0.726 \\

